A provable initialization and robust clustering method for general mixture models

Clustering is a fundamental tool in statistical machine learning in the presence of heterogeneous data. Most recent results focus primarily on optimal mislabeling guarantees when data are distributed around centroids with sub-Gaussian errors. Yet, the restrictive sub-Gaussian model is often invalid in practice since various real-world applications exhibit heavy tail distributions around the centroids or suffer from possible adversarial attacks that call for robust clustering with a robust data-driven initialization. In this paper, we present initialization and subsequent clustering methods that provably guarantee near-optimal mislabeling for general mixture models when the number of clusters and data dimensions are finite. We first introduce a hybrid clustering technique with a novel multivariate trimmed mean type centroid estimate to produce mislabeling guarantees under a weak initialization condition for general error distributions around the centroids. A matching lower bound is derived, up to factors depending on the number of clusters. In addition, our approach also produces similar mislabeling guarantees even in the presence of adversarial outliers. Our results reduce to the sub-Gaussian case in finite dimensions when errors follow sub-Gaussian distributions. To solve the problem thoroughly, we also present novel data-driven robust initialization techniques and show that, with probabilities approaching one, these initial centroid estimates are sufficiently good for the subsequent clustering algorithm to achieve the optimal mislabeling rates. Furthermore, we demonstrate that the Lloyd algorithm is suboptimal for more than two clusters even when errors are Gaussian and for two clusters when error distributions have heavy tails. Both simulated data and real data examples further support our robust initialization procedure and clustering algorithm.

==> tex/Preamble-aos.tex <==
\usepackage{float}

%\IEEEoverridecommandlockouts
% If the IEEEtran.cls has not been installed into the LaTeX system files,
% manually specify the path to it:
% \documentclass[conference]{IEEEtran}
%



%\usepackage[margin=1in]{geometry}  % set the margins to 1in on all sides
\usepackage{xspace,exscale,relsize}
\usepackage{fancybox,shadow}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption} % conflict with [subfigure]
\usepackage{xcolor}
% this is for \mathfrak & better working \mathbb
% this is for \gtrsim, \lesssim symbols (redefined as \simleq, \simgeq in my_style.sty)
%\usepackage{url}
%\usepackage{authblk}
\usepackage[title]{appendix}
\usepackage{caption}
\usepackage{extarrows}
\usepackage{comment}
\usepackage{booktabs} % To thicken table lines
% \usepackage{multirow}
\usepackage{makecell, multirow}
%automatic sorting/compression of citations
% noadjust -- to prevent automatic adding of ~ before \cite{}
%\usepackage[noadjust]{cite}


% amsmath is for align, multline env's.
%  -- cmex10 option directs TeX to use rescaled cmex10 for cmex7-9 fonts.
%  	This option is highly recommended by IEEEtran because older systems
%  	did not include Type1 font definitions for cmex7-9 fonts. However, on my
%  	systems it seems that DVIPS is instructed by 
%  	/usr/share/texmf-texlive/fonts/map/dvips/cmex/ttcmex.map:
%  		cmex7 TeX-cmex7 <fmex7.pfb
%		cmex8 TeX-cmex8 <fmex8.pfb
%		cmex9 TeX-cmex9 <fmex9.pfb
%	Thus, I _DO NOT_ need cmex10 option
%\usepackage[cmex10]{amsmath}
\usepackage{mathrsfs}
% AMSMath was so ample as to prohibit usage of \over, so we undo it
\makeatletter
\let\over=\@@over \let\overwithdelims=\@@overwithdelims
\let\atop=\@@atop \let\atopwithdelims=\@@atopwithdelims
\let\above=\@@above \let\abovewithdelims=\@@abovewithdelims
\makeatother
% Also, note that the amsmath package sets \interdisplaylinepenalty to 10000
% thus preventing page breaks from occurring within multiline equations. Use:
\interdisplaylinepenalty=10000
% after loading amsmath to restore such page breaks as IEEEtran.cls normally
% does. 





\usepackage{rotating}
% \usepackage{multirow}

%\usepackage{stfloats}
% stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e
% the ability to do double column floats at the bottom of the page as well
% as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in
% LaTeX2e). It also provides a command:
%\fnbelowfloat
% to enable the placement of footnotes below bottom floats (the standard
% LaTeX2e kernel puts them above bottom floats). This is an invasive package
% which rewrites many portions of the LaTeX2e float routines. It may not work
% with other packages that modify the LaTeX2e float routines. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/tex-archive/macros/latex/contrib/sttools/
% Documentation is contained in the stfloats.sty comments as well as in the
% presfull.pdf file. Do not use the stfloats baselinefloat ability as IEEE
% does not allow \baselineskip to stretch. Authors submitting work to the
% IEEE should note that IEEE rarely uses double column equations and
% that authors should try to avoid such use. Do not be tempted to use the
% cuted.sty or midfloat.sty packages (also by Sigitas Tolusis) as IEEE does
% not format its papers in such ways.

% correct bad hypheion here
%\hyphenation{op-tical net-works semi-conduc-tor}





%
\usepackage{ifpdf}

\usepackage{psfrag}

\usepackage{prettyref}
%\usepackage{enumitem}
%\usepackage[showerrors,table,dvipsnames*, svgnames*]{xcolor}


\usepackage{tikz}
\usetikzlibrary{arrows}
\tikzstyle{int}=[draw, fill=blue!20, minimum size=2em]
\tikzstyle{dot}=[circle, draw, fill=blue!20, minimum size=2em]
\tikzstyle{init} = [pin edge={to-,thin,black}]


\usepackage[%dvips,
CJKbookmarks=true,
bookmarksnumbered=true,
bookmarksopen=true,
%						bookmarks=false,
colorlinks=true,
citecolor=red,
linkcolor=blue,
anchorcolor=red,
urlcolor=blue
]{hyperref}

\usepackage[all]{xy}

\usepackage{paralist}
\usepackage{enumitem}

\usepackage{algorithm}
\usepackage{algpseudocode}

\usepackage{mathtools}
%\mathtoolsset{showonlyrefs}

\usepackage{ifthen}
\newboolean{aos}
\setboolean{aos}{FALSE}

\DeclarePairedDelimiter{\nint}\lfloor\rceil
% \DeclarePairedDelimiter{\abs}\lvert\rvert


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                                                          %%%%
%%%%                      Local defines                       %%%%
%%%%                                                          %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newcommand{\med}{\text{median}}
\newcommand{\mats}{\ensuremath{\mathcal{S}}}
\newcommand{\matc}{\ensuremath{\mathcal{C}}}
\newcommand{\matx}{\ensuremath{\mathcal{X}}}
\newcommand{\mata}{\ensuremath{\mathcal{A}}}
\newcommand{\mate}{\ensuremath{\mathcal{E}}}
\newcommand{\matu}{\ensuremath{\mathcal{U}}}
\newcommand{\matb}{\ensuremath{\mathcal{B}}}
\newcommand{\matr}{\ensuremath{\mathcal{R}}}
\newcommand{\maty}{\ensuremath{\mathcal{Y}}}
\newcommand{\matn}{\ensuremath{\mathcal{N}}}
\newcommand{\matf}{\ensuremath{\mathcal{F}}}
\newcommand{\matg}{\ensuremath{\mathcal{G}}}
\newcommand{\matp}{\ensuremath{\mathcal{P}}}
\newcommand{\matd}{\ensuremath{\mathcal{D}}}
\newcommand{\matK}{\ensuremath{\mathcal{K}}}
\newcommand{\matH}{\ensuremath{\mathcal{H}}}

\newcommand{\alx}{\textbf{\sf A}}
\newcommand{\alf}{\textbf{\sf F}}
\newcommand{\aly}{\textbf{\sf B}}
\newcommand{\alw}{\textbf{\sf W}}

\newcommand{\mymmh} {\frac{\mathsmaller M \mathsmaller - \mathsmaller 1}{\mathsmaller 2}} %%SV-apr26
\newcommand{\mymm} {{\mathsmaller M \mathsmaller - \mathsmaller 1 }} %%SV-apr26
\newcommand{\figref}[1]{Fig.~{\bf #1}}
\newcommand{\mreals}{\ensuremath{\mathbb{R}}}
\newcommand{\mconst}{\ensuremath{\mathrm{const}}}
\newcommand{\supp}{\ensuremath{\mathrm{supp}}}

\ifx\eqref\undefined
\newcommand{\eqref}[1]{~(\ref{#1})}
\fi
\ifx\mod\undefined
\def\mod{\mathop{\rm mod}}
\fi

\usepackage{bm}
\def\vect#1{\bm{#1}}
\newcommand{\transp}[1]{{#1^{\mbox{\scriptsize\rm T}}}}
\newcommand{\vecttr}[1]{{\bf #1^{\mbox{\scriptsize\rm T}}}}
\newcommand{\norm}[1]{{\left\Vert #1 \right\Vert_2}}
\newcommand{\Norm}[1]{{\Vert #1 \Vert}}

\def\eng{\fontencoding{OT1}\selectfont}
\def\yhat{{\hat y}}
\def\chat{{\hat c}}
\def\esssup{\mathop{\rm esssup}}
\def\argmin{\mathop{\rm argmin}}
\def\argmax{\mathop{\rm argmax}}
\def\dim{\mathop{\rm dim}}
\def\wt{\mathop{\rm wt}}
\def\exp{\mathop{\rm exp}}
\def\lspan{\mathop{\rm span}}
\def\tr{\mathop{\rm tr}}
\def\rank{\mathop{\rm rank}}
\def\cov{\mathop{\rm cov}}
\def\MM{{\bf\rm M}}
\def\EE{\Expect}
\DeclareMathOperator\sign{\rm sign}
\def\LVar{\mathbb{L}\,}
\def\Var{\mathrm{Var}}
\def\Cov{\mathrm{Cov}}
\def\DD{{\bf\rm D}}
\def\wth{\mathop{\rm wt}}
\def\PP{\mathbb{P}}
\def\FF{\mathbb{F}}
\def\QQ{\mathbb{Q}}
\def\vchat{\vect{\hat c}}
\def\vctil{\vect{\tilde c}}
\def\vectx{\vect{x}}
\def\vdelta{\vect{\delta}}
\def\vdeltil{\tilde \delta}
\def\vecty{\vect{y}}
\def\diag{\mathop{\rm diag}}
\def\eig{\mathop{\rm eig}}
\def\follows{\Longrightarrow}
\def\equiva{\Leftrightarrow}
\def\equival{\Longleftrightarrow}
%\def\eqdef{\stackrel{\triangle}{=}}
\def\eqdef{\triangleq}
\def\dd{\partial}
\def\upto{\nearrow}
\def\downto{\searrow}

\def\capf{\mathsf{C}}
\def\veef{\mathsf{V}}
\def\Leb{\mathrm{Leb}}
\def\simiid{\stackrel{iid}{\sim}}

%\def\co{{\mathrm{co}}}


\def\gacap#1{{1\over 2} \log\left(1+{#1}\right)}



%%%%%%%%%%%%%%%%%%%%%%%%%%% by Soham %%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\scr}[1]{\mathscr{#1}}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\trm}{\calM}
\newcommand{\newrisk}[1]{U_{#1}}
\newcommand{\mymat}{M}


%%% Bordermatrices with square brackets %%%


\makeatletter
\def\bbordermatrix#1{\begingroup \m@th
	\@tempdima 4.75\p@
	\setbox\z@\vbox{%
		\def\cr{\crcr\noalign{\kern2\p@\global\let\cr\endline}}%
		\ialign{$##$\hfil\kern2\p@\kern\@tempdima&\thinspace\hfil$##$\hfil
			&&\quad\hfil$##$\hfil\crcr
			\omit\strut\hfil\crcr\noalign{\kern-\baselineskip}%
			#1\crcr\omit\strut\cr}}%
	\setbox\tw@\vbox{\unvcopy\z@\global\setbox\@ne\lastbox}%
	\setbox\tw@\hbox{\unhbox\@ne\unskip\global\setbox\@ne\lastbox}%
	\setbox\tw@\hbox{$\kern\wd\@ne\kern-\@tempdima\left[\kern-\wd\@ne
		\global\setbox\@ne\vbox{\box\@ne\kern2\p@}%
		\vcenter{\kern-\ht\@ne\unvbox\z@\kern-\baselineskip}\,\right]$}%
	\null\;\vbox{\kern\ht\@ne\box\tw@}\endgroup}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%% by Soham %%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%% by Wu %%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\M}{M}

\newcommand{\id}{\text{id}}

\newcommand{\zeros}{\mathbf{0}}
\newcommand{\ones}{\mathbf{1}}
\newcommand{\stepa}[1]{\overset{\rm (a)}{#1}}
\newcommand{\stepb}[1]{\overset{\rm (b)}{#1}}
\newcommand{\stepc}[1]{\overset{\rm (c)}{#1}}
\newcommand{\stepd}[1]{\overset{\rm (d)}{#1}}
\newcommand{\stepe}[1]{\overset{\rm (e)}{#1}}

\newcommand{\I}{\text{(I)}}
\newcommand{\II}{\text{(II)}}
\newcommand{\III}{\text{(III)}}
\newcommand{\IV}{\text{(IV)}}


%\newcommand{\ones}{\mathbf{1}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\btheta}{\vect{\theta}}
\newcommand{\Poi}{\mathrm{Poi}}
\newcommand{\subG}{\mathsf{SubG}}
\newcommand{\out}{\mathsf{out}}

\newcommand{\maxcor}{\mathrm{maxcor}}
\newcommand{\Unif}{\mathrm{Uniform}}
\newcommand{\hV}{\hat{V}}
\newcommand{\hW}{\hat{W}}
\newcommand{\cost}{\sfM}
\newcommand{\costi}{\cost^{-1}}
\newcommand{\floor}[1]{{\left\lfloor {#1} \right \rfloor}}
\newcommand{\ceil}[1]{{\left\lceil {#1} \right \rceil}}

\newcommand{\blambda}{\bar{\lambda}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\complex}{\mathbb{C}}
\newcommand{\Expect}{\mathbb{E}}
\newcommand{\expect}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\prob}[1]{\mathbb{P}\left[#1\right]}
\newcommand{\pprob}[1]{\mathbb{P}[#1]}
\newcommand{\intd}{{\rm d}}
\newcommand{\TV}{{\rm TV}}
\newcommand{\Aff}{{\rm Aff}}
\newcommand{\Mu}{M}
\newcommand{\dbar}{\bar{d}}
\newcommand{\LC}{{\sf LC}}
\newcommand{\PW}{{\sf PW}}
\newcommand{\htheta}{\hat{\theta}}
\newcommand{\eexp}{{\rm e}}
\newcommand{\expects}[2]{\mathbb{E}_{#2}\left[ #1 \right]}
\newcommand{\diff}{{\rm d}}
\newcommand{\eg}{e.g.\xspace}
\newcommand{\ie}{i.e.\xspace}
\newcommand{\iid}{iid\xspace}
\newcommand{\ind}{ind.\xspace}
\newcommand{\fracp}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\fracpk}[3]{\frac{\partial^{#3} #1}{\partial #2^{#3}}}
\newcommand{\fracd}[2]{\frac{\diff #1}{\diff #2}}
\newcommand{\fracdk}[3]{\frac{\diff^{#3} #1}{\diff #2^{#3}}}
\newcommand{\renyi}{R\'enyi\xspace}
\newcommand{\lpnorm}[1]{\left\|{#1} \right\|_{p}}
\newcommand{\linf}[1]{\left\|{#1} \right\|_{\infty}}
\newcommand{\lnorm}[2]{\left\|{#1} \right\|_{{#2}}}
\newcommand{\Lploc}[1]{L^{#1}_{\rm loc}}
\newcommand{\hellinger}{d_{\rm H}}
\newcommand{\Fnorm}[1]{\lnorm{#1}{\rm F}}
%% parenthesis
\newcommand{\pth}[1]{\left( #1 \right)}
\newcommand{\qth}[1]{\left[ #1 \right]}
\newcommand{\sth}[1]{\left\{ #1 \right\}}
\newcommand{\bpth}[1]{\Bigg( #1 \Bigg)}
\newcommand{\bqth}[1]{\Bigg[ #1 \Bigg]}
\newcommand{\bsth}[1]{\Bigg\{ #1 \Bigg\}}
\newcommand{\xxx}{\textbf{xxx}\xspace}
\newcommand{\toprob}{{\xrightarrow{\Prob}}}
\newcommand{\tolp}[1]{{\xrightarrow{L^{#1}}}}
\newcommand{\toas}{{\xrightarrow{{\rm a.s.}}}}
\newcommand{\toae}{{\xrightarrow{{\rm a.e.}}}}
\newcommand{\todistr}{{\xrightarrow{{\rm D}}}}
\newcommand{\eqdistr}{{\stackrel{\rm D}{=}}}
\newcommand{\eqlaw}{{\stackrel{\rm law}{=}}}
\newcommand{\iiddistr}{{\stackrel{\text{\iid}}{\sim}}}
\newcommand{\inddistr}{{\stackrel{\text{\ind}}{\sim}}}
\newcommand{\var}{\Var}
\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\Bern}{\text{Bern}}
\newcommand{\Binom}{\text{Binom}}
\newcommand{\Bino}{\Binom}
\newcommand{\iprod}[2]{\left \langle #1, #2 \right\rangle}
\newcommand{\Iprod}[2]{\langle #1, #2 \rangle}
\newcommand{\indc}[1]{{\mathbf{1}_{\left\{{#1}\right\}}}}
\newcommand{\Indc}{\mathbf{1}}

\definecolor{myblue}{rgb}{.8, .8, 1}
\definecolor{mathblue}{rgb}{0.2472, 0.24, 0.6} % mathematica's Color[1, 1--3]
\definecolor{mathred}{rgb}{0.6, 0.24, 0.442893}
\definecolor{mathyellow}{rgb}{0.6, 0.547014, 0.24}
\def\yp#1{\textcolor{mathyellow}{#1}}


\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}
\newcommand{\nb}[1]{{\sf\blue[#1]}}
\newcommand{\nbr}[1]{{\sf\red[#1]}}
\newcommand{\nbo}[1]{{\sf\orange[#1]}}
\newcommand{\nbwu}[1]{{\sf\red[YW: #1]}}
\newcommand{\yh}[1]{{\sf\blue[YH: #1]}}

\newcommand{\tmu}{{\tilde{\mu}}}
\newcommand{\tf}{{\tilde{f}}}
\newcommand{\tp}{\tilde{p}}
\newcommand{\tilh}{{\tilde{h}}}
\newcommand{\tu}{{\tilde{u}}}
\newcommand{\tx}{{\tilde{x}}}
\newcommand{\ty}{{\tilde{y}}}
\newcommand{\tz}{{\tilde{z}}}
\newcommand{\tA}{{\tilde{A}}}
\newcommand{\tB}{{\tilde{B}}}
\newcommand{\tC}{{\tilde{C}}}
\newcommand{\tD}{{\tilde{D}}}
\newcommand{\tE}{{\tilde{E}}}
\newcommand{\tF}{{\tilde{F}}}
\newcommand{\tG}{{\tilde{G}}}
\newcommand{\tH}{{\tilde{H}}}
\newcommand{\tI}{{\tilde{I}}}
\newcommand{\tJ}{{\tilde{J}}}
\newcommand{\tK}{{\tilde{K}}}
\newcommand{\tL}{{\tilde{L}}}
\newcommand{\tM}{{\tilde{M}}}
\newcommand{\tN}{{\tilde{N}}}
\newcommand{\tO}{{\tilde{O}}}
\newcommand{\tP}{{\tilde{P}}}
\newcommand{\tQ}{{\tilde{Q}}}
\newcommand{\tR}{{\tilde{R}}}
\newcommand{\tS}{{\tilde{S}}}
\newcommand{\tT}{{\tilde{T}}}
\newcommand{\tU}{{\tilde{U}}}
\newcommand{\tV}{{\tilde{V}}}
\newcommand{\tW}{{\tilde{W}}}
\newcommand{\tX}{{\tilde{X}}}
\newcommand{\tY}{{\tilde{Y}}}
\newcommand{\tZ}{{\tilde{Z}}}

\newcommand{\sfa}{{\mathsf{a}}}
\newcommand{\sfb}{{\mathsf{b}}}
\newcommand{\sfc}{{\mathsf{c}}}
\newcommand{\sfd}{{\mathsf{d}}}
\newcommand{\sfe}{{\mathsf{e}}}
\newcommand{\sff}{{\mathsf{f}}}
\newcommand{\sfg}{{\mathsf{g}}}
\newcommand{\sfh}{{\mathsf{h}}}
\newcommand{\sfi}{{\mathsf{i}}}
\newcommand{\sfj}{{\mathsf{j}}}
\newcommand{\sfk}{{\mathsf{k}}}
\newcommand{\sfl}{{\mathsf{l}}}
\newcommand{\sfm}{{\mathsf{m}}}
\newcommand{\sfn}{{\mathsf{n}}}
\newcommand{\sfo}{{\mathsf{o}}}
\newcommand{\sfp}{{\mathsf{p}}}
\newcommand{\sfq}{{\mathsf{q}}}
\newcommand{\sfr}{{\mathsf{r}}}
\newcommand{\sfs}{{\mathsf{s}}}
\newcommand{\sft}{{\mathsf{t}}}
\newcommand{\sfu}{{\mathsf{u}}}
\newcommand{\sfv}{{\mathsf{v}}}
\newcommand{\sfw}{{\mathsf{w}}}
\newcommand{\sfx}{{\mathsf{x}}}
\newcommand{\sfy}{{\mathsf{y}}}
\newcommand{\sfz}{{\mathsf{z}}}
\newcommand{\sfA}{{\mathsf{A}}}
\newcommand{\sfB}{{\mathsf{B}}}
\newcommand{\sfC}{{\mathsf{C}}}
\newcommand{\sfD}{{\mathsf{D}}}
\newcommand{\sfE}{{\mathsf{E}}}
\newcommand{\sfF}{{\mathsf{F}}}
\newcommand{\sfG}{{\mathsf{G}}}
\newcommand{\sfH}{{\mathsf{H}}}
\newcommand{\sfI}{{\mathsf{I}}}
\newcommand{\sfJ}{{\mathsf{J}}}
\newcommand{\sfK}{{\mathsf{K}}}
\newcommand{\sfL}{{\mathsf{L}}}
\newcommand{\sfM}{{\mathsf{M}}}
\newcommand{\sfN}{{\mathsf{N}}}
\newcommand{\sfO}{{\mathsf{O}}}
\newcommand{\sfP}{{\mathsf{P}}}
\newcommand{\sfQ}{{\mathsf{Q}}}
\newcommand{\sfR}{{\mathsf{R}}}
\newcommand{\sfS}{{\mathsf{S}}}
\newcommand{\sfT}{{\mathsf{T}}}
\newcommand{\sfU}{{\mathsf{U}}}
\newcommand{\sfV}{{\mathsf{V}}}
\newcommand{\sfW}{{\mathsf{W}}}
\newcommand{\sfX}{{\mathsf{X}}}
\newcommand{\sfY}{{\mathsf{Y}}}
\newcommand{\sfZ}{{\mathsf{Z}}}


\newcommand{\calA}{{\mathcal{A}}}
\newcommand{\calB}{{\mathcal{B}}}
\newcommand{\calC}{{\mathcal{C}}}
\newcommand{\calD}{{\mathcal{D}}}
\newcommand{\calE}{{\mathcal{E}}}
\newcommand{\calF}{{\mathcal{F}}}
\newcommand{\calG}{{\mathcal{G}}}
\newcommand{\calH}{{\mathcal{H}}}
\newcommand{\calI}{{\mathcal{I}}}
\newcommand{\calJ}{{\mathcal{J}}}
\newcommand{\calK}{{\mathcal{K}}}
\newcommand{\calL}{{\mathcal{L}}}
\newcommand{\calM}{{\mathcal{M}}}
\newcommand{\calN}{{\mathcal{N}}}
\newcommand{\calO}{{\mathcal{O}}}
\newcommand{\calP}{{\mathcal{P}}}
\newcommand{\calQ}{{\mathcal{Q}}}
\newcommand{\calR}{{\mathcal{R}}}
\newcommand{\calS}{{\mathcal{S}}}
\newcommand{\calT}{{\mathcal{T}}}
\newcommand{\calU}{{\mathcal{U}}}
\newcommand{\calV}{{\mathcal{V}}}
\newcommand{\calW}{{\mathcal{W}}}
\newcommand{\calX}{{\mathcal{X}}}
\newcommand{\calY}{{\mathcal{Y}}}
\newcommand{\calZ}{{\mathcal{Z}}}

\newcommand{\bara}{{\bar{a}}}
\newcommand{\barb}{{\bar{b}}}
\newcommand{\barc}{{\bar{c}}}
\newcommand{\bard}{{\bar{d}}}
\newcommand{\bare}{{\bar{e}}}
\newcommand{\barf}{{\bar{f}}}
\newcommand{\barg}{{\bar{g}}}
\newcommand{\barh}{{\bar{h}}}
\newcommand{\bari}{{\bar{i}}}
\newcommand{\barj}{{\bar{j}}}
\newcommand{\bark}{{\bar{k}}}
\newcommand{\barl}{{\bar{l}}}
\newcommand{\barm}{{\bar{m}}}
\newcommand{\barn}{{\bar{n}}}
%\newcommand{\baro}{{\bar{o}}}
\newcommand{\barp}{{\bar{p}}}
\newcommand{\barq}{{\bar{q}}}
\newcommand{\barr}{{\bar{r}}}
\newcommand{\bars}{{\bar{s}}}
\newcommand{\bart}{{\bar{t}}}
\newcommand{\baru}{{\bar{u}}}
\newcommand{\barv}{{\bar{v}}}
\newcommand{\barw}{{\bar{w}}}
\newcommand{\barx}{{\bar{x}}}
\newcommand{\bary}{{\bar{y}}}
\newcommand{\barz}{{\bar{z}}}
\newcommand{\barA}{{\bar{A}}}
\newcommand{\barB}{{\bar{B}}}
\newcommand{\barC}{{\bar{C}}}
\newcommand{\barD}{{\bar{D}}}
\newcommand{\barE}{{\bar{E}}}
\newcommand{\barF}{{\bar{F}}}
\newcommand{\barG}{{\bar{G}}}
\newcommand{\barH}{{\bar{H}}}
\newcommand{\barI}{{\bar{I}}}
\newcommand{\barJ}{{\bar{J}}}
\newcommand{\barK}{{\bar{K}}}
\newcommand{\barL}{{\bar{L}}}
\newcommand{\barM}{{\bar{M}}}
\newcommand{\barN}{{\bar{N}}}
\newcommand{\barO}{{\bar{O}}}
\newcommand{\barP}{{\bar{P}}}
\newcommand{\barQ}{{\bar{Q}}}
\newcommand{\barR}{{\bar{R}}}
\newcommand{\barS}{{\bar{S}}}
\newcommand{\barT}{{\bar{T}}}
\newcommand{\barU}{{\bar{U}}}
\newcommand{\barV}{{\bar{V}}}
\newcommand{\barW}{{\bar{W}}}
\newcommand{\barX}{{\bar{X}}}
\newcommand{\barY}{{\bar{Y}}}
\newcommand{\barZ}{{\bar{Z}}}



\newcommand{\hX}{\hat{X}}

\newcommand{\trans}{^{\rm T}}
\newcommand{\Th}{{^{\rm th}}}
\newcommand{\diverge}{\to \infty}
\newcommand{\mmse}{\mathsf{mmse}}

% for prettyref
\newrefformat{eq}{(\ref{#1})}
\newrefformat{thm}{Theorem~\ref{#1}}
\newrefformat{th}{Theorem~\ref{#1}}
\newrefformat{chap}{Chapter~\ref{#1}}
\newrefformat{sec}{Section~\ref{#1}}
\newrefformat{seca}{Section~\ref{#1}}
\newrefformat{algo}{Algorithm~\ref{#1}}
\newrefformat{fig}{Fig.~\ref{#1}}
\newrefformat{tab}{Table~\ref{#1}}
\newrefformat{rmk}{Remark~\ref{#1}}
\newrefformat{clm}{Claim~\ref{#1}}
\newrefformat{def}{Definition~\ref{#1}}
\newrefformat{cor}{Corollary~\ref{#1}}
\newrefformat{lmm}{Lemma~\ref{#1}}
\newrefformat{prop}{Proposition~\ref{#1}}
\newrefformat{pr}{Proposition~\ref{#1}}
\newrefformat{property}{Property~\ref{#1}}
\newrefformat{app}{Appendix~\ref{#1}}
\newrefformat{apx}{Appendix~\ref{#1}}
\newrefformat{ex}{Example~\ref{#1}}
\newrefformat{exer}{Exercise~\ref{#1}}
\newrefformat{soln}{Solution~\ref{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% by Wu %%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\unifto{\mathop{{\mskip 3mu plus 2mu minus 1mu%
			\setbox0=\hbox{$\mathchar"3221$}%
			\raise.6ex\copy0\kern-\wd0%
			\lower0.5ex\hbox{$\mathchar"3221$}}\mskip 3mu plus 2mu minus 1mu}}

\def\ds{\displaystyle}

%% These two are defined in amssymb package
\ifx\lesssim\undefined
\def\simleq{{{\mskip 3mu plus 2mu minus 1mu%
			\setbox0=\hbox{$\mathchar"013C$}%
			\raise.2ex\copy0\kern-\wd0%
			\lower0.9ex\hbox{$\mathchar"0218$}}\mskip 3mu plus 2mu minus 1mu}}
\else
\def\simleq{\lesssim}
\fi

\ifx\gtrsim\undefined
\def\simgeq{{{\mskip 3mu plus 2mu minus 1mu%
			\setbox0=\hbox{$\mathchar"013E$}%
			\raise.2ex\copy0\kern-\wd0%
			\lower0.9ex\hbox{$\mathchar"0218$}}\mskip 3mu plus 2mu minus 1mu}}
\else
\def\simgeq{\gtrsim}
\fi


% beautiful system of 2 alternatives preceded by {
	\newcommand{\systalt}[4]{\left\{%
		\vcenter{%
			\hbox{%
				\vbox{\hbox{$#1$}\hbox{$#3$}}%
				\quad%
				\vbox{\hbox{$#2$}\hbox{$#4$}}%
			}%
		} \right.%
	}
	\newcommand{\trisystalt}[6]{\left\{%
		\vcenter{%
			\hbox{%
				\vbox{\hbox{$#1$}\hbox{$#3$}\hbox{$#5$}}%
				\quad%
				\vbox{\hbox{$#2$}\hbox{$#4$}\hbox{$#6$}}%
			}%
		} \right.%
	}
	
	\def\tsub{\mathtt{t}}
	
	\def\dperp{\perp\!\!\!\perp}
	
	\def\delchi{\delta_{\chi^2}}
	\def\delTV{\delta_{TV}}
	
	% Macro to show off newstuff to authors
	\long\def\newstuff#1{{\color{mathred}#1}}
	
	\newtheorem{theorem}{Theorem}
	\newtheorem{lemma}[theorem]{Lemma}
	\newtheorem{corollary}[theorem]{Corollary}
	\newtheorem{coro}[theorem]{Corollary}
	\newtheorem{proposition}[theorem]{Proposition}
	\newtheorem{prop}[theorem]{Proposition}
	
	\theoremstyle{definition}
	\newtheorem{definition}{Definition}
	\newtheorem{example}{Example}
	\newtheorem{remark}{Remark}
	\newtheorem*{observation}{Observation}
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%% CONDITIONAL COMPILATION TRICK %%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%% Usage: \ifmapx TEXT \fi 
	%%%%%%%%%%%% The "TEXT" will only appear if *_apx.tex is compiled   
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%
	% Ok, all this pain is to produce the name "xxx_apx" with characters
	% of category 12, since this is what jobname expands to. What I used is the
	% trick that \string\abc produces a sequence of tokens (\,a,b,c) all of category 12, 
	% so I only need to kill the front \_12 which is what mkillslash macro doing.
	%
	%%%%%%%%%%%%
	\newif\ifmapx
	{\catcode`/=0 \catcode`\\=12/gdef/mkillslash\#1{#1}}
	\edef\jobnametmp{\expandafter\string\csname ic_apx\endcsname}
	\edef\jobnameapx{\expandafter\mkillslash\jobnametmp}
	\edef\jobnameexpand{\jobname}
	\ifx\jobnameexpand\jobnameapx
	\mapxtrue
	\else
	\mapxfalse
	\fi
	
	\long\def\apxonly#1{\ifmapx{\color{blue}#1}\fi}
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%                                                          %%%%
	%%%%                Document begins here                      %%%%
	%%%%                                                          %%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\newcommand{\Lip}{\mathop{\mathrm{Lip}}}
	\newcommand{\co}{\mathop{\mathrm{co}}}
	
	
	\newcommand{\decay}{G}
	\newcommand{\bfH}{\mathbf{H}}
	
	\newcommand{\poly}{\mathsf{poly}}
	\newcommand{\polylog}{\mathsf{polylog}}
	
	\newcommand{\Regret}{\mathsf{Regret}}
	\newcommand{\AvgRegret}{\mathsf{AvgRegret}}
	\newcommand{\AccRegret}{\mathsf{AccRegret}}
	
	\newcommand{\Red}{\mathsf{Red}}
	\newcommand{\Risk}{\mathsf{Risk}}
	
	\newcommand{\SubG}{\mathsf{SubG}}
	
	\renewcommand{\hat}{\widehat}
	\renewcommand{\tilde}{\widetilde}
	
	\renewcommand{\calO}{O}
	
	\newcommand{\Rpm}{\calR_m}
	
	\newcommand{\lss}{\mathsf{Lloyd~Subset~select}}
	
%	\newcommand{\cod}{{\sf Clustering~via~Ordered~Distances}~}
	
	\newcommand{\cod}{{\sf COD}~}
	\newcommand{\codelta}{{$\sf COD_\delta$}~}
	\newcommand{\vX}{\boldsymbol X}
	
	\newcommand{\snr}{\mathsf{SNR}}
	
	\newcommand{\enorm}{\calE^{\sf{norm}}}
	\newcommand{\econ}{\calE^{\sf{con}}}
	\newcommand{\eEigen}{\calE^{\sf{eigen}}}
	
	\newcommand{\hdp}{${\sf HDP}$}
	\newcommand{\dist}{{\sf dist}}
	\newcommand{\totdist}{{\sf totdist}}
	\newcommand{\iod}{{\sf IOD}~}
	
	\newcommand{\eord}{\calE^{\sf{ord}}}
	\newcommand{\lcomed}{$k$-medians-hybrid~}
	\newcommand{\kmed}{$k$-medians-${\ell}_1$~}
	

==> tex/Preamble.tex <==
\usepackage{float}

%\IEEEoverridecommandlockouts
% If the IEEEtran.cls has not been installed into the LaTeX system files,
% manually specify the path to it:
% \documentclass[conference]{IEEEtran}
%

\usepackage{amsthm,amsmath,amsfonts,amssymb}


\usepackage[margin=1in]{geometry}  % set the margins to 1in on all sides
\usepackage{xspace,exscale,relsize}
\usepackage{fancybox,shadow}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption} % conflict with [subfigure]
\usepackage{xcolor}
% this is for \mathfrak & better working \mathbb
% this is for \gtrsim, \lesssim symbols (redefined as \simleq, \simgeq in my_style.sty)
%\usepackage{url}
%\usepackage{authblk}
\usepackage[title]{appendix}
\usepackage{caption}
\usepackage{extarrows}
\usepackage{comment}
\usepackage{booktabs} % To thicken table lines
% \usepackage{multirow}
\usepackage{makecell, multirow}
%automatic sorting/compression of citations
% noadjust -- to prevent automatic adding of ~ before \cite{}
%\usepackage[noadjust]{cite}


% amsmath is for align, multline env's.
%  -- cmex10 option directs TeX to use rescaled cmex10 for cmex7-9 fonts.
%  	This option is highly recommended by IEEEtran because older systems
%  	did not include Type1 font definitions for cmex7-9 fonts. However, on my
%  	systems it seems that DVIPS is instructed by 
%  	/usr/share/texmf-texlive/fonts/map/dvips/cmex/ttcmex.map:
%  		cmex7 TeX-cmex7 <fmex7.pfb
%		cmex8 TeX-cmex8 <fmex8.pfb
%		cmex9 TeX-cmex9 <fmex9.pfb
%	Thus, I _DO NOT_ need cmex10 option
%\usepackage[cmex10]{amsmath}
\usepackage{mathrsfs}
% AMSMath was so ample as to prohibit usage of \over, so we undo it
\makeatletter
\let\over=\@@over \let\overwithdelims=\@@overwithdelims
\let\atop=\@@atop \let\atopwithdelims=\@@atopwithdelims
\let\above=\@@above \let\abovewithdelims=\@@abovewithdelims
\makeatother
% Also, note that the amsmath package sets \interdisplaylinepenalty to 10000
% thus preventing page breaks from occurring within multiline equations. Use:
\interdisplaylinepenalty=10000
% after loading amsmath to restore such page breaks as IEEEtran.cls normally
% does. 





\usepackage{rotating}
% \usepackage{multirow}

%\usepackage{stfloats}
% stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e
% the ability to do double column floats at the bottom of the page as well
% as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in
% LaTeX2e). It also provides a command:
%\fnbelowfloat
% to enable the placement of footnotes below bottom floats (the standard
% LaTeX2e kernel puts them above bottom floats). This is an invasive package
% which rewrites many portions of the LaTeX2e float routines. It may not work
% with other packages that modify the LaTeX2e float routines. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/tex-archive/macros/latex/contrib/sttools/
% Documentation is contained in the stfloats.sty comments as well as in the
% presfull.pdf file. Do not use the stfloats baselinefloat ability as IEEE
% does not allow \baselineskip to stretch. Authors submitting work to the
% IEEE should note that IEEE rarely uses double column equations and
% that authors should try to avoid such use. Do not be tempted to use the
% cuted.sty or midfloat.sty packages (also by Sigitas Tolusis) as IEEE does
% not format its papers in such ways.

% correct bad hypheion here
%\hyphenation{op-tical net-works semi-conduc-tor}





%
\usepackage{ifpdf}

\usepackage{psfrag}

\usepackage{prettyref}
%\usepackage{enumitem}
%\usepackage[showerrors,table,dvipsnames*, svgnames*]{xcolor}


\usepackage{tikz}
\usetikzlibrary{arrows}
\tikzstyle{int}=[draw, fill=blue!20, minimum size=2em]
\tikzstyle{dot}=[circle, draw, fill=blue!20, minimum size=2em]
\tikzstyle{init} = [pin edge={to-,thin,black}]


\usepackage[%dvips,
CJKbookmarks=true,
bookmarksnumbered=true,
bookmarksopen=true,
%						bookmarks=false,
colorlinks=true,
citecolor=red,
linkcolor=blue,
anchorcolor=red,
urlcolor=blue
]{hyperref}

\usepackage[all]{xy}

\usepackage{paralist}
\usepackage{enumitem}

\usepackage{algorithm}
\usepackage{algpseudocode}

\usepackage{mathtools}
%\mathtoolsset{showonlyrefs}

\usepackage{ifthen}
\newboolean{aos}
\setboolean{aos}{FALSE}

\DeclarePairedDelimiter{\nint}\lfloor\rceil
% \DeclarePairedDelimiter{\abs}\lvert\rvert


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                                                          %%%%
%%%%                      Local defines                       %%%%
%%%%                                                          %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newcommand{\med}{\text{median}}
\newcommand{\mats}{\ensuremath{\mathcal{S}}}
\newcommand{\matc}{\ensuremath{\mathcal{C}}}
\newcommand{\matx}{\ensuremath{\mathcal{X}}}
\newcommand{\mata}{\ensuremath{\mathcal{A}}}
\newcommand{\mate}{\ensuremath{\mathcal{E}}}
\newcommand{\matu}{\ensuremath{\mathcal{U}}}
\newcommand{\matb}{\ensuremath{\mathcal{B}}}
\newcommand{\matr}{\ensuremath{\mathcal{R}}}
\newcommand{\maty}{\ensuremath{\mathcal{Y}}}
\newcommand{\matn}{\ensuremath{\mathcal{N}}}
\newcommand{\matf}{\ensuremath{\mathcal{F}}}
\newcommand{\matg}{\ensuremath{\mathcal{G}}}
\newcommand{\matp}{\ensuremath{\mathcal{P}}}
\newcommand{\matd}{\ensuremath{\mathcal{D}}}
\newcommand{\matK}{\ensuremath{\mathcal{K}}}
\newcommand{\matH}{\ensuremath{\mathcal{H}}}

\newcommand{\alx}{\textbf{\sf A}}
\newcommand{\alf}{\textbf{\sf F}}
\newcommand{\aly}{\textbf{\sf B}}
\newcommand{\alw}{\textbf{\sf W}}

\newcommand{\mymmh} {\frac{\mathsmaller M \mathsmaller - \mathsmaller 1}{\mathsmaller 2}} %%SV-apr26
\newcommand{\mymm} {{\mathsmaller M \mathsmaller - \mathsmaller 1 }} %%SV-apr26
\newcommand{\figref}[1]{Fig.~{\bf #1}}
\newcommand{\mreals}{\ensuremath{\mathbb{R}}}
\newcommand{\mconst}{\ensuremath{\mathrm{const}}}
\newcommand{\supp}{\ensuremath{\mathrm{supp}}}

\ifx\eqref\undefined
\newcommand{\eqref}[1]{~(\ref{#1})}
\fi
\ifx\mod\undefined
\def\mod{\mathop{\rm mod}}
\fi

\usepackage{bm}
\def\vect#1{\bm{#1}}
\newcommand{\transp}[1]{{#1^{\mbox{\scriptsize\rm T}}}}
\newcommand{\vecttr}[1]{{\bf #1^{\mbox{\scriptsize\rm T}}}}
\newcommand{\norm}[1]{{\left\Vert #1 \right\Vert_2}}
\newcommand{\Norm}[1]{{\Vert #1 \Vert}}

\def\eng{\fontencoding{OT1}\selectfont}
\def\yhat{{\hat y}}
\def\chat{{\hat c}}
\def\esssup{\mathop{\rm esssup}}
\def\argmin{\mathop{\rm argmin}}
\def\argmax{\mathop{\rm argmax}}
\def\dim{\mathop{\rm dim}}
\def\wt{\mathop{\rm wt}}
\def\exp{\mathop{\rm exp}}
\def\lspan{\mathop{\rm span}}
\def\tr{\mathop{\rm tr}}
\def\rank{\mathop{\rm rank}}
\def\cov{\mathop{\rm cov}}
\def\MM{{\bf\rm M}}
\def\EE{\Expect}
\DeclareMathOperator\sign{\rm sign}
\def\LVar{\mathbb{L}\,}
\def\Var{\mathrm{Var}}
\def\Cov{\mathrm{Cov}}
\def\DD{{\bf\rm D}}
\def\wth{\mathop{\rm wt}}
\def\PP{\mathbb{P}}
\def\FF{\mathbb{F}}
\def\QQ{\mathbb{Q}}
\def\vchat{\vect{\hat c}}
\def\vctil{\vect{\tilde c}}
\def\vectx{\vect{x}}
\def\vdelta{\vect{\delta}}
\def\vdeltil{\tilde \delta}
\def\vecty{\vect{y}}
\def\diag{\mathop{\rm diag}}
\def\eig{\mathop{\rm eig}}
\def\follows{\Longrightarrow}
\def\equiva{\Leftrightarrow}
\def\equival{\Longleftrightarrow}
%\def\eqdef{\stackrel{\triangle}{=}}
\def\eqdef{\triangleq}
\def\dd{\partial}
\def\upto{\nearrow}
\def\downto{\searrow}

\def\capf{\mathsf{C}}
\def\veef{\mathsf{V}}
\def\Leb{\mathrm{Leb}}
\def\simiid{\stackrel{iid}{\sim}}

%\def\co{{\mathrm{co}}}


\def\gacap#1{{1\over 2} \log\left(1+{#1}\right)}



%%%%%%%%%%%%%%%%%%%%%%%%%%% by Soham %%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\scr}[1]{\mathscr{#1}}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\trm}{\calM}
\newcommand{\newrisk}[1]{U_{#1}}
\newcommand{\mymat}{M}


%%% Bordermatrices with square brackets %%%


\makeatletter
\def\bbordermatrix#1{\begingroup \m@th
	\@tempdima 4.75\p@
	\setbox\z@\vbox{%
		\def\cr{\crcr\noalign{\kern2\p@\global\let\cr\endline}}%
		\ialign{$##$\hfil\kern2\p@\kern\@tempdima&\thinspace\hfil$##$\hfil
			&&\quad\hfil$##$\hfil\crcr
			\omit\strut\hfil\crcr\noalign{\kern-\baselineskip}%
			#1\crcr\omit\strut\cr}}%
	\setbox\tw@\vbox{\unvcopy\z@\global\setbox\@ne\lastbox}%
	\setbox\tw@\hbox{\unhbox\@ne\unskip\global\setbox\@ne\lastbox}%
	\setbox\tw@\hbox{$\kern\wd\@ne\kern-\@tempdima\left[\kern-\wd\@ne
		\global\setbox\@ne\vbox{\box\@ne\kern2\p@}%
		\vcenter{\kern-\ht\@ne\unvbox\z@\kern-\baselineskip}\,\right]$}%
	\null\;\vbox{\kern\ht\@ne\box\tw@}\endgroup}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%% by Soham %%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%% by Wu %%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\M}{M}

\newcommand{\id}{\text{id}}

\newcommand{\zeros}{\mathbf{0}}
\newcommand{\ones}{\mathbf{1}}
\newcommand{\stepa}[1]{\overset{\rm (a)}{#1}}
\newcommand{\stepb}[1]{\overset{\rm (b)}{#1}}
\newcommand{\stepc}[1]{\overset{\rm (c)}{#1}}
\newcommand{\stepd}[1]{\overset{\rm (d)}{#1}}
\newcommand{\stepe}[1]{\overset{\rm (e)}{#1}}

\newcommand{\I}{\text{(I)}}
\newcommand{\II}{\text{(II)}}
\newcommand{\III}{\text{(III)}}
\newcommand{\IV}{\text{(IV)}}


%\newcommand{\ones}{\mathbf{1}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\btheta}{\vect{\theta}}
\newcommand{\Poi}{\mathrm{Poi}}
\newcommand{\subG}{\mathsf{SubG}}
\newcommand{\out}{\mathsf{out}}

\newcommand{\maxcor}{\mathrm{maxcor}}
\newcommand{\Unif}{\mathrm{Uniform}}
\newcommand{\hV}{\hat{V}}
\newcommand{\hW}{\hat{W}}
\newcommand{\cost}{\sfM}
\newcommand{\costi}{\cost^{-1}}
\newcommand{\floor}[1]{{\left\lfloor {#1} \right \rfloor}}
\newcommand{\ceil}[1]{{\left\lceil {#1} \right \rceil}}

\newcommand{\blambda}{\bar{\lambda}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\complex}{\mathbb{C}}
\newcommand{\Expect}{\mathbb{E}}
\newcommand{\expect}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\prob}[1]{\mathbb{P}\left[#1\right]}
\newcommand{\pprob}[1]{\mathbb{P}[#1]}
\newcommand{\intd}{{\rm d}}
\newcommand{\TV}{{\rm TV}}
\newcommand{\Aff}{{\rm Aff}}
\newcommand{\Mu}{M}
\newcommand{\dbar}{\bar{d}}
\newcommand{\LC}{{\sf LC}}
\newcommand{\PW}{{\sf PW}}
\newcommand{\htheta}{\hat{\theta}}
\newcommand{\eexp}{{\rm e}}
\newcommand{\expects}[2]{\mathbb{E}_{#2}\left[ #1 \right]}
\newcommand{\diff}{{\rm d}}
\newcommand{\eg}{e.g.\xspace}
\newcommand{\ie}{i.e.\xspace}
\newcommand{\iid}{iid\xspace}
\newcommand{\ind}{ind.\xspace}
\newcommand{\fracp}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\fracpk}[3]{\frac{\partial^{#3} #1}{\partial #2^{#3}}}
\newcommand{\fracd}[2]{\frac{\diff #1}{\diff #2}}
\newcommand{\fracdk}[3]{\frac{\diff^{#3} #1}{\diff #2^{#3}}}
\newcommand{\renyi}{R\'enyi\xspace}
\newcommand{\lpnorm}[1]{\left\|{#1} \right\|_{p}}
\newcommand{\linf}[1]{\left\|{#1} \right\|_{\infty}}
\newcommand{\lnorm}[2]{\left\|{#1} \right\|_{{#2}}}
\newcommand{\Lploc}[1]{L^{#1}_{\rm loc}}
\newcommand{\hellinger}{d_{\rm H}}
\newcommand{\Fnorm}[1]{\lnorm{#1}{\rm F}}
%% parenthesis
\newcommand{\pth}[1]{\left( #1 \right)}
\newcommand{\qth}[1]{\left[ #1 \right]}
\newcommand{\sth}[1]{\left\{ #1 \right\}}
\newcommand{\bpth}[1]{\Bigg( #1 \Bigg)}
\newcommand{\bqth}[1]{\Bigg[ #1 \Bigg]}
\newcommand{\bsth}[1]{\Bigg\{ #1 \Bigg\}}
\newcommand{\xxx}{\textbf{xxx}\xspace}
\newcommand{\toprob}{{\xrightarrow{\Prob}}}
\newcommand{\tolp}[1]{{\xrightarrow{L^{#1}}}}
\newcommand{\toas}{{\xrightarrow{{\rm a.s.}}}}
\newcommand{\toae}{{\xrightarrow{{\rm a.e.}}}}
\newcommand{\todistr}{{\xrightarrow{{\rm D}}}}
\newcommand{\eqdistr}{{\stackrel{\rm D}{=}}}
\newcommand{\eqlaw}{{\stackrel{\rm law}{=}}}
\newcommand{\iiddistr}{{\stackrel{\text{\iid}}{\sim}}}
\newcommand{\inddistr}{{\stackrel{\text{\ind}}{\sim}}}
\newcommand{\var}{\Var}
\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\Bern}{\text{Bern}}
\newcommand{\Binom}{\text{Binom}}
\newcommand{\Bino}{\Binom}
\newcommand{\iprod}[2]{\left \langle #1, #2 \right\rangle}
\newcommand{\Iprod}[2]{\langle #1, #2 \rangle}
\newcommand{\indc}[1]{{\mathbf{1}_{\left\{{#1}\right\}}}}
\newcommand{\Indc}{\mathbf{1}}

\definecolor{myblue}{rgb}{.8, .8, 1}
\definecolor{mathblue}{rgb}{0.2472, 0.24, 0.6} % mathematica's Color[1, 1--3]
\definecolor{mathred}{rgb}{0.6, 0.24, 0.442893}
\definecolor{mathyellow}{rgb}{0.6, 0.547014, 0.24}
\def\yp#1{\textcolor{mathyellow}{#1}}


\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}
\newcommand{\nb}[1]{{\sf\blue[#1]}}
\newcommand{\nbr}[1]{{\sf\red[#1]}}
\newcommand{\nbo}[1]{{\sf\orange[#1]}}
\newcommand{\nbwu}[1]{{\sf\red[YW: #1]}}
\newcommand{\yh}[1]{{\sf\blue[YH: #1]}}

\newcommand{\tmu}{{\tilde{\mu}}}
\newcommand{\tf}{{\tilde{f}}}
\newcommand{\tp}{\tilde{p}}
\newcommand{\tilh}{{\tilde{h}}}
\newcommand{\tu}{{\tilde{u}}}
\newcommand{\tx}{{\tilde{x}}}
\newcommand{\ty}{{\tilde{y}}}
\newcommand{\tz}{{\tilde{z}}}
\newcommand{\tA}{{\tilde{A}}}
\newcommand{\tB}{{\tilde{B}}}
\newcommand{\tC}{{\tilde{C}}}
\newcommand{\tD}{{\tilde{D}}}
\newcommand{\tE}{{\tilde{E}}}
\newcommand{\tF}{{\tilde{F}}}
\newcommand{\tG}{{\tilde{G}}}
\newcommand{\tH}{{\tilde{H}}}
\newcommand{\tI}{{\tilde{I}}}
\newcommand{\tJ}{{\tilde{J}}}
\newcommand{\tK}{{\tilde{K}}}
\newcommand{\tL}{{\tilde{L}}}
\newcommand{\tM}{{\tilde{M}}}
\newcommand{\tN}{{\tilde{N}}}
\newcommand{\tO}{{\tilde{O}}}
\newcommand{\tP}{{\tilde{P}}}
\newcommand{\tQ}{{\tilde{Q}}}
\newcommand{\tR}{{\tilde{R}}}
\newcommand{\tS}{{\tilde{S}}}
\newcommand{\tT}{{\tilde{T}}}
\newcommand{\tU}{{\tilde{U}}}
\newcommand{\tV}{{\tilde{V}}}
\newcommand{\tW}{{\tilde{W}}}
\newcommand{\tX}{{\tilde{X}}}
\newcommand{\tY}{{\tilde{Y}}}
\newcommand{\tZ}{{\tilde{Z}}}

\newcommand{\sfa}{{\mathsf{a}}}
\newcommand{\sfb}{{\mathsf{b}}}
\newcommand{\sfc}{{\mathsf{c}}}
\newcommand{\sfd}{{\mathsf{d}}}
\newcommand{\sfe}{{\mathsf{e}}}
\newcommand{\sff}{{\mathsf{f}}}
\newcommand{\sfg}{{\mathsf{g}}}
\newcommand{\sfh}{{\mathsf{h}}}
\newcommand{\sfi}{{\mathsf{i}}}
\newcommand{\sfj}{{\mathsf{j}}}
\newcommand{\sfk}{{\mathsf{k}}}
\newcommand{\sfl}{{\mathsf{l}}}
\newcommand{\sfm}{{\mathsf{m}}}
\newcommand{\sfn}{{\mathsf{n}}}
\newcommand{\sfo}{{\mathsf{o}}}
\newcommand{\sfp}{{\mathsf{p}}}
\newcommand{\sfq}{{\mathsf{q}}}
\newcommand{\sfr}{{\mathsf{r}}}
\newcommand{\sfs}{{\mathsf{s}}}
\newcommand{\sft}{{\mathsf{t}}}
\newcommand{\sfu}{{\mathsf{u}}}
\newcommand{\sfv}{{\mathsf{v}}}
\newcommand{\sfw}{{\mathsf{w}}}
\newcommand{\sfx}{{\mathsf{x}}}
\newcommand{\sfy}{{\mathsf{y}}}
\newcommand{\sfz}{{\mathsf{z}}}
\newcommand{\sfA}{{\mathsf{A}}}
\newcommand{\sfB}{{\mathsf{B}}}
\newcommand{\sfC}{{\mathsf{C}}}
\newcommand{\sfD}{{\mathsf{D}}}
\newcommand{\sfE}{{\mathsf{E}}}
\newcommand{\sfF}{{\mathsf{F}}}
\newcommand{\sfG}{{\mathsf{G}}}
\newcommand{\sfH}{{\mathsf{H}}}
\newcommand{\sfI}{{\mathsf{I}}}
\newcommand{\sfJ}{{\mathsf{J}}}
\newcommand{\sfK}{{\mathsf{K}}}
\newcommand{\sfL}{{\mathsf{L}}}
\newcommand{\sfM}{{\mathsf{M}}}
\newcommand{\sfN}{{\mathsf{N}}}
\newcommand{\sfO}{{\mathsf{O}}}
\newcommand{\sfP}{{\mathsf{P}}}
\newcommand{\sfQ}{{\mathsf{Q}}}
\newcommand{\sfR}{{\mathsf{R}}}
\newcommand{\sfS}{{\mathsf{S}}}
\newcommand{\sfT}{{\mathsf{T}}}
\newcommand{\sfU}{{\mathsf{U}}}
\newcommand{\sfV}{{\mathsf{V}}}
\newcommand{\sfW}{{\mathsf{W}}}
\newcommand{\sfX}{{\mathsf{X}}}
\newcommand{\sfY}{{\mathsf{Y}}}
\newcommand{\sfZ}{{\mathsf{Z}}}


\newcommand{\calA}{{\mathcal{A}}}
\newcommand{\calB}{{\mathcal{B}}}
\newcommand{\calC}{{\mathcal{C}}}
\newcommand{\calD}{{\mathcal{D}}}
\newcommand{\calE}{{\mathcal{E}}}
\newcommand{\calF}{{\mathcal{F}}}
\newcommand{\calG}{{\mathcal{G}}}
\newcommand{\calH}{{\mathcal{H}}}
\newcommand{\calI}{{\mathcal{I}}}
\newcommand{\calJ}{{\mathcal{J}}}
\newcommand{\calK}{{\mathcal{K}}}
\newcommand{\calL}{{\mathcal{L}}}
\newcommand{\calM}{{\mathcal{M}}}
\newcommand{\calN}{{\mathcal{N}}}
\newcommand{\calO}{{\mathcal{O}}}
\newcommand{\calP}{{\mathcal{P}}}
\newcommand{\calQ}{{\mathcal{Q}}}
\newcommand{\calR}{{\mathcal{R}}}
\newcommand{\calS}{{\mathcal{S}}}
\newcommand{\calT}{{\mathcal{T}}}
\newcommand{\calU}{{\mathcal{U}}}
\newcommand{\calV}{{\mathcal{V}}}
\newcommand{\calW}{{\mathcal{W}}}
\newcommand{\calX}{{\mathcal{X}}}
\newcommand{\calY}{{\mathcal{Y}}}
\newcommand{\calZ}{{\mathcal{Z}}}

\newcommand{\bara}{{\bar{a}}}
\newcommand{\barb}{{\bar{b}}}
\newcommand{\barc}{{\bar{c}}}
\newcommand{\bard}{{\bar{d}}}
\newcommand{\bare}{{\bar{e}}}
\newcommand{\barf}{{\bar{f}}}
\newcommand{\barg}{{\bar{g}}}
\newcommand{\barh}{{\bar{h}}}
\newcommand{\bari}{{\bar{i}}}
\newcommand{\barj}{{\bar{j}}}
\newcommand{\bark}{{\bar{k}}}
\newcommand{\barl}{{\bar{l}}}
\newcommand{\barm}{{\bar{m}}}
\newcommand{\barn}{{\bar{n}}}
%\newcommand{\baro}{{\bar{o}}}
\newcommand{\barp}{{\bar{p}}}
\newcommand{\barq}{{\bar{q}}}
\newcommand{\barr}{{\bar{r}}}
\newcommand{\bars}{{\bar{s}}}
\newcommand{\bart}{{\bar{t}}}
\newcommand{\baru}{{\bar{u}}}
\newcommand{\barv}{{\bar{v}}}
\newcommand{\barw}{{\bar{w}}}
\newcommand{\barx}{{\bar{x}}}
\newcommand{\bary}{{\bar{y}}}
\newcommand{\barz}{{\bar{z}}}
\newcommand{\barA}{{\bar{A}}}
\newcommand{\barB}{{\bar{B}}}
\newcommand{\barC}{{\bar{C}}}
\newcommand{\barD}{{\bar{D}}}
\newcommand{\barE}{{\bar{E}}}
\newcommand{\barF}{{\bar{F}}}
\newcommand{\barG}{{\bar{G}}}
\newcommand{\barH}{{\bar{H}}}
\newcommand{\barI}{{\bar{I}}}
\newcommand{\barJ}{{\bar{J}}}
\newcommand{\barK}{{\bar{K}}}
\newcommand{\barL}{{\bar{L}}}
\newcommand{\barM}{{\bar{M}}}
\newcommand{\barN}{{\bar{N}}}
\newcommand{\barO}{{\bar{O}}}
\newcommand{\barP}{{\bar{P}}}
\newcommand{\barQ}{{\bar{Q}}}
\newcommand{\barR}{{\bar{R}}}
\newcommand{\barS}{{\bar{S}}}
\newcommand{\barT}{{\bar{T}}}
\newcommand{\barU}{{\bar{U}}}
\newcommand{\barV}{{\bar{V}}}
\newcommand{\barW}{{\bar{W}}}
\newcommand{\barX}{{\bar{X}}}
\newcommand{\barY}{{\bar{Y}}}
\newcommand{\barZ}{{\bar{Z}}}



\newcommand{\hX}{\hat{X}}

\newcommand{\trans}{^{\rm T}}
\newcommand{\Th}{{^{\rm th}}}
\newcommand{\diverge}{\to \infty}
\newcommand{\mmse}{\mathsf{mmse}}

% for prettyref
\newrefformat{eq}{(\ref{#1})}
\newrefformat{thm}{Theorem~\ref{#1}}
\newrefformat{th}{Theorem~\ref{#1}}
\newrefformat{chap}{Chapter~\ref{#1}}
\newrefformat{sec}{Section~\ref{#1}}
\newrefformat{seca}{Section~\ref{#1}}
\newrefformat{algo}{Algorithm~\ref{#1}}
\newrefformat{fig}{Fig.~\ref{#1}}
\newrefformat{tab}{Table~\ref{#1}}
\newrefformat{rmk}{Remark~\ref{#1}}
\newrefformat{clm}{Claim~\ref{#1}}
\newrefformat{def}{Definition~\ref{#1}}
\newrefformat{cor}{Corollary~\ref{#1}}
\newrefformat{lmm}{Lemma~\ref{#1}}
\newrefformat{prop}{Proposition~\ref{#1}}
\newrefformat{pr}{Proposition~\ref{#1}}
\newrefformat{property}{Property~\ref{#1}}
\newrefformat{app}{Appendix~\ref{#1}}
\newrefformat{apx}{Appendix~\ref{#1}}
\newrefformat{ex}{Example~\ref{#1}}
\newrefformat{exer}{Exercise~\ref{#1}}
\newrefformat{soln}{Solution~\ref{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% by Wu %%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\unifto{\mathop{{\mskip 3mu plus 2mu minus 1mu%
			\setbox0=\hbox{$\mathchar"3221$}%
			\raise.6ex\copy0\kern-\wd0%
			\lower0.5ex\hbox{$\mathchar"3221$}}\mskip 3mu plus 2mu minus 1mu}}

\def\ds{\displaystyle}

%% These two are defined in amssymb package
\ifx\lesssim\undefined
\def\simleq{{{\mskip 3mu plus 2mu minus 1mu%
			\setbox0=\hbox{$\mathchar"013C$}%
			\raise.2ex\copy0\kern-\wd0%
			\lower0.9ex\hbox{$\mathchar"0218$}}\mskip 3mu plus 2mu minus 1mu}}
\else
\def\simleq{\lesssim}
\fi

\ifx\gtrsim\undefined
\def\simgeq{{{\mskip 3mu plus 2mu minus 1mu%
			\setbox0=\hbox{$\mathchar"013E$}%
			\raise.2ex\copy0\kern-\wd0%
			\lower0.9ex\hbox{$\mathchar"0218$}}\mskip 3mu plus 2mu minus 1mu}}
\else
\def\simgeq{\gtrsim}
\fi


% beautiful system of 2 alternatives preceded by {
	\newcommand{\systalt}[4]{\left\{%
		\vcenter{%
			\hbox{%
				\vbox{\hbox{$#1$}\hbox{$#3$}}%
				\quad%
				\vbox{\hbox{$#2$}\hbox{$#4$}}%
			}%
		} \right.%
	}
	\newcommand{\trisystalt}[6]{\left\{%
		\vcenter{%
			\hbox{%
				\vbox{\hbox{$#1$}\hbox{$#3$}\hbox{$#5$}}%
				\quad%
				\vbox{\hbox{$#2$}\hbox{$#4$}\hbox{$#6$}}%
			}%
		} \right.%
	}
	
	\def\tsub{\mathtt{t}}
	
	\def\dperp{\perp\!\!\!\perp}
	
	\def\delchi{\delta_{\chi^2}}
	\def\delTV{\delta_{TV}}
	
	% Macro to show off newstuff to authors
	\long\def\newstuff#1{{\color{mathred}#1}}
	
	\newtheorem{theorem}{Theorem}
	\newtheorem{lemma}[theorem]{Lemma}
	\newtheorem{corollary}[theorem]{Corollary}
	\newtheorem{coro}[theorem]{Corollary}
	\newtheorem{proposition}[theorem]{Proposition}
	\newtheorem{prop}[theorem]{Proposition}
	
	\theoremstyle{definition}
	\newtheorem{definition}{Definition}
	\newtheorem{example}{Example}
	\newtheorem{remark}{Remark}
	\newtheorem*{observation}{Observation}
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%% CONDITIONAL COMPILATION TRICK %%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%% Usage: \ifmapx TEXT \fi 
	%%%%%%%%%%%% The "TEXT" will only appear if *_apx.tex is compiled   
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%
	% Ok, all this pain is to produce the name "xxx_apx" with characters
	% of category 12, since this is what jobname expands to. What I used is the
	% trick that \string\abc produces a sequence of tokens (\,a,b,c) all of category 12, 
	% so I only need to kill the front \_12 which is what mkillslash macro doing.
	%
	%%%%%%%%%%%%
	\newif\ifmapx
	{\catcode`/=0 \catcode`\\=12/gdef/mkillslash\#1{#1}}
	\edef\jobnametmp{\expandafter\string\csname ic_apx\endcsname}
	\edef\jobnameapx{\expandafter\mkillslash\jobnametmp}
	\edef\jobnameexpand{\jobname}
	\ifx\jobnameexpand\jobnameapx
	\mapxtrue
	\else
	\mapxfalse
	\fi
	
	\long\def\apxonly#1{\ifmapx{\color{blue}#1}\fi}
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%                                                          %%%%
	%%%%                Document begins here                      %%%%
	%%%%                                                          %%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\newcommand{\Lip}{\mathop{\mathrm{Lip}}}
	\newcommand{\co}{\mathop{\mathrm{co}}}
	
	
	\newcommand{\decay}{G}
	\newcommand{\bfH}{\mathbf{H}}
	
	\newcommand{\poly}{\mathsf{poly}}
	\newcommand{\polylog}{\mathsf{polylog}}
	
	\newcommand{\Regret}{\mathsf{Regret}}
	\newcommand{\AvgRegret}{\mathsf{AvgRegret}}
	\newcommand{\AccRegret}{\mathsf{AccRegret}}
	
	\newcommand{\Red}{\mathsf{Red}}
	\newcommand{\Risk}{\mathsf{Risk}}
	
	\newcommand{\SubG}{\mathsf{SubG}}
	
	\renewcommand{\hat}{\widehat}
	\renewcommand{\tilde}{\widetilde}
	
	\renewcommand{\calO}{O}
	
	\newcommand{\Rpm}{\calR_m}
	
	\newcommand{\lss}{\mathsf{Lloyd~Subset~select}}
	
%	\newcommand{\cod}{{\sf Clustering~via~Ordered~Distances}~}
	
	\newcommand{\cod}{{\sf COD}~}
	\newcommand{\codelta}{{$\sf COD_\delta$}~}
	\newcommand{\vX}{\boldsymbol X}
	
	\newcommand{\snr}{\mathsf{SNR}}
	
	\newcommand{\enorm}{\calE^{\sf{norm}}}
	\newcommand{\econ}{\calE^{\sf{con}}}
	\newcommand{\eEigen}{\calE^{\sf{eigen}}}
	
	\newcommand{\hdpalpha}{${\sf HDP}_\alpha~$}
	\newcommand{\dist}{{\sf dist}}
	\newcommand{\totdist}{{\sf totdist}}
	\newcommand{\iod}{{\sf IOD}}
	
	\newcommand{\eord}{\calE^{\sf{ord}}}
	\newcommand{\lcomed}{$k$-medians-hybrid~}

==> tex/abstract.tex <==
\begin{abstract}
	Clustering is a fundamental tool in statistical machine learning in the presence of heterogeneous data.  Many recent results focus primarily on optimal mislabeling guarantees, when data are distributed around centroids with sub-Gaussian errors. Yet, the restrictive sub-Gaussian model is often invalid in practice, since various real-world applications exhibit heavy tail distributions around the centroids or suffer from possible adversarial attacks that call for robust clustering with a robust data-driven initialization.  In this paper, we introduce a hybrid clustering technique with a novel multivariate trimmed mean type centroid estimate to produce mislabeling guarantees under a weak initialization condition for general error distributions around the centroids. A matching lower bound is derived, up to factors depending on the number of clusters. In addition, our approach also produces the optimal mislabeling even in the presence of adversarial outliers. Our results reduce to the sub-Gaussian case when errors follow sub-Gaussian distributions.  To solve the problem thoroughly, we also present novel data-driven robust initialization techniques and show that, with probabilities approaching one, these initial centroid estimates are sufficiently good for the subsequent clustering algorithm to achieve the optimal mislabeling rates.  Furthermore, we demonstrate that the Lloyd algorithm is suboptimal for more than two clusters even when errors are Gaussian, and for two clusters when errors distributions have heavy tails.  Both simulated data and real data examples lend further support to both of our robust initialization procedure and clustering algorithm.
\end{abstract}

==> tex/app_proof_initialization.tex <==
\section{Proof of the initialization algorithms}

\subsection{Preparation}

\label{app:n_i-conc_results}

Our proofs in this section rely on the following high probability guarantees.

\begin{lemma}\label{lmm:E-conc-init-k}
	Let $\beta$ be as in either \prettyref{thm:proof-algo-2} or \prettyref{thm:proof-algo-k}. There is an event $\tilde \calE_k$ with 
	$
	\PP\qth{\tilde \calE_k}\geq 1-2ke^{-{\min_{g\in [k]} n_g^*\over 4k}}
	$
	on which the following holds:
	\begin{enumerate}[label=(\roman*)]
		\item $\abs{\calB(\theta_i,\sigma \decay^{-1}(e^{-{5\over 4\beta^2}}))\cap \sth{Y_i:i\in T_i}}\geq n_i(1-{\beta^2})$ for each $i\in [k]$,
		\item $\abs{\calB(\theta_i,{\Delta\over 16 k})\cap \sth{Y_i:i\in T_i}}\geq n_i\pth{1-{5\over 4\log\pth{1/G\pth{\Delta/ (16\sigma k)}}}}$ for each $i\in [k]$.
	\end{enumerate} 
\end{lemma}

\begin{proof}
	The proof of part (i) follows from the proof of \prettyref{lmm:E-conc-genr} by choosing $\epsilon_0^2={\sigma\over \Delta} \decay^{-1}(e^{-{5\over 4\beta^2}})$ in the lemma. The proof of part (ii) follows from the proof of \prettyref{lmm:E-conc-genr} by choosing $\epsilon_0^2=\frac 1{16k}$ in the lemma.
\end{proof}

\subsection{Proof of \prettyref{thm:proof-algo-2}}
\label{app:proof-init-2}
In the proof below, we assume that all the mentioned constants  depend on $\decay,\alpha,\sigma$, unless otherwise specified. In addition, for our entire analysis we will assume that the event $\tilde \calE$ holds, which has a high probability guarantee. We will extensively use the following definition of order statistics: Given any set $V$ of real numbers and fraction $0<p<1$, let $V^{\sth{p}}$ define the $\ceil{p|V|}$-th smallest number in $V$. The proof is a combination of the following results.

\begin{lemma}\label{lmm:centroid1}
	There is one $\theta_i$, such that $\|\theta_i-\mu_1^{(1)}\|\leq C$ for some constant $C>0$.
\end{lemma}

\begin{lemma}\label{lmm:first-jump}
	There is a stage $\ell+1$, with $\ell\geq 1$,  such that $\dist_1^{(\ell+1)}> {\Delta\over 16}$.	
\end{lemma}

\begin{lemma}\label{lmm:small-totdist}
	Suppose that $\ell=\min\sth{r\geq 1:\dist_1^{(r+1)}> {\Delta\over 16}}$. Then $\totdist_{\ell}\leq \Delta/16$.
\end{lemma}	

\begin{lemma}\label{lmm:apprx-centroid}
	If $\totdist_\ell\leq {\Delta\over 8}$, then there is a permutation $\pi$ of $\{1,2\}$ such that $$\max_{i=1,2} {\|\mu_i^{(\ell)}-\theta_{\pi(i)}\|}\leq {\Delta\over 3}.$$
\end{lemma}

\begin{proof}[Proof of \prettyref{lmm:centroid1}]
	In view of \prettyref{lmm:E-conc-init-k}, there is a constant $c_1=\sigma \decay^{-1}(e^{-{5\over 4\beta^2}})$ such that
	\begin{align}\label{eq:init1}
		|\sth{j\in [n]:Y_j\in \calB(\theta_i,c_1)}|\geq n_i\pth{1-\beta^2},\quad i\in \{1,2\}.
	\end{align}
	As we have $n_1,n_2>n\alpha$ by assumption, it follows that there is a point $Y_i$ such that 
	$$|\sth{j\in [n]:Y_j\in \calB(Y_i,2c_{1})}|\geq m_1 \geq {n\alpha\over 4}.$$
	Hence, the tightest neighborhood around any point $Y_i,i\in [n]$, that contains at least $n\alpha/4$ points from $Y_1,\dots,Y_n$, has a radius of at most $2c_{1}$ around that $Y_i$. Define
	\begin{align}\label{eq:distance}
		D({x},S)=\sth{\|x-Y_{i}\|:i\in S},\quad x\in \reals^d,S\subseteq [n].
	\end{align} 
	Let $i^*$ be one such index in $[n]$ that satisfies 
	\begin{align}
		\sth{D(Y_{i^*},[n])}^{\sth{1-\beta}} = \min_{j\in [n]} \sth{D(Y_{j},[n])}^{\sth{1-\beta}}.
	\end{align} 
	Then $\calB(Y_{i^*},2c_{1})$ and $\cup_{i=1,2}\calB(\theta_i,c_{1})$ can not be disjoint, as in view of \eqref{eq:init1} it will imply that their union will contain more than $n$ points from $Y_1,\dots,Y_n$
	\begin{align*}
		&\abs{\sth{i\in [n]:Y_i\in \calB(Y_{i^*},2c_1)}\cup\qth{\cup_{j=1,2}\sth{i\in [n]:Y_i\in \calB(\theta_j,c_1)}}}
		\nonumber\\
		&\geq m_1 + \sum_{i=1,2}n_i\pth{1-\beta^2}
		\geq n+n\pth{\frac \alpha4 - {\alpha^2\over 16}} > n,
	\end{align*}	
	where we use the fact that $\sth{i\in [n]:Y_i\in \calB(\theta_i,c_1)},i=1,2$ are disjoint sets as $\|\theta_1-\theta_2\|\geq \Delta$. Hence, $Y_{i^*}$ is at a distance at most $3c_{1}$ from one of the centroids. Without loss of we can pick $\mu_1^{(1)} = Y_{i^*}$ and we assume that $\theta_1$ is the closer to $\mu_1^{(1)}$ than $\theta_2$.	
\end{proof}



\begin{proof}[Proof of \prettyref{lmm:first-jump}]
	In view of \prettyref{lmm:centroid1}, let us assume that $\theta_1$ is the closest centroid to $\mu_1^{(1)}$ and define $c_1=\sigma \decay^{-1}(e^{-{5\over 4\beta^2}})$ as before in the proof of \prettyref{lmm:apprx-centroid} to have
	\begin{align}\label{eq:init0}
		\mu_1^{(1)}\in \calB\pth{\theta_1,3c_1},\quad 
		\abs{\{Y_j:j\in T_i\}\cap\calB\pth{\theta_i,c_1}}\geq n_i\pth{1-\beta^2},i\in \{1,2\}.
	\end{align}
	We observe the following: 
	\begin{itemize}
		\item In view of $\calB(\mu_1^{(1)},4c_1)\supset\calB(\theta_1,c_1)$ we get
		\begin{align*}
			\abs{\sth{Y_i:i\in [n]}\cap \calB(\mu_1^{(1)},4c_1)}
			\geq \abs{\sth{Y_i:i\in [n]}\cap\calB(\theta_1,c_1)}
			\geq n\alpha(1-\beta^2).
		\end{align*}
		As the size of $\calP_1^{(1)}$ is at most $m_1 \leq \ceil{n\alpha\over 4}$ the distance of $\mu_1^{(1)}$ to any point in $\calP_1^{(1)}$ is less than $4c_1$, which implies $\dist_1^{(1)}\leq {\Delta\over 16}$.
		\item At the last step, say $\tilde \ell$, in our algorithm, $\calP_1^{(\tilde \ell)}$ will have at least $n-m = n-{n\alpha^2\over 16}$ many points. In view of \eqref{eq:init0} we also have
		\begin{align*}
			|\sth{Y_j:j\in [n],Y_j\in \calB(\theta_2,c_1)}\cap \calP_1^{(\tilde\ell)}|
			&\geq
			|\sth{Y_j:j\in [n],Y_j\in \calB(\theta_2,c_1)}|-  |\overline{\calP_1^{(\tilde\ell)}}|
			\nonumber\\
			&\geq n_2\pth{1-{\beta^2}}-{n\alpha^2\over 16}
			\geq n\alpha-{n\alpha^2\over 16}-{n\alpha\beta^2}.
		\end{align*}
		\end{itemize} 
		As we have
		\begin{itemize}
			\item the tightest neighborhood in the data set around $\mu_1^{(1)}$ with a size at least $(1-\beta)|\calP_1^{(\tilde\ell)}|$, say, $N$, will include at least $(1-\beta)(n-{n\alpha^2\over 16})\geq n-{n\beta}-{n\alpha^2\over 16}$ points
			\item \eqref{eq:init0} implies that $\{Y_j:j\in T_2\}\cap\calB\pth{\theta_2,c_1}$ will contain at least ${n\alpha\over 2}$ points
		\end{itemize}
	 	we get that
	 	$$
	 	|N|+\abs{\{Y_j:j\in T_2\}\cap\calB\pth{\theta_2,c_1}} \geq n + {n\alpha\over 4}.
	 	$$ 
	 	This implies $N\cap \{Y_j: j\in T_2,\calB\pth{\theta_2,c_1}\}$ is nonempty. Suppose that $y$ is an entry in the above set. Then we have that the distance of $y$ from $\mu_1^{(\tilde\ell)}$ is at least $\Delta-4c_1$, 
		\begin{align*}
			\|\mu_1^{(\tilde\ell)}-y\|
			\geq \|\theta_1-\theta_2\|-\|\mu_1^{(\tilde\ell)}-\theta_1\|-\|\theta_2-y\|
			\geq \Delta - 4c_1.
		\end{align*}
\end{proof}

\begin{proof}[Proof of \prettyref{lmm:small-totdist}]
	Without a loss of generality we assume that $\theta_1$ is the closest centroid to $\mu_1^{(1)}$ and \eqref{eq:init0} holds for some $c_1>0$. We first prove the following claims:
	\begin{align}
		\abs{\calP_1^{(\ell)}\cap \{Y_i:i\in T_1\}}&\geq n_1-m-{5n\over 4\log(1/(G(\Delta/32\sigma)))}
		\label{eq:init-claim1}\\
		\abs{\calP_1^{(\ell)}\cap \{Y_i:i\in T_2\}}&\leq n\beta + {5n\over 4\log(1/(G(\Delta/32\sigma)))}.
		\label{eq:init-claim2}
	\end{align}
	The first claim \eqref{eq:init-claim1} follows from the following sequence of arguments
	\begin{itemize}
		\item Using $\mu_1^{(\ell)}=\mu_1^{(\ell+1)}$ we get $\dist_1^{(\ell+1)}=\sth{D(\mu_1^{(\ell)},\calP_1^{(\ell+1)})}^{\sth{1-\beta}} > {\Delta\over 16},$
		which implies 
		\begin{align}\label{eq:init6}
			\calP_1^{(\ell+1)}\supseteq \{Y_i:i\in [n]\}\cap \calB\pth{\mu_1^{(\ell)},{\Delta\over 16}}.
		\end{align}
		As we have $\calP_1^{(\ell)}\subset \calP_1^{(\ell+1)}$ and $|\calP_1^{(\ell)}|\leq |\calP_1^{(\ell+1)}|\leq |\calP_1^{(\ell)}|+m$, we get that there is a set $A\subseteq \{Y_i:i\in [n]\}$ that satisfies
		$$
		\calP_1^{(\ell)}\supseteq\calP_1^{(\ell+1)}/A,\quad |A|\leq {n\alpha^2\over 16}.
		$$
		In view of \eqref{eq:init6} the last display implies
		$$
		\calP_1^{(\ell)}\cap\{Y_i:i\in T_1\}\supseteq\calP_1^{(\ell+1)}\cap\{Y_i:i\in T_1\}/A
		\supseteq \calB\pth{\mu_1^{(\ell)},{\Delta\over 16}}\cap\{Y_i:i\in T_1\}/A,
		$$
		and hence
		\begin{align}\label{eq:init7}
			\abs{\calP_1^{(\ell)}\cap\{Y_i:i\in T_1\}}&\geq \abs{\calB\pth{\mu_1^{(\ell)},{\Delta\over 16}}\cap\{Y_i:i\in T_1\}}-|A|
			\nonumber\\
			& \geq \abs{\calB\pth{\mu_1^{(\ell)},{\Delta\over 16}}\cap\{Y_i:i\in T_1\}}-m.
		\end{align}
		
		\item As we have from \eqref{eq:init0}:
		\begin{align}
			\begin{gathered}
				\calB\pth{\mu_1^{(\ell)},{\Delta\over 16}}\supseteq \calB\pth{\theta_1,{\Delta\over 16}-3c_1}
				\supseteq \calB\pth{\theta_1,{\Delta\over 32}},
			\end{gathered}	
		\end{align}
		in view of \prettyref{lmm:E-conc-init-k}(ii) we get
		\begin{align}\label{eq:init8}
			&\abs{\calB\pth{\mu_1^{(\ell)},{\Delta\over 16}}\cap \{Y_i:i\in T_1\}}
			\geq \abs{\calB\pth{\theta_1,{\Delta\over 32}}\cap \{Y_i:i\in T_1\}}
			\nonumber\\
			&\geq n_1\pth{1-{5\over 4\log\pth{1/G\pth{\Delta\over 32\sigma}}}}
			\geq n_1-{5n\over 4\log(1/(G(\Delta/32\sigma)))}. 
		\end{align}
	\end{itemize}
	Combining \eqref{eq:init7} and \eqref{eq:init8} we get \eqref{eq:init-claim1}.
	Next, to prove the claim \eqref{eq:init-claim2}, we note that:
	\begin{itemize}
		\item In view of \prettyref{lmm:E-conc-init-k} there are at most ${5n\over 4\log(1/(G(\Delta/32\sigma)))}$ many points from $\sth{Y_i:i\in T_2}$ outside $\calB(\theta_2,{\Delta\over 32})$. As \eqref{eq:init0} implies $\calB\pth{\mu_1^{(\ell)},{\Delta\over 16}}\subseteq \calB\pth{\theta_1,{\Delta\over 16}+3c_1}$ and  $\calB(\theta_2,{\Delta\over 32})$ are disjoint, we have
		\begin{align}\label{eq:init9}
			\abs{\calP_1^{(\ell)}\cap \{Y_i:i\in T_2\}\cap \calB\pth{\mu_1^{(\ell)},{\Delta\over 16}}}
			\leq \abs{\{Y_i:i\in T_2\}/ \calB\pth{\theta_2,{\Delta\over 32}}}
			\leq {5n\over 4\log(1/(G(\Delta/32\sigma)))} .
		\end{align}
		\item On the other hand,
		$\dist_1^{(\ell)}=\sth{D(\mu_1^{(\ell)},\calP_1^{(\ell)})}^{\sth{1-\beta}}\leq {\Delta\over 16}$
		implies that
		\begin{align}\label{eq:init10}
			\abs{\calP_1^{(\ell)}\cap \{Y_i:i\in T_2\}/ \calB\pth{\mu_1^{(\ell)},{\Delta\over 16}}}\leq n\beta.
		\end{align}
	\end{itemize}
	Combining \eqref{eq:init9} and \eqref{eq:init10} we get \eqref{eq:init-claim2}.
	
	Hence, we have proven the inequalities \eqref{eq:init-claim1} and \eqref{eq:init-claim2}. These inequalities together imply
	\begin{align}
		\abs{\overline{\calP_1^{(\ell)}}\cap \{Y_i:i\in T_2\}}&\geq n_2- n\beta-{5n\over 4\log(1/(G(\Delta/32\sigma)))}
		\label{eq:init-claim3}\\
		\abs{\overline{\calP_1^{(\ell)}}\cap \{Y_i:i\in T_1\}}&\leq m +{5n\over 4\log(1/(G(\Delta/32\sigma)))}.
		\label{eq:init-claim4}
	\end{align}
	In view of $\abs{\sth{Y_i:i\in T_2}/ \calB(\theta_2,{\Delta/32})}\leq {5n\over 4\log(1/(G(\Delta/32\sigma)))}$ from \prettyref{lmm:E-conc-init-k}, we have  
	\begin{align*}
		&\abs{\overline{\calP_1^{(\ell)}}/\calB(\theta_2,{\Delta/ 32})}
		\nonumber\\
		&=\abs{\sth{\overline{\calP_1^{(\ell)}}\cap \{Y_i:i\in T_2\}/{\calB(\theta_2,{\Delta/ 32})}}
			\cup \sth{\overline{\calP_1^{(\ell)}}\cap \{Y_i:i\in T_1\}/ {\calB(\theta_2,{\Delta/ 32})}}}
		\nonumber\\
		&\leq \abs{\{Y_i:i\in T_2\}/ \sth{\calB(\theta_2,{\Delta/ 32})}}
		+ \abs{\overline{\calP_1^{(\ell)}}\cap \{Y_i:i\in T_1\}}
		\nonumber\\
		&\leq \abs{\sth{Y_i:i\in T_2}/ \calB(\theta_2,{\Delta/32})} + m +{5n\over 4\log(1/(G(\Delta/32\sigma)))}
		\nonumber\\
		&\leq  {n\alpha^2\over 16}+{5n\over 2\log(1/(G(\Delta/32\sigma)))}.
	\end{align*}
	As $\abs{\overline{\calP_1^{(\ell)}}}\geq{n\alpha}-{n\beta}-{n\alpha\over 16}\geq {11n\alpha\over 16}$ from \eqref{eq:init-claim3}, any subset of $\overline{\calP_1^{(\ell)}}$ with size ${\pth{1-\beta}|\overline{\calP_1^{(\ell)}}|}$, discards a set of size at least ${11n\alpha\beta\over 16}\geq {n\alpha^2\over 6}$. Hence the tightest subset of $\overline{\calP_1^{(\ell)}}$ with size ${\pth{1-\beta}|\overline{\calP_1^{(\ell)}}|}$ will have a diameter of at most $\Delta\over 16$. This implies $\dist_2^{(\ell)}\leq \Delta/16$.
\end{proof}

\begin{proof}[Proof of \prettyref{lmm:apprx-centroid}]
	As $\totdist_\ell\leq {\Delta\over 8}$, we have $\dist_i^{(\ell)}\leq {\Delta\over 8}$ for $i\in \{1,2\}$. First we show that both $\mu_1^{(\ell)}$ and $\mu_2^{(\ell)}$ lies in $\cup_{i=1,2}\calB(\theta_i,{\Delta/ 3})$. If not, without loss of generality let $\mu_2^{(\ell)}$ lie outside  $\cup_{i=1,2}\calB(\theta_i,\Delta/3)$. Then we have
	\begin{align}\label{eq:init3}
		\calB\pth{\mu_2^{(\ell)},{\Delta\over 8}}\cap \sth{\cup_{i\in \{1,2\}}\calB\pth{\theta_i,{\Delta\over 8}}}=\phi,.
	\end{align} 
	As we have $\dist_2^{(\ell)}\leq {\Delta\over 8}$, we get that 
	\begin{align}\label{eq:init4}
		\abs{\overline{\calP_1^{(\ell)}} \cap \calB\pth{\mu_2^{(\ell)},{\Delta\over 8}}}\geq \pth{1-\frac \alpha4}\abs{\overline{\calP_1^{(\ell)}}}.
	\end{align}
	Using \prettyref{lmm:E-conc-init-k} we get that 
	\begin{align}\label{eq:init5}
		\abs{\{Y_i:i\in [n]\}/ \sth{\cup_{i\in \{1,2\}}\calB\pth{\theta_i,{\Delta\over 8}}}}\leq {5n\over 4\log(1/(G(\Delta/32\sigma)))}.
	\end{align}
	In view of the last display, using \eqref{eq:init3} and\eqref{eq:init4} we get
	\begin{align*}
		\abs{\overline{\calP_1^{(\ell)}}}
		&\leq \frac 1{1-\beta}\abs{\overline{\calP_1^{(\ell)}} \cap \calB\pth{\mu_2^{(\ell)},{\Delta\over 8}}}
		\nonumber\\
		&\leq \frac 1{1-\beta}
		\abs{\{Y_i:i\in [n]\}/ \sth{\cup_{i\in \{1,2\}}\calB\pth{\theta_i,{\Delta\over 8}}}}
		\leq {5n\over 2\log(1/(G(\Delta/32\sigma)))}.
	\end{align*}
	The last display implies 
	$$
	|{\calP_1^{(\ell)}}|\geq n-{5n\over 2\log(1/(G(\Delta/32\sigma)))}.
	$$ 
	In view of \eqref{eq:init5} with $\cap_{i\in \{1,2\}}\calB\pth{\theta_i,{\Delta\over 8}}=\phi$ and $n_1,n_2\geq n\alpha$, we get that given any set $\calS\subseteq \{Y_i:i\in [n]\}$ of size at least $n-{n\alpha\over 2}$, there will be at least two points in $\calS$ that are at least $\Delta-{\Delta\over 4}$ distance away. We choose $\calS = \{i\in [n]:Y_i\in \calB(\mu_1^{(\ell)},\dist_1^{(\ell)})\}$ and note that
	$$
	|\calS|\geq n-{n\beta}- {5n\over 2\log(1/(G(\Delta/32\sigma)))}\geq n-{n\alpha\over 2},
	$$
	as $\abs{\calP_1^{(\ell)}/\calB(\mu_1^{(\ell)},\dist_1^{(\ell)})}\leq {n\beta}$. Suppose $x,y$ are the farthest away points in $\calS$. This leads to a contradiction as 
	$$
	\Delta-{\Delta\over 4}\leq \|x-y\|\leq \|x-\mu_1^{(\ell)}\|+\|y-\mu_1^{(\ell)}\|
	\leq 2\cdot \dist_1^{(\ell)}\leq {\Delta\over 4}.
	$$
	Now it remains to show that $\mu_1^{(\ell)},\mu_2^{(\ell)}$ lies in different balls among $\calB(\theta_1,\Delta/3)$ and $\calB(\theta_2,\Delta/3)$. If not, then suppose that both lie in $\calB(\theta_1,\Delta/3)$. Note that either $\calP_1^{(\ell)}$ or $\overline{\calP_1^{(\ell)}}$ will contain more than half the points from $\{Y_i:i\in T_2\}\cap \calB\pth{\theta_2,{\Delta\over 8}}$. Suppose that without loss of generality $\overline{\calP_1^{(\ell)}}$ is the partition with more than half of the points in $\{Y_i:i\in T_2\}\cap \calB\pth{\theta_2,{\Delta\over 8}}$. Then we have the following
	\begin{itemize}
		\item $\calB\pth{\mu_2^{(\ell)},\dist_2^{(\ell)}}
		\subseteq \calB\pth{\mu_2^{(\ell)},{\Delta\over 8}}\subseteq \calB\pth{\theta_1,{\Delta\over 3}+{\Delta\over 8}} = \calB\pth{\theta_1,{11\Delta\over 24}}$
		\item $\calB\pth{\theta_2,{\Delta\over 8}}\cap \calB\pth{\mu_2^{(\ell)},\dist_2^{(\ell)}}\subseteq \calB\pth{\theta_2,{\Delta\over 8}}\cap \calB\pth{\theta_1,{11\Delta\over 24}}=\phi$,
		\item $\frac 12 \abs{\{Y_i:i\in T_2\}\cap \calB\pth{\theta_2,{\Delta\over 8}}}\geq {n\alpha\over 2}-{5n\over 8\log(1/(G(\Delta/32\sigma)))}\geq {n\alpha\over 3}$
	\end{itemize} 
	However, this leads to a contradiction, as 
	$$
	\abs{\overline{\calP_1^{(\ell)}}\cap \calB\pth{\theta_2,{\Delta\over 8}}}
	\leq \abs{\overline{\calP_1^{(\ell)}}/ \sth{Y_i: i\in [n]Y_i\in  \calB\pth{\mu_2^{(\ell)},\dist_2^{(\ell)}}}}
	\leq {n\alpha\over 4},
	$$
	but on the other hand, 
	$$
	\abs{\overline{\calP_1^{(\ell)}}\cap \calB\pth{\theta_2,{\Delta\over 8}}}
	\geq \frac 12 \abs{\{Y_i:i\in T_2\}\cap \calB\pth{\theta_2,{\Delta\over 8}}}\geq {n\alpha\over 3}.
	$$
\end{proof}

\subsection{Proof of \prettyref{thm:proof-algo-k}}
\label{app:proof-init-k}
In the proof below, we assume that all the mentioned constants depend on $\decay,\alpha,\sigma,k$, unless otherwise specified. In addition, for our entire analysis we will assume that the event $\tilde \calE_k$ holds, which has a high probability guarantee. Similar to before, we will extensively use the following definition of order statistics: Given any set $V$ of real numbers and fraction $0<\beta<1$, let $V^{\sth{\beta}}$ define the $\ceil{\beta|V|}$-th smallest number in $V$. . We make the following observations for simplifying the notation. Whenever we call the \iod algorithm to find $j$ centroids from the remaining data set, it contains a {\it for-loop} with the loop counter denoted by $\ell_j$. As a result, whenever we find a set of centroids $\hat \mu_k,\dots,\hat\mu_1$ it corresponds to a set of loop counts $\tilde \ell_k,\dots,\tilde\ell_2$
\begin{align}
	(\hat \mu_k,\dots,\hat\mu_2,\hat\mu_1)
	= (\mu_k^{(k,\tilde \ell_k)},\dots,\mu_2^{(2,\tilde \ell_2)},\mu_1^{(1,\tilde \ell_2)}),
\end{align}
and vice-versa. In view of this relation, in the proofs below we will interchangeably use the centroids and the indices.

The proof is a combination of the following results.

\begin{lemma}\label{lmm:centroid1-k}
	There is one $\theta_i$, such that $\|\theta_i-\mu_k^{(k,1)}\|\leq C$ for some constant $C>0$.
\end{lemma}

\begin{lemma}\label{lmm:first-jump-k}
	There is a stage $\bar \ell_k+1$, with $\bar \ell_k\geq 1$,  such that $\dist_k^{(\bar \ell_k+1)}> {\Delta\over 8k},\dist_k^{(\bar \ell_k)}\leq  {\Delta\over 8k}$.	
\end{lemma}


\begin{lemma} \label{lmm:small-totdist-k}
	There exists steps $\ell_{k},\dots,\ell_2$ such that for each $i=2,\dots,k$, at the $\ell_i$-th step the distance to the $(1-\beta)|\calP_i^{(\ell_i)}|$-th closest point from $\mu_i^{(i,\ell_i)}$, within the set $\calP_i^{(\ell_i)}$ will all be smaller than $\Delta\over 8k$ and the $(1-\beta)|\overline{\calP_2^{(\ell_2)}}|$-th closest point from $\mu_1^{(1,1)}$, within the set $\overline{\calP_2^{(\ell_2)}}$ will be smaller than $\Delta\over 8k$.
\end{lemma} 

\begin{lemma}\label{lmm:apprx-centroid-k}
	If $\totdist_k^{(\ell_k)}\leq {\Delta\over 16}$ for some $\ell_k$, then there is a permutation $\pi$ of $[k]$ such that $$\max_{i\in [k]} {\|\mu_i^{(\ell)}-\theta_{\pi(i)}\|}\leq {\Delta\over 3}.$$
\end{lemma}

\begin{proof}[Proof of \prettyref{lmm:centroid1-k}]
	
	In view of \prettyref{lmm:E-conc-init-k}, there is a constant $c_1>0$ such that
	\begin{align}\label{eq:init1-k}
		|\sth{j\in [n]:Y_j\in \calB(\theta_i,c_1)}|\geq n_i\pth{1-\beta^2},\quad i\in [k].
	\end{align}
	As we have $n_i>{n\alpha\over k}$ by assumption, it follows that there is a point $Y_i$ such that 
	$$|\sth{j\in [n]:Y_j\in \calB(Y_i,2c_{1})}|\geq {n\alpha\over 4k} (=m_1).$$
	Hence, the tightest neighborhood around any point $Y_i,i\in [n]$, that contains at least ${n\alpha\over 4k}$ points from $Y_1,\dots,Y_n$, has a radius of at most $2c_{1}$ around that $Y_i$. Using the definition \eqref{eq:distance}
	\begin{align}
		D({x},S)=\sth{\|x-Y_{i}\|:i\in S},\quad x\in \reals^d,S\subseteq [n],
	\end{align} 
	pick $i^*\in [n]$ that satisfies 
	\begin{align}
		\sth{D(Y_{i^*},[n])}^{\sth{1-\frac {m_1}n}} = \min_{j\in [n]} \sth{D(Y_{j},[n])}^{\sth{1-\frac {m_1}n}}.
	\end{align} 
	Then $\calB(Y_{i^*},2c_{1})$ and $\cup_{j\in [k]}\calB(\theta_j,c_{1})$ can not be disjoint, as in view of \eqref{eq:init1-k} it will imply that their union will contain more than $n$ points from $Y_1,\dots,Y_n$
	\begin{align}
		&\abs{\sth{i\in [n]:Y_i\in \calB(Y_{i^*},2c_1)}\cup\qth{\cup_{j\in [k]}\sth{i\in [n]:Y_i\in \calB(\theta_j,c_1)}}}
		\nonumber\\
		&\geq {n\alpha\over 4k} + \sum_{j\in [k]}n_j\pth{1-{\beta^2}}
		\geq n+n\pth{\frac \alpha{4k} - {\alpha^2\over 16k^2}} > n,
	\end{align}	
	where we use the fact that $\sth{i\in [n]:Y_i\in \calB(\theta_j,c_1)},j\in [k]$ are disjoint sets as $\min_{g\neq h\in [k]}\|\theta_g-\theta_h\|\geq \Delta$. Hence, $Y_{i^*}$ is at a distance at most $3c_{1}$ from one of the centroids. Without loss of we can pick $\mu_k^{(k,1)} = Y_{i^*}$ and we assume that $\theta_k$ is the closer to $\mu_k^{(k,1)}$ than the other centroids.	
\end{proof}


\begin{proof}[Proof of \prettyref{lmm:first-jump-k}]
	In view of \prettyref{lmm:centroid1-k} we have for some constant $c_1>0$
	\begin{align}\label{eq:init0-k}
		\mu_k^{(k,1)}\in \calB\pth{\theta_k,3c_1},\quad 
		\abs{\{Y_i:i\in T_j\}\cap\calB\pth{\theta_j,c_1}}\geq n_j\pth{1-\beta^2},j\in [k].
	\end{align}
	We observe the following: 
	\begin{itemize}
		\item The set $\calB(\mu_k^{(k,1)},4c_1)$ contains $\calB(\theta_k,c_1)$, which contains at least ${n\alpha\over k}(1-\beta^2)$ points from $\{Y_i:i\in T_k\}$. As the size of $\calP_k^{(1)}$ is at most $\ceil{n\alpha\over 4k}$ the distance of $\mu_k^{(k,1)}$ to any point in $\calP_k^{(1)}$ is less than $4c_1$, which implies $\dist_k^{(1)}\leq {\Delta\over 8k}$.
		\item In view of \eqref{eq:init0-k} we have for $j=1,\dots,k-1$
		\begin{align}
			&|\sth{Y_i:i\in [n],Y_i\in \calB(\theta_j,c_1)}\cap \calP_k^{(\tilde\ell_k)}|
			\nonumber\\
			&\geq
			|\sth{Y_i:i\in [n],Y_i\in \calB(\theta_j,c_1)}|-  |\overline{\calP_k^{(\tilde\ell_k)}}|
			\nonumber\\
			&\geq n_j\pth{1-\beta^2}-m
			\geq {n\alpha\over k}-{n\beta^2\alpha\over k} -{n\beta ^2\over 2}.
		\end{align}
		At the last step, say $\tilde \ell_k$, in the for loop indexed by $\ell_k$, $\calP_k^{(\tilde \ell_k)}$ will have at least $n-m$ many points, we get: 
		\begin{enumerate}[label=(\alph*)]
			\item The tightest neighborhood (say $N$) around $\mu_k^{(k,1)}$ with a size at least $(1-\beta)|\calP_k^{(\tilde\ell_k)}|$ will include at least $(1-\beta)(n-m)\geq n-n\beta-m$ points,
			\item \eqref{eq:init0-k} implies that $\cup_{j\in [k-1]}\sth{\{Y_i:i\in T_j\}\cap\calB\pth{\theta_j,c_1}}$ will contain at least ${n\alpha\over 2k}$ points.
		\end{enumerate}
		Hence we get that this neighborhood $N$ will contain at least one point $y$ from the set $\cup_{j\in [k-1]}\sth{Y_i:i\in [n],Y_i\in \calB(\theta_j,c_1)}$. Let that $y\in \sth{Y_i:i\in [n],Y_i\in \calB(\theta_j,c_1)}$ for some $j\in [k-1]$. Then the distance of $y$ from $\mu_k^{(\tilde\ell)}$ is at least $\Delta-4c_1$, 
		\begin{align}\label{eq:init2-k}
			\|\mu_k^{(\tilde\ell_k)}-y\|
			\geq \|\theta_k-\theta_j\|-\|\mu_k^{(\tilde\ell_k)}-\theta_k\|-\|\theta_j-y\|
			\geq \Delta - 4c_1.
		\end{align}
	\end{itemize} 
	Hence we have that there exist some $1\leq \ell_k\leq n-1$ such that $\dist_k^{(\ell_k+1)} > {\Delta\over 8k}$. Then the following choice of $\bar \ell_k$ finishes the proof
	$$
	\bar \ell_k=\min\sth{r\geq 1:\dist_k^{(r+1)}> {\Delta\over 8k}}.
	$$
\end{proof}


\begin{proof}[Proof of \prettyref{lmm:small-totdist-k}]
	The result be verified using an induction argument. 
	We claim that the following: there exists indices $\ell_j$ corresponding the the $j$-th loop, for $j=k,\dots,2$ such that the corresponding centroids $\mu_k^{(k,\ell_k)},\dots,\mu_i^{(i,\ell_i)}$ satisfy, for each $i=k,k-1,\dots,2$
	\begin{enumerate}[label=(Q\arabic*)]
		
		\item \label{prop:good-centroid} There is one $\theta_g$, such that $\|\theta_g-\mu_g^{(g,\ell_g)}\|\leq C$ for some constant $C>0$ and $g=k,k-1,\dots,i$.
		
		\item \label{prop:low-dist} At the $\ell_i$-th step the distance to the $(1-\beta)|\calP_i^{(\ell_i)}|$-th closest point from $\mu_i^{(i,1)}$, within the set $\calP_i^{(\ell_i)}$ will all be smaller than $\Delta\over 8k$.
		
		\item \label{prop:more-in-complement} For $h=1,\dots,i-1$ 
		$$\abs{\overline{\calP_i^{(\bar \ell_i)}}\cap {\{Y_j:j\in T_h\}}}
		\geq n_h- (k-i+1)n\beta -{5(k-i+1)n_h\over 4\log(1/(G(\Delta/16\sigma k)))}.$$
		\item \label{prop:less-in-complement}  $\abs{\overline{\calP_{i}^{(\bar \ell_i)}}\cap \sth{\cup_{g=i}^k\{Y_j:j\in T_g\}}}\leq (k-i+1){n\beta^2\over 2}+{5\sum_{g=i}^k n_g\over 4\log(1/G(\Delta/(16k\sigma)))}.$
		
		%			\item \label{prop:good-centroid-in-complement} There is a constant $\tilde C$ such that $\mu_{i-1}^{(i-1,1)}$ lies inside $\calB(\theta_{i-1},\tilde C)$.
	\end{enumerate}
	
	\paragraph*{\textbf{Base case $i=k$}} 
	Note that our algorithm starts by picking the tightest neighborhood with $m_1$ points, and then we keep adding $m$ points from $\overline{\calP_k^{(\ell_k)}}$ to $\calP_k^{(\ell_k)}$ at each step. In view of \prettyref{lmm:centroid1-k} we get that the approximate $\mu_k^{(k,1)}$ lies within a constant radius of $\theta_k$, and hence \ref{prop:good-centroid} is satisfied. In view of \prettyref{lmm:first-jump-k}, when we run the $k$-th for loop at the iteration $\bar \ell_k$, we get $\dist_k^{(\bar \ell_k)}\leq {\Delta\over 8k}$, and hence \ref{prop:low-dist} is satisfied.
	
	Let $\bar \ell_k$ is as in \prettyref{lmm:first-jump-k}. Without a loss of generality we assume that $\theta_k$ is the closest centroid to $\mu_k^{(k,1)}$ and \eqref{eq:init0-k} holds for some $c_1>0$.
	We first prove the following claims:
	\begin{align}
		\abs{\calP_k^{(\bar \ell_k)}\cap \{Y_i:i\in T_k\}}&\geq n_k-{n\beta^2\over 2}-{5n_k\over 4\log(1/(G(\Delta/16\sigma k)))}
		\label{eq:init-claim1-k}\\
		\abs{\calP_k^{(\bar \ell_k)}\cap {\{Y_i:i\in T_j\}}}&\leq n\beta + {5n_j\over 4\log(1/(G(\Delta/16\sigma k)))},\quad j\in [k-1].
		\label{eq:init-claim2-k}
	\end{align}
	The first claim \eqref{eq:init-claim1-k} follows from the following sequence of arguments (note the definition in \eqref{eq:distance})
	\begin{itemize}
		\item Using $\mu_k^{(k,\bar \ell_k)}=\mu_k^{(k,\bar \ell_k+1)}$ we get $\dist_k^{(\bar \ell_k+1)}=\sth{D(\mu_k^{(k,\bar \ell_k)},\calP_k^{(\bar \ell_k+1)})}^{\sth{1-\beta}} > {\Delta\over 8k},$
		which implies 
		\begin{align}\label{eq:init6-k}
			\calP_k^{(\bar \ell_k+1)}\supseteq \{Y_i:i\in [n]\}\cap \calB\pth{\mu_k^{(k,\bar \ell_k)},{\Delta\over 8k}}.
		\end{align}
		As we have $\calP_k^{(\bar \ell_k)}\subset \calP_k^{(\bar \ell_k+1)}$ and $|\calP_k^{(\bar \ell_k)}|\leq |\calP_k^{(\bar \ell_k+1)}|\leq |\calP_k^{(\bar \ell_k)}|+{n\beta^2\over 2}$, we get that there is a set $A\subseteq \{Y_i:i\in [n]\}$ that satisfies
		$$
		\calP_k^{(\bar \ell_k)}\supseteq\calP_k^{(\bar \ell_k+1)}/A,\quad |A|\leq {n\beta^2\over 2}.
		$$
		In view of \eqref{eq:init6-k} the last display implies
		\begin{align}
			\sth{\calP_k^{(\bar \ell_k)}\cap\{Y_i:i\in T_k\}}
			&\supseteq \sth{\calP_k^{(\bar \ell_k+1)}\cap\{Y_i:i\in T_k\}/A}
			\nonumber\\
			&\supseteq \sth{\calB\pth{\mu_k^{(k,\bar \ell_k)},{\Delta\over 8k}}\cap\{Y_i:i\in T_k\}/A},
		\end{align}
		and hence
		\begin{align}\label{eq:init7-k}
			\abs{\calP_k^{(\bar \ell_k)}\cap\{Y_i:i\in T_k\}}&\geq \abs{\calB\pth{\mu_k^{(k,\bar \ell_k)},{\Delta\over 8k}}\cap\{Y_i:i\in T_k\}}-|A|
			\nonumber\\
			& \geq \abs{\calB\pth{\mu_k^{(k,\bar \ell_k)},{\Delta\over 8k}}\cap\{Y_i:i\in T_k\}}-{n\beta^2\over 2}.
		\end{align}
		
		\item As we have from \eqref{eq:init0-k}:
		\begin{align}
			\begin{gathered}
				\calB\pth{\mu_k^{(k,\bar \ell_k)},{\Delta\over 8k}}\supseteq \calB\pth{\theta_k,{\Delta\over 8k}-3c_1}
				\supseteq \calB\pth{\theta_k,{\Delta\over 16k}},
			\end{gathered}	
		\end{align}
		in view of \prettyref{lmm:E-conc-init-k}(ii) we get
		\begin{align}\label{eq:init8-k}
			&\abs{\calB\pth{\mu_k^{(k,\bar \ell_k)},{\Delta\over 8k}}\cap \{Y_i:i\in T_k\}}
			\geq \abs{\calB\pth{\theta_k,{\Delta\over 16k}}\cap \{Y_i:i\in T_k\}}
			\nonumber\\
			&\geq n_k\pth{1-{5\over 4\log\pth{1/G\pth{\Delta\over 16\sigma k}}}}
			\geq n_k-{5n_k\over 4\log(1/(G(\Delta/16\sigma k)))}. 
		\end{align}
	\end{itemize}
	Combining \eqref{eq:init7-k} and \eqref{eq:init8-k} we get \eqref{eq:init-claim1-k}.
	
	Next, to prove the claim \eqref{eq:init-claim2-k}, we note that:
	\begin{itemize}
		\item In view of \prettyref{lmm:E-conc-init-k}, for each $j=1,\dots,k-1$, there are at most ${5n_j\over 4\log(1/(G(\Delta/16\sigma k)))}$ many points from $\sth{Y_i:i\in T_j}$ outside $\calB(\theta_j,{\Delta\over 16k})$. As \eqref{eq:init0-k} implies $\calB\pth{\mu_k^{(k,\bar \ell_k)},{\Delta\over 8k}}\pth{\subseteq \calB\pth{\theta_k,{\Delta\over 8k}+3c_1}}$ and  $\cup_{j=1}^{k-1}\calB(\theta_j,{\Delta\over 16k})$ are disjoint, we have for each $j=1,\dots,k-1$
		\begin{align}\label{eq:init9-k}
			&\abs{\calP_k^{(\bar \ell_k)}\cap {\{Y_i:i\in T_j\}}\cap \calB\pth{\mu_k^{(k,\bar \ell_k)},{\Delta\over 8k}}}
			\nonumber\\
			&\leq \abs{{\{Y_i:i\in T_j\}}/ {\cup_{j=1}^{k-1}\calB\pth{\theta_j,{\Delta\over 16k}}}}
			\leq {5n_j\over 4\log(1/(G(\Delta/16\sigma k)))} .
		\end{align}
		\item On the other hand,
		$\dist_k^{(\bar \ell_k)}=\sth{D(\mu_k^{(k,\bar \ell_k)},\calP_k^{(\bar \ell_k)})}^{\sth{1-\beta}}\leq {\Delta\over 8k}$
		implies that for each $j\in [k-1]$
		\begin{align}\label{eq:init10-k}
			\abs{\calP_k^{(\bar \ell_k)}\cap {\{Y_i:i\in T_j\}}/ \calB\pth{\mu_k^{(k,\bar \ell_k)},{\Delta\over 8k}}}
			\leq {n\beta}.
		\end{align}
	\end{itemize}
	Combining \eqref{eq:init9-k} and \eqref{eq:init10-k} we get \eqref{eq:init-claim2-k}.
	
	Hence, we have proven the inequalities \eqref{eq:init-claim1-k} and \eqref{eq:init-claim2-k}. These inequalities together imply
	\begin{align}
		\abs{\overline{\calP_k^{(\bar \ell_k)}}\cap {\{Y_i:i\in T_j\}}}
		&\geq n_j- n\beta -{5n_j\over 4\log(1/(G(\Delta/16\sigma k)))},\quad j\in [k-1]
		\label{eq:init-claim3-k}\\
		\abs{\overline{\calP_k^{(\bar \ell_k)}}\cap \{Y_i:i\in T_k\}}&\leq {n\beta^2\over 2}+{5n_k\over 4\log(1/(G(\Delta/16\sigma k)))}.
		\label{eq:init-claim4-k}
	\end{align}
	The first inequality above verifies \ref{prop:more-in-complement} and the second inequality verifies \ref{prop:less-in-complement}. 
	
	
	%			
	%			
	%			Note that at some stage $\ell$, before we exhaust all the points, the distance to the $(1-{\beta})|\calP_k^{(\ell)}|$-th closest point from $\mu_k^{(k,1)}$, within the set $\calP_k^{(\ell)}$ will exceed ${\Delta\over 8k}$. This is because of the following reasoning. Note that $\calP_k^{(\floor{n-m_1\over m})}$ will contain at least $n-m$ points and in the data set there are at least $32k^2(k-1)m$ points coming from the clusters with centroids $\theta_1,\dots,\theta_{k-1}$. As a result, the set of points that are closer to $\mu_k^{(k,\floor{n-m_1\over m})}$ than the $(1-{\beta})|\calP_k^{(\floor{n-m_1\over m})}|$-th closest point in $\calP_k^{(\floor{n-m_1\over m})}$ will contain at least $32k^2(k-1)-m$ points from those other clusters. In addition we note that $\mu_k^{(k,\floor{n-m_1\over m})}$ is within $c_{k,\alpha,G}$ distance of $\theta_k$ and $$\abs{\cup_{i=2}^k\calB(\theta_i,{\Delta\over 4k})}\geq 32k^2(k-1)m-{nk\over \log(1/G(\Delta/4k))}\geq 16k^2(k-1)m.$$
	%			Hence the $(1-{\beta})|\calP_k^{(\floor{n-m_1\over m})}|$-th closest distance from a $\mu_k^{(k,\floor{n-m_1\over m})}$ will be at least $\Delta - c_{k,\alpha,G}-{\Delta\over 4k}$. 
	%			
	%			Suppose that at the $(\ell_k+1)$-th step the distance to the $(1-\beta)|\calP_k^{(\ell_k+1)}|$-th closest point from $\mu_k^{(k,1)}$, within the set $\calP_k^{(\ell_k+1)}$, will exceed $\Delta\over 50k$. Hence at the $\ell_k$-th step the distance to the $(1-\beta)|\calP_k^{(\ell_k+1)}|$-th closest point from $\mu_k^{(k,1)}$, within the set $\calP_k^{(\ell_k)}$ will still be smaller than $\Delta\over 50k$.
	%			Note that in $\calP_k^{(\ell_k)}$ there are at least $n_k-m-{n\over \log(1/(G(\Delta/4k)))}$ points from $T_k$ and at most ${n\beta} + {n(k-1)\over \log(1/(G(\Delta/4k)))}$ points from each of $T_i,i=1,\dots,k-1$. The first claim follows from the fact that in the step $\ell_k$, the $(1-\beta)|\calP_k^{(\ell)}|$-th closest point in $\calP_k^{(\ell)}$ are still within $\Delta\over 100k$ radius of $\mu_k^{(k,1)}$ and the set $\calB(\mu_k^{(k,1)},\Delta/100k)$, which contains the set $\calB(\theta_1,3c_{k,\alpha,G}+\Delta/200k)$, has at least $n_k-{n\over \log(1/(G(\Delta/200k)))}$ points from $T_k$. This implies that if the size of $\calP_k^{(\ell_k)}$ is at most $n_k-m-{n\over \log(1/(G(\Delta/200k)))}$, we could have still added $m$ points from $T_k$ without increasing $\dist_1^{(\ell_k+1)}$ beyond $\Delta\over 50k$, providing a contradiction. Next, to prove the claim that $\calP_k^{(\ell_k)}$ contains at most ${n\beta} +{n\over \log(1/(G(\Delta/200k)))}$ points from each of the remaining clusters $T_i,i=1,\dots,k-1$, we first note that for each $i=1,\dots,k-1$ there are at most ${n\over \log(1/(G(\Delta/200k)))}$ many points outside $\calB(\theta_i,\Delta/200k)$, which can be within the $\Delta/100k$ radius of $\mu_k^{(k,1)}$, and the size of points in $\calP_k^{(\ell_k)}$ that are not in $\calB(\mu_k^{(k,1)},\Delta/100k)$ is at most $n\beta$. Hence, we have proven that $\overline{\calP_k^{(\ell_k)}}$ contains at least ${n\alpha\over k}-n\beta-{n\over \log(1/(G(\Delta/200k)))}$ points from each of $T_i,i=1,\dots,k-1$ and at most $m+{n\over \log(1/(G(\Delta/200k)))}$ points from $T_k$. Finally, as $\overline{\calP_k^{(\ell_k)}}$ contains at most $m+{n\over \log(1/(G(\Delta/4k)))}$ points from $T_k$, with  $m={\floor{n\alpha^2\over 32k^3}}$, and at least ${n\alpha\over k}-n\beta-{nk\over \log(1/G(\Delta/4k))}$ many points from each of the remaining clusters, with $\beta={\alpha\over 8k^2}$, when we pick the tightest neighborhood with $m_1=\ceil{n\alpha\over 2k}$ many points,  we get that $\mu_{k-1}^{k-1,1}$ to be in the set $\cup_{i=1}^{k-1}\calB(\theta_i,\tilde c_{k,\alpha,G})$ for some constant $\tilde c_{k,\alpha,G}$.
	
	\paragraph*{\textbf{Induction step from $i$ to $i-1$}} To complete the induction argument, let us suppose that the statement holds for some $3\leq i\leq k$ and we intend to prove the case of $i-1$. The proof of \ref{prop:good-centroid} follows from the following general result. The proof is essentially a repetition of argument as in the proof of \prettyref{lmm:centroid1-k}, and is presented at the end of this section.
	\begin{lemma}\label{lmm:good-centroid-in-complement}
		Suppose that we have for $i\geq 3$ and $h=1,\dots,i-1$
		\begin{align*}
			\abs{\overline{\calP_i^{(\bar \ell_i)}}\cap {\{Y_j:j\in T_h\}}}
			&\geq {3n_h\over 5}, \quad
			\abs{\overline{\calP_i^{(\bar \ell_i)}}\cap \sth{\cup_{g=i}^k\{Y_j:j\in T_g\}}}
			\leq {n\alpha\beta\over 5k}.
		\end{align*} 
		Then there is a constant $\tilde C$ and a centroid $\theta_{i-1}$ such that $\|\mu_{i-1}^{(i-1,1)}-\theta_{i-1}\|\leq \tilde C$.
	\end{lemma}
	
	
	Next we prove \ref{prop:low-dist} for the loop indexed by $\ell_{i-1}$. In view of the above we note that there is a constant $C$ with
	\begin{align}\label{eq:init0-k-induction}
		\mu_{i-1}^{(i-1,1)}\in \calB\pth{\theta_{i-1}, C},\quad 
		\abs{\{Y_j:j\in T_h\}\cap\calB\pth{\theta_h,C}}\geq n_h\pth{1-\beta^2},h\in [i-1].
	\end{align}
	
	As we keep adding $m$ points from $\overline{\calP_{i-1}^{(\ell_{i-1})}}$ to $\calP_{i-1}^{(\ell_{i-1})}$ at each step $\ell_{i-1}=2,\dots,\floor{n'- m_1\over m}$, note that at some stage $\ell_{i-1}$, before we exhaust all the points, the distance to the $(1-{\beta})|\calP_{i-1}^{(\ell_{i-1})}|$-th closest point from $\mu_{i-1}^{(i-1,1)}$, within the set $\calP_{i-1}^{(\ell_{i-1})}$ will exceed ${\Delta\over 8k}$. This is because of a reasoning similar as in the proof of \prettyref{lmm:first-jump-k}. 
	To prove our claim we observe the following: 
	\begin{itemize}
		\item In view of \eqref{eq:init0-k-induction} we have $\calB(\mu_{i-1}^{(i-1,1)},2C)\supseteq\calB(\theta_{i-1},C)$, which implies
		\begin{align}
			\abs{\{Y_j:j\in T_{i-1}\}/\calB(\mu_{i-1}^{(i-1,1)},2C)}
			\leq \abs{\{Y_j:j\in T_{i-1}\}/\calB(\theta_{i-1},C)}
			\leq n_{i-1}\beta^2.
		\end{align}
		In view of the assumption \ref{prop:more-in-complement} at the induction step $i$ the last display implies 
		\begin{align}
			&\abs{\overline{\calP_i^{(\bar \ell_i)}}\cap \{Y_j:j\in T_{i-1}\}\cap \calB(\mu_{i-1}^{(i-1,1)},2C)}
			\nonumber\\
			&=\abs{\overline{\calP_i^{(\bar \ell_i)}}\cap \{Y_j:j\in T_{i-1}\}}-\abs{\overline{\calP_i^{(\bar \ell_i)}}\cap \{Y_j:j\in T_{i-1}\}/ \calB(\mu_{i-1}^{(i-1,1)},2C)}
			\nonumber\\
			&\geq \abs{\overline{\calP_i^{(\bar \ell_i)}}\cap \{Y_j:j\in T_{i-1}\}}-\abs{\{Y_j:j\in T_{i-1}\}/ \calB(\mu_{i-1}^{(i-1,1)},2C)}
			\nonumber\\
			&\geq n_{i-1}- (k-i+1)n\beta - n_{i-1}\beta^2 -{5(k-i+1)n_{i-1}\over 4\log(1/(G\pth{{\Delta\over 16\sigma k}}))}
			\geq {n\alpha\over 2k}.
		\end{align}
		As the size of $\calP_{i-1}^{(1)}$ is at most $\ceil{n\alpha\over 4k}$ the distance of $\mu_{i-1}^{({i-1},1)}$ to any point in $\calP_{i-1}^{(1)}$ is less than $2C$, which implies $\dist_{i-1}^{(1)}\leq {\Delta\over 8k}$.
		\item At the last step, say $\tilde \ell_{i-1}$, in the for loop indexed by $\ell_{i-1}$, $\overline{\calP_{i-1}^{(\tilde \ell_{i-1})}}$ will have at most $m$ many points, in view of \ref{prop:more-in-complement} and $n_1\geq 4n\beta$ we get
		\begin{align}\label{eq:init11-k}
			&\abs{\calP_{i-1}^{(\tilde \ell_{i-1})}\cap \{Y_j:j\in T_{1}\}}
			\nonumber\\
			&\geq \abs{\overline{\calP_i^{(\bar \ell_i)}}\cap \{Y_j:j\in T_{1}\}} - m
			\geq n_1 - kn\beta - {n\beta^2\over 2} - {5kn_1\over 4\log(1/\decay({\Delta\over 16\sigma k}))}
			\geq 2n\beta.
		\end{align} 
		As the tightest neighborhood (say $N$) around $\mu_{i-1}^{(i-1,1)}$ with a size at least $(1-\beta)|\calP_{i-1}^{(\tilde\ell_{i-1})}|$ will exclude at most $n\beta$ points from $\calP_{i-1}^{(\tilde\ell_{i-1})}$, in view of \eqref{eq:init11-k} we get that the neighborhood $N$ will include at least $n\beta$ points from $\{Y_j:j\in T_{1}\}$. Now, \eqref{eq:init0-k} implies that $\{Y_i:i\in T_1\}\cap\calB\pth{\theta_1,C}$ will contain at lest $n_1(1-\beta^2)$ points from $\{Y_j:j\in T_{1}\}$, hence we get that the above neighborhood $N$ will contain at least one point $y\in \sth{Y_j:j\in [n],Y_i\in \calB(\theta_1,C)}$. Then the distance of $y$ from $\mu_{i-1}^{(i-1,\tilde\ell_{i-1})}$ is at least $\Delta-2C$, 
		\begin{align}
			\|\mu_{i-1}^{(i-1,\tilde\ell_{i-1})}-y\|
			\geq \|\theta_1-\theta_{i-1}\|-\|\mu_{i-1}^{(i-1,\tilde\ell_{i-1})}-\theta_{i-1}\|-\|\theta_1-y\|
			\geq \Delta - 2C.
		\end{align}
	\end{itemize} 
	Hence we have that there exist some $1\leq \ell_{i-1}\leq n-1$ such that $\dist_{i-1}^{(\ell_{i-1}+1)} > {\Delta\over 8k}$. Choose $\bar \ell_{i-1}$ as
	$$
	\bar \ell_{i-1}=\min\sth{r\geq 1:\dist_{i-1}^{(r+1)}> {\Delta\over 8k}}.
	$$
	to satisfy the condition \ref{prop:low-dist}.
	%The set $\calP_{i-1}^{(\floor{n'-m_1\over m})}$ will contain at least $n'-m$ points and in the data set there are at least $32k^2(i-2)m$ points coming from the clusters with centroids $\theta_1,\dots,\theta_{i-2}$. As a result, the set of points that are closer to $\mu_{i-1}^{(i-1,\floor{n'-m_1\over m})}$ than the $(1-{\beta})|\calP_{i-1}^{(\floor{n'-m_1\over m})}|$-th closest point in $\calP_{i-1}^{(\floor{n'-m_1\over m})}$ will contain at least $32k^2(i-2)m-m$ points from those other clusters. In addition we note that $\mu_{i-1}^{({i-1},\floor{n'-m_1\over m})}$ is within $c_{k,\alpha,G}$ distance of $\theta_{i-1}$ and $$\abs{\cup_{j=1}^{i-2}\calB(\theta_j,{\Delta\over 4k})}\geq 32k^2(i-2)m-{nk\over \log(1/G(\Delta/4k))}\geq 16k^2(i-2)m.$$
	%	Hence the $(1-{\beta})|\calP_{i-1}^{(\floor{n'-m_1\over m})}|$-th closest distance from a $\mu_{i-1}^{(k,\floor{n'-m_1\over m})}$ will be at least $\Delta - c_{k,\alpha,G}-{\Delta\over 4k}$. 
	%	
	
	Next we establish \ref{prop:more-in-complement} and \ref{prop:less-in-complement} for the induction level ${i-1}$. 
	Let $\bar \ell_{i-1}$ is as in the last definition.
	We prove the following claims:
	For $h=1,\dots,i-2$
	\begin{align}
		\abs{\overline{\calP_{i-1}^{(\bar \ell_{i-1})}}\cap {\{Y_j:j\in T_{h}\}}}
		&\geq n_h- (k-i+2)n\beta -{5(k-i+2)n_h\over 4\log(1/(G(\Delta/16\sigma k)))},
		\label{eq:init-claim3-k-induction}
		\\
		\abs{\overline{\calP_{i-1}^{(\bar \ell_{i-1})}}\cap \{Y_j:j\in T_{i-1}\}}&\leq {n\beta^2\over 2}+{5n_{i-1}\over 4\log(1/(G(\Delta/16\sigma k)))}.
		\label{eq:init-claim4-k-induction}
	\end{align}
	To prove the claim \eqref{eq:init-claim3-k-induction}, we note that:
	\begin{itemize}
		\item In view of \prettyref{lmm:E-conc-init-k}, for each $h=1,\dots,i-2$, there are at most ${5n_h\over 4\log(1/(G({\Delta\over 16\sigma k})))}$ many points from $\sth{Y_j:j\in T_h}$ outside $\calB(\theta_h,{\Delta\over 16k})$. As \eqref{eq:init0-k-induction} implies $\calB\pth{\mu_{i-1}^{({i-1},\bar \ell_{i-1})},{\Delta\over 8k}}\pth{\subseteq \calB\pth{\theta_{i-1},{\Delta\over 8k}+2C}}$ and  $\cup_{h=1}^{i-2}\calB(\theta_h,{\Delta\over 16k})$ are disjoint, we have for each $h=1,\dots,i-2$
		\begin{align}\label{eq:init9-k-induction}
			&\abs{\calP_{i-1}^{(\bar \ell_{i-1})}\cap {\{Y_j:j\in T_h\}}\cap \calB\pth{\mu_{i-1}^{(i-1,\bar \ell_{i-1})},{\Delta\over 8k}}}
			\nonumber\\
			&\leq \abs{{\{Y_j:j\in T_h\}}/ {\cup_{h=1}^{i-2}\calB\pth{\theta_h,{\Delta\over 16k}}}}
			\leq {5n_h\over 4\log(1/(G(\Delta/16\sigma k)))}.
		\end{align}
		\item On the other hand,
		$\dist_{i-1}^{(\bar \ell_{i-1})}=\sth{D(\mu_{i-1}^{(i-1,\bar \ell_{i-1})},\calP_{i-1}^{(\bar \ell_{i-1})})}^{\sth{1-\beta}}\leq {\Delta\over 8k}$
		implies that for each $h\in [i-2]$
		\begin{align}\label{eq:init10-k-induction}
			\abs{\calP_{i-1}^{(\bar \ell_{i-1})}\cap {\{Y_j:j\in T_h\}}/ \calB\pth{\mu_{i-1}^{(i-1,\bar \ell_{i-1})},{\Delta\over 8k}}}
			\leq {n\beta}.
		\end{align}
	\end{itemize}
	Combining \eqref{eq:init9-k} and \eqref{eq:init10-k} we get
	\begin{align*}
		&\abs{\calP_{i-1}^{(\bar \ell_{i-1})}\cap {\{Y_j:j\in T_h\}}}
		\nonumber\\
		&\leq 
		\abs{\calP_{i-1}^{(\bar \ell_{i-1})}\cap {\{Y_j:j\in T_h\}}\cap \calB\pth{\mu_{i-1}^{(i-1,\bar \ell_{i-1})},{\Delta\over 8k}}}+\abs{\calP_{i-1}^{(\bar \ell_{i-1})}\cap {\{Y_j:j\in T_h\}}/ \calB\pth{\mu_{i-1}^{(i-1,\bar \ell_{i-1})},{\Delta\over 8k}}}
		\nonumber\\
		&\leq {n\beta} + {5n_h\over 4\log(1/(G(\Delta/16\sigma k)))}.
	\end{align*}
	Combining the above display with \ref{prop:more-in-complement} at the induction level $i$ we get for each $h\in [i-2]$
	\begin{align}
		\abs{\overline{\calP_{i-1}^{(\bar \ell_{i-1})}}\cap {\{Y_j:j\in T_{h}\}}}
		&=\abs{\overline{\calP_{i}^{(\bar \ell_{i})}}\cap {\{Y_j:j\in T_{h}\}}}
		-\abs{\calP_{i-1}^{(\bar \ell_{i-1})}\cap {\{Y_j:j\in T_h\}}}
		\nonumber\\
		&\geq n_h- (k-i+2)n\beta -{5(k-i+2)n_h\over 4\log(1/(G(\Delta/16\sigma k)))}.
	\end{align}
	This completes the verification of \ref{prop:more-in-complement} for the level $i-1$.
	
	The claim \eqref{eq:init-claim4-k-induction} follows from the following sequence of arguments (note the definition in \eqref{eq:distance})
	\begin{itemize}
		\item Using $\mu_{i-1}^{(i-1,\bar \ell_{i-1})}=\mu_{i-1}^{(i-1,\bar \ell_{i-1}+1)}$ we get $\dist_{i-1}^{(\bar \ell_{i-1}+1)}=\sth{D(\mu_{i-1}^{({i-1},\bar \ell_{i-1})},\calP_{i-1}^{(\bar \ell_{i-1}+1)})}^{\sth{1-\beta}} > {\Delta\over 8k},$
		which implies 
		\begin{align}\label{eq:init6-k-iterate}
			\calP_{i-1}^{(\bar \ell_{i-1}+1)}\supseteq \overline{\calP_{i}^{(\bar \ell_{i})}}\cap \calB\pth{\mu_{i-1}^{({i-1},\bar \ell_{i-1})},{\Delta\over 8k}}.
		\end{align}
		As we have $\calP_{i-1}^{(\bar \ell_{i-1})}\subset \calP_{i-1}^{(\bar \ell_{i-1}+1)}$ and $|\calP_{i-1}^{(\bar \ell_{i-1})}|\leq |\calP_{i-1}^{(\bar \ell_{i-1}+1)}|\leq |\calP_{i-1}^{(\bar \ell_{i-1})}|+{n\beta^2\over 2}$, we get that there is a set $A\subseteq \{Y_i:i\in [n]\}$ that satisfies
		$$
		\calP_{i-1}^{(\bar \ell_{i-1})}\supseteq\calP_{i-1}^{(\bar \ell_{i-1}+1)}/A,\quad |A|\leq {n\beta^2\over 2}.
		$$
		In view of \eqref{eq:init6-k-iterate} the last display implies
		\begin{align}
			\sth{\calP_{i-1}^{(\bar \ell_{i-1})}\cap\{Y_j:j\in T_{i-1}\}}
			&\supseteq
			\sth{\calP_{i-1}^{(\bar \ell_{i-1}+1)}\cap\{Y_j:j\in T_{i-1}\}/A}
			\nonumber\\
			&\supseteq 
			\sth{\overline{\calP_{i}^{(\bar \ell_{i})}}\cap \calB\pth{\mu_{i-1}^{({i-1},\bar \ell_{i-1})},{\Delta\over 8k}}\cap\{Y_j:j\in T_{i-1}\}/A},
		\end{align}
		and hence
		\begin{align}\label{eq:init7-k-induction}
			\abs{\calP_{i-1}^{(\bar \ell_{i-1})}\cap\{Y_j:j\in T_{i-1}\}}&\geq \abs{\overline{\calP_{i}^{(\bar \ell_{i})}}\cap\calB\pth{\mu_{i-1}^{({i-1},\bar \ell_{i-1})},{\Delta\over 8k}}\cap\{Y_j:j\in T_{i-1}\}}-|A|
			\nonumber\\
			& \geq \abs{\overline{\calP_{i}^{(\bar \ell_{i})}}\cap\calB\pth{\mu_{i-1}^{({i-1},\bar \ell_{i-1})},{\Delta\over 8k}}\cap\{Y_j:j\in T_{i-1}\}}-{n\beta^2\over 2}.
		\end{align}
		
		\item As we have from \eqref{eq:init0-k-induction}:
		\begin{align}
			\begin{gathered}
				\calB\pth{\mu_{i-1}^{({i-1},\bar \ell_{i-1})},{\Delta\over 8k}}\supseteq \calB\pth{\theta_{i-1},{\Delta\over 8k}-C}
				\supseteq \calB\pth{\theta_{i-1},{\Delta\over 16k}},
			\end{gathered}	
		\end{align}
		in view of \prettyref{lmm:E-conc-init-k}(ii) and the identity of sets 
		$$
		\abs{A\cap B\cap C} =\abs{\{A\cap C\}/\{B/C\}}
		\geq \abs{A\cap C}-\abs{B/C}
		$$ 
		with $A=\overline{\calP_{i}^{(\bar \ell_{i})}},B=\{Y_j:j\in T_{i-1}\},C=\calB\pth{\theta_{i-1},{\Delta\over 8k}}$ we get
		\begin{align}\label{eq:init8-k-induction}
			&\abs{\overline{\calP_{i}^{(\bar \ell_{i})}}\cap\calB\pth{\mu_{i-1}^{({i-1},\bar \ell_{i-1})},{\Delta\over 8k}}\cap \{Y_j:j\in T_{i-1}\}}
			\nonumber\\
			&\geq \abs{\overline{\calP_{i}^{(\bar \ell_{i})}}\cap\calB\pth{\theta_{i-1},{\Delta\over 16k}}\cap \{Y_j:j\in T_{i-1}\}}
			\nonumber\\
			& {\geq} \abs{\overline{\calP_{i}^{(\bar \ell_{i})}}\cap \{Y_j:j\in T_{i-1}\}}
			- \abs{\{Y_j:j\in T_{i-1}\}/\calB\pth{\theta_{i-1},{\Delta\over 16k}}}
			\nonumber\\
			&\geq \abs{\overline{\calP_{i}^{(\bar \ell_{i})}}\cap \{Y_j:j\in T_{i-1}\}}
			- {5n_{i-1}\over 4\log(1/(G(\Delta/16\sigma k)))}.
		\end{align}
	\end{itemize}
	Combining \eqref{eq:init7-k-induction} and \eqref{eq:init8-k-induction} we get
	\begin{align*}
		\abs{\overline{\calP_{i-1}^{(\bar \ell_{i-1})}}\cap \{Y_j:j\in T_{i-1}\}}
		&= \abs{\overline{\calP_{i}^{(\bar \ell_{i})}}\cap \{Y_j:j\in T_{i-1}\}}
		-	\abs{\calP_{i-1}^{(\bar \ell_{i-1})}\cap\{Y_j:j\in T_{i-1}\}}
		\nonumber\\
		&\leq {n\beta^2\over 2}+{5n_{i-1}\over 4\log(1/(G(\Delta/16\sigma k)))}.
	\end{align*}
	In view of \ref{prop:less-in-complement} for the induction level $i$, with $\overline{\calP_{i-1}^{(\bar \ell_{i-1})}}\subseteq \overline{\calP_{i}^{(\bar \ell_{i})}}$ we get
	\begin{align}
		\abs{\overline{\calP_{i-1}^{(\bar \ell_{i-1})}}\cap \sth{\cup_{g=i-1}^k\{Y_j:j\in T_g\}}}
		&\leq \abs{\overline{\calP_{i}^{(\bar \ell_i)}}\cap \sth{\cup_{g=i}^k\{Y_j:j\in T_g\}}} + \abs{\overline{\calP_{i-1}^{(\bar \ell_{i-1})}}\cap \{Y_j:j\in T_{i-1}\}}
		\nonumber\\
		&\leq (k-i+2){n\beta^2\over 2}+{5\sum_{g=i-1}^k n_g\over 4\log(1/G(\Delta/(16k\sigma)))}.
	\end{align}
	This concludes the checking of \ref{prop:less-in-complement} for the induction level $i-1$. This also concludes the proof of the induction results.
	
	
	
	
	%	Note that in $\calP_{i-1}^{(\ell_{i-1})}$ there are at least $n_{i-1}'- m-{n\over \log(1/(G(\Delta/4k)))}$ points from $T_{i-1}$ and at most ${n\beta} + {n\over \log(1/(G(\Delta/4k)))}$ points from $\cup_{j=1}^{i-1}T_j$. The first claim follows from the fact that in the step $\ell_{i-1}$, the $(1-\beta)|\calP_{i-1}^{(\ell_{i-1})}|$-th closest point in $\calP_{i-1}^{(\ell_{i-1})}$ are still within $\Delta\over 100k$ radius of $\mu_{i-1}^{(i-1,1)}$ and the set $\calB(\mu_{i-1}^{(i-1,1)},\Delta/100k)$, which contains the set $\calB(\theta_{i-1},\tilde c_{k,\alpha,G}+\Delta/200k)$, has at least $n_{i-1}'-{n\over \log(1/(G(\Delta/200k)))}$ points from $T_{i-1}$. This implies that if the size of $\calP_{i-1}^{(\ell_{i-1})}$ is at most $n_{i-1}'-m-{n\over \log(1/(G(\Delta/200k)))}$, we could have still added $m$ points from $T_k$ without increasing $\dist_1^{(\ell_k+1)}$ beyond $\Delta\over 50k$, providing a contradiction. 
	
	
	%	Next, to prove the claim that $\calP_{i-1}^{(\ell_{i-1})}$ contains at most ${n\beta} +{n\over \log(1/(G(\Delta/200k)))}$ points from each of the remaining clusters $T_j,j=1,\dots,i-2$, we first note that for each $j=1,\dots,i-2$ there are at most ${n\over \log(1/(G(\Delta/200k)))}$ many points outside $\calB(\theta_j,\Delta/200k)$, which can be within the $\Delta/100k$ radius of $\mu_{i-1}^{(i-1,1)}$, and the size of points in $\calP_{i-1}^{(\ell_{i-1})}$ that are not in $\calB(\mu_{i-1}^{(i-1,1)},\Delta/100k)$ is at most $n\beta$. 
	
	
	%	\nb{Revise from here} Hence, we have proven that $\overline{\calP_{i-1}^{(\ell_{i-1})}}$ contains at least ${n\alpha\over k}-n\beta-{n\over \log(1/(G(\Delta/200k)))}$ points from each of $T_j,i=1,\dots,i-2$ and at most $m+{n\over \log(1/(G(\Delta/200k)))}$ points from $T_{i-1}$. Hence we get that $\overline{\calP_{i-1}^{(\ell_{i-1})}}$ contains at most $m(k-i+1)+{n(k-i+1)\over \log(1/(G(\Delta/200k)))}$ points from $\cup_{j=i-1}^kT_{j}$. Finally, as $\overline{\calP_{i-2}^{(\ell_{i-2})}}$ contains at most $m(k-i+1)+{n(k-i+2)\over \log(1/(G(\Delta/200k)))}$ points from $T_{i-1}$, with $m={\floor{n\alpha^2\over 32k^3}}$, and at least ${n\alpha\over k}-n\beta-{n\over \log(1/G(\Delta/4k))}$ many points from each of the remaining clusters, with $\beta={\alpha\over 8k^2}$, when we pick the tightest neighborhood with $m_1=\ceil{n\alpha\over 2k}$ many points,  we get that $\mu_{i-2}^{i-2,1}$ to be in the set $\calB(\theta_j,\tilde c_{k,\alpha,G})$ for some constant $\tilde c_{k,\alpha,G}$ and $j\in [i-2]$. Without loss of generality we can pick $j=i-2$. This completes the analysis. 
	
	In view of the induction arguments, we have that 
	\begin{align}\label{eq:primary-distances-k}
		\dist_i^{(\bar \ell_i)}\leq {\Delta\over 8k},\quad i=k,k-1,\dots,2.
	\end{align} 
	Finally, to complete the proof of \prettyref{lmm:small-totdist-k} it remains to show that $\dist_1^{(\ell_2)}\leq {\Delta\over 8k}$. In view of the induction statement we have that 
	\begin{enumerate}
		\item $\abs{\overline{\calP_2^{(\bar \ell_2)}}\cap {\{Y_j:j\in T_1\}}}
		\geq n_1- (k-1)n\beta -{5(k-1)n_1\over 4\log(1/(G(\Delta/16\sigma k)))}.$
		\item $\abs{\overline{\calP_{2}^{(\bar \ell_2)}}\cap \sth{\cup_{g=2}^k\{Y_j:j\in T_g\}}}\leq (k-1){n\beta^2\over 2}+{5\sum_{g=2}^k n_g\over 4\log(1/G(\Delta/(16\sigma k)))}
		\leq {n\alpha\beta\over 8k}+{5\sum_{g=2}^k n_g\over 4\log(1/G(\Delta/(16\sigma k)))}.$
	\end{enumerate}
	According to our algorithm, in the final stage, to find $\mu_1^{(1,\bar \ell_2)}$ we deploy the ${\sf HDP}_{1-\beta}$ algorithm. In view of 
	$$
	\abs{\sth{Y_j:j\in T_1}/ \calB\pth{\theta_1,{\Delta\over 16k}}}\leq {5n_1\over 4\log(1/(G(\Delta/16\sigma k)))}
	$$ 
	from \prettyref{lmm:E-conc-init-k}, we have  
	\begin{align*}
		&\abs{\overline{\calP_{2}^{(\bar \ell_2)}}/\calB\pth{\theta_1,{\Delta\over 16k}}}
		\nonumber\\
		&=\abs{\sth{\overline{\calP_{2}^{(\bar \ell_2)}}\cap \{Y_j:j\in T_1\}/\calB\pth{\theta_1,{\Delta\over 16k}}}
			\cup \sth{\overline{\calP_{2}^{(\bar \ell_2)}}\cap \sth{\cup_{g=2}^k\{Y_j:j\in T_g\}}/\calB\pth{\theta_1,{\Delta\over 16k}}}}
		\nonumber\\
		&\leq \abs{\{Y_j:j\in T_1\}/\calB\pth{\theta_1,{\Delta\over 16k}}}
		+ \abs{\overline{\calP_{2}^{(\bar \ell_2)}}\cap \sth{\cup_{g=2}^k\{Y_j:j\in T_g\}}}
		\nonumber\\
		&\leq {5n_1\over 4\log(1/(G(\Delta/16\sigma k)))} + (k-1){n\beta^2\over 2}+{5\sum_{g=2}^k n_g\over 4\log(1/G(\Delta/(16\sigma k)))}
		\nonumber\\
		&\leq  {n\alpha\beta\over 8k}+{5n\over 2\log(1/(G(\Delta/(16\sigma k))))}
		\leq {n_1\beta\over 4}.
	\end{align*}
	As we have
	\begin{align}
		\abs{\overline{\calP_2^{(\bar \ell_2)}}}\geq \abs{\overline{\calP_2^{(\bar \ell_2)}}\cap {\{Y_j:j\in T_1\}}}\geq {n_1\over 2},
	\end{align} 
	any subset of $\overline{\calP_2^{(\bar \ell_2)}}$ with size $\pth{1-\beta}\abs{\overline{\calP_2^{(\bar \ell_2)}}}$, discards a set of size at least ${n_1\beta\over 2}$ from $\overline{\calP_2^{(\bar \ell_2)}}$. Hence the tightest subset of $\overline{\calP_2^{(\bar \ell_2)}}$ with size $\pth{1-{\beta}}\abs{\overline{\calP_1^{(\ell)}}}$ will have a diameter of at most $\Delta\over 16k$. This implies $\dist_1^{(\bar \ell_2)}\leq {\Delta\over 16 k}$. In view of \eqref{eq:primary-distances-k} this proves that there is a path of indices $\bar \ell_k,\dots\bar\ell_2$ such that $\dist_1^{(\bar\ell_2)}+\sum_{h=2}^k\dist_h^{(\bar \ell_h)}\leq {\Delta\over 8}$. Hence, when we pick the indices to optimize $\totdist$, we get $\min_{\ell_k}\totdist_k^{(\ell_k)}\leq {\Delta\over 8}$, as required.
\end{proof}




\begin{lemma}
	Suppose that for a sequence of indices $\ell_1,\dots,\ell_k$ we have $\sum_{i=1}^k\dist_{i}^{(\ell_i)}\leq {\Delta\over 8}$. Then if the corresponding centroids are $\{\mu_i^{(i,\ell_i)}\}_{i=1}^k$, with $\ell_2=\ell_1$, we get that there is a permutation $\pi$ of $[k]$ such that $\mu_i\in \calB(\theta_{\pi(i)},\Delta/7)$ for each $i\in 1,\dots, k$.
\end{lemma}

\begin{proof}
	
	
	
	
	First we show that all of the centroids lie in $\cup_{i=1}^k\calB(\theta_i,\Delta/3)$. If not, without loss of generality let $\mu_1^{(1,\ell_1)}$ lie outside  $\cup_{i=1}^k\calB(\theta_i,\Delta/3)$. Then we have
	\begin{align}\label{eq:init12-k}
		\abs{\{Y_i:i\in [n]\}\cap \calB\pth{\mu_1^{(1,\ell_1)}, {\Delta\over 8}}}
		\leq {n\over \log(1/(G(\Delta/16\sigma k)))}.
	\end{align} 
	For an ease of notation, throughout the proof we define 
	\begin{align}
		\ell_1\eqdef\ell_2,\quad \calP_1^{(\ell_{1})}\eqdef\overline{\calP_1^{(\ell_{2})}},\quad
		\mu_1^{(1,\ell_1)}
		\eqdef \mu_1^{(1,\ell_2)}.
	\end{align}
	Note that in terms of the indices $\ell_2,\dots,\ell_k$ we have the partition of $\{Y_i:i\in [n]\}$ as
	\begin{align}
		\{Y_i:i\in [n]\}={\cup_{g=1}^k{\calP_g^{(\ell_g)}}},\quad
		\calP_g^{(\ell_g)}\cap \calP_h^{(\ell_h)}=\phi,g\neq h\in [k].
	\end{align}
	In view of the assumption $\dist_1^{(\ell_1)}\leq {\Delta\over 8}$ and the fact that the $\abs{\calP_1^{(\ell_1)}\cap\calB\pth{\mu_1^{(1,\ell_1)},\dist_1^{(\ell_1)}}}\geq (1-\beta)\abs{\calP_1^{(\ell_1)}}$ we have 
	\begin{align}
		\abs{\calP_1^{(\ell_1)}/ \calB\pth{\mu_1^{(1,\ell_1)}, {\Delta\over 8}}}
		\leq 
		\abs{\calP_1^{(\ell_1)}/ \calB\pth{\mu_1^{(1,\ell_1)}, \dist_1^{(\ell_1)}}}
		\leq n\beta.
	\end{align}
	In view of \eqref{eq:init12-k} the last display implies
	\begin{align}
		\abs{\calP_1^{(\ell_1)}}
		&\leq \abs{\calP_1^{(\ell_1)}/ \calB\pth{\mu_1^{(1,\ell_1)}, {\Delta\over 8}}}
		+	\abs{\{Y_i:i\in [n]\}\cap \calB\pth{\mu_1^{(1,\ell_1)}, {\Delta\over 8}}}
		\nonumber\\
		&\leq n\beta + {n\over \log(1/(G(\Delta/16\sigma k)))}. 
	\end{align}
	As $\cup_{i=2}^{k}\calP_i^{(\ell_i)}$ and $\calP_1^{(\ell_1)}$ are disjoint, the last display implies for any $j=2,\dots,k$
	\begin{align}\label{eq:init13-k}
		\abs{\{Y_i:i\in T_j\}\cap\sth{\cup_{g=2}^{k}\calP_g^{(\ell_g)}}}\geq n_j-{n\beta}-{n\over \log(1/(G(\Delta/16\sigma k)))}
		\geq {7n\alpha\over 8k}.
	\end{align}
	Then we have for $j=1,\dots,k$
	\begin{align}
		&\abs{\{Y_i:i\in T_j\}\cap\qth{\cup_{g=2}^{k}\sth{\calP_g^{(\ell_g)}\cap \calB(\mu_g^{(g,\ell_g)},\dist_g^{(\ell_g)})}}}
		\nonumber\\
		&=\abs{\{Y_i:i\in T_j\}\cap \sth{\cup_{g=2}^{k}\calP_g^{(\ell_g)}}\cap\qth{\cup_{g=2}^{k}\sth{\calP_g^{(\ell_g)}\cap \calB(\mu_g^{(g,\ell_g)},\dist_g^{(\ell_g)})}}}
		\nonumber\\
		&= \abs{\{Y_i:i\in T_j\}\cap \sth{\cup_{g=2}^{k}\calP_g^{(\ell_g)}}}\nonumber\\
		&\quad -\abs{\{Y_i:i\in T_j\}\cap \sth{\cup_{g=2}^{k}\calP_g^{(\ell_g)}}/\qth{\cup_{g=2}^{k}\sth{\calP_g^{(\ell_g)}\cap \calB(\mu_g^{(g,\ell_g)},\dist_g^{(\ell_g)})}}}
		\nonumber\\
		&\geq \abs{\{Y_i:i\in T_j\}\cap \sth{\cup_{g=2}^{k}\calP_g^{(\ell_g)}}}\nonumber\\
		&\quad-\abs{ \sth{\cup_{g=2}^{k}\calP_g^{(\ell_g)}}/\qth{\cup_{g=2}^{k}\sth{\calP_g^{(\ell_g)}\cap \calB(\mu_g^{(g,\ell_g)},\dist_g^{(\ell_g)})}}}
		\nonumber\\
		&\stepa{\geq} {7n\alpha\over 8k}
		-\abs{\cup_{g=2}^{k}\sth{\calP_g^{(\ell_g)}/ \calB(\mu_g^{(g,\ell_g)},\dist_g^{(\ell_g)})}}
		\nonumber\\
		& = {7n\alpha\over 8k}
		-\sum_{g=2}^{k}\abs{\calP_g^{(\ell_g)}/ \calB(\mu_g^{(g,\ell_g)},\dist_g^{(\ell_g)})}
		\stepb{\geq} {7n\alpha\over 8k}-n\beta
		\geq {3n\alpha\over 4k},
		\label{eq:init14-k}
	\end{align}
	where (a) followed \eqref{eq:init13-k} and the fact that $\{\calP_g^{(\ell_g)}\}_{g=2}^k$ are disjoint and (b) followed from as
	$$
	\sum_{g=2}^{k}\abs{\calP_g^{(\ell_g)}/ \calB(\mu_g^{(g,\ell_g)},\dist_g^{(\ell_g)})}
	\leq 
	\beta\sum_{g=2}^{k}\abs{\calP_g^{(\ell_g)}}\leq n\beta.
	$$
	As we have for each $j=1,\dots,k$
	\begin{align*}
		&\{Y_i:i\in T_{j}\}\cap \qth{\cup_{g=2}^{k}\sth{\calP_g^{(\ell_g)}\cap \calB(\mu_g^{(g,\ell_g)},\dist_g^{(\ell_g)})}}
		\nonumber\\
		&=\cup_{g=2}^{k} \sth{\{Y_i:i\in T_{j}\}\cap\calP_g^{(\ell_g)}\cap \calB(\mu_g^{(g,\ell_g)},\dist_g^{(\ell_g)})}
	\end{align*} 
	with the union on right side of the above display is disjoint, by the pigeon hole principle there exists indices $g,j_1,j_2$ such that
	\begin{align*}
		&\abs{\sth{\calP_g^{(\ell_g)}\cap \calB(\mu_g^{(g,\ell_g)},\dist_g^{(\ell_g)})}\cap \{Y_i:i\in T_{j}\}}
		\nonumber\\
		&\geq {\min_{j=1}^k\abs{\{Y_i:i\in T_j\}\cap\qth{\cup_{g=2}^{k}\sth{\calP_g^{(\ell_g)}\cap \calB(\mu_g^{(g,\ell_g)},\dist_g^{(\ell_g)})}}}
			\over k}
		\geq {3n\alpha\over 4k^2},
		\quad j=j_1,j_2.
	\end{align*}
	However, as 
	$$\abs{\{Y_i:i\in T_j\}/\calB(\theta_{j},\Delta/3)}
	\leq {n_j\over \log(1/G(\Delta/16\sigma k))}
	\leq {n\alpha\over 4k^2}, \quad j=j_1,j_2,
	$$ 
	we get that for $j=j_1,j_2$
	\begin{align*}
		&\abs{\sth{\calP_g^{(\ell_g)}\cap \calB(\mu_g^{(g,\ell_g)},\dist_g^{(\ell_g)})}\cap \{Y_i:i\in T_{j}\}\cap \calB(\theta_{j},\Delta/3)}
		\nonumber\\
		&\geq \abs{\sth{\calP_g^{(\ell_g)}\cap \calB(\mu_g^{(g,\ell_g)},\dist_g^{(\ell_g)})}\cap \{Y_i:i\in T_{j}\}}
		-\abs{\{Y_i:i\in T_{j}\} /\calB(\theta_{j},\Delta/3)}
		\geq {n\alpha\over 2k^2}.
	\end{align*}
	Hence, there exists $x,y\in \{Y_i:i\in [n]\}$ such that 
	\begin{align}
		x&\in \sth{\calP_g^{(\ell_g)}\cap \calB(\mu_g^{(g,\ell_g)},\dist_g^{(\ell_g)})}\cap\{Y_i:i\in T_{j_1}\}\cap \calB(\theta_{j_1},\Delta/3),
		\nonumber\\
		y&\in \sth{\calP_g^{(\ell_g)}\cap \calB(\mu_g^{(g,\ell_g)},\dist_g^{(\ell_g)})}\cap\{Y_i:i\in T_{j_2}\}\cap \calB(\theta_{j_2},\Delta/3).
	\end{align} 	
	As we have $\dist_g^{(\ell_g)}\leq {\Delta\over 8}$ and $\|\theta_{j_1}-\theta_{j_2}\|\geq \Delta$ we get a contradiction
	\begin{align}
		\|x-y\|&\geq
		\|\theta_{j_1}-\theta_{j_2}\|
		-\|x-\theta_{j_1}\|
		-\|y-\theta_{j_2}\|
		\geq {\Delta\over 3}.
		\nonumber\\
		\|x-y\|&\leq \|x-\mu_g^{(g,\ell_g)}\|
		+\|y-\mu_g^{(g,\ell_g)}\|\leq 2\dist_g^{(\ell_g)}\leq {\Delta\over 4}.
	\end{align}
	Hence all of the centroids lie in $\cup_{i=1}^k\calB(\theta_i,\Delta/3)$.
	
	
	
	
	Now it remains to show that $\sth{\mu_g^{(g,\ell_g)}}_{g=1}^k$ lie in different balls among $\sth{\calB(\theta_g,\Delta/3)}_{g=1}^k$. If not, then without loss of generality let $\calB\pth{\theta_1,{\Delta\over 3}}$ contains two of the centroids, say $\mu_{j_1}^{(j_1,\ell_{j_1})},\mu_{j_2}^{(j_2,\ell_{j_2})}$.
	Also, as $\calB\pth{\theta_g,{\Delta\over 3}}$ contains two centroids, by the pigeonhole principle we get that there is an index $g\neq 1$ such that 
	$$
	\mu_j^{(j,\ell_j)}\notin \calB\pth{\theta_g,{\Delta\over 3}},\quad j=1,\dots,k.
	$$ 
	In view of the disjoint union $\sth{\calB\pth{\theta_g,{\Delta\over8}}}_{g=1}^k$,and $\dist_j^{(\ell_j)}\leq{\Delta\over 8}$ the above implies
	\begin{align}
		\calB\pth{\theta_g,{\Delta\over 8}}\cap 
		\calB\pth{\mu_j^{(j,\ell_j)},\dist_j^{(\ell_j)}}=\phi,\quad j=1,\dots,k.
	\end{align}  
	Note that by \prettyref{lmm:E-conc-init-k}
	\begin{align}\label{eq:init15-k}
		\abs{\{Y_i:i\in [n]\}\cap \calB\pth{\theta_g,{\Delta\over 8}}}
		\geq {n\alpha\over 2k}.
	\end{align}
	As the disjoint union $\cup_{m=1}^k\calP_m^{(\ell_m)}$ is the entire set of data points, 
	we get
	\begin{align}
		\{Y_i:i\in [n]\}\cap \calB\pth{\theta_g,{\Delta\over 8}}
		&=\sth{\cup_{j=1}^k\calP_j^{(\ell_j)}}
		\cap \calB\pth{\theta_g,{\Delta\over 8}}
		\nonumber\\
		&= \cup_{j=1}^k\sth{\calP_j^{(\ell_j)}
			\cap \calB\pth{\theta_g,{\Delta\over 8}}}
		\subseteq 
		\cup_{j=1}^k\sth{\calP_j^{(\ell_j)}
			/ \calB\pth{\mu_j^{(j,\ell_j)},\dist_j^{(\ell_j)}}},
	\end{align}
	which implies 
	\begin{align}
		\abs{\{Y_i:i\in [n]\}\cap \calB\pth{\theta_g,{\Delta\over 8}}}
		&\leq \sum_{j=1}^k
		\sth{\calP_j^{(\ell_j)}
			/ \calB\pth{\mu_j^{(j,\ell_j)},\dist_j^{(\ell_j)}}}
		\nonumber\\
		&\leq \sum_{j=1}^k \beta\abs{\calP_j^{(\ell_j)}}
		\leq n\beta={n\alpha\over 4k^2}.
	\end{align}
	This provides a contradiction to \eqref{eq:init15-k}. Hence, all the centroids must lie in different $\calB\pth{\theta_j,{\Delta\over 3}}$ sets.
\end{proof}


\begin{proof}[Proof of \prettyref{lmm:good-centroid-in-complement}]
	
	In view of \prettyref{lmm:E-conc-init-k}, there is a constant $c_1>0$ such that
	\begin{align}\label{eq:init1-k-induction}
		\abs{\{Y_j:j\in T_h\}/\calB(\theta_h,c_1)}\leq n_h\beta^2,\quad h\in [k].
	\end{align}
	Hence we get that for $h\in [i-1]$
	\begin{align}
		&\abs{\overline{\calP_i^{(\bar \ell_i)}}\cap {\{Y_j:j\in T_h\}}\cap\calB(\theta_h,c_1)}
		\nonumber\\
		& \geq 	\abs{\overline{\calP_i^{(\bar \ell_i)}}\cap {\{Y_j:j\in T_h\}}} -\abs{{\{Y_j:j\in T_h\}}/\calB(\theta_h,c_1)}
		\nonumber\\
		& \geq 	\abs{\overline{\calP_i^{(\bar \ell_i)}}\cap {\{Y_j:j\in T_h\}}} 
		- n_h\beta^2
		\label{eq:init16-k}\\
		&\geq n_h- (k-i+1)n\beta -{5(k-i+1)n_h\over 4\log(1/(G(\Delta/16\sigma k)))}
		-n_h\beta^2
		\geq m_1.
		\nonumber
	\end{align}
	As we have 
	\begin{align}
		\label{eq:init18-k}
		\abs{\overline{\calP_i^{(\bar \ell_i)}}\cap \sth{\cup_{g=i}^k\{Y_j:j\in T_g\}}}
		&\leq {2n\alpha\beta\over 5k}
		\leq {m_1\over 2},
	\end{align}
	we get that the tightest neighborhood around any point in $\overline{\calP_i^{(\bar \ell_i)}}$ with a size $m_1$ will have a radius of at most $2c_{1}$ around that $Y_i$. Let $\mu_{i-1}^{(i-1,1)} = Y_{i^*}$ be the chosen centroid. Hence $\abs{\sth{\overline{\calP_i^{(\bar \ell_i)}}\cap \calB(Y_{i^*},2c_1)}}\geq m_1$. Then $\calB(Y_{i^*},2c_{1})$ and $\cup_{j\in [i-1]}\calB(\theta_j,c_{1})$ can not be disjoint, as in view of \eqref{eq:init16-k} it will imply that
	\begin{align}
		\abs{\overline{\calP_i^{(\bar \ell_i)}}}
		&\geq\abs{\sth{\overline{\calP_i^{(\bar \ell_i)}}\cap \calB(Y_{i^*},2c_1)}\cup\sth{\overline{\calP_i^{(\bar \ell_i)}}\cap\sth{\cup_{h\in [i-1]}\calB(\theta_h,c_1)}}}
		\nonumber\\
		&\geq m_1+ \sum_{h\in [i-1]} \abs{\overline{\calP_i^{(\bar \ell_i)}}\cap {\{Y_j:j\in T_h\}}\cap\calB(\theta_h,c_1)}
		\nonumber\\
		&\geq m_1-n\beta^2+ \sum_{h\in [i-1]} \abs{\overline{\calP_i^{(\bar \ell_i)}}\cap {\{Y_j:j\in T_h\}}} 
		\nonumber\\
		&= m_1-n\beta^2+ \abs{\overline{\calP_i^{(\bar \ell_i)}}}-
		\abs{\overline{\calP_i^{(\bar \ell_i)}}\cap \sth{\cup_{g=i}^k\{Y_j:j\in T_g\}}} 
		\nonumber\\
		&= {m_1\over 2}-n\beta^2+ \abs{\overline{\calP_i^{(\bar \ell_i)}}}
		\geq  \abs{\overline{\calP_i^{(\bar \ell_i)}}} + {m_1\over 4}.
		\label{eq:init17-k}
	\end{align}	
	where we use the fact that $\sth{i\in [n]:Y_i\in \calB(\theta_j,c_1)},j\in [k]$ are disjoint sets as $\min_{g\neq h\in [k]}\|\theta_g-\theta_h\|\geq \Delta$ and \eqref{eq:init17-k} followed from \eqref{eq:init18-k}. Hence, $Y_{i^*}$ is at a distance at most $3c_{1}$ from one of the centroids. Without loss of we can the closest centroid to be $\theta_{i-1}$. 
	
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%Define 
%\begin{align}
%	p={\ceil{\frac {n_g^{(s)}}2}-\ceil{{(\frac 12 -\gamma)} {n_g^{(s)}}}\over n_g^{(s)}}.
%\end{align}
%Note that $n_g^{(s)} p\geq 10$ by our assumptions
%and 
%\begin{align}
%	p \leq {\frac{n_g^{(s)}+1}{2}-{(\frac 12 -\gamma)}n_g^{(s)}\over n_g^{(s)}} = \frac 12 +\frac 1{2n_g^{(s)}}-{(\frac 12 -\gamma)}
%	=\gamma+\frac 1{n_{g}^{(s)}} < \frac 12.
%\end{align}
%Define the term
%\begin{align}
%	\eta_g^+(t)=\Phi(\Phi^{-1}(1-p)+t)-(1-p),.
%\end{align}
%Then using \cite[Theorem 2]{xia2019non} we get 
%\begin{align}
%	\PP\qth{\tilde w^{(np)} \geq \Phi^{-1}(1-p)+t}
%	&\leq  \exp\pth{-2n_g^{(s)}\qth{\eta_g^+(t)}^2}
%	\label{eq:result-upper-tail}
%\end{align}
%Note that for any $t>0$ we have
%\begin{align}
%	\label{eq:km0}
%	\abs{\eta_g^+(t)}
%	&=\abs{\Phi(\Phi^{-1}(1-p)+t)-\Phi(\Phi^{-1}(1-p))}
%	= \int_{\Phi^{-1}(1-p)}^{\Phi^{-1}(1-p)+t} \phi(x) dx
%	\geq t \phi (\Phi^{-1}(1-p)+t),
%\end{align}
%where the last equality followed as $\phi(\cdot)$ is decreasing in $[0,\infty)$ and $p<\frac 12$. Using \prettyref{lmm:gaussian-quantile-bound} we get for $t\leq \frac 12$
%\begin{align}
%	\phi(\Phi^{-1}(1-p)+t)
%	=
%	&\frac 1{\sqrt{2\pi}} \exp\sth{-{(\Phi^{-1}(1-p)+t)^2\over 2}}
%	\nonumber\\
%	&\geq \frac 1{\sqrt{2\pi}} \exp\sth{-(\Phi^{-1}(1-p))^2-t^2}
%	\geq {e^{-\frac 14}\over \sqrt{2\pi}}
%	{p^2\log\frac 1p}\cdot \exp\sth{-t^2}.
%\end{align}
%Choosing
%\begin{align}
%	t= {2e\sqrt{\pi\beta} }\cdot {1\over p^2 \log \frac 1p},
%\end{align}
%in view of \eqref{eq:km0} and \eqref{eq:km1} we continue \eqref{eq:result-upper-tail}
%\begin{align}\label{eq:bound_upper}
%	\PP\qth{\tilde w^{(np)} \geq \Phi^{-1}(1-p)+ {2e\sqrt{\pi\beta}}\cdot {1\over p^2 \log \frac 1p}
	%		\cdot \sqrt {\log n_g^{(s)}\over n_g^{(s)}}}
%	\leq \exp\sth{-4\beta\log (n_g^{(s)})}
%	\leq \frac 1{n^4}.
%\end{align}
%consider the concentration guarantee on $\tilde w^{(\ceil{\frac {n_g^{(s)}}2}+\ceil{{(\frac 12 -\gamma)} {n_g^{(s)}}})}$. Define 
%\begin{align}
%	q={\ceil{\frac {n_g^{(s)}}2}+\ceil{{(\frac 12 -\gamma)} {n_g^{(s)}}}\over n_g^{(s)}}.
%\end{align}
%Note that $n_g^{(s)} q\leq n_g^{(s)}-10$ by our assumptions and 
%\begin{align}
%	q \geq {\frac{n_g^{(s)}}{2}+{(\frac 12 -\gamma)}n_g^{(s)}\over n_g^{(s)}}= \frac 12+{(\frac 12 -\gamma)}\geq \frac 12.
%\end{align}
%Define the term
%\begin{align}
%	\eta_g^-(t)=\Phi(\Phi^{-1}(1-q)-t)-(1-q).
%\end{align}
%Then using \cite[Theorem 2]{xia2019non} we get 
%\begin{align}
%	\PP\qth{\tilde w^{(nq)} \leq \Phi^{-1}(1-q)-t}
%	\leq  \exp\pth{-2n_g^{(s)}\qth{\eta_g^-(t)}^2}
%	\label{eq:result-lower-tail}.
%\end{align}
%Note that for any $t>0$ we have
%\begin{align}
%	\label{eq:km2}
%	\abs{\eta_g^-(t)}
%	&=\abs{\Phi(\Phi^{-1}(1-q)-t)-\Phi(\Phi^{-1}(1-q))}
%	= \int_{\Phi^{-1}(1-q)-t}^{\Phi^{-1}(1-q)} \phi(x) dx
%	\geq t \phi (\Phi^{-1}(1-q)-t),
%\end{align}
%where the last equality followed as $\phi(\cdot)$ is increasing in $(-\infty,0]$ and $q\geq\frac 12$. Using \prettyref{lmm:gaussian-quantile-bound} we get
%\begin{align}
%	\label{eq:km3}
%	\phi(\Phi^{-1}(1-q)-t)
%	=
%	&\frac 1{\sqrt{2\pi}} \exp\sth{-{(\Phi^{-1}(1-q)+t)^2\over 2}}
%	\nonumber\\
%	&\geq \frac 1{\sqrt{2\pi}} \exp\sth{-(\Phi^{-1}(1-q))^2-t^2}
%	\nonumber\\
%	&=\frac 1{\sqrt{2\pi}} \exp\sth{-(\Phi^{-1}(q))^2-t^2}
%	\geq {1\over \sqrt{2\pi}e}
%	{(1-q)^2\log\frac 1{(1-q)}}.
%\end{align}
%Choosing
%\begin{align}
%	t= {2e\sqrt{\pi\beta} }\cdot {1\over {(1-q)}^2 \log \frac 1{(1-q)}}
%	\cdot \sqrt {\log n_g^{(s)}\over n_g^{(s)}},
%\end{align}
%in view of \eqref{eq:km2} and \eqref{eq:km3} we continue \eqref{eq:result-lower-tail}
%\begin{align}\label{eq:bound_lower}
%	\PP\qth{\tilde w^{(n{(1-q)})} \leq \Phi^{-1}(1-q)+ {2e\sqrt{\pi\beta}}\cdot {1\over {(1-q)}^2 \log \frac 1{(1-q)}}
	%		\cdot \sqrt {\log n_g^{(s)}\over n_g^{(s)}}}
%	\leq \exp\sth{-4\beta\log (n_g^{(s)})}
%	\leq \frac 1{n^4}.
%\end{align}
%Combining \eqref{eq:bound_lower} and \eqref{eq:bound_upper} we get with probability at least $1-\frac 2{n^4}$
%\begin{align}
%	&\abs{\tilde w^{(\ceil{\frac {n_g^{(s)}}2}-\ceil{{(\frac 12 -\gamma)} {n_g^{(s)}}})} - \tilde w^{(\ceil{\frac {n_g^{(s)}}2}+\ceil{{(\frac 12 -\gamma)} {n_g^{(s)}}})}}
%	\nonumber\\
%	&\leq
%	{\Phi^{-1}(1-p)-\Phi^{-1}(1-q)}+
%	{2e\sqrt{\pi\beta}} \pth{{1\over p^2 \log \frac 1p}
	%		+ {1\over {(1-q)}^2 \pth{\log \frac 1{1-q}}}}\sqrt {\log n_g^{(s)}\over n_g^{(s)}}.
%\end{align}
%We note the following
%\begin{itemize}
%	\item $\frac 12-{(\frac 12 -\gamma)}-\frac 1{n_g^{(s)}}\leq p\leq \frac 12-{(\frac 12 -\gamma)}+\frac 1{2n_g^{(s)}}$,
%	\item $\frac 12+{(\frac 12 -\gamma)}\leq q\leq \frac 12+{(\frac 12 -\gamma)}+\frac 3{2n_g^{(s)}}$,
%	\item In view of \prettyref{lmm:gaussian-quantile-bound}, \begin{align}
	%		\Phi^{-1}(1-p)&\leq \Phi^{-1}\pth{\frac 12+{(\frac 12 -\gamma)}+\frac 1{n_g^{(s)}}}
	%		\leq \sqrt{2\log\pth{1\over \frac 12-{(\frac 12 -\gamma)}-\frac 1{n_g^{(s)}}}},
	%		\\
	%		-\Phi^{-1}(1-q)&=\Phi^{-1}(q)\leq \Phi^{-1}\pth{\frac 12+{(\frac 12 -\gamma)}+\frac 3{2n_g^{(s)}}}
	%		\leq \sqrt{2\log\pth{1\over \frac 12-{(\frac 12 -\gamma)}-\frac 3{2n_g^{(s)}}}}
	%	\end{align}
%\end{itemize}	
%Combining the above results with $(a+b)^2\leq 2(a^2+b^2)$ we get
%\begin{align}
%	&\abs{\tilde w^{(\ceil{\frac {n_g^{(s)}}2}-\ceil{{(\frac 12 -\gamma)} {n_g^{(s)}}})} - \tilde w^{(\ceil{\frac {n_g^{(s)}}2}+\ceil{{(\frac 12 -\gamma)} {n_g^{(s)}}})}}
%	\nonumber\\
%	&\leq
%	4\pth{\sqrt{2\log\pth{1\over\frac 12-{(\frac 12 -\gamma)}-\frac 3{2n_g^{(s)}}}}+
	%		{2e\sqrt{\pi\beta}}\cdot \pth{\log\pth{\frac 12-{(\frac 12 -\gamma)}}\over \pth{\frac 12-{(\frac 12 -\gamma)}-\frac 3{2n_g^{(s)}}}^2}\cdot \sqrt {\log n_g^{(s)}\over n_g^{(s)}}}^2
%	\nonumber\\
%	&\leq 16\pth{\log\pth{1\over\frac 12-{(\frac 12 -\gamma)}-\frac 3{2n_g^{(s)}}}
	%		+2e^2\pi\beta\cdot \pth{\pth{\log\pth{\frac 12-{(\frac 12 -\gamma)}}}^2\over \pth{\frac 12-{(\frac 12 -\gamma)}-\frac 3{2n_g^{(s)}}}^4}\cdot {\log n_g^{(s)}\over n_g^{(s)}}}.
%\end{align}
%Finally using $n_g^{(s)}\geq n_{gg}^{s}\geq (1-{(\frac 12 -\gamma)})n_g^*=\frac {n_g^*}2$ and noting that ${\log x\over x}$ is decreasing in $x\geq e$ we get that whenever $n_g^*\geq 2e$
%\begin{align}
%	&\abs{\tilde w^{(\ceil{\frac {n_g^{(s)}}2}-\ceil{{(\frac 12 -\gamma)} {n_g^{(s)}}})} - \tilde w^{(\ceil{\frac {n_g^{(s)}}2}+\ceil{{(\frac 12 -\gamma)} {n_g^{(s)}}})}}
%	\nonumber\\
%	&\leq 16\pth{\log\pth{1\over\frac 12-{(\frac 12 -\gamma)}-\frac 3{n_g^*}}
	%		+2e^2\pi\beta\cdot \pth{\pth{\log\pth{\frac 12-{(\frac 12 -\gamma)}}}^2\over \pth{\frac 12-{(\frac 12 -\gamma)}-\frac 3{n_g^*}}^4}\cdot {2\log (n_g^*/2)\over n_g*}}.
%\end{align}

==> tex/heavy-tail.tex <==






\section{Notation} 
We will call a random vector $w\in \reals^d$ satisfies the spherical $p$ moment constraint with parameter $\sigma>0$ (here and below denoted by $w\in \calR_p(\sigma)$) if it has mean zero and
\begin{itemize}
	\item ${w\over \|w\|_2}$ is uniformly distributed on the unit sphere $\sfS^{d-1}$,
	\item $\EE\qth{\|w\|_2^{p}}<\sigma^p$.
\end{itemize}
For our paper we assume $p\geq 2$. We observe independent samples $Y_1,\dots,Y_n\in \reals^d$ from a mixture of $k$ many $\calR_p(\sigma)$ distributions
\begin{align}
	Y_i=\theta_{z_i}+w_i,\ i=1,\dots,n,\quad w_i\in \calR_p(\sigma),
\end{align}
where $ z=\sth{z_i}_{i=1}^n\in[k]^n$ denote the underlying labels, $\theta_1,\dots,\theta_k$ are the unknown centers of those $k$ distributions. Suppose that after $s$-steps the estimated centers are $\hat\theta^{(s)}_1,\dots,\hat\theta^{(s)}_k$ and the estimated labels are $\hat z^{(s)}=\sth{\hat z^{(s)}_1,\dots,\hat z^{(s)}_k}$. The initialization for the parameters correspond to $s=0$. 
We study the loss function
\begin{align}
	\ell(\hat z^{(s)},z) = \inf_{\pi\in \calS_k}\qth{\frac 1n \sum_{i=1}^n\indc{\pi(z^{(s)}_i)\neq z_i}},
\end{align}
where $\calS_k$ is the set of all permutations on $\{1,\dots,k\}$. Next we define notations for the different clusters in ground truth as well as during the iterations. For all $h,g\in [k]$, define
\begin{equation}\label{eq:cluster-def}
	\begin{gathered}
		T_h^*=\sth{Y_i:i\in [n],z_i=h},
		\hat T_h^{(s)}=\sth{Y_i:i\in [n],z_i^{(s-1)}=h}\\
		n^*_h = \abs{T^*_h}, n^{(s)}_h = \abs{T^{(s)}_h}, n^{(s)}_{hg} = \abs{T^*_h \cap T^{(s)}_g}
	\end{gathered}
\end{equation}
Note that for $s\geq 1$ this implies
\begin{align}
	T_h^{(s)}=\sth{Y_i:i\in[n], \|Y_i-\hat\theta_h^{(s-1)}\|\leq \|Y_i-\hat\theta_a^{(s-1)}\|,a\in[k]}.
\end{align}
with tie broken arbitrarily.

 Our clustering algorithm is the following.

\begin{algorithm}[H]
	\caption{The $\loa$}\label{algo:lloyd-rob}
	{\bf Input}:  Data $Y_1,\dots,Y_n$. Initial centroid estimates $(\hat \theta_1^{(0)},\dots,\hat \theta_k^{(0)})$. Error threshold $\epsilon$. Truncation level $\delta\in (0,\frac 12)$. Here we choose $\delta=0.49$.\\
	{\bf Steps}: 
	\begin{algorithmic}[1]
		\While{$\frac 1k\sum_{h=1}^k \|\hat\theta_h^{(s)}-\hat\theta_h^{(s-1)}\|_2^2 > \epsilon$,}
		\For{$h\in \sth{1,2,\dots,k}}$
		\State \textbf{Labeling step}:
		$$T_h^{(s)}=\sth{Y_i:i\in \sth{1,\dots,n}, \|Y_i-\hat\theta_h^{(s-1)}\|_2\leq \|Y_i-\hat\theta_a^{(s-1)}\|_2,a\in\{1,\dots,k\}, a\neq h}.$$
		\State \textbf{Estimation step:} 
		\begin{enumerate}[label=\alph*)]
			\item Compute the subset $V$ using
			$$
			V=\argmin_{S\subseteq T_h^{(s)},|S|=(1-\delta)n_h^{(s)}}
			\sum_{i:Y_i\in S} \left\|Y_i - \frac 1{(1-\delta)n_h^{(s)}}\sum_{i:Y_i\in S} Y_i\right\|_2^2,
			$$
			with tie broken arbitrarily.
			\item $\hat\theta_h^{(s)}= \frac 1{(1-\delta)n_h^{(s)}}\sum_{i:Y_i\in V} Y_i$.
		\end{enumerate}
		\EndFor
		\State $s=s+1$
		\EndWhile
	\end{algorithmic}
	{\bf Output}: $(\hat \theta_1^{(s)},\dots,\hat \theta_k^{(s)})$ and label estimate for $Y_i$ given by $\hat z_i^{(s)} = \argmin_{h\in\{1,\dots,k\}}\|Y_i-\hat\theta_h^{(s)}\|_2,$ with tie broken arbitrarily.
\end{algorithm}


%\begin{algorithm}[H]
%	\caption{The $\lss$ clustering algorithm}\label{algo:lloyd-rob}
%	{\bf Input}:  Data $Y_1,\dots,Y_n$. Initial centroid estimates $(\hat \theta_1^{(0)},\dots,\hat \theta_k^{(0)})$. Error threshold $\epsilon$. Truncation level $\delta\in (0,\frac 12)$. Here we choose $\delta=0.49$.\\
%	{\bf Steps}: 
%	\begin{algorithmic}[1]
%		\While{$\frac 1k\sum_{h=1}^k \|\hat\theta_h^{(s)}-\hat\theta_h^{(s-1)}\|_2^2 > \epsilon$,}
%		\For{$h\in \sth{1,2,\dots,k}}$
%		\State \textbf{Labeling step}:
%		$$T_h^{(s)}=\sth{Y_i:i\in \sth{1,\dots,n}, \|Y_i-\hat\theta_h^{(s-1)}\|_2\leq \|Y_i-\hat\theta_a^{(s-1)}\|_2,a\in\{1,\dots,k\}, a\neq h}.$$
%		\State \textbf{Estimation step:} 
%		\begin{enumerate}[label=\alph*)]
%			\item Compute the subset $V$ using
%			$$
%			V=\argmin_{S\subseteq T_h^{(s)},|S|=(1-\delta)n_h^{(s)}}
%			\sum_{i:Y_i\in S} \left\|Y_i - \frac 1{(1-\delta)n_h^{(s)}}\sum_{i:Y_i\in S} Y_i\right\|_2^2,
%			$$
%			with tie broken arbitrarily.
%			\item $\hat\theta_h^{(s)}= \frac 1{(1-\delta)n_h^{(s)}}\sum_{i:Y_i\in V} Y_i$.
%		\end{enumerate}
%%		\begin{enumerate}
%%			\item Define $T_{\epsilon} = \epsilon^{-\frac 1p}e^{-{C_2\over \epsilon p\alpha}}$, with $\epsilon = 0.3$
%%			\item Compute 
%%			$$
%%			\hat \theta_h^{(s)} = \argmin_{\theta\in \reals^d} \sum_{i:Y_i\in T_h^{(s)}} \ell_{T_{\epsilon}}(\|X_i-\theta\|_2),\quad h\in \sth{1,\dots,k},$$
%%			where 
%%			$
%%			\ell_\tau(x) = x^2\indc{x\leq \tau}+\tau^2\indc{x>\tau}.
%%			$
%%		\end{enumerate}
%		\EndFor
%		\State $s=s+1$
%		\EndWhile
%	\end{algorithmic}
%	{\bf Output}: $(\hat \theta_1^{(s)},\dots,\hat \theta_k^{(s)})$ and label estimate for $Y_i$ given by $\hat z_i^{(s)} = \argmin_{h\in\{1,\dots,k\}}\|Y_i-\hat\theta_h^{(s)}\|_2,$ with tie broken arbitrarily.
%\end{algorithm}

\section{Results}

Denote the minimum separation between the centers by $\Delta$
\begin{align}
	\Delta=\min_{g,h\in[k],g\neq h}\|\theta_g-\theta_h\|_2.
\end{align}
We denote the signal to noise ratio as
\begin{align}
\snr = {\Delta\over 2\sigma}.
\end{align}
Let $\Lambda_s$ denote the error rate of estimating the centers at iteration $s$
\begin{align}
	\Lambda_s = \max_{h\in[k]}\frac 1{\Delta} \|\hat \theta_h^{(s)}-\theta_h\|_2.
\end{align}
Let us define the minimum fraction of points in the data set that come from a single component in the Gaussian mixture as
\begin{align}
	\alpha=\min_{g\in[k]} {n_{g}^*\over n}.
\end{align}
Define the cluster-wise mis-clustering rate as
\begin{align}\label{eq:mislabel}
	G_s=\max_{g\in [k]} \sth{\max\sth{{\sum_{h\in[k]\atop h\neq g} n_{gh}^{(s)}\over n_g^*},{\sum_{h\in[k]\atop h\neq g} n_{hg}^{(s)}\over n_g^{(s)}}}}
\end{align}
Our main result is the following.
\begin{theorem}
	\label{thm:main}
	Suppose that $n\alpha\geq c\log n$ for some $c>0$. There exists absolute constants $c_1,c_2>0$ such that the followings are satisfied. If the clustering initialization satisfies  
	$$\Lambda_0\leq \frac 12-{e^{25/(4p\alpha)}\over (\snr)^{1/2}},$$
	then whenever $\snr\geq c_1(0.3)^{-\frac 1p}e^{\frac {10(1+20/7\alpha)}{3p}}=M$ 
	we have $$\EE\qth{\ell(\hat z^{(s)},z)}\leq 2k^2{\pth{1-{c_2\over M}}^{-p}\over (\snr)^p}
	+ 4kn^{-c/4}+16e^{-0.3n},
		\quad s\geq 1.
		$$
\end{theorem}

\section{Proof strategy}

The proof on the $\lss$ algorithm is primarily based in the following two stages: 
\begin{enumerate}[label=(\alph*)]
	\item analyzing accuracy of the clustering method based on current center estimates,
	\item analysis of the next center updates based on current labels.
\end{enumerate} 
We obtain results on these steps separately and then combine them to prove \prettyref{thm:main}. Our analysis depends on high-probability events of the following type. For any symmetric matrix $A$ let $\lambda_{\max}(A)$ denote its maximum eigen value.
\begin{lemma}
	\label{lmm:E-prob}
	Fix $0<\tau,\epsilon_0<\frac 12$. There is a set $\calE_{\tau,\epsilon_0}$ with $\PP\qth{\calE_{\tau,\epsilon_0}}\geq 1-kn^{-c/2}-e^{-0.3n}$ on which the following holds: 
	\begin{enumerate}[label=(\roman*)]
		\item For any $\tau>0$ and any $S\subseteq [n]$ with $|S|>\beta n$, the cardinality of the set 
		$$\sth{i\in S: \norm{w_i}\leq {\sigma}\tau^{-\frac 1p}e^{\frac 1{\tau p}(1+\frac 1\beta)}}$$
		is at least $(1-\tau)|S|$.
		
		\item For any $\epsilon\in[\epsilon_0,1/2]$ and $g,h\in[k]$ we have
		$$\sum_{i:Y_i\in T_g^*}\indc{\epsilon^2\Delta\leq \|w_i\|}
		\leq \frac {5}{2p \alpha\log(\epsilon_0^2\Delta/\sigma)}.$$
	\end{enumerate}
\end{lemma}
\begin{proof}
	For each of the cases we separately construct sets of high probability on which the results hold. Then taking intersection we get the result. The individual analyses have been provided in \prettyref{lmm:norm-concentration}, \prettyref{lmm:Chernoff-binom} in \prettyref{app:main-lemma-proof}.
\end{proof}

The following lemma provides results that show upper bound on $G_{s+1}$ based on $\Lambda_s$ and establish upper bound on $\Lambda_{s}$ in terms of $G_s$. 

\begin{lemma}\label{lmm:Gs-Ls-bound}
	Fix $\epsilon_0\in (0,\frac 12]$. Then on the set $\calE_{\epsilon_0}=\calE_{0.5,\epsilon_0}$, which has probability at least $1-n^{-c/2}-ke^{-0.3n}$, we have for all $s\geq 0$
	\begin{enumerate}[label=(\roman*)]
		\item If $\Lambda_s\leq \frac 12-\epsilon_0$ then $G_{s+1} \leq \frac {5}{2p \alpha\log(\epsilon_0^2\Delta/\sigma)}$,
		\item If $G_{s+1}\leq 0.2$ then $\Lambda_{s+1}\leq {3\sigma\over \Delta}(0.3)^{-\frac 1p}e^{\frac {10(1+\frac 5{4\alpha})}{3p}}$.
	\end{enumerate}
\end{lemma}



\begin{proof}[Proof of \prettyref{lmm:Gs-Ls-bound}]
	The proof of \prettyref{lmm:Gs-Ls-bound}(i) has been presented in \prettyref{app:Gs-Ls-i}. We present below the proof of \prettyref{lmm:Gs-Ls-bound}(ii). We prove this using contradiction. For simplicity of notation we denote 
	$$D={\sigma\over \Delta}(0.3)^{-\frac 1p}e^{\frac {10(1+\frac 5{4\alpha})}{3p}}.$$ 
	Let us assume $\Lambda_{s+1} > {3D\over \Delta}$. This implies that there exists a cluster $h$ such that the centroid estimation error satisfies 
	$$\|\hat \theta_h^{(s+1)}-\theta_h\|> {3D}.$$ 
	As $G_{s+1}\leq 0.2$ we know that $n_{hh}^{(s)}\geq 0.8 n_h^{(s)}$. As we are on the set $\calE_{\epsilon_0}$, we use \prettyref{lmm:E-prob} with 
	$$
	 \tau =0.3,\quad S=\{i\in [n]:Y_i\in T_{h}^{(s)}\cap T_{h}^*\}, \quad \beta = {0.8 \alpha} < {n_{hh}^{(s)}\over n}.
	$$ 
	This gives us that there are at least $0.7n_{hh}^{(s)}(=0.56 n_h^{(s)})$ many points within a radius $D$ of $\theta_h$. As our subset selection strategy guarantees that we choose $0.55 n_h^{(s)}$ points within a radius $D$ of the estimator $\hat \theta_h^{(s)}$, we get a contradiction.
\end{proof}

\section{Proof of \prettyref{thm:main}}

The mis-clustering rate at step $s$ is given by 
\begin{align}
	A_s=\frac 1n \sum_{i=1}^n\indc{z^{(s)}_i\neq z_i}
	=\frac 1n \sum_{h\neq g \in [k]} n_{hg}^{(s)}.
\end{align} 
For $c_1$ to be chosen later, we define
$$\epsilon_0={c_2\over (\Delta/2\sigma)^{1/2}}.$$
Then from \prettyref{lmm:Gs-Ls-bound} it follows that we can choose $c_1,c_2>0$ such that on the set $\calE_{\epsilon_0}$ we have that if $\Lambda_0\leq \frac 12-\epsilon_0$ then $G_1\leq 0.2$.
A second application of \prettyref{lmm:Gs-Ls-bound} guarantees that we can choose $c_3$ large enough such that if  
$${\Delta\over \sigma}(0.3)^{\frac 1p}e^{-\frac {10(1+\frac 5{4\alpha})}{3p}}\geq M\geq c_3$$
then on the set $\calE_{0.2}$ we have,
\begin{enumerate}[label=(P\arabic*)]
	\item \label{eq:P1} $G_s\leq \frac {5}{2p \alpha\log(\epsilon_0^2\Delta/\sigma)}\leq 0.2$ for all $s\geq 1$
	\item $\Lambda_s\leq {3\sigma\over \Delta}(0.3)^{-\frac 1p}e^{\frac {10(1+\frac 5{4\alpha})}{3p}}\leq {C_1\over M} \leq 0.2$ for all $s\geq 1$.
\end{enumerate}
Combining the above displays we get that on the set
\begin{align}
	\label{eq:Prob-E}
	\calE&=\calE_{\epsilon_0}\cap \calE_{0.2}\text{ with }
	\PP\qth{\calE}
	\geq 1-4kn^{-c/4}-e^{-0.3n}
\end{align} 
we have
\begin{align}
	\label{eq:km14}
	\Lambda_s\leq 0.2,G_{s}\leq 0.2 \text{ for all } s\ge 1.
\end{align}
We will show that $\PP\qth{\left.z_i\neq \hat z_i^{(s+1)}\right|\calE}$ is small for each $i\in [n]$.
Note that $$\indc{z_i\neq\hat z_i^{(s+1)}}
=\frac 12\sum_{g,h\in [k]\atop g\neq} \indc{\hat z_i^{(s+1)}=h,z_i=g}.$$ Fix a choice for $z_i$, say equal to $g\in [k]$. Then 
For any $h\in[k],h\neq g$,
\begin{align}\label{eq:km21}
	\indc{z_i=g,\hat z_i^{(s+1)}=h}
	&\leq \indc{\|Y_i-\hat\theta_h^{(s)}\|^2
		\leq \|Y_i-\hat\theta_g^{(s)}\|^2, Y_i\in T_g^*}
	\nonumber\\
	&=\indc{\|\theta_g+w_i-\hat\theta_h^{(s)}\|^2
		\leq \|\theta_g+w_i-\hat\theta_g^{(s)}\|^2}
	=\indc{\|\theta_g-\hat\theta_h^{(s)}\|^2-\|\theta_g-\hat\theta_g^{(s)}\|^2\leq 2\langle w_i,\hat\theta_h^{(s)}-\hat\theta_g^{(s)}\rangle}.
\end{align}
Triangle inequality implies
\begin{align}
	\|\theta_g-\hat\theta_h^{(s)}\|^2\geq \pth{\|\theta_g-\theta_h\|-\|\theta_h-\hat\theta_h^{(s)}\|}^2
	\geq (1-\Lambda_s)^2\|\theta_g-\theta_h\|^2.
\end{align}
Using $$\|\theta_g-\hat\theta_g^{(s)}\|\leq \Lambda_s\Delta
\leq \Lambda_s\|\theta_g-\theta_h\|$$
and the fact that $(1-x)^2-y^2\geq (1-x-y)^2$ when $y(1-x-y)\geq 0$, we obtain
\begin{align}
	&\|\theta_g-\hat\theta_h^{(s)}\|^2-\|\theta_g-\hat\theta_g^{(s)}\|^2
	\geq (1-\Lambda_s)^2\|\theta_g-\theta_h\|^2
	-\Lambda_s^2\|\theta_g-\theta_h\|^2
	\geq (1-2\Lambda_s)^2\|\theta_g-\theta_h\|^2.
\end{align}
In view of \eqref{eq:ht21} the last display implies
\begin{align}
	\label{eq:km10}
	\indc{z_i=g,\hat z_i^{(s+1)}=h}
	\leq \indc{(1-2\Lambda_s)^2\|\theta_g-\theta_h\|^2\leq 2\langle w_i,\hat\theta^{(s)}_h-\hat\theta^{(s)}_g \rangle}.
\end{align}
Using Property \ref{eq:P1} and 
\begin{align*}
	|\langle w_i,\hat\theta^{(s)}_h-\hat\theta^{(s)}_g\rangle|
	&\leq \|w_i\|\cdot \|\hat\theta^{(s)}_h-\hat\theta^{(s)}_g\|
	\nonumber\\
	&\leq \|w_i\|\cdot(\|\hat\theta^{(s)}_h-\theta_h\|+\|\hat\theta^{(s)}_h-\theta_h\|+\|\theta_g-\theta_h\|)
	\leq \|w_i\|(2\Lambda_s\Delta+\Delta)
	\leq 2\|w_i\|\Delta,
\end{align*}
we get that
\begin{align*}
	\indc{z_i=g,\hat z_i^{(s+1)}=h}
	\leq \indc{(1-2\Lambda_s)^2\Delta\leq 2\|w_i\|}
	\leq \indc{\frac 12\pth{1-{2C_1\over M}}\Delta\leq \|w_i\|}.
\end{align*}
Taking expectation conditioned on $\calE$ we get
	\begin{align}
		\PP\qth{\left.z_i\neq \hat z_i^{(s+1)}\right|\calE}
		&\leq
		k^2 \max_{g,h\in [k]\atop g\neq h}\PP\qth{\left.z_i=g, \hat z_i^{(s+1)}=h \right|\calE}
		\leq 2k^2{\pth{1-{2C_1\over M}}^{-p}\over (\Delta/2\sigma)^p}
	\end{align}
	This implies
	\begin{align}
		\EE\qth{A_{s+1}|\calE}
		=\frac 1n\sum_{i=1}^n\PP\qth{\left.z_i\neq z_i^{(s+1)}\right| \calE}\leq 2k^2{\pth{1-{2C_1\over M}}^{-p}\over (\Delta/2\sigma)^p}.
	\end{align}
Combining the above with \eqref{eq:Prob-E} we get
\begin{align}
	\EE\qth{A_s}&\leq4 kn^{-c/4}+16e^{-0.3n}+2k^2{\pth{1-{2C_1\over M}}^{-p}\over (\Delta/2\sigma)^p}.
\end{align}

\section{Lower bound}
\begin{theorem}
	 For an absolute constant $C>0$ such that the following holds true. If the error distributions are chosen from $\calR_p(\sigma)$, then
	 $$\inf_{\hat z}\sup\EE_{z\in[k]^n}\qth{\ell(\hat z,z)}
	\geq {C\alpha\over k^2p }\cdot{1\over (\snr)^{p}(\log (\snr))^{1.5}}.$$
\end{theorem}
\begin{proof}
	We follow the proof technique of \cite[Theorem 3.3]{lu2016statistical}. For any $z\in [k]^n$, let us define $n_u(z)=\sum_{i=1}^n \indc{z_i=u}$. Let $z^*\in [k]^n$ satisfying $n_1(z^*)\leq n_2(z^*)\leq\dots\leq n_k(z^*)$, with $n_1(z^*)=n_2(z^*)=\floor{\alpha n}$. It is easy to check the existence of $z^*$. For each $u\in [k]$ we choose a subset of $\{i\in [n]: z^*(i)=u\}$ with cardinality $\ceil{n_u(z^*)-{\alpha n\over 4k}},$ denoted by $T_u$. Define $T=\cup_{u=1}^k T_u$ and
	$\calZ^* = \sth{z\in \calZ,z_i=z_i^* \text{ for all } i\in T}$. 
	A key observation is that for any $z\neq \tilde z\in\calZ^*$, we have $\frac 1n\sum_{i=1}^n\indc{z_i\neq \tilde z_i}\leq \frac kn\cdot \frac {\alpha n}{4k}=\frac \alpha 4$, and 
	$$
	\frac 1n\sum_{i=1}^n\indc{\pi(z_i)\neq \tilde z_i}\geq \frac 1n(\alpha n-{\alpha n\over 4k})\geq {\alpha\over 2}
	$$
	for all $\pi\in \calS_k$ which is not the identity permutation. Thus, $\ell(\tilde z,z)=\frac 1n\sum_{i=1}^n \indc{z_i\neq \tilde z_i}$ for all $z,\tilde z\in \calZ^*$. Then following the same arguments in the proof of \cite[Theorem 2]{gao2018community}, we can obtain
	\begin{align}\label{eq:gao2018}
	\inf_{\hat z}\sup_{z\in \calZ} \EE\qth{\ell(\hat z,z)}
	\geq {\alpha\over 6}
	\frac 1{T^c}\sum_{i\in T^c}\qth{\frac 1{2k^2}\inf_{\hat z_i}(\PP_1\qth{\hat z_i=2}+\PP_2\qth{\hat z_i=1})}.
	\end{align}
	Here $\PP_t,t\in \{1,2\}$ denote the probability distribution of our data given $z_i=t$. By Neyman-Pearson Lemma, the infimum of the right hand side of the last display is achieved by the likelihood ratio test 
	$$
	\hat z_i = \argmin_{g\in \{1,2\}}\|Y_i-\theta_g\|^2.
	$$
	Thus,
	$$
	\inf_{\hat z_i}\pth{\frac 12 \PP_1\qth{\qth{\hat z_i=2}+\frac 12\PP_2\qth{\hat z_i=1}}}
	=\PP\qth{\|\theta_1+w_i-\theta_2\|^2\leq \|w_i\|^2}
	=\PP\qth{\|\theta_1-\theta_2\|^2\leq 2\langle w_i,\theta_1-\theta_2\rangle}.
	$$
	 Note that as $|\langle w_i,\theta_1-\theta_2\rangle|\leq \|w_i\|\cdot\|\theta_1-\theta_2\|$, from the last display we get
	\begin{align}
		\label{eq:lb1}
	\inf_{\hat z_i}\pth{\frac 12 \PP_1\qth{\qth{\hat z_i=2}+\frac 12\PP_2\qth{\hat z_i=1}}}
	\geq \PP\qth{\|w_i\|\geq \frac 12\|\theta_1-\theta_2\|}
	\geq \PP\qth{\|w_i\|\geq \Delta/2}.
	\end{align}
	Next we choose all the errors to have the distribution
	\begin{align*}
	\begin{gathered}
		\{w_i\}_{i=1}^n\simiid R\cdot \Unif(\calS_{d-1}),\\ R = \sigma\pth{\xi\over pa\log a}^{\frac 1p}\tilde R,
	\ \PP\qth{\tilde R\geq r}=\frac {a(\log a)^{1+\xi}\indc{r\geq 0}}{(1+r^{p-1})(a+r)(\log(a+r))^{1+\xi}},\ a>1,\xi>0.
	\end{gathered}
	\end{align*}
	where $R$ is the radial distribution and $\Unif(\calS_{d-1})$ is the uniform distribution over the unit sphere, and they are independent.
	The $p$-th moment of $R$ is bounded from above by $\sigma^p$ follows from the fact that the $p$-th moment of $\tilde R$ is bounded from above as
	$$
	\EE\qth{\tilde R^{p}}
	=p\int_{0}^\infty  r^{p-1} \PP\qth{\tilde R > r} dr
	\leq \frac {pa\log a}\xi.
	$$
	This implies, with $a=2,\xi=\frac 12$, for an absolute constant $C>0$
	$$
	\PP\qth{\|w_i\|\geq \Delta/2}
	=\PP\qth{\tilde R\geq \frac{\Delta}{2\sigma}\pth{\xi\over pa\log a}^{-\frac 1p}}
	\geq C {1\over p(\Delta/2\sigma)^{p}(\log (\Delta/2\sigma))^{1.5}},
	$$
	where we used $\abs{\log\pth{\pth{\xi\over pa\log a}^{-1/p}}}\leq c$ for a small constant $c>0$. Thus using \eqref{eq:gao2018} and \eqref{eq:lb1} we conclude the result.
\end{proof}

\section{Minimax optimality with Sub-Gaussian mixtures}
In this section we prove that our algorithm achieves the optimal misclustering rate when the errors are generated from Sub-Gaussian mixture. In our model, the observed data $Y_1,\dots,Y_n\in \reals^d$ are distributed as
\begin{align}
	Y_i=\theta_{z_i}+w_i,\ i=1,\dots,n,
\end{align}
where $\sth{z_i}_{i=1}^n\in[k]^n$ denote the underlying unknown component labels of the points, and $w_i$-s denote the error variables. We assume that $w_i$-s are independent 0 mean Sub-Gaussian vectors with parameter $\sigma>0$, i.e.,
\begin{align}\label{eq:subg-defn}
	\EE\qth{e^{\langle a,w_i \rangle}}
	\leq e^{\sigma^2\|a\|^2\over 2}, \text{ for all $i\in \sth{1,\dots,n}$ and $a\in \reals^d$}.
\end{align}
We show the following.
Define the cluster-wise correct classification proportion at step $s$ as
\begin{align}
	H_s=\min_{g\in [k]}\sth{\min\sth{{n_{gg}^{(s)}\over n_g^*},{n_{gg}^{(s)}\over n_{g}^{(s)}}}}.
\end{align}
Our result is the following.
\begin{theorem}
	\label{thm:main-subg}
	There exists absolute constants $c_0,c_1,c_2,c_3,c_4>0$ such that the followings are satisfied.
	\begin{enumerate}[label=(\alph*)]
		\item \textbf{$\snr< c_0\sqrt {d/\alpha}$:} Assume $n\alpha^2\geq Ck\log n$ and ${\snr}\sqrt{\alpha\over 1+{dk\over n}}\geq C\sqrt k$ for a sufficiently large constant $C$. If the clustering initialization satisfies either one of the following conditions
		$${H_0}\geq 1-\frac 2{\sigma\sqrt d}\pth{\frac 12 - \frac {c_1/{\alpha}^{1/4}}{\pth{\snr}^{1/2}}}\quad  \text{ or } \quad \Lambda_0\leq \frac 12-{c_2/{\alpha}^{1/4}\over \pth{\snr}^{1/2}}.$$
		Then whenever $\snr\sqrt \alpha \geq M\geq c_3$,  we have $$\EE\qth{\ell(\hat z^{(s)},z)}\leq \exp\sth{-\frac 12\pth{1-{c_4\over \sqrt \snr}}(\snr)^2},
		\quad s\geq 3\log n.
		$$
		
		\item \textbf{$\snr\geq c_0\sqrt {d/\alpha}$:} Suppose the clustering initialization satisfies either one of the following conditions
		$${H_0}\geq \frac 12 +\gamma_0 \text{ with } \gamma_0>2.1\alpha \quad  \text{ or } \quad \Lambda_0\leq \frac 12-{c_2/{\alpha}^{1/4}\over \pth{\snr}^{1/2}}.$$
		Then whenever $\snr\sqrt \alpha \geq M\geq c_3$,  the $\lss$ algorithm with $\delta=\frac 12-{\gamma_0\over 4}$ achieves the misclustering rate
		$$
		\EE\qth{\ell(\hat z^{(s)},z)}\leq \exp\sth{-\frac 12\pth{1-{c_4\over \sqrt \snr}}{(\snr)^2}},
		\quad s\geq 1.
		$$
	\end{enumerate}
	
\end{theorem}
\begin{remark}
	The result \cite[Theorem 3.4]{lu2016statistical} shows that it is not possible to improve the misclustering error beyond the rate $e^{-\frac 12(1+o(1)){(\snr)^2}}$. This establishes the optimality of the coordinate-wise median based Lloyd algorithm.
\end{remark}

\begin{proof}[Proof of \prettyref{thm:main-subg}]
	The proof of part (a) is essentially the same as the proof of the similar result \cite[Theorem 3.2]{lu2016statistical} for usual $k$-means. This is because the part of the cluster, the mean of which we use to construct our centroid estimates, is of similar order as the full clusters themselves. As a result we can use the similar concentration bounds that were used to analyze the mean of the full sample in the classical $k$-means problems. We omit the proof here.
	
	To prove part (b), we use the following key lemma.
	\begin{lemma}
		\label{lmm:E-prob-subg}
		Fix $0<\tau,\epsilon_0<\frac 12$. There is a set $\calE_{\tau,\epsilon_0}$ with $\PP\qth{\calE_{\tau,\epsilon_0}}\geq 1-kn^{-c/2}-4e^{-0.3n}$ on which the following holds: 
		\begin{enumerate}[label=(\roman*)]
			\item For any $S\subseteq [n]$ with $|S|>\beta n$, the cardinality of the set 
			$$\sth{i\in S: \|{w_i}\|\leq \sigma \pth{\sqrt d + \sqrt{2\pth{\frac 1\tau\pth{1+\frac 1\beta}+\log(1/\tau)}}}}$$ 
			is at least $(1-\tau)|S|$.
			\item For any $\epsilon\in[\epsilon_0,1/2]$ and $g,h\in[k]$ we have
			$$\sum_{i:Y_i\in T_g^*}\indc{\epsilon^2\|\theta_g-\theta_h\|^2\leq \langle w_i,\theta_h-\theta_g\rangle}
			\leq \frac {5n_g^*}{4\epsilon_0^4(\Delta/\sigma)^2}$$
			\item For any symmetric matrix $A$, let $\lambda_{\max}(A)$ denote its maximum eigen value. Then 
			$$\lambda_{\max}\pth{\sum_{i:Y_i\in T_g^*} w_iw_i^{\sfT}}\leq 6\sigma^2(n_g^*+d) \text{ for all } g\in [k].$$
		\end{enumerate}
	\end{lemma} 
	To prove the above lemma, for each of the cases we separately construct sets of high probability on which the results hold. Then taking intersection we get the result. The analysis of (i) has been provided in \prettyref{lmm:norm-concentration-subg}, the statements (ii),(iii) are the exact results from \cite[Lemma 12, Lemma 13]{JKY2023}.
	
	Based on the above result we get the following results on step-wise clustering errors due to mislabelling.

\begin{lemma}\label{lmm:Gs-Ls-bound-subg}
	Fix $0<\epsilon_0\leq \frac 12,\frac 5{n\alpha} <\gamma_0 \leq \frac 12$. Let $r_k={\Delta\over\sigma}\sqrt{\alpha\over 1+{dk/n}}$. Then on the set $\calE_{\tau,\epsilon_0}$ with $\tau={\gamma_0\over 1+2\gamma_0}$ we have
	\begin{enumerate}[label=(\roman*)]
		\item If $\Lambda_s\leq \frac 12-\epsilon_0$ then $H_{s+1} \geq 1-{5\over \epsilon_0^4 r_k^2}
		-{48\Lambda_s^2\over \epsilon_0^4r_k^2}$,
		\item If $H_s\geq \frac 12+\gamma_0$ then $\Lambda_s\leq {3\sigma\over \Delta} \pth{\sqrt d + \sqrt{2\pth{{1+2\gamma_0\over \gamma_0}\pth{1+\frac 1\beta}+\log\pth{1+2\gamma_0\over \gamma_0}}}}$.
	\end{enumerate}
\end{lemma}

The proof of above result is straightforward. The proof of \prettyref{lmm:Gs-Ls-bound-subg}(i) is exactly the same as in \cite[Appendix C]{JKY2023}, so we skip it here. 
	We present below the proof of \prettyref{lmm:Gs-Ls-bound}(ii). We prove this using contradiction. For simplicity of notation we denote 
	$$D={\sigma} \pth{\sqrt d + \sqrt{2\pth{{1+2\gamma_0\over \gamma_0}\pth{1+\frac 1\beta}+\log\pth{1+2\gamma_0\over \gamma_0}}}}.$$ 
	Let us assume $\Lambda_{s} > 3D$. This implies that there exists a cluster $h$ such that the centroid estimation error satisfies 
	$$\|\hat \theta_h^{(s+1)}-\theta_h\|> {3D}.$$ 
	As $H_{s}\geq \frac 12+\gamma_0$ we know that $n_{hh}^{(s)}\geq \pth{\frac 12+\gamma_0} n_h^{(s)}$. As we are on the set $\calE_{\tau,\epsilon_0}$, we use \prettyref{lmm:E-prob-subg} with 
	$$
	\tau = {\gamma_0\over 1+2\gamma_0},\quad S=\{i\in [n]:Y_i\in T_{h}^{(s)}\cap T_{h}^*\}, \quad \beta = {\pth{\frac 12+\gamma_0} \alpha} < {n_{hh}^{(s)}\over n}.
	$$ 
	This gives us that there are at least $\pth{1-{\gamma_0\over 1+2\gamma_0}}n_{hh}^{(s)}(=\pth{\frac 12+{\gamma_0\over 2}} n_h^{(s)})$ many points within a radius $D$ of $\theta_h$. As our subset selection strategy guarantees that we choose $\pth{\frac 12+{\gamma_0\over 4}} n_h^{(s)}$ points within a radius $D$ of the estimator $\hat \theta_h^{(s)}$, we get a contradiction.


Next we use the above results to prove \prettyref{thm:main-subg}(ii). For $c_1$ to be chosen later, we define
$$\epsilon_0={c_1/\alpha^{1/4}\over \pth{\snr}^{1/2}}.$$
Let $G_s$ be the mislabeling proportion as defined before in \eqref{eq:mislabel}. Then from \prettyref{lmm:Gs-Ls-bound-subg} it follows that we can choose $c_0,c_1>0$ such that on the set $\calE_{{\gamma_0\over 1+2\gamma_0},\epsilon_0}$:
\begin{itemize}
	\item if $H_0\geq \frac 12+\gamma_0$ then $\Lambda_0\leq 0.3$,
	\item if $\Lambda_0\leq \frac 12-\epsilon_0$ then $H_1\geq 0.7$.
\end{itemize}
A second application of \prettyref{lmm:Gs-Ls-bound-subg} guarantees that we can choose $c_0$ large enough such that if  
$\snr\geq c_0\sqrt{d/\alpha}$
then on the set $\calE_{{5\over 26},0.2}$, with $\epsilon_1=\gamma_1=0.2$,
\begin{itemize}
	\item if $G_s\leq 0.3$ then
	\begin{align}
		\label{eq:Ls}
		\Lambda_s&\leq {12\sqrt 2/\alpha^{1/2}\over \sqrt{0.2}\snr} \leq 0.3,
	\end{align}
	\item if $\Lambda_s\leq 0.3$ then
	\begin{align}
		\label{eq:Gs}
		G_{s+1}&\leq {5/\alpha\over (0.2)^4(\snr)^2}+{48(0.3)^2/\alpha\over (0.2)^4(\snr)^2}\leq 0.3.
	\end{align}		
\end{itemize}
and whenever 
Combining the above displays we get that on the set
\begin{align}
	\label{eq:Prob-E}
	\calE&=\calE_{{\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{{5\over 26},0.2}
	\nonumber\\
	\PP\qth{\calE}
	&\geq 1-4kn^{-c/4}-4e^{-0.3n}
\end{align} 
we have
\begin{align}
	\label{eq:ht14}
	\Lambda_s\leq 0.3,G_{s+1}\leq 0.3 \text{ for all } s\ge 0.
\end{align}
The rest of the analysis is 
identical to that of the proof of \cite[Theorem 1]{JKY2023} where it is shown that once we achieve $\Lambda_s\leq 0.3$ for all $s\geq 3$, the mislabeling rate follows. We omit it here.
\end{proof}


\section{Clustering in presence of adversarial outliers \nb{TBD}}

\subsection{Error distributions with moment constraints}

\subsection{Sub-Gaussian error distributions}
Suppose that an adversary adds $n^{\out}$ many points to our existing data set. Then we have the following guarantees.
\begin{theorem}
	\label{thm:optim-outl}
	Suppose that $n\alpha\geq c\log n$ for some $c>0$. There exists absolute constants $c_1,c_2,c_3,c_4,c_5>0$ such that the followings are satisfied. For any $\eta\in(0,1]$, if the clustering initialization satisfies either one of the following conditions
	$${H_0}\geq \frac 12+\frac {c_1/\alpha}{\pth{\snr}^2}\quad  \text{ or } \quad \Lambda_0\leq \frac 12-{c_2/\alpha\over \pth{\snr}^{\frac 12(1-\eta)}},$$
	then whenever $$\snr\sqrt\alpha\geq M\geq c_3,$$ 
	for any $n^{\out}\leq n\alpha(1-c_4M^{-2\eta})$ our algorithm guarantees $$\EE\qth{\ell(\hat z^{(s)},z)}\leq \exp\sth{-\frac 12\pth{1-{c_5\over \sqrt M}}{(\snr)^2}},
	\quad s\geq 1.
	$$
\end{theorem}


\subsection{Step-wise clustering errors due to mislabelling (in presence of outliers)}
The proof of the above theorem hinges on the following lemma, similar to \prettyref{lmm:Gs-Ls-bound}.

\begin{lemma}\label{eq:HsLs-bound}
	Fix $\epsilon_0,\gamma_0\in (0,\frac 12]$ and suppose that an adversary added $n\beta$ many outliers with $\beta\leq\alpha(1-\delta)$ for some $\delta>0$. Let $r_k={\Delta\over\sigma}\sqrt{\alpha\over 1+{dk/n}}$. Then on the set $\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0} $ we have
	\begin{enumerate}[label=(\roman*)]
		\item If $\Lambda_s\leq \frac 12-\epsilon_0$ then $H_{s+1} \geq \frac 12 +\min\sth{{\delta-2\tau\over 2(2-\delta)},1-\tau}$ where $\tau={5\over 2\epsilon_0^4 r_k^2}
		+{24\Lambda_s^2\over \epsilon_0^4r_k^2}$,
		\item If $H_s\geq \frac 12+\gamma_0$ then $\Lambda_s\leq {3\sigma\over \Delta} \pth{\sqrt d + \sqrt{2\pth{{1+2\gamma_0\over \gamma_0}\pth{1+\frac 1\beta}+\log\pth{1+2\gamma_0\over \gamma_0}}}}$.
	\end{enumerate}
\end{lemma}

\begin{proof}
	
	The proof of part (i) borrows results from the proof of \prettyref{lmm:Gs-Ls-bound}(i). Notice that we can show for each $h\neq g$
	\begin{align}
		\label{eq:km22}
		n_{gh}^{(s+1)}
		&\leq 
		\frac{5n_g^*\sigma^2}{4\epsilon_0^4\Delta^2}
		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2}\pth{{n_g^*}+  d}.
	\end{align}
	Using the last display and noting that $k\leq \frac 1{\alpha}$ and $n_g^*\geq n\alpha$ we get
	\begin{align}\label{eq:km23}
		{\sum_{h\in[k]\atop h\neq g}n_{gh}^{(s+1)}\over n_g^*}
		\leq \tau,\quad \tau=
		\frac{5\sigma^2}{2\epsilon_0^4\Delta^2\alpha}
		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2\alpha}\pth{1+ {dk\over n}}.
	\end{align}
	Using $n_g^{*}=\sum_{h\in [k]}n_{gh}^{(s+1)}$ for all $s\geq 0$, we get 
	\begin{align}\label{eq:km24}
		{n_{gg}^{(s+1)}\over n_g^*}\geq 1-\tau.
	\end{align}	 
	Next we switch $g,h$ in \eqref{eq:km22} and sum over $h\in [k], h\neq g$. We get
	\begin{align}
		\sum_{h\in[k]\atop h\neq g}n_{hg}^{(s+1)}
		\leq \frac{5n\sigma^2}{2\epsilon_0^4\Delta^2}
		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2}\pth{n+ kd}
		\leq n\alpha\tau.
	\end{align}
	Using the above and noticing that in addition to the points in $\cup_{h\in[k]}\sth{T_{h}^*\cap T_g^{(s+1)}}$, $T_g^{(s+1)}$ can at most have $n\beta$ many extra points, accounting for the outliers, we get
	\begin{align}
		{n_{gg}^{(s+1)}\over n_g^{(s+1)}}\geq {n_{gg}^{(s+1)}\over n_{gg}^{(s+1)}+n\alpha\tau+n^{\out}}
		\geq \frac 1{1+{n_g^*(1-\delta+\tau)\over n_{gg}^{(s+1)}}}
		\geq \frac 1{1+{1-\delta+\tau\over 1-\tau}}
		=\frac 12 + {\delta-2\tau\over 2(2-\delta)}.
	\end{align}
	Combining the last display with \eqref{eq:km24} we get
	\begin{align*}
		H_{s+1}=\min_{g\in [k]}\sth{\min\sth{{n_{gg}^{(s)}\over n_g^*},{n_{gg}^{(s)}\over n_{g}^{(s)}}}}
		\geq \frac 12+\min\sth{{\delta-2\tau\over 2(2-\delta)},\frac 12-\tau},
	\end{align*}
	as required.
	
	The proof of (ii) follows a similar strategy as in the proof of \prettyref{lmm:Gs-Ls-bound}, part (ii). Define as before
\end{proof}
\subsection{Proof of \prettyref{thm:optim-outl}}
Let $\beta=\alpha(1-\delta)$.  For $c_1,c_2$ to be chosen later, we define
$$\gamma_0=\frac {c_1}{\pth{{\Delta\over \sigma}\sqrt{\alpha\over d}}^2},\quad \epsilon_0={c_2\over \pth{{\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}^{\frac 12(1-\eta)}}.$$
Then from \prettyref{lmm:Gs-Ls-bound} it follows that, we can choose $c_1,c_2,c_3,c_4>0$ such that whenever $M>c_3$ and $\delta\geq c_4M^{-2\eta}$, on the set $\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0}$:
\begin{itemize}
	\item if $\Lambda_0\leq \frac 12-\epsilon_0$ then $H_1\geq \frac 12 + {\delta\over 6}$.
	\item if $H_0\geq \frac 12+\gamma_0$ then $\Lambda_0\leq 0  .3$,
\end{itemize}
A second application of \prettyref{lmm:Gs-Ls-bound} guarantees that we can choose $c_3$ large enough such that if  
$$M=\min \sth{{\Delta\over \sigma}\sqrt{\alpha\over d},{\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}\geq c_3$$
then on the set $\calE_{{2\gamma_1\over 1+2\gamma_1},\epsilon_1}\cap \calE_{\frac 14,\epsilon_1}$, with $\epsilon_1=\gamma_1=0.2$, if $H_{s}\geq \frac 12 +\frac \delta6$ then $\Lambda_s\leq {12\sqrt 2\over \sqrt{0.2}M} \leq 0.3$ and if $\Lambda_s\leq 0.3$ then $H_{s+1}\geq \frac 12 +\frac \delta6$.
Combining the above displays we get that on the set
\begin{align}
	\label{eq:Prob-E2}
	\calE&=\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0} \cap \calE_{{2\gamma_1\over 1+2\gamma_1},\epsilon_1}\cap \calE_{\frac 14,\epsilon_1}
	\nonumber\\
	\PP\qth{\calE}
	&\geq 1-4(k^2+k)n^{-c/4}-16de^{-0.3n}
\end{align} 
we have
\begin{align}
	\label{eq:km27}
	\Lambda_s\leq 0.3,\quad H_{s+1}\geq \frac 12 +\frac \delta6 \text{ for all } s\ge 2.
\end{align}
We will show that $\PP\qth{\left.z_i\neq \hat z_i^{(s+1)}\right|\calE}$ is small for each $i\in [n]$. This will imply that on the set $\calE$, $A_{s+1}=\frac 1n\sum_{i=1}^n\indc{z_i\neq \hat z_i^{(s+1)}}$ is also small in probability. From this, using a Markov inequality we will conclude the result. The analysis is 
identical to that of the proof of \cite[Theorem 1]{JKY2023} where it is shown that once we achieve $\Lambda_s\leq 0.3$ for all $s\geq 3$, the mislabeling rate follows. We omit it here.

\section{A computable clustering algorithm \nb{TBD}}

We need to use the fact that if initialized at good centroids, we can use a SCAD type loss around it to create the clusters.

\begin{algorithm}[H]
	\caption{The computable $\lss$ clustering algorithm}\label{algo:lloyd-rob-computable}
	{\bf Input}:  Data $Y_1,\dots,Y_n$. Initial centroid estimates $(\hat \theta_1^{(0)},\dots,\hat \theta_k^{(0)})$. Error threshold $\epsilon$. Truncation level $\delta\in (0,\frac 12)$. Here we choose $\delta=0.45$.\\
	{\bf Steps}: 
	\begin{algorithmic}[1]
		\While{$\frac 1k\sum_{h=1}^k \|\hat\theta_h^{(s)}-\hat\theta_h^{(s-1)}\|_2^2 > \epsilon$,}
		\For{$h\in \sth{1,2,\dots,k}}$
		\State \textbf{Labeling step}:
		$$T_h^{(s)}=\sth{Y_i:i\in \sth{1,\dots,n}, \|Y_i-\hat\theta_h^{(s-1)}\|_2\leq \|Y_i-\hat\theta_a^{(s-1)}\|_2,a\in\{1,\dots,k\}, a\neq h}.$$
		\State \textbf{Estimation step:} 
		\begin{enumerate}[label=\alph*)]
			\item Compute $R_h$ as the $(1-\delta)n_h^{(s)}$-th order statistics of the set $Q = \sth{i\in T_h^{(s)}: \|Y_i-\hat \theta^{(s-1)}\|}$.
			\item Compute the set $V$ of $Y_i$-s in $T_h^{(s)}$ such that $\|Y_i-\hat \theta_h^{(s-1)}\|$ is smaller than $R$,
			with tie broken arbitrarily.
			\item $\hat\theta_h^{(s)}= \frac 1{(1-\delta)n_h^{(s)}}\sum_{i:Y_i\in V} Y_i$.
		\end{enumerate}
		\EndFor
		\State $s=s+1$
		\EndWhile
	\end{algorithmic}
	{\bf Output}: $(\hat \theta_1^{(s)},\dots,\hat \theta_k^{(s)})$ and label estimate for $Y_i$ given by $\hat z_i^{(s)} = \argmin_{h\in\{1,\dots,k\}}\|Y_i-\hat\theta_h^{(s)}\|_2,$ with tie broken arbitrarily.
	\end{algorithm}


%
%\section{Related estimation guarantees in absence of outliers}
%\label{sec:other-est-no-outliers}
%%We mention the centrality property here:
%%
%%\begin{enumerate}[label=(Q)]
%%	\item \label{eq:Q}(Quantile detection) Given a real random variable $W$ and $q\in(0,\frac 12]$, we say $x,y$ are sufficient to detect its $q,1-q$-th quantiles if
%%	\begin{align*}
%%		\PP\qth{W\geq x}\leq q,\quad \PP\qth{W\leq y}\leq 1-q.
%%	\end{align*}
%%\end{enumerate}
%
%\begin{theorem}
%	Let $F_{ij}$ denote the distribution of the $j$-th coordinate of the $i$-th data point $Y_i$. Suppose that $n\alpha\geq c\log n$ for some $c>0$ and the constraints in \prettyref{thm:main} on $G_s,\Lambda_s$ are satisfied. Then given any $\tau >0$, there exists absolute constants $C:=C(\tau)>0$ such that whenever $M=\min \sth{{\Delta\over \sigma}\sqrt{\alpha\over d}, {\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}\geq C$
%	with probability at least $1-\frac 1n-4(k^2+k)n^{-(c/2-2)}-16dn^4e^{-0.3n}- 2k^2\exp\sth{-{\Delta\over 8\sigma}}$ we have
%	$$
%	\|\hat \theta_g^{(s)}-\theta_g\|^2\leq {d}
%	\qth{\max_{i:Y_i\in T_g^*}\max_{j\in [d]} \max\sth{\abs{F_{ij}^{-1}\pth{\frac 12 +x_0}},\abs{F_{ij}^{-1}\pth{\frac 12 -x_0}}}}^2,\quad s\geq 2,
%	$$
%	where 
%	$x_0= \sqrt{3\log n\over n_g^*}+e^{-{\Delta^2\over (8+\tau)\sigma^2}}$.
%\end{theorem}
%
%\begin{remark} \nb{EDIT THIS FOR NEW NOTATIONS}
%	In particular, if the errors of the $g$-th cluster are distributed as the univariate Gaussian distribution with variance $\sigma^2$, then for any value of $n_g^*$ the conditions in the above theorems are satisfied with $$x_0=C\sigma\pth{{\sqrt{\log n\over {n_g^*}}+e^{-{\Delta^2\over 24\sigma^2}}}}$$ for some large constant $C>0$. This implies that when $\Delta\gtrsim \sigma\log n$ we achieve the optimal rate of estimating the centroids.
%\end{remark}
%\begin{proof}
%	The results in the last section implies that there is an absolute constant $C>0$ such that whenever 
%	$$
%	\min\sth{{\Delta\over \sigma}\sqrt{\alpha\over d},{\Delta\over \sigma}\sqrt{\alpha\over 1+{kd/n}}}\geq C
%	$$
%	we get for any $g\in [k]$
%	\begin{align}
%		\max\sth{\sum_{h\in[k]\atop h\ne g}n_{hg}^{(s)},\sum_{h\in[k]\atop h\ne g}n_{gh}^{(s)}}
%		\leq \sum_{i=1}^n\indc{\hat z_i^{(s)}\neq z_i}
%		=nA_s, \quad s\geq 3.
%	\end{align}
%	Using the above we get
%	\begin{align}
%		G_s=\max_{g\in [k]} \sth{\max\sth{{\sum_{h\in[k]\atop h\neq g} n_{gh}^{(s)}\over n_g^*},{\sum_{h\in[k]\atop h\neq g} n_{hg}^{(s)}\over n_g^{(s)}}}}
%		\leq nA_s\cdot \max_{g\in [k]}\sth{\max\sth{\frac 1{n_g^*},\frac 1{n_g^{(s)}}}}.
%	\end{align}
%	As $G_s\leq \frac 12$ for all $s\geq 3$, we get $n\alpha\leq n_g^*\leq 2n_{gg}^{(s)}\leq 2n_{g}^{(s)}$. Using this we have
%	\begin{align}\label{eq:km26}
%		n_{g}^*\geq n_{gg}^{(s)}\geq n_g^{(s)}-nA_s\geq n_g^{(s)}\pth{1-\frac 2\alpha A_s},
%		\quad n_{g}^{(s)}\geq n_{gg}^{(s)}\geq n_g^*-nA_s\geq n_g^*\pth{1-\frac 1\alpha A_s}.
%	\end{align}
%	Fix $g\in [k]$. Let $U_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^{(s)}$, $V_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^*\cap T_g^{(s)}$, and $W_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^*$. Then we get
%	\begin{align*}
%		U_j^{(\ceil{ {n_g^{(s)}/2}})}
%		&\stepa{\leq} V_j^{(\ceil{n_g^{(s)}/2}-n_g^{(s)}+n_{gg}^{(s)})}
%		\nonumber\\
%		&\stepb{\leq }
%		V_j^{(\floor{{n_g^{(s)}\over 2}-nA_s})}
%		\stepc{\leq} W_j^{(\floor{{n_g^{(s)}\over 2}-nA_s})}
%		\stepd{\leq} W_j^{(\floor{{n_g^{*}\over 2}-{3nA_s\over 2}})}
%		\stepe{\leq} W_j^{(\floor{{n_g^*}(\frac 12-\frac 1\alpha A_s)})},
%	\end{align*}
%	where
%	\begin{itemize}
%		\item (a) followed using \prettyref{lmm:ord-stat_after_addn} with
%		$
%		X=V_j,\ \tilde X=U_j,\ \ell=n_g^{(s)}-n_{gg}^{(s)},\ t=\ceil{n_g^{(s)}\over 2},
%		$
%		\item (b) followed using $n_g^{(s)}-n_{gg}^{(s)}\leq nA_s$ and $\ceil{x}-y\geq \floor{x-y}$ for $x,y\geq 0$
%		
%		\item (c) followed using \prettyref{lmm:ord-stat_after_addn} with 
%		$X=V_j,\ \tilde X=W_j,\ \ell=n_g^*-n_{gg}^{(s)},\ t=\floor{{n_g^{(s)}\over 2} -nA_s},$
%		
%		\item (d) followed using \eqref{eq:km26} and (e) followed using $n_g^*\geq n\alpha$.
%	\end{itemize}
%	Similarly we also have
%	\begin{align*}
%		U_j^{(\ceil{ {n_g^{(s)}/2}})}
%		&\stepa{\geq} V_j^{(\ceil{n_g^{(s)}/2})}
%		\nonumber\\
%		&\stepb{\geq} 
%		V_j^{(\ceil{{n_g^*\over 2}\cdot \frac 1{1-{2A_s/\alpha}}})}
%		\stepc{\geq} 
%		V_j^{(\ceil{{n_g^*}(\frac 12+\frac 2\alpha A_s)})}
%		\stepd{\geq} W_j^{(\ceil{{n_g^*}(\frac 12+\frac 2\alpha A_s)}+\sum_{h=[k]\atop h\neq k}n_{gh})}
%		\stepe{\geq} W_j^{(\ceil{{n_g^*}(\frac 12+\frac 3\alpha A_s)})}.
%	\end{align*}
%	\begin{itemize}
%		\item (a) followed using \prettyref{lmm:ord-stat_after_addn} with
%		$
%		X=V_j,\ \tilde X=U_j,\ \ell=n_g^{(s)}-n_{gg}^{(s)},\ t=\ceil{n_g^{(s)}\over 2},
%		$
%		
%		\item (b) followed using \eqref{eq:km26} and (c) followed using $(1-x)^{-1}\leq 1+2x$ for $x=\frac 2\alpha A_s\leq \frac 12$.
%		
%		\item (d) used \prettyref{lmm:ord-stat_after_addn} with 
%		$X=V_j,\ \tilde X=W_j,\ \ell=\sum_{h=[k]\atop h\neq k}n_{gh},\ t=\ceil{{n_g^*\over 2}(1+\frac 4\alpha A_s)}+\sum_{h=[k]\atop h\neq k}n_{gh},$
%		
%		
%		\item (e) used that for any $x>0$ and positive integer $y$, $\ceil{x}+y = \ceil{x+y}$, and $\sum_{h=[k]\atop h\neq k}n_{gh}\leq nA_s$.
%	\end{itemize}
%	Then \prettyref{thm:main} implies that given any $\tau>0$, there exists $C:=C(\tau)$ such that whenever $M\geq C(\tau)$, we have $\frac 6\alpha A_s\leq e^{-{\Delta^2\over (8+\tau)\sigma^2}}$. Using this we combine the last two displays to get
%	\begin{align}
%		W_j^{(\ceil{{n_g^*\pth{\frac 12+e^{-{\Delta^2\over (8+\tau)\sigma^2}}}}})}
%		\leq U_j^{(\floor{{n_g^{(s)}/2}})}\leq W_j^{(\floor{{n_g^*\pth{\frac 12-e^{-{\Delta^2\over (8+\tau)\sigma^2}}}}})}.
%	\end{align}
%	Then using the result \prettyref{lmm:order-concentration-smallx} on the concentration of the order statistics
%	we conclude our results.
%\end{proof}
%
%\nb{TBD: Add a remark about spectral initialization}
%
%\section{Optimality in the presence of outliers}
%
% Suppose that an adversary adds $n^{\out}$ many points to our existing data set. Our results for the adversarial addition regime is based on the cluster-wise correct classification proportion at step $s$, defined as
%\begin{align}
%	H_s=\min_{g\in [k]}\sth{\min\sth{{n_{gg}^{(s)}\over n_g^*},{n_{gg}^{(s)}\over n_{g}^{(s)}}}}.
%\end{align}
%\begin{theorem}
%	\label{thm:optim-outl}
%	 Suppose that $n\alpha\geq c\log n$ for some $c>0$. There exists absolute constants $c_1,c_2,c_3,c_4,c_5>0$ such that the followings are satisfied. For any $\eta\in(0,1]$, if the clustering initialization satisfies either one of the following conditions
%	$${H_0}\geq \frac 12+\frac {c_1}{\pth{{\Delta\over \sigma}\sqrt{\alpha\over d}}^2}\quad  \text{ or } \quad \Lambda_0\leq \frac 12-{c_2\over \pth{{\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}^{\frac 12(1-\eta)}},$$
%	then whenever $$M=\min \sth{{\Delta\over \sigma}\sqrt{\alpha\over d}, {\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}\geq c_3,$$ 
%	for any $n^{\out}\leq n\alpha(1-c_4M^{-2\eta})$ our algorithm guarantees $$A_s\leq \exp\sth{-\pth{1-{c_5\over \sqrt M}}{\Delta^2\over 8\sigma^2}+{\Delta\over \sigma}},
%	\quad s\geq 2
%	$$
%	with probability $1-4(k^2+k)n^{-(c/2-2)}-16dn^4e^{-0.3n}- 2k^2\exp\sth{-{\Delta\over 8\sigma}}.$
%\end{theorem}
%
%\begin{remark}
%    When we initialize with the constraint on $H_0$ we can allow $\eta=1$.\nb{Check proof}
%\end{remark}
%
%The proof of the above theorem hinges on the following lemma, similar to \prettyref{lmm:Gs-Ls-bound}.
%
%\begin{lemma}\label{eq:HsLs-bound}
%	Fix $\epsilon_0,\gamma_0\in (0,\frac 12]$ and suppose that an adversary added $n\beta$ many outliers with $\beta\leq\alpha(1-\delta)$ for some $\delta>0$. Let $r_k={\Delta\over\sigma}\sqrt{\alpha\over 1+{dk/n}}$. Then on the set $\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0} $ we have
%	\begin{enumerate}[label=(\roman*)]
%		\item If $\Lambda_s\leq \frac 12-\epsilon_0$ then $H_{s+1} \geq \frac 12 +\min\sth{{\delta-2\tau\over 2(2-\delta)},1-\tau}$ where $\tau={5\over 2\epsilon_0^4 r_k^2}
%		+{24\Lambda_s^2\over \epsilon_0^4r_k^2}$,
%		\item If $H_s\geq \frac 12+\gamma_0$ then $\Lambda_s\leq {12\sqrt 2\over \Delta/\sigma}\sqrt{d \over  {\gamma_0\alpha}}$.
%	\end{enumerate}
%\end{lemma}
%
%\begin{proof}
%	
%	The proof of part (i) borrows results from the proof of \prettyref{lmm:Gs-Ls-bound}(i). Notice that we can show for each $h\neq g$
%	\begin{align}
%		\label{eq:km22}
%		n_{gh}^{(s+1)}
%		&\leq 
%		\frac{5n_g^*\sigma^2}{4\epsilon_0^4\Delta^2}
%		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2}\pth{{n_g^*}+  d}.
%	\end{align}
%	Using the last display and noting that $k\leq \frac 1{\alpha}$ and $n_g^*\geq n\alpha$ we get
%	\begin{align}\label{eq:km23}
%		{\sum_{h\in[k]\atop h\neq g}n_{gh}^{(s+1)}\over n_g^*}
%		\leq \tau,\quad \tau=
%		\frac{5\sigma^2}{2\epsilon_0^4\Delta^2\alpha}
%		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2\alpha}\pth{1+ {dk\over n}}.
%	\end{align}
%	Using $n_g^{*}=\sum_{h\in [k]}n_{gh}^{(s+1)}$ for all $s\geq 0$, we get 
%	\begin{align}\label{eq:km24}
%		{n_{gg}^{(s+1)}\over n_g^*}\geq 1-\tau.
%	\end{align}	 
%	Next we switch $g,h$ in \eqref{eq:km22} and sum over $h\in [k], h\neq g$. We get
%	\begin{align}
%		\sum_{h\in[k]\atop h\neq g}n_{hg}^{(s+1)}
%		\leq \frac{5n\sigma^2}{2\epsilon_0^4\Delta^2}
%		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2}\pth{n+ kd}
%		\leq n\alpha\tau.
%	\end{align}
%	Using the above and noticing that in addition to the points in $\cup_{h\in[k]}\sth{T_{h}^*\cap T_g^{(s+1)}}$, $T_g^{(s+1)}$ can at most have $n\beta$ many extra points, accounting for the outliers, we get
%	\begin{align}
%		{n_{gg}^{(s+1)}\over n_g^{(s+1)}}\geq {n_{gg}^{(s+1)}\over n_{gg}^{(s+1)}+n\alpha\tau+n^{\out}}
%		\geq \frac 1{1+{n_g^*(1-\delta+\tau)\over n_{gg}^{(s+1)}}}
%		\geq \frac 1{1+{1-\delta+\tau\over 1-\tau}}
%		=\frac 12 + {\delta-2\tau\over 2(2-\delta)}.
%	\end{align}
%	Combining the last display with \eqref{eq:km24} we get
%	\begin{align*}
%		H_{s+1}=\min_{g\in [k]}\sth{\min\sth{{n_{gg}^{(s)}\over n_g^*},{n_{gg}^{(s)}\over n_{g}^{(s)}}}}
%		\geq \frac 12+\min\sth{{\delta-2\tau\over 2(2-\delta)},\frac 12-\tau},
%	\end{align*}
%	as required.
%	
%	The proof of (ii) follows a similar strategy as in the proof of \prettyref{lmm:Gs-Ls-bound}, part (ii). Define as before
%	\begin{align}
%		\begin{gathered}
%			\hat \theta_g^{(s)}=\med(T_g^{(s)}),\quad \tilde \theta_g^{(s)}=\med(T_g^{(s)}\cap T_g^*)\\
%			U_j=\text{the set of $j^{\rm{th}}$ coordinates of $T_g^{(s)}$},\quad
%			V_j=\text{the set of $j^{\rm{th}}$ coordinates of $T_g^{(s)}\cap T_g^*$}.
%		\end{gathered}
%	\end{align} 
%%	Then as we have
%%	\begin{align}
%%			n_{gg}^{(s)}\geq (\frac 12+\gamma_0)n_g^{(s)}\geq {n_g^{(s)}\over 2}+5,\quad
%%			n_{g}^{(s)}-n_{gg}^{(s)}\leq (\frac 12-\gamma_0)n_g^{(s)}\leq {n_g^{(s)}\over 2}-5
%%	\end{align}
%%	we can use \prettyref{lmm:ord-stat_after_addn} with
%%	$X=V_j,\tilde X=U_j,m=n_{gg}^{(s)},\ell=n_{g}^{(s)}-n_{gg}^{(s)},
%%	t=\ceil{n_g^{(s)}\over 2}$
%%	to get
%%	\begin{align}
%%		V_j^{(\ceil{ {n_g^{(s)}/2}})}
%%		\leq \med(U_j)
%%		\leq V_j^{(\floor{\gamma_0 n_{g}^{(s)}})}.
%%	\end{align}
%%	Using the definition of order statistics we also have
%%	\begin{align}
%%	V_j^{(\ceil{ {n_g^{(s)}/2}})}
%%	\leq V_j^{(\ceil{n_{gg}^{(s)}/2})}=\med(V_j)
%%	\leq  V_j^{(\floor{\gamma_0 n_{g}^{(s)}})}.
%%	\end{align}
%%	Combining the last two displays we get
%	Then using essentially the same strategy we show
%	\begin{align}\label{eq:km32}
%	\|\hat \theta_g^{(s)}-\tilde\theta_g^{(s)}\|_2^2\leq \sum_{j=1}^d\abs{\med(U_j)-\med(V_j)}^2
%	&\leq \abs{V_j^{(\floor{\gamma_0 n_g^{(s)}})}-V_j^{(\ceil{ {n_g^{(s)}/2}})}}.
%	\end{align}
%	Then as $H_s\geq \frac 12+\gamma_0$ guarantees ${1\over 1+2\gamma_0}n_{gg}^{(s)} \geq {n_g^{(s)}\over 2}\leq \gamma_0 n_g^{(s)}\geq \gamma_0 n_{gg}^{(s)}$, we get that
%	\begin{align}
%		\|\hat \theta_g^{(s)}-\tilde\theta_g^{(s)}\|_2^2
%		\leq \sum_{j=1}^d\abs{V_j^{(\floor{\gamma_0 n_{gg}^{(s)}})}-V_j^{(\ceil{{1\over 1+2\gamma_0}n_{gg}^{(s)}})}}^2
%	\end{align}
%	The rest of the proof then follows using the concentration bound of order statistics for the sets $V_1,\dots,V_d$ As these sets do not involve any outliers, our usual concentration bound for $\subG(\sigma^2)$, provided in \prettyref{lmm:order-concentration}, applies.
%	
%\end{proof}
%
%\begin{proof}[Proof of \prettyref{thm:optim-outl}]
%	Let $\beta=\alpha(1-\delta)$.  For $c_1,c_2$ to be chosen later, we define
%	$$\gamma_0=\frac {c_1}{\pth{{\Delta\over \sigma}\sqrt{\alpha\over d}}^2},\quad \epsilon_0={c_2\over \pth{{\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}^{\frac 12(1-\eta)}}.$$
%	Then from \prettyref{lmm:Gs-Ls-bound} it follows that, we can choose $c_1,c_2,c_3,c_4>0$ such that whenever $M>c_3$ and $\delta\geq c_4M^{-2\eta}$, on the set $\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0}$:
%	\begin{itemize}
%		\item if $\Lambda_0\leq \frac 12-\epsilon_0$ then $H_1\geq \frac 12 + {\delta\over 6}$.
%		\item if $H_0\geq \frac 12+\gamma_0$ then $\Lambda_0\leq 0  .3$,
%	\end{itemize}
%	A second application of \prettyref{lmm:Gs-Ls-bound} guarantees that we can choose $c_3$ large enough such that if  
%	$$M=\min \sth{{\Delta\over \sigma}\sqrt{\alpha\over d},{\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}\geq c_3$$
%	then on the set $\calE_{{2\gamma_1\over 1+2\gamma_1},\epsilon_1}\cap \calE_{\frac 14,\epsilon_1}$, with $\epsilon_1=\gamma_1=0.2$, if $H_{s}\geq \frac 12 +\frac \delta6$ then $\Lambda_s\leq {12\sqrt 2\over \sqrt{0.2}M} \leq 0.3$ and if $\Lambda_s\leq 0.3$ then $H_{s+1}\geq \frac 12 +\frac \delta6$.
%	Combining the above displays we get that on the set
%	\begin{align}
%		\label{eq:Prob-E2}
%		\calE&=\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0} \cap \calE_{{2\gamma_1\over 1+2\gamma_1},\epsilon_1}\cap \calE_{\frac 14,\epsilon_1}
%		\nonumber\\
%		\PP\qth{\calE}
%		&\geq 1-4(k^2+k)n^{-c/4}-16de^{-0.3n}
%	\end{align} 
%	we have
%	\begin{align}
%		\label{eq:km27}
%		\Lambda_s\leq 0.3,\quad H_{s+1}\geq \frac 12 +\frac \delta6 \text{ for all } s\ge 2.
%	\end{align}
%	We will show that $\PP\qth{\left.z_i\neq \hat z_i^{(s+1)}\right|\calE}$ is small for each $i\in [n]$. This will imply that on the set $\calE$, $A_{s+1}=\frac 1n\sum_{i=1}^n\indc{z_i\neq \hat z_i^{(s+1)}}$ is also small in probability. From this, using a Markov inequality we will conclude the result. The analysis is 
%	identical to that of the proof of \prettyref{thm:main} after \eqref{eq:km14} which relies solely on the fact that $\Lambda_s\leq 0.3$ for all $s\geq 3$. We omit it here.
%\end{proof}
%
%
%
%\subsection*{Adversarial data corruption}
%	
%	\begin{remark}
%		Mention that it is equivalent to adversarial data addition but the result changes a bit
%	\end{remark}
%
%\section{Centroid estimation in presence of outliers}
%For this section, let us define the ratio of total outliers with respect to individual clusters as
%\begin{align}
%    \beta_g^\out = {n^{\out}\over n_g^*},\quad g=1,2,\dots,k.
%\end{align}
%Note that in order to identify all the clusters accurately we require $\max_g\beta_g^\out<1$; otherwise, given any algorithm, an adversary can always create a constellation involving only the outliers that will force the algorithm to detect it as an individual cluster.
%
%\begin{theorem} 
%	Suppose that $n\alpha\geq c\log n$ for some $c>0$ and the constraints in \prettyref{thm:optim-outl} on $H_s,\Lambda_s$ are satisfied. Then given any $\tau >0$, there exists absolute constants $C:=C(\tau)>0$ such that whenever $M=\min \sth{{\Delta\over \sigma}\sqrt{\alpha\over d}, {\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}\geq C$, then
%	with probability at least $1-\frac 1n-4(k^2+k)n^{-(c/2-2)}-16dn^4e^{-0.3n}- 2k^2\exp\sth{-{\Delta\over 8\sigma}}$ we have
%	$$
%	\|\hat \theta_g^{(s)}-\theta_g\|^2\leq {d}
%	\qth{\max_{i:Y_i\in T_g^*}\max_{j\in [d]} \max\sth{\abs{F_{ij}^{-1}\pth{\frac 12 +x_0}},\abs{F_{ij}^{-1}\pth{\frac 12 -x_0}}}}^2,\quad s\geq 2,
%	$$
%	where 
%	$x_0= \sqrt{3\log n\over n_g^*}+e^{-{\Delta^2\over (8+\tau)\sigma^2}}+{\beta_g^\out\over 1+\beta_g^\out}$.
%\end{theorem}
%
%\begin{remark} \nb{EDIT THIS FOR NEW NOTATIONS}
%	In particular, if the errors of the $g$-th cluster are distributed as the multivariate Gaussian distribution with variance $\sigma^2$, then for any $\beta_g^{\out}\leq c \pth{\sqrt{3\log n\over n_g^*}+e^{-{\Delta^2\over (8+\tau)\sigma^2}}}$ the conditions in the above theorems are satisfied with $$x_0=C\sigma\pth{{\sqrt{\log n\over {n_g^*}}+e^{-{\Delta^2\over 24\sigma^2}}}}$$ for some large constant $C>0$. This implies that when $\Delta\gtrsim \sigma\log n$ we achieve the optimal rate of estimating the centroids.
%\end{remark}
%\begin{proof}
%	From the definition of $A_s$ we have
%	we get for any $g\in [k]$
%	\begin{align}\label{eq:29}
%		\max\sth{\sum_{h\in[k]\atop h\ne g}n_{hg}^{(s)},\sum_{h\in[k]\atop h\ne g}n_{gh}^{(s)}}
%		\leq \sum_{i=1}^n\indc{\hat z_i^{(s)}\neq z_i}
%		=nA_s, \quad s\geq 3.
%	\end{align}
%	Note that using $n\leq {n_g^*\over \alpha}$ and $n_{gg}^{(s)}\geq n_{g}^*-nA_s\geq n_g^*(1-A_s/\alpha)$, using the last display we can write
%	\begin{align*}
%		{n_{gg}^{(s)}\over n_g^{(s)}}\geq {n_{gg}^{(s)}\over n_{gg}^{(s)}+\sum_{h\in[k]\atop h\ne g}n_{hg}^{(s)}+n^{\out}}
%		\geq \frac 1{1+{n_g^*(\frac 1\alpha A_s+\beta_g^{\out})\over n_{gg}^{(s+1)}}}
%		\geq \frac 1{1+{\beta_g^{\out}+ A_s/\alpha\over 1-A_s/\alpha}}
%		=\frac 12 + {1-\beta_g^{\out}-\frac 2\alpha A_s\over 2(1+{\beta_g^{\out}})},
%	\end{align*}
%	which implies
%	\begin{align}\label{eq:km30}
%		\ceil{ {n_g^{(s)}/2}}-n_g^{(s)}+n_{gg}^{(s)}\geq n_{gg}^{(s)}-{n_g^{(s)}\over 2}
%		\geq \pth{1-\beta_g^{\out}-\frac 2\alpha A_s\over 1+\beta_g^{\out}}{n_g^{(s)}\over 2}
%		= \pth{\frac 12-{\beta_g^{\out}+A_s/\alpha \over 1+\beta_g^{\out}}}{n_g^{(s)}}
%	\end{align}
%	As $n_g^*\geq n\alpha$, the above implies for all $g\in [k]$
%	\begin{gather}
%			n_g^{(s)}\geq 	n_{gg}^{(s)}=n_g^*-\sum_{h\in[k]\atop h\ne g}n_{gh}^{(s)}
%			\geq n_g^*-nA_s \geq n_g^*\pth{1-\frac 1\alpha A_s}
%			\label{eq:km31}
%	\end{gather}
%	Fix $g\in [k]$. Let $U_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^{(s)}$, $V_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^*\cap T_g^{(s)}$, and $W_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^*$.Then we get
%	\begin{align*}
%		U_j^{(\ceil{ {n_g^{(s)}/2}})}
%		&\stepa{\leq} V_j^{(\ceil{n_g^{(s)}/2}-n_g^{(s)}+n_{gg}^{(s)})}
%		\nonumber\\
%		&\stepb{\leq }
%		V_j^{(\floor{\pth{1-\beta_g^{\out}-\frac 2\alpha A_s\over 1+\beta_g^{\out}}{n_g^{(s)}\over 2}})}
%		\nonumber\\
%		&\stepc{\leq} W_j^{(\floor{\pth{1-\beta_g^{\out}-\frac 2\alpha A_s\over 1+\beta_g^{\out}}{n_g^{(s)}\over 2}})}
%		\stepd{\leq} W_j^{(\floor{{n_g^{*}}\pth{\frac 12-{\beta_g^{\out}+A_s/\alpha \over 1+\beta_g^{\out}}}\pth{1-\frac 1\alpha A_s}})}
%		\leq W_j^{(\floor{{n_g^{*}}\pth{\frac 12-{\beta_g^{\out}\over 1+\beta_g^{\out}}-\frac 5{2\alpha}A_s}})},
%	\end{align*}
%	where
%	\begin{itemize}
%		\item (a) followed using \prettyref{lmm:ord-stat_after_addn} with
%		$
%		X=V_j,\ \tilde X=U_j,\ \ell=n_g^{(s)}-n_{gg}^{(s)},\ t=\ceil{n_g^{(s)}\over 2},
%		$
%		\item (b) followed using \eqref{eq:km32} \eqref{eq:km30} and $\ceil{x}-y\geq \floor{x-y}$ for $x,y\geq 0$
%		
%		\item (c) followed using \prettyref{lmm:ord-stat_after_addn} with 
%		$X=V_j,\ \tilde X=W_j,\ \ell=n_g^*-n_{gg}^{(s)},\ t=\floor{\pth{\frac 12-{\beta_g^{\out}+ A_s/\alpha\over 1+\beta_g^{\out}}}{n_g^{(s)}}},$
%		
%		\item (d) followed using \eqref{eq:km31}.
%	\end{itemize}
%	Similarly, we also have
%	\begin{align*}
%		U_j^{(\ceil{ {n_g^{(s)}/2}})}
%		&\stepa{\geq} V_j^{(\ceil{n_g^{(s)}/2})}
%		\nonumber\\
%		&\stepb{\geq} 
%		V_j^{(\ceil{{n_g^*\over 2}\cdot \frac 1{1-{2A_s/\alpha}}})}
%		\stepc{\geq} 
%		V_j^{(\ceil{{n_g^*}(\frac 12+\frac 2\alpha A_s)})}
%		\stepd{\geq} W_j^{(\ceil{{n_g^*}(\frac 12+\frac 2\alpha A_s)}+\sum_{h=[k]\atop h\neq k}n_{gh})}
%		\stepe{\geq} W_j^{(\ceil{{n_g^*}(\frac 12+\frac 3\alpha A_s)})}.
%	\end{align*}
%	\begin{itemize}
%		\item (a) followed using \prettyref{lmm:ord-stat_after_addn} with
%		$
%		X=V_j,\ \tilde X=U_j,\ \ell=n_g^{(s)}-n_{gg}^{(s)},\ t=\ceil{n_g^{(s)}\over 2},
%		$
%		
%		\item (b) followed using \eqref{eq:km31} and (c) followed using $(1-x)^{-1}\leq 1+2x$ for $x=\frac 2\alpha A_s\leq \frac 12$.
%		
%		\item (d) used \prettyref{lmm:ord-stat_after_addn} with 
%		$X=V_j,\ \tilde X=W_j,\ \ell=\sum_{h=[k]\atop h\neq k}n_{gh},\ t=\ceil{{n_g^*\over 2}(1+\frac 4\alpha A_s)}+\sum_{h=[k]\atop h\neq k}n_{gh},$
%		
%		
%		\item (e) used that for any $x>0$ and positive integer $y$, $\ceil{x}+y = \ceil{x+y}$, and $\sum_{h=[k]\atop h\neq k}n_{gh}\leq nA_s$.
%	\end{itemize}
%	Then \prettyref{thm:main} implies that given any $\tau>0$, there exists $C:=C(\tau)$ such that whenever $M\geq C(\tau)$, we have $\frac 6\alpha A_s\leq e^{-{\Delta^2\over (8+\tau)\sigma^2}}$. Using this we combine the last two displays to get
%	\begin{align}
%		W_j^{(\ceil{{n_g^*\pth{\frac 12+e^{-{\Delta^2\over (8+\tau)\sigma^2}}}}})}
%		\leq U_j^{(\floor{{n_g^{(s)}/2}})}\leq W_j^{(\floor{{n_g^*\pth{\frac 12-{\beta_g^{\out}\over 1+\beta_g^{\out}}-e^{-{\Delta^2\over (8+\tau)\sigma^2}}}}})}.
%	\end{align}
%	Then using the result \prettyref{lmm:order-concentration-smallx} on the concentration of the order statistics
%	we conclude our results.
%\end{proof}

==> tex/low-moment.tex <==






\section{Notation} 
We will call a random vector $w\in \reals^d$ satisfies the spherical $p$ moment constraint with parameter $\sigma>0$ (here and below denoted by $w\in \calR_p(\sigma)$) if it has mean zero and
\begin{itemize}
	\item ${w\over \|w\|_2}$ is uniformly distributed on the unit sphere $\sfS^{d-1}$,
	\item $\EE\qth{\|w\|_2^{p}}<\sigma^p$.
\end{itemize}
For our paper we assume $p\geq 2$. We observe independent samples $Y_1,\dots,Y_n\in \reals^d$ from a mixture of $k$ many $\calR_p(\sigma)$ distributions
\begin{align}
	Y_i=\theta_{z_i}+w_i,\ i=1,\dots,n,\quad w_i\in \calR_p(\sigma),
\end{align}
where $ z=\sth{z_i}_{i=1}^n\in[k]^n$ denote the underlying labels, $\theta_1,\dots,\theta_k$ are the unknown centers of those $k$ distributions. Suppose that after $s$-steps the estimated centers are $\hat\theta^{(s)}_1,\dots,\hat\theta^{(s)}_k$ and the estimated labels are $\hat z^{(s)}=\sth{\hat z^{(s)}_1,\dots,\hat z^{(s)}_k}$. The initialization for the parameters correspond to $s=0$. 
We study the loss function
\begin{align}
	\ell(\hat z^{(s)},z) = \inf_{\pi\in \calS_k}\qth{\frac 1n \sum_{i=1}^n\indc{\pi(z^{(s)}_i)\neq z_i}},
\end{align}
where $\calS_k$ is the set of all permutations on $\{1,\dots,k\}$. Next we define notations for the different clusters in ground truth as well as during the iterations. For all $h,g\in [k]$, define
\begin{equation}\label{eq:cluster-def}
	\begin{gathered}
		T_h^*=\sth{Y_i:i\in [n],z_i=h},
		\hat T_h^{(s)}=\sth{Y_i:i\in [n],z_i^{(s-1)}=h}\\
		n^*_h = \abs{T^*_h}, n^{(s)}_h = \abs{T^{(s)}_h}, n^{(s)}_{hg} = \abs{T^*_h \cap T^{(s)}_g}
	\end{gathered}
\end{equation}
Note that for $s\geq 1$ this implies
\begin{align}
	T_h^{(s)}=\sth{Y_i:i\in[n], \|Y_i-\hat\theta_h^{(s-1)}\|\leq \|Y_i-\hat\theta_a^{(s-1)}\|,a\in[k]}.
\end{align}
with tie broken arbitrarily.

 Our clustering algorithm is the following.

\begin{algorithm}[H]
	\caption{The $\loa$}\label{algo:lloyd-rob}
	{\bf Input}:  Data $Y_1,\dots,Y_n$. Initial centroid estimates $(\hat \theta_1^{(0)},\dots,\hat \theta_k^{(0)})$. Error threshold $\epsilon$. Truncation level $\delta\in (0,\frac 12)$. Here we choose $\delta=0.49$.\\
	{\bf Steps}: 
	\begin{algorithmic}[1]
		\While{$\frac 1k\sum_{h=1}^k \|\hat\theta_h^{(s)}-\hat\theta_h^{(s-1)}\|_2^2 > \epsilon$,}
		\For{$h\in \sth{1,2,\dots,k}}$
		\State \textbf{Labeling step}:
		$$T_h^{(s)}=\sth{Y_i:i\in \sth{1,\dots,n}, \|Y_i-\hat\theta_h^{(s-1)}\|_2\leq \|Y_i-\hat\theta_a^{(s-1)}\|_2,a\in\{1,\dots,k\}, a\neq h}.$$
		\State \textbf{Estimation step:} 
		\begin{enumerate}[label=\alph*)]
			\item Compute the subset $V$ using
			$$
			V=\argmin_{S\subseteq T_h^{(s)},|S|=(1-\delta)n_h^{(s)}}
			\sum_{i:Y_i\in S} \left\|Y_i - \frac 1{(1-\delta)n_h^{(s)}}\sum_{i:Y_i\in S} Y_i\right\|_2^2,
			$$
			with tie broken arbitrarily.
			\item $\hat\theta_h^{(s)}= \frac 1{(1-\delta)n_h^{(s)}}\sum_{i:Y_i\in V} Y_i$.
		\end{enumerate}
		\EndFor
		\State $s=s+1$
		\EndWhile
	\end{algorithmic}
	{\bf Output}: $(\hat \theta_1^{(s)},\dots,\hat \theta_k^{(s)})$ and label estimate for $Y_i$ given by $\hat z_i^{(s)} = \argmin_{h\in\{1,\dots,k\}}\|Y_i-\hat\theta_h^{(s)}\|_2,$ with tie broken arbitrarily.
\end{algorithm}


%\begin{algorithm}[H]
%	\caption{The $\lss$ clustering algorithm}\label{algo:lloyd-rob}
%	{\bf Input}:  Data $Y_1,\dots,Y_n$. Initial centroid estimates $(\hat \theta_1^{(0)},\dots,\hat \theta_k^{(0)})$. Error threshold $\epsilon$. Truncation level $\delta\in (0,\frac 12)$. Here we choose $\delta=0.49$.\\
%	{\bf Steps}: 
%	\begin{algorithmic}[1]
%		\While{$\frac 1k\sum_{h=1}^k \|\hat\theta_h^{(s)}-\hat\theta_h^{(s-1)}\|_2^2 > \epsilon$,}
%		\For{$h\in \sth{1,2,\dots,k}}$
%		\State \textbf{Labeling step}:
%		$$T_h^{(s)}=\sth{Y_i:i\in \sth{1,\dots,n}, \|Y_i-\hat\theta_h^{(s-1)}\|_2\leq \|Y_i-\hat\theta_a^{(s-1)}\|_2,a\in\{1,\dots,k\}, a\neq h}.$$
%		\State \textbf{Estimation step:} 
%		\begin{enumerate}[label=\alph*)]
%			\item Compute the subset $V$ using
%			$$
%			V=\argmin_{S\subseteq T_h^{(s)},|S|=(1-\delta)n_h^{(s)}}
%			\sum_{i:Y_i\in S} \left\|Y_i - \frac 1{(1-\delta)n_h^{(s)}}\sum_{i:Y_i\in S} Y_i\right\|_2^2,
%			$$
%			with tie broken arbitrarily.
%			\item $\hat\theta_h^{(s)}= \frac 1{(1-\delta)n_h^{(s)}}\sum_{i:Y_i\in V} Y_i$.
%		\end{enumerate}
%%		\begin{enumerate}
%%			\item Define $T_{\epsilon} = \epsilon^{-\frac 1p}e^{-{C_2\over \epsilon p\alpha}}$, with $\epsilon = 0.3$
%%			\item Compute 
%%			$$
%%			\hat \theta_h^{(s)} = \argmin_{\theta\in \reals^d} \sum_{i:Y_i\in T_h^{(s)}} \ell_{T_{\epsilon}}(\|X_i-\theta\|_2),\quad h\in \sth{1,\dots,k},$$
%%			where 
%%			$
%%			\ell_\tau(x) = x^2\indc{x\leq \tau}+\tau^2\indc{x>\tau}.
%%			$
%%		\end{enumerate}
%		\EndFor
%		\State $s=s+1$
%		\EndWhile
%	\end{algorithmic}
%	{\bf Output}: $(\hat \theta_1^{(s)},\dots,\hat \theta_k^{(s)})$ and label estimate for $Y_i$ given by $\hat z_i^{(s)} = \argmin_{h\in\{1,\dots,k\}}\|Y_i-\hat\theta_h^{(s)}\|_2,$ with tie broken arbitrarily.
%\end{algorithm}

\section{Results}

Denote the minimum separation between the centers by $\Delta$
\begin{align}
	\Delta=\min_{g,h\in[k],g\neq h}\|\theta_g-\theta_h\|_2.
\end{align}
We denote the signal to noise ratio as
\begin{align}
\snr = {\Delta\over 2\sigma}.
\end{align}
Let $\Lambda_s$ denote the error rate of estimating the centers at iteration $s$
\begin{align}
	\Lambda_s = \max_{h\in[k]}\frac 1{\Delta} \|\hat \theta_h^{(s)}-\theta_h\|_2.
\end{align}
Let us define the minimum fraction of points in the data set that come from a single component in the Gaussian mixture as
\begin{align}
	\alpha=\min_{g\in[k]} {n_{g}^*\over n}.
\end{align}
Define the cluster-wise mis-clustering rate as
\begin{align}\label{eq:mislabel}
	G_s=\max_{g\in [k]} \sth{\max\sth{{\sum_{h\in[k]\atop h\neq g} n_{gh}^{(s)}\over n_g^*},{\sum_{h\in[k]\atop h\neq g} n_{hg}^{(s)}\over n_g^{(s)}}}}
\end{align}
Our main result is the following.
\begin{theorem}
	\label{thm:main}
	Suppose that $n\alpha\geq c\log n$ for some $c>0$. There exists absolute constants $c_1,c_2>0$ such that the followings are satisfied. If the clustering initialization satisfies  
	$$\Lambda_0\leq \frac 12-{e^{25/(4p\alpha)}\over (\snr)^{1/2}},$$
	then whenever $\snr\geq c_1(0.3)^{-\frac 1p}e^{\frac {10(1+20/7\alpha)}{3p}}=M$ 
	we have $$\EE\qth{\ell(\hat z^{(s)},z)}\leq 2k^2{\pth{1-{c_2\over M}}^{-p}\over (\snr)^p}
	+ 4kn^{-c/4}+16e^{-0.3n},
		\quad s\geq 1.
		$$
\end{theorem}

\section{Proof strategy}

The proof on the $\lss$ algorithm is primarily based in the following two stages: 
\begin{enumerate}[label=(\alph*)]
	\item analyzing accuracy of the clustering method based on current center estimates,
	\item analysis of the next center updates based on current labels.
\end{enumerate} 
We obtain results on these steps separately and then combine them to prove \prettyref{thm:main}. Our analysis depends on high-probability events of the following type. For any symmetric matrix $A$ let $\lambda_{\max}(A)$ denote its maximum eigen value.
\begin{lemma}
	\label{lmm:E-prob}
	Fix $0<\tau,\epsilon_0<\frac 12$. There is a set $\calE_{\tau,\epsilon_0}$ with $\PP\qth{\calE_{\tau,\epsilon_0}}\geq 1-kn^{-c/2}-e^{-0.3n}$ on which the following holds: 
	\begin{enumerate}[label=(\roman*)]
		\item For any $\tau>0$ and any $S\subseteq [n]$ with $|S|>\beta n$, the cardinality of the set 
		$$\sth{i\in S: \norm{w_i}\leq {\sigma}\tau^{-\frac 1p}e^{\frac 1{\tau p}(1+\frac 1\beta)}}$$
		is at least $(1-\tau)|S|$.
		
		\item For any $\epsilon\in[\epsilon_0,1/2]$ and $g,h\in[k]$ we have
		$$\sum_{i:Y_i\in T_g^*}\indc{\epsilon^2\Delta\leq \|w_i\|}
		\leq \frac {5}{2p \alpha\log(\epsilon_0^2\Delta/\sigma)}.$$
	\end{enumerate}
\end{lemma}
\begin{proof}
	For each of the cases we separately construct sets of high probability on which the results hold. Then taking intersection we get the result. The individual analyses have been provided in \prettyref{lmm:norm-concentration}, \prettyref{lmm:Chernoff-binom} in \prettyref{app:main-lemma-proof}.
\end{proof}

The following lemma provides results that show upper bound on $G_{s+1}$ based on $\Lambda_s$ and establish upper bound on $\Lambda_{s}$ in terms of $G_s$. 

\begin{lemma}\label{lmm:Gs-Ls-bound}
	Fix $\epsilon_0\in (0,\frac 12]$. Then on the set $\calE_{\epsilon_0}=\calE_{0.5,\epsilon_0}$, which has probability at least $1-n^{-c/2}-ke^{-0.3n}$, we have for all $s\geq 0$
	\begin{enumerate}[label=(\roman*)]
		\item If $\Lambda_s\leq \frac 12-\epsilon_0$ then $G_{s+1} \leq \frac {5}{2p \alpha\log(\epsilon_0^2\Delta/\sigma)}$,
		\item If $G_{s+1}\leq 0.2$ then $\Lambda_{s+1}\leq {3\sigma\over \Delta}(0.3)^{-\frac 1p}e^{\frac {10(1+\frac 5{4\alpha})}{3p}}$.
	\end{enumerate}
\end{lemma}



\begin{proof}[Proof of \prettyref{lmm:Gs-Ls-bound}]
	The proof of \prettyref{lmm:Gs-Ls-bound}(i) has been presented in \prettyref{app:Gs-Ls-i}. We present below the proof of \prettyref{lmm:Gs-Ls-bound}(ii). We prove this using contradiction. For simplicity of notation we denote 
	$$D={\sigma\over \Delta}(0.3)^{-\frac 1p}e^{\frac {10(1+\frac 5{4\alpha})}{3p}}.$$ 
	Let us assume $\Lambda_{s+1} > {3D\over \Delta}$. This implies that there exists a cluster $h$ such that the centroid estimation error satisfies 
	$$\|\hat \theta_h^{(s+1)}-\theta_h\|> {3D}.$$ 
	As $G_{s+1}\leq 0.2$ we know that $n_{hh}^{(s)}\geq 0.8 n_h^{(s)}$. As we are on the set $\calE_{\epsilon_0}$, we use \prettyref{lmm:E-prob} with 
	$$
	 \tau =0.3,\quad S=\{i\in [n]:Y_i\in T_{h}^{(s)}\cap T_{h}^*\}, \quad \beta = {0.8 \alpha} < {n_{hh}^{(s)}\over n}.
	$$ 
	This gives us that there are at least $0.7n_{hh}^{(s)}(=0.56 n_h^{(s)})$ many points within a radius $D$ of $\theta_h$. As our subset selection strategy guarantees that we choose $0.55 n_h^{(s)}$ points within a radius $D$ of the estimator $\hat \theta_h^{(s)}$, we get a contradiction.
\end{proof}

\section{Proof of \prettyref{thm:main}}

The mis-clustering rate at step $s$ is given by 
\begin{align}
	A_s=\frac 1n \sum_{i=1}^n\indc{z^{(s)}_i\neq z_i}
	=\frac 1n \sum_{h\neq g \in [k]} n_{hg}^{(s)}.
\end{align} 
For $c_1$ to be chosen later, we define
$$\epsilon_0={c_2\over (\Delta/2\sigma)^{1/2}}.$$
Then from \prettyref{lmm:Gs-Ls-bound} it follows that we can choose $c_1,c_2>0$ such that on the set $\calE_{\epsilon_0}$ we have that if $\Lambda_0\leq \frac 12-\epsilon_0$ then $G_1\leq 0.2$.
A second application of \prettyref{lmm:Gs-Ls-bound} guarantees that we can choose $c_3$ large enough such that if  
$${\Delta\over \sigma}(0.3)^{\frac 1p}e^{-\frac {10(1+\frac 5{4\alpha})}{3p}}\geq M\geq c_3$$
then on the set $\calE_{0.2}$ we have,
\begin{enumerate}[label=(P\arabic*)]
	\item \label{eq:P1} $G_s\leq \frac {5}{2p \alpha\log(\epsilon_0^2\Delta/\sigma)}\leq 0.2$ for all $s\geq 1$
	\item $\Lambda_s\leq {3\sigma\over \Delta}(0.3)^{-\frac 1p}e^{\frac {10(1+\frac 5{4\alpha})}{3p}}\leq {C_1\over M} \leq 0.2$ for all $s\geq 1$.
\end{enumerate}
Combining the above displays we get that on the set
\begin{align}
	\label{eq:Prob-E}
	\calE&=\calE_{\epsilon_0}\cap \calE_{0.2}\text{ with }
	\PP\qth{\calE}
	\geq 1-4kn^{-c/4}-e^{-0.3n}
\end{align} 
we have
\begin{align}
	\label{eq:km14}
	\Lambda_s\leq 0.2,G_{s}\leq 0.2 \text{ for all } s\ge 1.
\end{align}
We will show that $\PP\qth{\left.z_i\neq \hat z_i^{(s+1)}\right|\calE}$ is small for each $i\in [n]$.
Note that $$\indc{z_i\neq\hat z_i^{(s+1)}}
=\frac 12\sum_{g,h\in [k]\atop g\neq} \indc{\hat z_i^{(s+1)}=h,z_i=g}.$$ Fix a choice for $z_i$, say equal to $g\in [k]$. Then 
For any $h\in[k],h\neq g$,
\begin{align}\label{eq:km21}
	\indc{z_i=g,\hat z_i^{(s+1)}=h}
	&\leq \indc{\|Y_i-\hat\theta_h^{(s)}\|^2
		\leq \|Y_i-\hat\theta_g^{(s)}\|^2, Y_i\in T_g^*}
	\nonumber\\
	&=\indc{\|\theta_g+w_i-\hat\theta_h^{(s)}\|^2
		\leq \|\theta_g+w_i-\hat\theta_g^{(s)}\|^2}
	=\indc{\|\theta_g-\hat\theta_h^{(s)}\|^2-\|\theta_g-\hat\theta_g^{(s)}\|^2\leq 2\langle w_i,\hat\theta_h^{(s)}-\hat\theta_g^{(s)}\rangle}.
\end{align}
Triangle inequality implies
\begin{align}
	\|\theta_g-\hat\theta_h^{(s)}\|^2\geq \pth{\|\theta_g-\theta_h\|-\|\theta_h-\hat\theta_h^{(s)}\|}^2
	\geq (1-\Lambda_s)^2\|\theta_g-\theta_h\|^2.
\end{align}
Using $$\|\theta_g-\hat\theta_g^{(s)}\|\leq \Lambda_s\Delta
\leq \Lambda_s\|\theta_g-\theta_h\|$$
and the fact that $(1-x)^2-y^2\geq (1-x-y)^2$ when $y(1-x-y)\geq 0$, we obtain
\begin{align}
	&\|\theta_g-\hat\theta_h^{(s)}\|^2-\|\theta_g-\hat\theta_g^{(s)}\|^2
	\geq (1-\Lambda_s)^2\|\theta_g-\theta_h\|^2
	-\Lambda_s^2\|\theta_g-\theta_h\|^2
	\geq (1-2\Lambda_s)^2\|\theta_g-\theta_h\|^2.
\end{align}
In view of \eqref{eq:ht21} the last display implies
\begin{align}
	\label{eq:km10}
	\indc{z_i=g,\hat z_i^{(s+1)}=h}
	\leq \indc{(1-2\Lambda_s)^2\|\theta_g-\theta_h\|^2\leq 2\langle w_i,\hat\theta^{(s)}_h-\hat\theta^{(s)}_g \rangle}.
\end{align}
Using Property \ref{eq:P1} and 
\begin{align*}
	|\langle w_i,\hat\theta^{(s)}_h-\hat\theta^{(s)}_g\rangle|
	&\leq \|w_i\|\cdot \|\hat\theta^{(s)}_h-\hat\theta^{(s)}_g\|
	\nonumber\\
	&\leq \|w_i\|\cdot(\|\hat\theta^{(s)}_h-\theta_h\|+\|\hat\theta^{(s)}_h-\theta_h\|+\|\theta_g-\theta_h\|)
	\leq \|w_i\|(2\Lambda_s\Delta+\Delta)
	\leq 2\|w_i\|\Delta,
\end{align*}
we get that
\begin{align*}
	\indc{z_i=g,\hat z_i^{(s+1)}=h}
	\leq \indc{(1-2\Lambda_s)^2\Delta\leq 2\|w_i\|}
	\leq \indc{\frac 12\pth{1-{2C_1\over M}}\Delta\leq \|w_i\|}.
\end{align*}
Taking expectation conditioned on $\calE$ we get
	\begin{align}
		\PP\qth{\left.z_i\neq \hat z_i^{(s+1)}\right|\calE}
		&\leq
		k^2 \max_{g,h\in [k]\atop g\neq h}\PP\qth{\left.z_i=g, \hat z_i^{(s+1)}=h \right|\calE}
		\leq 2k^2{\pth{1-{2C_1\over M}}^{-p}\over (\Delta/2\sigma)^p}
	\end{align}
	This implies
	\begin{align}
		\EE\qth{A_{s+1}|\calE}
		=\frac 1n\sum_{i=1}^n\PP\qth{\left.z_i\neq z_i^{(s+1)}\right| \calE}\leq 2k^2{\pth{1-{2C_1\over M}}^{-p}\over (\Delta/2\sigma)^p}.
	\end{align}
Combining the above with \eqref{eq:Prob-E} we get
\begin{align}
	\EE\qth{A_s}&\leq4 kn^{-c/4}+16e^{-0.3n}+2k^2{\pth{1-{2C_1\over M}}^{-p}\over (\Delta/2\sigma)^p}.
\end{align}

\section{Lower bound}
\begin{theorem}
	 For an absolute constant $C>0$ such that the following holds true. If the error distributions are chosen from $\calR_p(\sigma)$, then
	 $$\inf_{\hat z}\sup\EE_{z\in[k]^n}\qth{\ell(\hat z,z)}
	\geq {C\alpha\over k^2p }\cdot{1\over (\snr)^{p}(\log (\snr))^{1.5}}.$$
\end{theorem}
\begin{proof}
	We follow the proof technique of \cite[Theorem 3.3]{lu2016statistical}. For any $z\in [k]^n$, let us define $n_u(z)=\sum_{i=1}^n \indc{z_i=u}$. Let $z^*\in [k]^n$ satisfying $n_1(z^*)\leq n_2(z^*)\leq\dots\leq n_k(z^*)$, with $n_1(z^*)=n_2(z^*)=\floor{\alpha n}$. It is easy to check the existence of $z^*$. For each $u\in [k]$ we choose a subset of $\{i\in [n]: z^*(i)=u\}$ with cardinality $\ceil{n_u(z^*)-{\alpha n\over 4k}},$ denoted by $T_u$. Define $T=\cup_{u=1}^k T_u$ and
	$\calZ^* = \sth{z\in \calZ,z_i=z_i^* \text{ for all } i\in T}$. 
	A key observation is that for any $z\neq \tilde z\in\calZ^*$, we have $\frac 1n\sum_{i=1}^n\indc{z_i\neq \tilde z_i}\leq \frac kn\cdot \frac {\alpha n}{4k}=\frac \alpha 4$, and 
	$$
	\frac 1n\sum_{i=1}^n\indc{\pi(z_i)\neq \tilde z_i}\geq \frac 1n(\alpha n-{\alpha n\over 4k})\geq {\alpha\over 2}
	$$
	for all $\pi\in \calS_k$ which is not the identity permutation. Thus, $\ell(\tilde z,z)=\frac 1n\sum_{i=1}^n \indc{z_i\neq \tilde z_i}$ for all $z,\tilde z\in \calZ^*$. Then following the same arguments in the proof of \cite[Theorem 2]{gao2018community}, we can obtain
	\begin{align}\label{eq:gao2018}
	\inf_{\hat z}\sup_{z\in \calZ} \EE\qth{\ell(\hat z,z)}
	\geq {\alpha\over 6}
	\frac 1{T^c}\sum_{i\in T^c}\qth{\frac 1{2k^2}\inf_{\hat z_i}(\PP_1\qth{\hat z_i=2}+\PP_2\qth{\hat z_i=1})}.
	\end{align}
	Here $\PP_t,t\in \{1,2\}$ denote the probability distribution of our data given $z_i=t$. By Neyman-Pearson Lemma, the infimum of the right hand side of the last display is achieved by the likelihood ratio test 
	$$
	\hat z_i = \argmin_{g\in \{1,2\}}\|Y_i-\theta_g\|^2.
	$$
	Thus,
	$$
	\inf_{\hat z_i}\pth{\frac 12 \PP_1\qth{\qth{\hat z_i=2}+\frac 12\PP_2\qth{\hat z_i=1}}}
	=\PP\qth{\|\theta_1+w_i-\theta_2\|^2\leq \|w_i\|^2}
	=\PP\qth{\|\theta_1-\theta_2\|^2\leq 2\langle w_i,\theta_1-\theta_2\rangle}.
	$$
	 Note that as $|\langle w_i,\theta_1-\theta_2\rangle|\leq \|w_i\|\cdot\|\theta_1-\theta_2\|$, from the last display we get
	\begin{align}
		\label{eq:lb1}
	\inf_{\hat z_i}\pth{\frac 12 \PP_1\qth{\qth{\hat z_i=2}+\frac 12\PP_2\qth{\hat z_i=1}}}
	\geq \PP\qth{\|w_i\|\geq \frac 12\|\theta_1-\theta_2\|}
	\geq \PP\qth{\|w_i\|\geq \Delta/2}.
	\end{align}
	Next we choose all the errors to have the distribution
	\begin{align*}
	\begin{gathered}
		\{w_i\}_{i=1}^n\simiid R\cdot \Unif(\calS_{d-1}),\\ R = \sigma\pth{\xi\over pa\log a}^{\frac 1p}\tilde R,
	\ \PP\qth{\tilde R\geq r}=\frac {a(\log a)^{1+\xi}\indc{r\geq 0}}{(1+r^{p-1})(a+r)(\log(a+r))^{1+\xi}},\ a>1,\xi>0.
	\end{gathered}
	\end{align*}
	where $R$ is the radial distribution and $\Unif(\calS_{d-1})$ is the uniform distribution over the unit sphere, and they are independent.
	The $p$-th moment of $R$ is bounded from above by $\sigma^p$ follows from the fact that the $p$-th moment of $\tilde R$ is bounded from above as
	$$
	\EE\qth{\tilde R^{p}}
	=p\int_{0}^\infty  r^{p-1} \PP\qth{\tilde R > r} dr
	\leq \frac {pa\log a}\xi.
	$$
	This implies, with $a=2,\xi=\frac 12$, for an absolute constant $C>0$
	$$
	\PP\qth{\|w_i\|\geq \Delta/2}
	=\PP\qth{\tilde R\geq \frac{\Delta}{2\sigma}\pth{\xi\over pa\log a}^{-\frac 1p}}
	\geq C {1\over p(\Delta/2\sigma)^{p}(\log (\Delta/2\sigma))^{1.5}},
	$$
	where we used $\abs{\log\pth{\pth{\xi\over pa\log a}^{-1/p}}}\leq c$ for a small constant $c>0$. Thus using \eqref{eq:gao2018} and \eqref{eq:lb1} we conclude the result.
\end{proof}

\section{Minimax optimality with Sub-Gaussian mixtures}
In this section we prove that our algorithm achieves the optimal misclustering rate when the errors are generated from Sub-Gaussian mixture. In our model, the observed data $Y_1,\dots,Y_n\in \reals^d$ are distributed as
\begin{align}
	Y_i=\theta_{z_i}+w_i,\ i=1,\dots,n,
\end{align}
where $\sth{z_i}_{i=1}^n\in[k]^n$ denote the underlying unknown component labels of the points, and $w_i$-s denote the error variables. We assume that $w_i$-s are independent 0 mean Sub-Gaussian vectors with parameter $\sigma>0$, i.e.,
\begin{align}\label{eq:subg-defn}
	\EE\qth{e^{\langle a,w_i \rangle}}
	\leq e^{\sigma^2\|a\|^2\over 2}, \text{ for all $i\in \sth{1,\dots,n}$ and $a\in \reals^d$}.
\end{align}
We show the following.
Define the cluster-wise correct classification proportion at step $s$ as
\begin{align}
	H_s=\min_{g\in [k]}\sth{\min\sth{{n_{gg}^{(s)}\over n_g^*},{n_{gg}^{(s)}\over n_{g}^{(s)}}}}.
\end{align}
Our result is the following.
\begin{theorem}
	\label{thm:main-subg}
	There exists absolute constants $c_0,c_1,c_2,c_3,c_4>0$ such that the followings are satisfied.
	\begin{enumerate}[label=(\alph*)]
		\item \textbf{$\snr< c_0\sqrt {d/\alpha}$:} Assume $n\alpha^2\geq Ck\log n$ and ${\snr}\sqrt{\alpha\over 1+{dk\over n}}\geq C\sqrt k$ for a sufficiently large constant $C$. If the clustering initialization satisfies either one of the following conditions
		$${H_0}\geq 1-\frac 2{\sigma\sqrt d}\pth{\frac 12 - \frac {c_1/{\alpha}^{1/4}}{\pth{\snr}^{1/2}}}\quad  \text{ or } \quad \Lambda_0\leq \frac 12-{c_2/{\alpha}^{1/4}\over \pth{\snr}^{1/2}}.$$
		Then whenever $\snr\sqrt \alpha \geq M\geq c_3$,  we have $$\EE\qth{\ell(\hat z^{(s)},z)}\leq \exp\sth{-\frac 12\pth{1-{c_4\over \sqrt \snr}}(\snr)^2},
		\quad s\geq 3\log n.
		$$
		
		\item \textbf{$\snr\geq c_0\sqrt {d/\alpha}$:} Suppose the clustering initialization satisfies either one of the following conditions
		$${H_0}\geq \frac 12 +\gamma_0 \text{ with } \gamma_0>2.1\alpha \quad  \text{ or } \quad \Lambda_0\leq \frac 12-{c_2/{\alpha}^{1/4}\over \pth{\snr}^{1/2}}.$$
		Then whenever $\snr\sqrt \alpha \geq M\geq c_3$,  the $\lss$ algorithm with $\delta=\frac 12-{\gamma_0\over 4}$ achieves the misclustering rate
		$$
		\EE\qth{\ell(\hat z^{(s)},z)}\leq \exp\sth{-\frac 12\pth{1-{c_4\over \sqrt \snr}}{(\snr)^2}},
		\quad s\geq 1.
		$$
	\end{enumerate}
	
\end{theorem}
\begin{remark}
	The result \cite[Theorem 3.4]{lu2016statistical} shows that it is not possible to improve the misclustering error beyond the rate $e^{-\frac 12(1+o(1)){(\snr)^2}}$. This establishes the optimality of the coordinate-wise median based Lloyd algorithm.
\end{remark}

\begin{proof}[Proof of \prettyref{thm:main-subg}]
	The proof of part (a) is essentially the same as the proof of the similar result \cite[Theorem 3.2]{lu2016statistical} for usual $k$-means. This is because the part of the cluster, the mean of which we use to construct our centroid estimates, is of similar order as the full clusters themselves. As a result we can use the similar concentration bounds that were used to analyze the mean of the full sample in the classical $k$-means problems. We omit the proof here.
	
	To prove part (b), we use the following key lemma.
	\begin{lemma}
		\label{lmm:E-prob-subg}
		Fix $0<\tau,\epsilon_0<\frac 12$. There is a set $\calE_{\tau,\epsilon_0}$ with $\PP\qth{\calE_{\tau,\epsilon_0}}\geq 1-kn^{-c/2}-4e^{-0.3n}$ on which the following holds: 
		\begin{enumerate}[label=(\roman*)]
			\item For any $S\subseteq [n]$ with $|S|>\beta n$, the cardinality of the set 
			$$\sth{i\in S: \|{w_i}\|\leq \sigma \pth{\sqrt d + \sqrt{2\pth{\frac 1\tau\pth{1+\frac 1\beta}+\log(1/\tau)}}}}$$ 
			is at least $(1-\tau)|S|$.
			\item For any $\epsilon\in[\epsilon_0,1/2]$ and $g,h\in[k]$ we have
			$$\sum_{i:Y_i\in T_g^*}\indc{\epsilon^2\|\theta_g-\theta_h\|^2\leq \langle w_i,\theta_h-\theta_g\rangle}
			\leq \frac {5n_g^*}{4\epsilon_0^4(\Delta/\sigma)^2}$$
			\item For any symmetric matrix $A$, let $\lambda_{\max}(A)$ denote its maximum eigen value. Then 
			$$\lambda_{\max}\pth{\sum_{i:Y_i\in T_g^*} w_iw_i^{\sfT}}\leq 6\sigma^2(n_g^*+d) \text{ for all } g\in [k].$$
		\end{enumerate}
	\end{lemma} 
	To prove the above lemma, for each of the cases we separately construct sets of high probability on which the results hold. Then taking intersection we get the result. The analysis of (i) has been provided in \prettyref{lmm:norm-concentration-subg}, the statements (ii),(iii) are the exact results from \cite[Lemma 12, Lemma 13]{JKY2023}.
	
	Based on the above result we get the following results on step-wise clustering errors due to mislabelling.

\begin{lemma}\label{lmm:Gs-Ls-bound-subg}
	Fix $0<\epsilon_0\leq \frac 12,\frac 5{n\alpha} <\gamma_0 \leq \frac 12$. Let $r_k={\Delta\over\sigma}\sqrt{\alpha\over 1+{dk/n}}$. Then on the set $\calE_{\tau,\epsilon_0}$ with $\tau={\gamma_0\over 1+2\gamma_0}$ we have
	\begin{enumerate}[label=(\roman*)]
		\item If $\Lambda_s\leq \frac 12-\epsilon_0$ then $H_{s+1} \geq 1-{5\over \epsilon_0^4 r_k^2}
		-{48\Lambda_s^2\over \epsilon_0^4r_k^2}$,
		\item If $H_s\geq \frac 12+\gamma_0$ then $\Lambda_s\leq {3\sigma\over \Delta} \pth{\sqrt d + \sqrt{2\pth{{1+2\gamma_0\over \gamma_0}\pth{1+\frac 1\beta}+\log\pth{1+2\gamma_0\over \gamma_0}}}}$.
	\end{enumerate}
\end{lemma}

The proof of above result is straightforward. The proof of \prettyref{lmm:Gs-Ls-bound-subg}(i) is exactly the same as in \cite[Appendix C]{JKY2023}, so we skip it here. 
	We present below the proof of \prettyref{lmm:Gs-Ls-bound}(ii). We prove this using contradiction. For simplicity of notation we denote 
	$$D={\sigma} \pth{\sqrt d + \sqrt{2\pth{{1+2\gamma_0\over \gamma_0}\pth{1+\frac 1\beta}+\log\pth{1+2\gamma_0\over \gamma_0}}}}.$$ 
	Let us assume $\Lambda_{s} > 3D$. This implies that there exists a cluster $h$ such that the centroid estimation error satisfies 
	$$\|\hat \theta_h^{(s+1)}-\theta_h\|> {3D}.$$ 
	As $H_{s}\geq \frac 12+\gamma_0$ we know that $n_{hh}^{(s)}\geq \pth{\frac 12+\gamma_0} n_h^{(s)}$. As we are on the set $\calE_{\tau,\epsilon_0}$, we use \prettyref{lmm:E-prob-subg} with 
	$$
	\tau = {\gamma_0\over 1+2\gamma_0},\quad S=\{i\in [n]:Y_i\in T_{h}^{(s)}\cap T_{h}^*\}, \quad \beta = {\pth{\frac 12+\gamma_0} \alpha} < {n_{hh}^{(s)}\over n}.
	$$ 
	This gives us that there are at least $\pth{1-{\gamma_0\over 1+2\gamma_0}}n_{hh}^{(s)}(=\pth{\frac 12+{\gamma_0\over 2}} n_h^{(s)})$ many points within a radius $D$ of $\theta_h$. As our subset selection strategy guarantees that we choose $\pth{\frac 12+{\gamma_0\over 4}} n_h^{(s)}$ points within a radius $D$ of the estimator $\hat \theta_h^{(s)}$, we get a contradiction.


Next we use the above results to prove \prettyref{thm:main-subg}(ii). For $c_1$ to be chosen later, we define
$$\epsilon_0={c_1/\alpha^{1/4}\over \pth{\snr}^{1/2}}.$$
Let $G_s$ be the mislabeling proportion as defined before in \eqref{eq:mislabel}. Then from \prettyref{lmm:Gs-Ls-bound-subg} it follows that we can choose $c_0,c_1>0$ such that on the set $\calE_{{\gamma_0\over 1+2\gamma_0},\epsilon_0}$:
\begin{itemize}
	\item if $H_0\geq \frac 12+\gamma_0$ then $\Lambda_0\leq 0.3$,
	\item if $\Lambda_0\leq \frac 12-\epsilon_0$ then $H_1\geq 0.7$.
\end{itemize}
A second application of \prettyref{lmm:Gs-Ls-bound-subg} guarantees that we can choose $c_0$ large enough such that if  
$\snr\geq c_0\sqrt{d/\alpha}$
then on the set $\calE_{{5\over 26},0.2}$, with $\epsilon_1=\gamma_1=0.2$,
\begin{itemize}
	\item if $G_s\leq 0.3$ then
	\begin{align}
		\label{eq:Ls}
		\Lambda_s&\leq {12\sqrt 2/\alpha^{1/2}\over \sqrt{0.2}\snr} \leq 0.3,
	\end{align}
	\item if $\Lambda_s\leq 0.3$ then
	\begin{align}
		\label{eq:Gs}
		G_{s+1}&\leq {5/\alpha\over (0.2)^4(\snr)^2}+{48(0.3)^2/\alpha\over (0.2)^4(\snr)^2}\leq 0.3.
	\end{align}		
\end{itemize}
and whenever 
Combining the above displays we get that on the set
\begin{align}
	\label{eq:Prob-E}
	\calE&=\calE_{{\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{{5\over 26},0.2}
	\nonumber\\
	\PP\qth{\calE}
	&\geq 1-4kn^{-c/4}-4e^{-0.3n}
\end{align} 
we have
\begin{align}
	\label{eq:ht14}
	\Lambda_s\leq 0.3,G_{s+1}\leq 0.3 \text{ for all } s\ge 0.
\end{align}
The rest of the analysis is 
identical to that of the proof of \cite[Theorem 1]{JKY2023} where it is shown that once we achieve $\Lambda_s\leq 0.3$ for all $s\geq 3$, the mislabeling rate follows. We omit it here.
\end{proof}


\section{Clustering in presence of adversarial outliers \nb{TBD}}

\subsection{Error distributions with moment constraints}

\subsection{Sub-Gaussian error distributions}
Suppose that an adversary adds $n^{\out}$ many points to our existing data set. Then we have the following guarantees.
\begin{theorem}
	\label{thm:optim-outl}
	Suppose that $n\alpha\geq c\log n$ for some $c>0$. There exists absolute constants $c_1,c_2,c_3,c_4,c_5>0$ such that the followings are satisfied. For any $\eta\in(0,1]$, if the clustering initialization satisfies either one of the following conditions
	$${H_0}\geq \frac 12+\frac {c_1/\alpha}{\pth{\snr}^2}\quad  \text{ or } \quad \Lambda_0\leq \frac 12-{c_2/\alpha\over \pth{\snr}^{\frac 12(1-\eta)}},$$
	then whenever $$\snr\sqrt\alpha\geq M\geq c_3,$$ 
	for any $n^{\out}\leq n\alpha(1-c_4M^{-2\eta})$ our algorithm guarantees $$\EE\qth{\ell(\hat z^{(s)},z)}\leq \exp\sth{-\frac 12\pth{1-{c_5\over \sqrt M}}{(\snr)^2}},
	\quad s\geq 1.
	$$
\end{theorem}


\subsection{Step-wise clustering errors due to mislabelling (in presence of outliers)}
The proof of the above theorem hinges on the following lemma, similar to \prettyref{lmm:Gs-Ls-bound}.

\begin{lemma}\label{eq:HsLs-bound}
	Fix $\epsilon_0,\gamma_0\in (0,\frac 12]$ and suppose that an adversary added $n\beta$ many outliers with $\beta\leq\alpha(1-\delta)$ for some $\delta>0$. Let $r_k={\Delta\over\sigma}\sqrt{\alpha\over 1+{dk/n}}$. Then on the set $\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0} $ we have
	\begin{enumerate}[label=(\roman*)]
		\item If $\Lambda_s\leq \frac 12-\epsilon_0$ then $H_{s+1} \geq \frac 12 +\min\sth{{\delta-2\tau\over 2(2-\delta)},1-\tau}$ where $\tau={5\over 2\epsilon_0^4 r_k^2}
		+{24\Lambda_s^2\over \epsilon_0^4r_k^2}$,
		\item If $H_s\geq \frac 12+\gamma_0$ then $\Lambda_s\leq {3\sigma\over \Delta} \pth{\sqrt d + \sqrt{2\pth{{1+2\gamma_0\over \gamma_0}\pth{1+\frac 1\beta}+\log\pth{1+2\gamma_0\over \gamma_0}}}}$.
	\end{enumerate}
\end{lemma}

\begin{proof}
	
	The proof of part (i) borrows results from the proof of \prettyref{lmm:Gs-Ls-bound}(i). Notice that we can show for each $h\neq g$
	\begin{align}
		\label{eq:km22}
		n_{gh}^{(s+1)}
		&\leq 
		\frac{5n_g^*\sigma^2}{4\epsilon_0^4\Delta^2}
		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2}\pth{{n_g^*}+  d}.
	\end{align}
	Using the last display and noting that $k\leq \frac 1{\alpha}$ and $n_g^*\geq n\alpha$ we get
	\begin{align}\label{eq:km23}
		{\sum_{h\in[k]\atop h\neq g}n_{gh}^{(s+1)}\over n_g^*}
		\leq \tau,\quad \tau=
		\frac{5\sigma^2}{2\epsilon_0^4\Delta^2\alpha}
		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2\alpha}\pth{1+ {dk\over n}}.
	\end{align}
	Using $n_g^{*}=\sum_{h\in [k]}n_{gh}^{(s+1)}$ for all $s\geq 0$, we get 
	\begin{align}\label{eq:km24}
		{n_{gg}^{(s+1)}\over n_g^*}\geq 1-\tau.
	\end{align}	 
	Next we switch $g,h$ in \eqref{eq:km22} and sum over $h\in [k], h\neq g$. We get
	\begin{align}
		\sum_{h\in[k]\atop h\neq g}n_{hg}^{(s+1)}
		\leq \frac{5n\sigma^2}{2\epsilon_0^4\Delta^2}
		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2}\pth{n+ kd}
		\leq n\alpha\tau.
	\end{align}
	Using the above and noticing that in addition to the points in $\cup_{h\in[k]}\sth{T_{h}^*\cap T_g^{(s+1)}}$, $T_g^{(s+1)}$ can at most have $n\beta$ many extra points, accounting for the outliers, we get
	\begin{align}
		{n_{gg}^{(s+1)}\over n_g^{(s+1)}}\geq {n_{gg}^{(s+1)}\over n_{gg}^{(s+1)}+n\alpha\tau+n^{\out}}
		\geq \frac 1{1+{n_g^*(1-\delta+\tau)\over n_{gg}^{(s+1)}}}
		\geq \frac 1{1+{1-\delta+\tau\over 1-\tau}}
		=\frac 12 + {\delta-2\tau\over 2(2-\delta)}.
	\end{align}
	Combining the last display with \eqref{eq:km24} we get
	\begin{align*}
		H_{s+1}=\min_{g\in [k]}\sth{\min\sth{{n_{gg}^{(s)}\over n_g^*},{n_{gg}^{(s)}\over n_{g}^{(s)}}}}
		\geq \frac 12+\min\sth{{\delta-2\tau\over 2(2-\delta)},\frac 12-\tau},
	\end{align*}
	as required.
	
	The proof of (ii) follows a similar strategy as in the proof of \prettyref{lmm:Gs-Ls-bound}, part (ii). Define as before
\end{proof}
\subsection{Proof of \prettyref{thm:optim-outl}}
Let $\beta=\alpha(1-\delta)$.  For $c_1,c_2$ to be chosen later, we define
$$\gamma_0=\frac {c_1}{\pth{{\Delta\over \sigma}\sqrt{\alpha\over d}}^2},\quad \epsilon_0={c_2\over \pth{{\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}^{\frac 12(1-\eta)}}.$$
Then from \prettyref{lmm:Gs-Ls-bound} it follows that, we can choose $c_1,c_2,c_3,c_4>0$ such that whenever $M>c_3$ and $\delta\geq c_4M^{-2\eta}$, on the set $\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0}$:
\begin{itemize}
	\item if $\Lambda_0\leq \frac 12-\epsilon_0$ then $H_1\geq \frac 12 + {\delta\over 6}$.
	\item if $H_0\geq \frac 12+\gamma_0$ then $\Lambda_0\leq 0  .3$,
\end{itemize}
A second application of \prettyref{lmm:Gs-Ls-bound} guarantees that we can choose $c_3$ large enough such that if  
$$M=\min \sth{{\Delta\over \sigma}\sqrt{\alpha\over d},{\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}\geq c_3$$
then on the set $\calE_{{2\gamma_1\over 1+2\gamma_1},\epsilon_1}\cap \calE_{\frac 14,\epsilon_1}$, with $\epsilon_1=\gamma_1=0.2$, if $H_{s}\geq \frac 12 +\frac \delta6$ then $\Lambda_s\leq {12\sqrt 2\over \sqrt{0.2}M} \leq 0.3$ and if $\Lambda_s\leq 0.3$ then $H_{s+1}\geq \frac 12 +\frac \delta6$.
Combining the above displays we get that on the set
\begin{align}
	\label{eq:Prob-E2}
	\calE&=\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0} \cap \calE_{{2\gamma_1\over 1+2\gamma_1},\epsilon_1}\cap \calE_{\frac 14,\epsilon_1}
	\nonumber\\
	\PP\qth{\calE}
	&\geq 1-4(k^2+k)n^{-c/4}-16de^{-0.3n}
\end{align} 
we have
\begin{align}
	\label{eq:km27}
	\Lambda_s\leq 0.3,\quad H_{s+1}\geq \frac 12 +\frac \delta6 \text{ for all } s\ge 2.
\end{align}
We will show that $\PP\qth{\left.z_i\neq \hat z_i^{(s+1)}\right|\calE}$ is small for each $i\in [n]$. This will imply that on the set $\calE$, $A_{s+1}=\frac 1n\sum_{i=1}^n\indc{z_i\neq \hat z_i^{(s+1)}}$ is also small in probability. From this, using a Markov inequality we will conclude the result. The analysis is 
identical to that of the proof of \cite[Theorem 1]{JKY2023} where it is shown that once we achieve $\Lambda_s\leq 0.3$ for all $s\geq 3$, the mislabeling rate follows. We omit it here.

\section{A computable clustering algorithm \nb{TBD}}

We need to use the fact that if initialized at good centroids, we can use a SCAD type loss around it to create the clusters.

\begin{algorithm}[H]
	\caption{The computable $\lss$ clustering algorithm}\label{algo:lloyd-rob-computable}
	{\bf Input}:  Data $Y_1,\dots,Y_n$. Initial centroid estimates $(\hat \theta_1^{(0)},\dots,\hat \theta_k^{(0)})$. Error threshold $\epsilon$. Truncation level $\delta\in (0,\frac 12)$. Here we choose $\delta=0.45$.\\
	{\bf Steps}: 
	\begin{algorithmic}[1]
		\While{$\frac 1k\sum_{h=1}^k \|\hat\theta_h^{(s)}-\hat\theta_h^{(s-1)}\|_2^2 > \epsilon$,}
		\For{$h\in \sth{1,2,\dots,k}}$
		\State \textbf{Labeling step}:
		$$T_h^{(s)}=\sth{Y_i:i\in \sth{1,\dots,n}, \|Y_i-\hat\theta_h^{(s-1)}\|_2\leq \|Y_i-\hat\theta_a^{(s-1)}\|_2,a\in\{1,\dots,k\}, a\neq h}.$$
		\State \textbf{Estimation step:} 
		\begin{enumerate}[label=\alph*)]
			\item Compute $R_h$ as the $(1-\delta)n_h^{(s)}$-th order statistics of the set $Q = \sth{i\in T_h^{(s)}: \|Y_i-\hat \theta^{(s-1)}\|}$.
			\item Compute the set $V$ of $Y_i$-s in $T_h^{(s)}$ such that $\|Y_i-\hat \theta_h^{(s-1)}\|$ is smaller than $R$,
			with tie broken arbitrarily.
			\item $\hat\theta_h^{(s)}= \frac 1{(1-\delta)n_h^{(s)}}\sum_{i:Y_i\in V} Y_i$.
		\end{enumerate}
		\EndFor
		\State $s=s+1$
		\EndWhile
	\end{algorithmic}
	{\bf Output}: $(\hat \theta_1^{(s)},\dots,\hat \theta_k^{(s)})$ and label estimate for $Y_i$ given by $\hat z_i^{(s)} = \argmin_{h\in\{1,\dots,k\}}\|Y_i-\hat\theta_h^{(s)}\|_2,$ with tie broken arbitrarily.
	\end{algorithm}


%
%\section{Related estimation guarantees in absence of outliers}
%\label{sec:other-est-no-outliers}
%%We mention the centrality property here:
%%
%%\begin{enumerate}[label=(Q)]
%%	\item \label{eq:Q}(Quantile detection) Given a real random variable $W$ and $q\in(0,\frac 12]$, we say $x,y$ are sufficient to detect its $q,1-q$-th quantiles if
%%	\begin{align*}
%%		\PP\qth{W\geq x}\leq q,\quad \PP\qth{W\leq y}\leq 1-q.
%%	\end{align*}
%%\end{enumerate}
%
%\begin{theorem}
%	Let $F_{ij}$ denote the distribution of the $j$-th coordinate of the $i$-th data point $Y_i$. Suppose that $n\alpha\geq c\log n$ for some $c>0$ and the constraints in \prettyref{thm:main} on $G_s,\Lambda_s$ are satisfied. Then given any $\tau >0$, there exists absolute constants $C:=C(\tau)>0$ such that whenever $M=\min \sth{{\Delta\over \sigma}\sqrt{\alpha\over d}, {\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}\geq C$
%	with probability at least $1-\frac 1n-4(k^2+k)n^{-(c/2-2)}-16dn^4e^{-0.3n}- 2k^2\exp\sth{-{\Delta\over 8\sigma}}$ we have
%	$$
%	\|\hat \theta_g^{(s)}-\theta_g\|^2\leq {d}
%	\qth{\max_{i:Y_i\in T_g^*}\max_{j\in [d]} \max\sth{\abs{F_{ij}^{-1}\pth{\frac 12 +x_0}},\abs{F_{ij}^{-1}\pth{\frac 12 -x_0}}}}^2,\quad s\geq 2,
%	$$
%	where 
%	$x_0= \sqrt{3\log n\over n_g^*}+e^{-{\Delta^2\over (8+\tau)\sigma^2}}$.
%\end{theorem}
%
%\begin{remark} \nb{EDIT THIS FOR NEW NOTATIONS}
%	In particular, if the errors of the $g$-th cluster are distributed as the univariate Gaussian distribution with variance $\sigma^2$, then for any value of $n_g^*$ the conditions in the above theorems are satisfied with $$x_0=C\sigma\pth{{\sqrt{\log n\over {n_g^*}}+e^{-{\Delta^2\over 24\sigma^2}}}}$$ for some large constant $C>0$. This implies that when $\Delta\gtrsim \sigma\log n$ we achieve the optimal rate of estimating the centroids.
%\end{remark}
%\begin{proof}
%	The results in the last section implies that there is an absolute constant $C>0$ such that whenever 
%	$$
%	\min\sth{{\Delta\over \sigma}\sqrt{\alpha\over d},{\Delta\over \sigma}\sqrt{\alpha\over 1+{kd/n}}}\geq C
%	$$
%	we get for any $g\in [k]$
%	\begin{align}
%		\max\sth{\sum_{h\in[k]\atop h\ne g}n_{hg}^{(s)},\sum_{h\in[k]\atop h\ne g}n_{gh}^{(s)}}
%		\leq \sum_{i=1}^n\indc{\hat z_i^{(s)}\neq z_i}
%		=nA_s, \quad s\geq 3.
%	\end{align}
%	Using the above we get
%	\begin{align}
%		G_s=\max_{g\in [k]} \sth{\max\sth{{\sum_{h\in[k]\atop h\neq g} n_{gh}^{(s)}\over n_g^*},{\sum_{h\in[k]\atop h\neq g} n_{hg}^{(s)}\over n_g^{(s)}}}}
%		\leq nA_s\cdot \max_{g\in [k]}\sth{\max\sth{\frac 1{n_g^*},\frac 1{n_g^{(s)}}}}.
%	\end{align}
%	As $G_s\leq \frac 12$ for all $s\geq 3$, we get $n\alpha\leq n_g^*\leq 2n_{gg}^{(s)}\leq 2n_{g}^{(s)}$. Using this we have
%	\begin{align}\label{eq:km26}
%		n_{g}^*\geq n_{gg}^{(s)}\geq n_g^{(s)}-nA_s\geq n_g^{(s)}\pth{1-\frac 2\alpha A_s},
%		\quad n_{g}^{(s)}\geq n_{gg}^{(s)}\geq n_g^*-nA_s\geq n_g^*\pth{1-\frac 1\alpha A_s}.
%	\end{align}
%	Fix $g\in [k]$. Let $U_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^{(s)}$, $V_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^*\cap T_g^{(s)}$, and $W_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^*$. Then we get
%	\begin{align*}
%		U_j^{(\ceil{ {n_g^{(s)}/2}})}
%		&\stepa{\leq} V_j^{(\ceil{n_g^{(s)}/2}-n_g^{(s)}+n_{gg}^{(s)})}
%		\nonumber\\
%		&\stepb{\leq }
%		V_j^{(\floor{{n_g^{(s)}\over 2}-nA_s})}
%		\stepc{\leq} W_j^{(\floor{{n_g^{(s)}\over 2}-nA_s})}
%		\stepd{\leq} W_j^{(\floor{{n_g^{*}\over 2}-{3nA_s\over 2}})}
%		\stepe{\leq} W_j^{(\floor{{n_g^*}(\frac 12-\frac 1\alpha A_s)})},
%	\end{align*}
%	where
%	\begin{itemize}
%		\item (a) followed using \prettyref{lmm:ord-stat_after_addn} with
%		$
%		X=V_j,\ \tilde X=U_j,\ \ell=n_g^{(s)}-n_{gg}^{(s)},\ t=\ceil{n_g^{(s)}\over 2},
%		$
%		\item (b) followed using $n_g^{(s)}-n_{gg}^{(s)}\leq nA_s$ and $\ceil{x}-y\geq \floor{x-y}$ for $x,y\geq 0$
%		
%		\item (c) followed using \prettyref{lmm:ord-stat_after_addn} with 
%		$X=V_j,\ \tilde X=W_j,\ \ell=n_g^*-n_{gg}^{(s)},\ t=\floor{{n_g^{(s)}\over 2} -nA_s},$
%		
%		\item (d) followed using \eqref{eq:km26} and (e) followed using $n_g^*\geq n\alpha$.
%	\end{itemize}
%	Similarly we also have
%	\begin{align*}
%		U_j^{(\ceil{ {n_g^{(s)}/2}})}
%		&\stepa{\geq} V_j^{(\ceil{n_g^{(s)}/2})}
%		\nonumber\\
%		&\stepb{\geq} 
%		V_j^{(\ceil{{n_g^*\over 2}\cdot \frac 1{1-{2A_s/\alpha}}})}
%		\stepc{\geq} 
%		V_j^{(\ceil{{n_g^*}(\frac 12+\frac 2\alpha A_s)})}
%		\stepd{\geq} W_j^{(\ceil{{n_g^*}(\frac 12+\frac 2\alpha A_s)}+\sum_{h=[k]\atop h\neq k}n_{gh})}
%		\stepe{\geq} W_j^{(\ceil{{n_g^*}(\frac 12+\frac 3\alpha A_s)})}.
%	\end{align*}
%	\begin{itemize}
%		\item (a) followed using \prettyref{lmm:ord-stat_after_addn} with
%		$
%		X=V_j,\ \tilde X=U_j,\ \ell=n_g^{(s)}-n_{gg}^{(s)},\ t=\ceil{n_g^{(s)}\over 2},
%		$
%		
%		\item (b) followed using \eqref{eq:km26} and (c) followed using $(1-x)^{-1}\leq 1+2x$ for $x=\frac 2\alpha A_s\leq \frac 12$.
%		
%		\item (d) used \prettyref{lmm:ord-stat_after_addn} with 
%		$X=V_j,\ \tilde X=W_j,\ \ell=\sum_{h=[k]\atop h\neq k}n_{gh},\ t=\ceil{{n_g^*\over 2}(1+\frac 4\alpha A_s)}+\sum_{h=[k]\atop h\neq k}n_{gh},$
%		
%		
%		\item (e) used that for any $x>0$ and positive integer $y$, $\ceil{x}+y = \ceil{x+y}$, and $\sum_{h=[k]\atop h\neq k}n_{gh}\leq nA_s$.
%	\end{itemize}
%	Then \prettyref{thm:main} implies that given any $\tau>0$, there exists $C:=C(\tau)$ such that whenever $M\geq C(\tau)$, we have $\frac 6\alpha A_s\leq e^{-{\Delta^2\over (8+\tau)\sigma^2}}$. Using this we combine the last two displays to get
%	\begin{align}
%		W_j^{(\ceil{{n_g^*\pth{\frac 12+e^{-{\Delta^2\over (8+\tau)\sigma^2}}}}})}
%		\leq U_j^{(\floor{{n_g^{(s)}/2}})}\leq W_j^{(\floor{{n_g^*\pth{\frac 12-e^{-{\Delta^2\over (8+\tau)\sigma^2}}}}})}.
%	\end{align}
%	Then using the result \prettyref{lmm:order-concentration-smallx} on the concentration of the order statistics
%	we conclude our results.
%\end{proof}
%
%\nb{TBD: Add a remark about spectral initialization}
%
%\section{Optimality in the presence of outliers}
%
% Suppose that an adversary adds $n^{\out}$ many points to our existing data set. Our results for the adversarial addition regime is based on the cluster-wise correct classification proportion at step $s$, defined as
%\begin{align}
%	H_s=\min_{g\in [k]}\sth{\min\sth{{n_{gg}^{(s)}\over n_g^*},{n_{gg}^{(s)}\over n_{g}^{(s)}}}}.
%\end{align}
%\begin{theorem}
%	\label{thm:optim-outl}
%	 Suppose that $n\alpha\geq c\log n$ for some $c>0$. There exists absolute constants $c_1,c_2,c_3,c_4,c_5>0$ such that the followings are satisfied. For any $\eta\in(0,1]$, if the clustering initialization satisfies either one of the following conditions
%	$${H_0}\geq \frac 12+\frac {c_1}{\pth{{\Delta\over \sigma}\sqrt{\alpha\over d}}^2}\quad  \text{ or } \quad \Lambda_0\leq \frac 12-{c_2\over \pth{{\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}^{\frac 12(1-\eta)}},$$
%	then whenever $$M=\min \sth{{\Delta\over \sigma}\sqrt{\alpha\over d}, {\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}\geq c_3,$$ 
%	for any $n^{\out}\leq n\alpha(1-c_4M^{-2\eta})$ our algorithm guarantees $$A_s\leq \exp\sth{-\pth{1-{c_5\over \sqrt M}}{\Delta^2\over 8\sigma^2}+{\Delta\over \sigma}},
%	\quad s\geq 2
%	$$
%	with probability $1-4(k^2+k)n^{-(c/2-2)}-16dn^4e^{-0.3n}- 2k^2\exp\sth{-{\Delta\over 8\sigma}}.$
%\end{theorem}
%
%\begin{remark}
%    When we initialize with the constraint on $H_0$ we can allow $\eta=1$.\nb{Check proof}
%\end{remark}
%
%The proof of the above theorem hinges on the following lemma, similar to \prettyref{lmm:Gs-Ls-bound}.
%
%\begin{lemma}\label{eq:HsLs-bound}
%	Fix $\epsilon_0,\gamma_0\in (0,\frac 12]$ and suppose that an adversary added $n\beta$ many outliers with $\beta\leq\alpha(1-\delta)$ for some $\delta>0$. Let $r_k={\Delta\over\sigma}\sqrt{\alpha\over 1+{dk/n}}$. Then on the set $\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0} $ we have
%	\begin{enumerate}[label=(\roman*)]
%		\item If $\Lambda_s\leq \frac 12-\epsilon_0$ then $H_{s+1} \geq \frac 12 +\min\sth{{\delta-2\tau\over 2(2-\delta)},1-\tau}$ where $\tau={5\over 2\epsilon_0^4 r_k^2}
%		+{24\Lambda_s^2\over \epsilon_0^4r_k^2}$,
%		\item If $H_s\geq \frac 12+\gamma_0$ then $\Lambda_s\leq {12\sqrt 2\over \Delta/\sigma}\sqrt{d \over  {\gamma_0\alpha}}$.
%	\end{enumerate}
%\end{lemma}
%
%\begin{proof}
%	
%	The proof of part (i) borrows results from the proof of \prettyref{lmm:Gs-Ls-bound}(i). Notice that we can show for each $h\neq g$
%	\begin{align}
%		\label{eq:km22}
%		n_{gh}^{(s+1)}
%		&\leq 
%		\frac{5n_g^*\sigma^2}{4\epsilon_0^4\Delta^2}
%		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2}\pth{{n_g^*}+  d}.
%	\end{align}
%	Using the last display and noting that $k\leq \frac 1{\alpha}$ and $n_g^*\geq n\alpha$ we get
%	\begin{align}\label{eq:km23}
%		{\sum_{h\in[k]\atop h\neq g}n_{gh}^{(s+1)}\over n_g^*}
%		\leq \tau,\quad \tau=
%		\frac{5\sigma^2}{2\epsilon_0^4\Delta^2\alpha}
%		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2\alpha}\pth{1+ {dk\over n}}.
%	\end{align}
%	Using $n_g^{*}=\sum_{h\in [k]}n_{gh}^{(s+1)}$ for all $s\geq 0$, we get 
%	\begin{align}\label{eq:km24}
%		{n_{gg}^{(s+1)}\over n_g^*}\geq 1-\tau.
%	\end{align}	 
%	Next we switch $g,h$ in \eqref{eq:km22} and sum over $h\in [k], h\neq g$. We get
%	\begin{align}
%		\sum_{h\in[k]\atop h\neq g}n_{hg}^{(s+1)}
%		\leq \frac{5n\sigma^2}{2\epsilon_0^4\Delta^2}
%		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2}\pth{n+ kd}
%		\leq n\alpha\tau.
%	\end{align}
%	Using the above and noticing that in addition to the points in $\cup_{h\in[k]}\sth{T_{h}^*\cap T_g^{(s+1)}}$, $T_g^{(s+1)}$ can at most have $n\beta$ many extra points, accounting for the outliers, we get
%	\begin{align}
%		{n_{gg}^{(s+1)}\over n_g^{(s+1)}}\geq {n_{gg}^{(s+1)}\over n_{gg}^{(s+1)}+n\alpha\tau+n^{\out}}
%		\geq \frac 1{1+{n_g^*(1-\delta+\tau)\over n_{gg}^{(s+1)}}}
%		\geq \frac 1{1+{1-\delta+\tau\over 1-\tau}}
%		=\frac 12 + {\delta-2\tau\over 2(2-\delta)}.
%	\end{align}
%	Combining the last display with \eqref{eq:km24} we get
%	\begin{align*}
%		H_{s+1}=\min_{g\in [k]}\sth{\min\sth{{n_{gg}^{(s)}\over n_g^*},{n_{gg}^{(s)}\over n_{g}^{(s)}}}}
%		\geq \frac 12+\min\sth{{\delta-2\tau\over 2(2-\delta)},\frac 12-\tau},
%	\end{align*}
%	as required.
%	
%	The proof of (ii) follows a similar strategy as in the proof of \prettyref{lmm:Gs-Ls-bound}, part (ii). Define as before
%	\begin{align}
%		\begin{gathered}
%			\hat \theta_g^{(s)}=\med(T_g^{(s)}),\quad \tilde \theta_g^{(s)}=\med(T_g^{(s)}\cap T_g^*)\\
%			U_j=\text{the set of $j^{\rm{th}}$ coordinates of $T_g^{(s)}$},\quad
%			V_j=\text{the set of $j^{\rm{th}}$ coordinates of $T_g^{(s)}\cap T_g^*$}.
%		\end{gathered}
%	\end{align} 
%%	Then as we have
%%	\begin{align}
%%			n_{gg}^{(s)}\geq (\frac 12+\gamma_0)n_g^{(s)}\geq {n_g^{(s)}\over 2}+5,\quad
%%			n_{g}^{(s)}-n_{gg}^{(s)}\leq (\frac 12-\gamma_0)n_g^{(s)}\leq {n_g^{(s)}\over 2}-5
%%	\end{align}
%%	we can use \prettyref{lmm:ord-stat_after_addn} with
%%	$X=V_j,\tilde X=U_j,m=n_{gg}^{(s)},\ell=n_{g}^{(s)}-n_{gg}^{(s)},
%%	t=\ceil{n_g^{(s)}\over 2}$
%%	to get
%%	\begin{align}
%%		V_j^{(\ceil{ {n_g^{(s)}/2}})}
%%		\leq \med(U_j)
%%		\leq V_j^{(\floor{\gamma_0 n_{g}^{(s)}})}.
%%	\end{align}
%%	Using the definition of order statistics we also have
%%	\begin{align}
%%	V_j^{(\ceil{ {n_g^{(s)}/2}})}
%%	\leq V_j^{(\ceil{n_{gg}^{(s)}/2})}=\med(V_j)
%%	\leq  V_j^{(\floor{\gamma_0 n_{g}^{(s)}})}.
%%	\end{align}
%%	Combining the last two displays we get
%	Then using essentially the same strategy we show
%	\begin{align}\label{eq:km32}
%	\|\hat \theta_g^{(s)}-\tilde\theta_g^{(s)}\|_2^2\leq \sum_{j=1}^d\abs{\med(U_j)-\med(V_j)}^2
%	&\leq \abs{V_j^{(\floor{\gamma_0 n_g^{(s)}})}-V_j^{(\ceil{ {n_g^{(s)}/2}})}}.
%	\end{align}
%	Then as $H_s\geq \frac 12+\gamma_0$ guarantees ${1\over 1+2\gamma_0}n_{gg}^{(s)} \geq {n_g^{(s)}\over 2}\leq \gamma_0 n_g^{(s)}\geq \gamma_0 n_{gg}^{(s)}$, we get that
%	\begin{align}
%		\|\hat \theta_g^{(s)}-\tilde\theta_g^{(s)}\|_2^2
%		\leq \sum_{j=1}^d\abs{V_j^{(\floor{\gamma_0 n_{gg}^{(s)}})}-V_j^{(\ceil{{1\over 1+2\gamma_0}n_{gg}^{(s)}})}}^2
%	\end{align}
%	The rest of the proof then follows using the concentration bound of order statistics for the sets $V_1,\dots,V_d$ As these sets do not involve any outliers, our usual concentration bound for $\subG(\sigma^2)$, provided in \prettyref{lmm:order-concentration}, applies.
%	
%\end{proof}
%
%\begin{proof}[Proof of \prettyref{thm:optim-outl}]
%	Let $\beta=\alpha(1-\delta)$.  For $c_1,c_2$ to be chosen later, we define
%	$$\gamma_0=\frac {c_1}{\pth{{\Delta\over \sigma}\sqrt{\alpha\over d}}^2},\quad \epsilon_0={c_2\over \pth{{\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}^{\frac 12(1-\eta)}}.$$
%	Then from \prettyref{lmm:Gs-Ls-bound} it follows that, we can choose $c_1,c_2,c_3,c_4>0$ such that whenever $M>c_3$ and $\delta\geq c_4M^{-2\eta}$, on the set $\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0}$:
%	\begin{itemize}
%		\item if $\Lambda_0\leq \frac 12-\epsilon_0$ then $H_1\geq \frac 12 + {\delta\over 6}$.
%		\item if $H_0\geq \frac 12+\gamma_0$ then $\Lambda_0\leq 0  .3$,
%	\end{itemize}
%	A second application of \prettyref{lmm:Gs-Ls-bound} guarantees that we can choose $c_3$ large enough such that if  
%	$$M=\min \sth{{\Delta\over \sigma}\sqrt{\alpha\over d},{\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}\geq c_3$$
%	then on the set $\calE_{{2\gamma_1\over 1+2\gamma_1},\epsilon_1}\cap \calE_{\frac 14,\epsilon_1}$, with $\epsilon_1=\gamma_1=0.2$, if $H_{s}\geq \frac 12 +\frac \delta6$ then $\Lambda_s\leq {12\sqrt 2\over \sqrt{0.2}M} \leq 0.3$ and if $\Lambda_s\leq 0.3$ then $H_{s+1}\geq \frac 12 +\frac \delta6$.
%	Combining the above displays we get that on the set
%	\begin{align}
%		\label{eq:Prob-E2}
%		\calE&=\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0} \cap \calE_{{2\gamma_1\over 1+2\gamma_1},\epsilon_1}\cap \calE_{\frac 14,\epsilon_1}
%		\nonumber\\
%		\PP\qth{\calE}
%		&\geq 1-4(k^2+k)n^{-c/4}-16de^{-0.3n}
%	\end{align} 
%	we have
%	\begin{align}
%		\label{eq:km27}
%		\Lambda_s\leq 0.3,\quad H_{s+1}\geq \frac 12 +\frac \delta6 \text{ for all } s\ge 2.
%	\end{align}
%	We will show that $\PP\qth{\left.z_i\neq \hat z_i^{(s+1)}\right|\calE}$ is small for each $i\in [n]$. This will imply that on the set $\calE$, $A_{s+1}=\frac 1n\sum_{i=1}^n\indc{z_i\neq \hat z_i^{(s+1)}}$ is also small in probability. From this, using a Markov inequality we will conclude the result. The analysis is 
%	identical to that of the proof of \prettyref{thm:main} after \eqref{eq:km14} which relies solely on the fact that $\Lambda_s\leq 0.3$ for all $s\geq 3$. We omit it here.
%\end{proof}
%
%
%
%\subsection*{Adversarial data corruption}
%	
%	\begin{remark}
%		Mention that it is equivalent to adversarial data addition but the result changes a bit
%	\end{remark}
%
%\section{Centroid estimation in presence of outliers}
%For this section, let us define the ratio of total outliers with respect to individual clusters as
%\begin{align}
%    \beta_g^\out = {n^{\out}\over n_g^*},\quad g=1,2,\dots,k.
%\end{align}
%Note that in order to identify all the clusters accurately we require $\max_g\beta_g^\out<1$; otherwise, given any algorithm, an adversary can always create a constellation involving only the outliers that will force the algorithm to detect it as an individual cluster.
%
%\begin{theorem} 
%	Suppose that $n\alpha\geq c\log n$ for some $c>0$ and the constraints in \prettyref{thm:optim-outl} on $H_s,\Lambda_s$ are satisfied. Then given any $\tau >0$, there exists absolute constants $C:=C(\tau)>0$ such that whenever $M=\min \sth{{\Delta\over \sigma}\sqrt{\alpha\over d}, {\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}\geq C$, then
%	with probability at least $1-\frac 1n-4(k^2+k)n^{-(c/2-2)}-16dn^4e^{-0.3n}- 2k^2\exp\sth{-{\Delta\over 8\sigma}}$ we have
%	$$
%	\|\hat \theta_g^{(s)}-\theta_g\|^2\leq {d}
%	\qth{\max_{i:Y_i\in T_g^*}\max_{j\in [d]} \max\sth{\abs{F_{ij}^{-1}\pth{\frac 12 +x_0}},\abs{F_{ij}^{-1}\pth{\frac 12 -x_0}}}}^2,\quad s\geq 2,
%	$$
%	where 
%	$x_0= \sqrt{3\log n\over n_g^*}+e^{-{\Delta^2\over (8+\tau)\sigma^2}}+{\beta_g^\out\over 1+\beta_g^\out}$.
%\end{theorem}
%
%\begin{remark} \nb{EDIT THIS FOR NEW NOTATIONS}
%	In particular, if the errors of the $g$-th cluster are distributed as the multivariate Gaussian distribution with variance $\sigma^2$, then for any $\beta_g^{\out}\leq c \pth{\sqrt{3\log n\over n_g^*}+e^{-{\Delta^2\over (8+\tau)\sigma^2}}}$ the conditions in the above theorems are satisfied with $$x_0=C\sigma\pth{{\sqrt{\log n\over {n_g^*}}+e^{-{\Delta^2\over 24\sigma^2}}}}$$ for some large constant $C>0$. This implies that when $\Delta\gtrsim \sigma\log n$ we achieve the optimal rate of estimating the centroids.
%\end{remark}
%\begin{proof}
%	From the definition of $A_s$ we have
%	we get for any $g\in [k]$
%	\begin{align}\label{eq:29}
%		\max\sth{\sum_{h\in[k]\atop h\ne g}n_{hg}^{(s)},\sum_{h\in[k]\atop h\ne g}n_{gh}^{(s)}}
%		\leq \sum_{i=1}^n\indc{\hat z_i^{(s)}\neq z_i}
%		=nA_s, \quad s\geq 3.
%	\end{align}
%	Note that using $n\leq {n_g^*\over \alpha}$ and $n_{gg}^{(s)}\geq n_{g}^*-nA_s\geq n_g^*(1-A_s/\alpha)$, using the last display we can write
%	\begin{align*}
%		{n_{gg}^{(s)}\over n_g^{(s)}}\geq {n_{gg}^{(s)}\over n_{gg}^{(s)}+\sum_{h\in[k]\atop h\ne g}n_{hg}^{(s)}+n^{\out}}
%		\geq \frac 1{1+{n_g^*(\frac 1\alpha A_s+\beta_g^{\out})\over n_{gg}^{(s+1)}}}
%		\geq \frac 1{1+{\beta_g^{\out}+ A_s/\alpha\over 1-A_s/\alpha}}
%		=\frac 12 + {1-\beta_g^{\out}-\frac 2\alpha A_s\over 2(1+{\beta_g^{\out}})},
%	\end{align*}
%	which implies
%	\begin{align}\label{eq:km30}
%		\ceil{ {n_g^{(s)}/2}}-n_g^{(s)}+n_{gg}^{(s)}\geq n_{gg}^{(s)}-{n_g^{(s)}\over 2}
%		\geq \pth{1-\beta_g^{\out}-\frac 2\alpha A_s\over 1+\beta_g^{\out}}{n_g^{(s)}\over 2}
%		= \pth{\frac 12-{\beta_g^{\out}+A_s/\alpha \over 1+\beta_g^{\out}}}{n_g^{(s)}}
%	\end{align}
%	As $n_g^*\geq n\alpha$, the above implies for all $g\in [k]$
%	\begin{gather}
%			n_g^{(s)}\geq 	n_{gg}^{(s)}=n_g^*-\sum_{h\in[k]\atop h\ne g}n_{gh}^{(s)}
%			\geq n_g^*-nA_s \geq n_g^*\pth{1-\frac 1\alpha A_s}
%			\label{eq:km31}
%	\end{gather}
%	Fix $g\in [k]$. Let $U_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^{(s)}$, $V_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^*\cap T_g^{(s)}$, and $W_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^*$.Then we get
%	\begin{align*}
%		U_j^{(\ceil{ {n_g^{(s)}/2}})}
%		&\stepa{\leq} V_j^{(\ceil{n_g^{(s)}/2}-n_g^{(s)}+n_{gg}^{(s)})}
%		\nonumber\\
%		&\stepb{\leq }
%		V_j^{(\floor{\pth{1-\beta_g^{\out}-\frac 2\alpha A_s\over 1+\beta_g^{\out}}{n_g^{(s)}\over 2}})}
%		\nonumber\\
%		&\stepc{\leq} W_j^{(\floor{\pth{1-\beta_g^{\out}-\frac 2\alpha A_s\over 1+\beta_g^{\out}}{n_g^{(s)}\over 2}})}
%		\stepd{\leq} W_j^{(\floor{{n_g^{*}}\pth{\frac 12-{\beta_g^{\out}+A_s/\alpha \over 1+\beta_g^{\out}}}\pth{1-\frac 1\alpha A_s}})}
%		\leq W_j^{(\floor{{n_g^{*}}\pth{\frac 12-{\beta_g^{\out}\over 1+\beta_g^{\out}}-\frac 5{2\alpha}A_s}})},
%	\end{align*}
%	where
%	\begin{itemize}
%		\item (a) followed using \prettyref{lmm:ord-stat_after_addn} with
%		$
%		X=V_j,\ \tilde X=U_j,\ \ell=n_g^{(s)}-n_{gg}^{(s)},\ t=\ceil{n_g^{(s)}\over 2},
%		$
%		\item (b) followed using \eqref{eq:km32} \eqref{eq:km30} and $\ceil{x}-y\geq \floor{x-y}$ for $x,y\geq 0$
%		
%		\item (c) followed using \prettyref{lmm:ord-stat_after_addn} with 
%		$X=V_j,\ \tilde X=W_j,\ \ell=n_g^*-n_{gg}^{(s)},\ t=\floor{\pth{\frac 12-{\beta_g^{\out}+ A_s/\alpha\over 1+\beta_g^{\out}}}{n_g^{(s)}}},$
%		
%		\item (d) followed using \eqref{eq:km31}.
%	\end{itemize}
%	Similarly, we also have
%	\begin{align*}
%		U_j^{(\ceil{ {n_g^{(s)}/2}})}
%		&\stepa{\geq} V_j^{(\ceil{n_g^{(s)}/2})}
%		\nonumber\\
%		&\stepb{\geq} 
%		V_j^{(\ceil{{n_g^*\over 2}\cdot \frac 1{1-{2A_s/\alpha}}})}
%		\stepc{\geq} 
%		V_j^{(\ceil{{n_g^*}(\frac 12+\frac 2\alpha A_s)})}
%		\stepd{\geq} W_j^{(\ceil{{n_g^*}(\frac 12+\frac 2\alpha A_s)}+\sum_{h=[k]\atop h\neq k}n_{gh})}
%		\stepe{\geq} W_j^{(\ceil{{n_g^*}(\frac 12+\frac 3\alpha A_s)})}.
%	\end{align*}
%	\begin{itemize}
%		\item (a) followed using \prettyref{lmm:ord-stat_after_addn} with
%		$
%		X=V_j,\ \tilde X=U_j,\ \ell=n_g^{(s)}-n_{gg}^{(s)},\ t=\ceil{n_g^{(s)}\over 2},
%		$
%		
%		\item (b) followed using \eqref{eq:km31} and (c) followed using $(1-x)^{-1}\leq 1+2x$ for $x=\frac 2\alpha A_s\leq \frac 12$.
%		
%		\item (d) used \prettyref{lmm:ord-stat_after_addn} with 
%		$X=V_j,\ \tilde X=W_j,\ \ell=\sum_{h=[k]\atop h\neq k}n_{gh},\ t=\ceil{{n_g^*\over 2}(1+\frac 4\alpha A_s)}+\sum_{h=[k]\atop h\neq k}n_{gh},$
%		
%		
%		\item (e) used that for any $x>0$ and positive integer $y$, $\ceil{x}+y = \ceil{x+y}$, and $\sum_{h=[k]\atop h\neq k}n_{gh}\leq nA_s$.
%	\end{itemize}
%	Then \prettyref{thm:main} implies that given any $\tau>0$, there exists $C:=C(\tau)$ such that whenever $M\geq C(\tau)$, we have $\frac 6\alpha A_s\leq e^{-{\Delta^2\over (8+\tau)\sigma^2}}$. Using this we combine the last two displays to get
%	\begin{align}
%		W_j^{(\ceil{{n_g^*\pth{\frac 12+e^{-{\Delta^2\over (8+\tau)\sigma^2}}}}})}
%		\leq U_j^{(\floor{{n_g^{(s)}/2}})}\leq W_j^{(\floor{{n_g^*\pth{\frac 12-{\beta_g^{\out}\over 1+\beta_g^{\out}}-e^{-{\Delta^2\over (8+\tau)\sigma^2}}}}})}.
%	\end{align}
%	Then using the result \prettyref{lmm:order-concentration-smallx} on the concentration of the order statistics
%	we conclude our results.
%\end{proof}

==> tex/ordered-diff-moment.tex <==






\section{Notation} 
We will call a random vector $w\in \reals^d$ satisfies the spherical $p$th order tail bound with parameter $\sigma>0$ (here and below denoted by $w\in \calR_p(\sigma)$) if it has mean zero and
\begin{itemize}
	\item ${w\over \|w\|_2}$ is uniformly distributed on the unit sphere $\sfS^{d-1}$,
	\item There exists $x_0>0$ such that $\PP\qth{\|w\|_2>x}<{\sigma^p\over x^p}$ for all $x\geq x_0$.
\end{itemize}
For our paper we assume $p\geq 2$. We observe independent samples $Y_1,\dots,Y_n\in \reals^d$ from a mixture of $k$ many $\calR_p(\sigma)$ distributions
\begin{align}
	Y_i=\theta_{z_i}+w_i,\ i=1,\dots,n,\quad w_i\in \calR_p(\sigma),
\end{align}
where $ z=\sth{z_i}_{i=1}^n\in[k]^n$ denote the underlying labels, $\theta_1,\dots,\theta_k$ are the unknown centers of those $k$ distributions. Suppose that after $s$-steps the estimated centers are $\hat\theta^{(s)}_1,\dots,\hat\theta^{(s)}_k$ and the estimated labels are $\hat z^{(s)}=\sth{\hat z^{(s)}_1,\dots,\hat z^{(s)}_k}$. The initialization for the parameters correspond to $s=0$. 
We study the loss function
\begin{align}
	\ell(\hat z^{(s)},z) = \inf_{\pi\in \calS_k}\qth{\frac 1n \sum_{i=1}^n\indc{\pi(z^{(s)}_i)\neq z_i}},
\end{align}
where $\calS_k$ is the set of all permutations on $\{1,\dots,k\}$. Next we define notations for the different clusters in ground truth as well as during the iterations. For all $h,g\in [k]$, define
\begin{equation}\label{eq:cluster-def}
	\begin{gathered}
		T_h^*=\sth{Y_i:i\in [n],z_i=h},
		\hat T_h^{(s)}=\sth{Y_i:i\in [n],z_i^{(s-1)}=h}\\
		n^*_h = \abs{T^*_h}, n^{(s)}_h = \abs{T^{(s)}_h}, n^{(s)}_{hg} = \abs{T^*_h \cap T^{(s)}_g}
	\end{gathered}
\end{equation}
Note that for $s\geq 1$ this implies
\begin{align}
	T_h^{(s)}=\sth{Y_i:i\in[n], \|Y_i-\hat\theta_h^{(s-1)}\|\leq \|Y_i-\hat\theta_a^{(s-1)}\|,a\in[k]}.
\end{align}
with tie broken arbitrarily.

 Our clustering algorithm is the following.

\begin{algorithm}[H]
	\caption{The {\sf Clustering via Ordered Distances} (\cod) - algorithm}\label{algo:cod}
	{\bf Input}:  Data $Y_1,\dots,Y_n$. Initial centroid estimates $(\hat \theta_1^{(0)},\dots,\hat \theta_k^{(0)})$. Error threshold $\epsilon$. Truncation level $\delta\in (0,\frac 12)$. Here we choose $\delta=0.45$.\\
	{\bf Steps}: 
	\begin{algorithmic}[1]
		\While{$\frac 1k\sum_{h=1}^k \|\hat\theta_h^{(s)}-\hat\theta_h^{(s-1)}\|_2^2 > \epsilon$,}
		\For{$h\in \sth{1,2,\dots,k}$}
		\State \textbf{Labeling step}:
		$$T_h^{(s)}=\sth{i\in \sth{1,\dots,n}: \|Y_i-\hat\theta_h^{(s-1)}\|_2\leq \|Y_i-\hat\theta_a^{(s-1)}\|_2,a\in\{1,\dots,k\}, a\neq h}.$$
		\State \textbf{Estimation step:} 
		\For{$i\in T_h^{(s)}$}
			\State Compute 
			$
			E_i= \sth{\|Y_j-Y_i\|:j\in T_h^{(s)}, j\neq i}
			$
			\State Compute $R_i^{(\delta)}$ as the $\floor{(1-\delta)n_h^{(s)}}$-th largest number in $E_i$
			\State Compute $i^* = \argmin_{i\in T_h^{(s)}} R_i^{(\delta)}$
		\EndFor
		\State Compute $\floor{(1-\delta)n_h^{(s)}}$-sized subset $V\subseteq T_h^{(s)}$, tie broken arbitrarily
		$$V=\sth{j\in T_h^{(s)}: \|Y_j-Y_{i^*}\|\leq R_{i^*}^{(\delta)},j\neq i_*}$$ 
		\State Update the new centroid as $\hat\theta_h^{(s)}= \frac {Y_{i^*}+\sum_{j\in V} Y_j}{\floor{(1-\delta)n_h^{(s)}}+1}$.
		\EndFor
		\State $s=s+1$
		\EndWhile
	\end{algorithmic}
	{\bf Output}: $(\hat \theta_1^{(s)},\dots,\hat \theta_k^{(s)})$ and label estimate for $Y_i$ given by $\hat z_i^{(s)} = \argmin_{h\in\{1,\dots,k\}}\|Y_i-\hat\theta_h^{(s)}\|_2,$ with tie broken arbitrarily.
\end{algorithm}


%\begin{algorithm}[H]
%	\caption{The $\lss$ clustering algorithm}\label{algo:lloyd-rob}
%	{\bf Input}:  Data $Y_1,\dots,Y_n$. Initial centroid estimates $(\hat \theta_1^{(0)},\dots,\hat \theta_k^{(0)})$. Error threshold $\epsilon$. Truncation level $\delta\in (0,\frac 12)$. Here we choose $\delta=0.49$.\\
%	{\bf Steps}: 
%	\begin{algorithmic}[1]
%		\While{$\frac 1k\sum_{h=1}^k \|\hat\theta_h^{(s)}-\hat\theta_h^{(s-1)}\|_2^2 > \epsilon$,}
%		\For{$h\in \sth{1,2,\dots,k}}$
%		\State \textbf{Labeling step}:
%		$$T_h^{(s)}=\sth{Y_i:i\in \sth{1,\dots,n}, \|Y_i-\hat\theta_h^{(s-1)}\|_2\leq \|Y_i-\hat\theta_a^{(s-1)}\|_2,a\in\{1,\dots,k\}, a\neq h}.$$
%		\State \textbf{Estimation step:} 
%		\begin{enumerate}[label=\alph*)]
%			\item Compute the subset $V$ using
%			$$
%			V=\argmin_{S\subseteq T_h^{(s)},|S|=(1-\delta)n_h^{(s)}}
%			\sum_{i:Y_i\in S} \left\|Y_i - \frac 1{(1-\delta)n_h^{(s)}}\sum_{i:Y_i\in S} Y_i\right\|_2^2,
%			$$
%			with tie broken arbitrarily.
%			\item $\hat\theta_h^{(s)}= \frac 1{(1-\delta)n_h^{(s)}}\sum_{i:Y_i\in V} Y_i$.
%		\end{enumerate}
%%		\begin{enumerate}
%%			\item Define $T_{\epsilon} = \epsilon^{-\frac 1p}e^{-{C_2\over \epsilon p\alpha}}$, with $\epsilon = 0.3$
%%			\item Compute 
%%			$$
%%			\hat \theta_h^{(s)} = \argmin_{\theta\in \reals^d} \sum_{i:Y_i\in T_h^{(s)}} \ell_{T_{\epsilon}}(\|X_i-\theta\|_2),\quad h\in \sth{1,\dots,k},$$
%%			where 
%%			$
%%			\ell_\tau(x) = x^2\indc{x\leq \tau}+\tau^2\indc{x>\tau}.
%%			$
%%		\end{enumerate}
%		\EndFor
%		\State $s=s+1$
%		\EndWhile
%	\end{algorithmic}
%	{\bf Output}: $(\hat \theta_1^{(s)},\dots,\hat \theta_k^{(s)})$ and label estimate for $Y_i$ given by $\hat z_i^{(s)} = \argmin_{h\in\{1,\dots,k\}}\|Y_i-\hat\theta_h^{(s)}\|_2,$ with tie broken arbitrarily.
%\end{algorithm}

\section{Results}

Denote the minimum separation between the centers by $\Delta$
\begin{align}
	\Delta=\min_{g,h\in[k],g\neq h}\|\theta_g-\theta_h\|_2.
\end{align}
We denote the signal to noise ratio as
\begin{align}
\snr = {\Delta\over 2\sigma}.
\end{align}
Let $\Lambda_s$ denote the error rate of estimating the centers at iteration $s$
\begin{align}
	\Lambda_s = \max_{h\in[k]}\frac 1{\Delta} \|\hat \theta_h^{(s)}-\theta_h\|_2.
\end{align}
Let us define the minimum fraction of points in the data set that come from a single component in the Gaussian mixture as
\begin{align}
	\alpha=\min_{g\in[k]} {n_{g}^*\over n}.
\end{align}
Define the cluster-wise mis-clustering rate as
\begin{align}\label{eq:mislabel}
	G_s=\max_{g\in [k]} \sth{\max\sth{{\sum_{h\in[k]\atop h\neq g} n_{gh}^{(s)}\over n_g^*},{\sum_{h\in[k]\atop h\neq g} n_{hg}^{(s)}\over n_g^{(s)}}}}
\end{align}
Our main result is the following.
\begin{theorem}
	\label{thm:main}
	Suppose that $n\alpha\geq c\log n$ for some $c>0$ and $\gamma\in (\frac 1{n\alpha},\frac 12)$. Then there exists absolute constants $c_1,c_2>0$ such that the followings are satisfied. If the clustering initialization satisfies  
	$$H_0\geq \frac 12+\gamma\quad \text{or}\quad \Lambda_0\leq \frac 12-{e^{25/(4p\alpha)}\over (\snr)^{1/2}},$$
	then whenever $\snr\geq c_1(0.3)^{-\frac 1p}e^{\frac {10(1+20/7\alpha)}{3p}}$ 
	we have that the \cod algorithm with $\delta=\frac 12-\frac \gamma4$ achieves the expected mislabeling rate $$\EE\qth{\ell(\hat z^{(s)},z)}\leq 2k^2{\pth{1-{c_2\over \snr}}^{-p}\over (\snr)^p}
	+ 4kn^{-c/4}+16e^{-0.3n},
		\quad s\geq 2.
		$$
\end{theorem}

\section{Proof strategy}

The proof on the $\cod$ algorithm is primarily based in the following two stages: 
\begin{enumerate}[label=(\alph*)]
	\item analyzing accuracy of the clustering method based on current center estimates,
	\item analysis of the next center updates based on current labels.
\end{enumerate} 
We obtain results on these steps separately and then combine them to prove \prettyref{thm:main}. Our analysis depends on high-probability events of the following type.

\begin{lemma}\label{lmm:norm-concentration}
	Suppose that $w_i$-s are independent random variables from $ \calR_p(\sigma)$. Then there is an event $\enorm$ with probability at least $1-e^{-0.3n}$ on which the following happens. For any $\tau>0$ and any $S\subseteq [n]$ with $|S|\geq {n\beta}$, the cardinality of the set $\sth{i\in S: \norm{w_i}\leq {\sigma}\tau^{-\frac 1p}e^{\frac 1{\tau p}(1+\frac 1\beta)}}$ is at least $(1-\tau)|S|$.
\end{lemma}

\begin{lemma}
	\label{lmm:Chernoff-binom}
	Fix $\epsilon_0 > 0$ and let $n\alpha\geq c\log n$. Then there is an event $\econ$ with probability at least $1-kn^{-c/4}$ on which 
	$$\sum_{i:Y_i\in T_g^*}\indc{\epsilon^2\Delta\leq \|w_i\|}
	\leq \frac {5n_g^*}{4 p \log(\epsilon_0^2\Delta/\sigma)}, \quad g\in [k].$$
\end{lemma}



The following lemma provides results that show upper bound on $G_{s+1}$ based on $\Lambda_s$ and establish upper bound on $\Lambda_{s}$ in terms of $G_s$. 

\begin{lemma}\label{lmm:Gs-Ls-bound}
	Fix $\epsilon_0\in (0,\frac 12),\gamma_0\in (\frac {10}{n\alpha},\frac 12)$. Then on the event $\calE_{\gamma_0,\epsilon_0}$, which has probability at least $1-n^{-c/2}-ke^{-0.3n}$, we have for all $s\geq 0$, the \cod algorithm with $\delta=\frac 12 - {\gamma_0\over 4}$ ensures:
	\begin{enumerate}[label=(\roman*)]
		\item if $\Lambda_s\leq \frac 12-\epsilon_0$ then $H_{s+1} \geq 1- \frac {5}{2p \alpha\log(\epsilon_0^2\Delta/\sigma)}$,
		\item if $H_{s+1}\geq \frac 12 + \gamma_0$ then $\Lambda_{s+1}\leq {8\sigma\over \Delta}\tau^{-\frac 1p}e^{\frac 1{\tau p}(1+\frac 1\beta)}$, where $\tau = {\gamma_0\over 1+2\gamma_0},\beta=(\frac 12+\gamma_0)\alpha$.
	\end{enumerate}
\end{lemma}

\begin{proof}[Proof of \prettyref{lmm:Gs-Ls-bound}]
	The proof of \prettyref{lmm:Gs-Ls-bound}(i) has been presented in \prettyref{app:Gs-Ls-i}. We present below the proof of \prettyref{lmm:Gs-Ls-bound}(ii). 
\end{proof}

%\begin{proof}[Proof of \prettyref{lmm:Gs-Ls-bound}]
%	The proof of \prettyref{lmm:Gs-Ls-bound}(i) has been presented in \prettyref{app:Gs-Ls-i}. We present below the proof of \prettyref{lmm:Gs-Ls-bound}(ii). We prove this using contradiction. For simplicity of notation we denote 
%	$$D={\sigma\over \Delta}(0.2)^{-\frac 1p}e^{\frac {10(1+\frac 5{4\alpha})}{3p}}.$$ 
%	Let us assume $\Lambda_{s+1} > {8D\over \Delta}$. This implies that there exists a cluster $h$ such that the centroid estimation error satisfies 
%	$$\|\hat \theta_h^{(s+1)}-\theta_h\|> {8D}.$$ 
%	As $H_{s+1}\geq 0.7$ we know that $n_{hh}^{(s+1)}\geq 0.7 n_h^{(s+1)}$. As we are on the set $\calE_{\epsilon_0}$, we use \prettyref{lmm:E-prob} with 
%	$$
%	 \tau =0.2,\quad S=\{i\in [n]:Y_i\in T_{h}^{(s+1)}\cap T_{h}^*\}, \quad \beta = {0.8 \alpha} < {n_{hh}^{(s+1)}\over n}.
%	$$ 
%	This gives us that there are at least $0.8n_{hh}^{(s+1)}(=0.56 n_h^{(s+1)})$ many points within a radius $D$ of $\theta_h$. Denote the set of these $0.56 n_h^{(s+1)}$ points by $W$
%	$$
%	W = \sth{j\in T_h^{(s+1)}: \|Y_j-\theta_h\|\leq D}. 
%	$$
%	Then given any $j_0\in W$, all the points in $\sth{Y_j:j\in W}$ are within $2D$ distance of $Y_{j_0}$. Hence, there are $0.56 n_h^{(s)}$ points within a radius $2D$ of $Y_{j_0}$. This also implies that $R_{i^*}^{(\delta)}\leq 2D$. We also get
%	$$
%	\|\hat \theta_h^{(s+1)}-Y_{j_0}\|\geq \|\hat \theta_h^{(s+1)}-\theta_h\|-\|Y_{j_0}-\theta_h\|\geq 7D.
%	$$
%	Note that our strategy guarantees that there are at least $0.55 n_h^{(s+1)}$ points within a radius $4D$ of the estimator $\hat \theta_h^{(s+1)}$: for the set $V$ in \prettyref{algo:cod}
%	\begin{align}
%	\|\hat\theta_h^{(s+1)}-Y_j\|
%	\leq \|\hat\theta_h^{(s)}-Y_{i^*}\|+\|Y_j-Y_{i^*}\|
%	\leq \frac {\sum_{j\in V}\| Y_j -Y_{i^*}\|}{\floor{(1-\delta)n_h^{(s+1)}}+1}
%	+R_{i^*}^{(\delta)}
%	\leq 2R_{i^*}^{(\delta)}
%	\leq 4D,\quad j\in V.
%	\end{align}
%\end{proof}

\begin{proposition}
	Suppose that given any $\tau,\beta\in (0,1)$, there is a event $\calF_{\tau}$ and a number $D_{\tau,\beta}>0$ such that, on $\calF_{\tau}$, for any $S\subseteq [n]$ with $|S|>\beta n$, the cardinality of the set 
	$\sth{i\in S: \norm{w_i}\leq D_{\tau,\beta}}$ is at least $(1-\tau)|S|$. Then for any $\gamma\in (10/{n\alpha},1/2)$, using $\tau={\gamma\over 1+2\gamma},\beta={\pth{\frac 12+\gamma} \alpha}$, we get that on the event $\calF_\tau$, if $H_{s}\geq \frac 12+\gamma$, then the \cod algorithm with any $\delta\geq\frac 12 -{\gamma\over 4}$ returns $\Lambda_{s}\leq {8D_{\tau,\beta}/\Delta}$.
\end{proposition}
\begin{proof}
	 We prove this using contradiction. Fix $\tau={\gamma\over 1+2\gamma},\beta={\pth{\frac 12+\gamma} \alpha}$ as specified. Our entire analysis will be on the event $\calF_\tau$. Let us assume $\Lambda_{s} > {8D_{\tau,\beta}/\Delta}$. This implies that there exists a cluster $h$ such that the centroid estimation error satisfies 
	$$\|\hat \theta_h^{(s)}-\theta_h\|> {8D_{\tau,\beta}}.$$ As $H_{s}\geq \frac 12+\gamma$, we know that $n_{hh}^{(s)}\geq \pth{\frac 12+\gamma} n_h^{(s)}$. As we are on the set $\calF_{\tau}$, we have
	$$
	S=T_{h}^{(s)}\cap T_{h}^*, \quad |S|=n_{hh}^{(s)} \geq {\pth{\frac 12+\gamma}n \alpha}.
	$$ 
	This gives us that there are at least $\pth{1-{\gamma\over 1+2\gamma}}n_{hh}^{(s)}(\geq\pth{\frac 12+{\gamma\over 2}} n_h^{(s)})$ many points in the cluster $T_h^{(s)}$ within a radius $D_{\tau,\beta}$ of $\theta_h$. Denote this set of points by $W$
	$$
	W = \sth{j\in T_h^{(s)}: \|Y_j-\theta_h\|\leq D_{\tau,\beta}}. 
	$$
	Then given any $j_0\in W$, all the points in $\sth{Y_j:j\in W}$ are within $2D_{\tau,\beta}$ distance of $Y_{j_0}$. This implies in the $\cod$ algorithm with $\delta=\frac 12 - {\gamma\over 4}$, we have $R_{i^*}^{(\delta)}\leq 2D_{\tau,\beta}$. 
	Note that our strategy guarantees that there are at least $(1-\delta)n_h^{(s)}=\pth{\frac 12 + {\gamma\over 4}}n_h^{(s)}$ points within a radius $4D_{\tau,\beta}$ of the estimator $\hat \theta_h^{(s)}$: for the set $V$ in \prettyref{algo:cod}
	\begin{align*}
		\|\hat\theta_h^{(s)}-Y_j\|
		\leq \|\hat\theta_h^{(s)}-Y_{i^*}\|+\|Y_j-Y_{i^*}\|
		\leq \frac {\sum_{j\in V}\| Y_j -Y_{i^*}\|}{\floor{(1-\delta)n_h^{(s)}}+1}
		+R_{i^*}^{(\delta)}
		\leq 2R_{i^*}^{(\delta)}
		\leq 4D_{\tau,\beta},\quad j\in V.
	\end{align*}
	Note that we also have
	$$
	\|\hat \theta_h^{(s)}-Y_{j_0}\|\geq \|\hat \theta_h^{(s)}-\theta_h\|-\|Y_{j_0}-\theta_h\|\geq 7D_{\tau,\beta}.
	$$
	Summarizing, we get
	\begin{itemize}
		\item there are at least $\pth{\frac 12+{\gamma\over 2}} n_h^{(s)}$ many points within a $2D_{\tau,\beta}$ radius of $Y_{j_0}$,
		\item there are at least $\pth{\frac 12+{\gamma\over 4}} n_h^{(s)}$ many points within a $4D_{\tau,\beta}$ radius of $\hat\theta_h^{(s)}$, and
		\item the distance between $\hat\theta_h^{(s)}$ and $Y_{j_0}$ is $7D_{\tau,\beta}$.
	\end{itemize}
	This leads to a contradiction.
\end{proof}

\section{Proof of \prettyref{thm:main}}

The mis-clustering rate at step $s$ is given by 
\begin{align}
	A_s=\frac 1n \sum_{i=1}^n\indc{z^{(s)}_i\neq z_i}
	=\frac 1n \sum_{h\neq g \in [k]} n_{hg}^{(s)}.
\end{align} 
For $c_1$ to be chosen later, we define
$$\epsilon_0={c_2\over (\Delta/2\sigma)^{1/2}}.$$
Then from \prettyref{lmm:Gs-Ls-bound} it follows that we can choose $c_1,c_2>0$ such that on the set $\calE_{\epsilon_0}$ we have that if $\Lambda_0\leq \frac 12-\epsilon_0$ then $G_1\leq 0.2$.
A second application of \prettyref{lmm:Gs-Ls-bound} guarantees that we can choose $c_3$ large enough such that if  
$${\Delta\over \sigma}(0.3)^{\frac 1p}e^{-\frac {10(1+\frac 5{4\alpha})}{3p}}\geq M\geq c_3$$
then on the set $\calE_{0.2}$ we have,
\begin{enumerate}[label=(P\arabic*)]
	\item \label{eq:P1} $G_s\leq \frac {5}{2p \alpha\log(\epsilon_0^2\Delta/\sigma)}\leq 0.2$ for all $s\geq 1$
	\item $\Lambda_s\leq {8\sigma\over \Delta}(0.3)^{-\frac 1p}e^{\frac {10(1+\frac 5{4\alpha})}{3p}}\leq {C_1\over M} \leq 0.2$ for all $s\geq 1$.
\end{enumerate}
Combining the above displays we get that on the set
\begin{align}
	\label{eq:Prob-E-new}
	\calE&=\calE_{\epsilon_0}\cap \calE_{0.2}\text{ with }
	\PP\qth{\calE}
	\geq 1-4kn^{-c/4}-e^{-0.3n}
\end{align} 
we have
\begin{align}
	\label{eq:km14}
	\Lambda_s\leq 0.2,G_{s}\leq 0.2 \text{ for all } s\ge 1.
\end{align}
We will show that $\PP\qth{\left.z_i\neq \hat z_i^{(s+1)}\right|\calE}$ is small for each $i\in [n]$.
Note that $$\indc{z_i\neq\hat z_i^{(s+1)}}
=\frac 12\sum_{g,h\in [k]\atop g\neq} \indc{\hat z_i^{(s+1)}=h,z_i=g}.$$ Fix a choice for $z_i$, say equal to $g\in [k]$. Then 
For any $h\in[k],h\neq g$,
\begin{align}\label{eq:km21}
	\indc{z_i=g,\hat z_i^{(s+1)}=h}
	&\leq \indc{\|Y_i-\hat\theta_h^{(s)}\|^2
		\leq \|Y_i-\hat\theta_g^{(s)}\|^2, Y_i\in T_g^*}
	\nonumber\\
	&=\indc{\|\theta_g+w_i-\hat\theta_h^{(s)}\|^2
		\leq \|\theta_g+w_i-\hat\theta_g^{(s)}\|^2}
	=\indc{\|\theta_g-\hat\theta_h^{(s)}\|^2-\|\theta_g-\hat\theta_g^{(s)}\|^2\leq 2\langle w_i,\hat\theta_h^{(s)}-\hat\theta_g^{(s)}\rangle}.
\end{align}
Triangle inequality implies
\begin{align}
	\|\theta_g-\hat\theta_h^{(s)}\|^2\geq \pth{\|\theta_g-\theta_h\|-\|\theta_h-\hat\theta_h^{(s)}\|}^2
	\geq (1-\Lambda_s)^2\|\theta_g-\theta_h\|^2.
\end{align}
Using $$\|\theta_g-\hat\theta_g^{(s)}\|\leq \Lambda_s\Delta
\leq \Lambda_s\|\theta_g-\theta_h\|$$
and the fact that $(1-x)^2-y^2\geq (1-x-y)^2$ when $y(1-x-y)\geq 0$, we obtain
\begin{align}
	&\|\theta_g-\hat\theta_h^{(s)}\|^2-\|\theta_g-\hat\theta_g^{(s)}\|^2
	\geq (1-\Lambda_s)^2\|\theta_g-\theta_h\|^2
	-\Lambda_s^2\|\theta_g-\theta_h\|^2
	\geq (1-2\Lambda_s)^2\|\theta_g-\theta_h\|^2.
\end{align}
In view of \eqref{eq:km21} the last display implies
\begin{align}
	\label{eq:km10}
	\indc{z_i=g,\hat z_i^{(s+1)}=h}
	\leq \indc{(1-2\Lambda_s)^2\|\theta_g-\theta_h\|^2\leq 2\langle w_i,\hat\theta^{(s)}_h-\hat\theta^{(s)}_g \rangle}.
\end{align}
Using Property \ref{eq:P1} and 
\begin{align*}
	|\langle w_i,\hat\theta^{(s)}_h-\hat\theta^{(s)}_g\rangle|
	&\leq \|w_i\|\cdot \|\hat\theta^{(s)}_h-\hat\theta^{(s)}_g\|
	\nonumber\\
	&\leq \|w_i\|\cdot(\|\hat\theta^{(s)}_h-\theta_h\|+\|\hat\theta^{(s)}_h-\theta_h\|+\|\theta_g-\theta_h\|)
	\leq \|w_i\|(2\Lambda_s\Delta+\Delta)
	\leq 2\|w_i\|\Delta,
\end{align*}
we get that
\begin{align*}
	\indc{z_i=g,\hat z_i^{(s+1)}=h}
	\leq \indc{(1-2\Lambda_s)^2\Delta\leq 2\|w_i\|}
	\leq \indc{\frac 12\pth{1-{2C_1\over M}}\Delta\leq \|w_i\|}.
\end{align*}
Taking expectation conditioned on $\calE$ we get
	\begin{align}
		\PP\qth{\left.z_i\neq \hat z_i^{(s+1)}\right|\calE}
		&\leq
		k^2 \max_{g,h\in [k]\atop g\neq h}\PP\qth{\left.z_i=g, \hat z_i^{(s+1)}=h \right|\calE}
		\leq 2k^2{\pth{1-{2C_1\over M}}^{-p}\over (\Delta/2\sigma)^p}
	\end{align}
	This implies
	\begin{align}
		\EE\qth{A_{s+1}|\calE}
		=\frac 1n\sum_{i=1}^n\PP\qth{\left.z_i\neq z_i^{(s+1)}\right| \calE}\leq 2k^2{\pth{1-{2C_1\over M}}^{-p}\over (\Delta/2\sigma)^p}.
	\end{align}
Combining the above with \eqref{eq:Prob-E-new} we get
\begin{align}
	\EE\qth{A_s}&\leq4 kn^{-c/4}+16e^{-0.3n}+2k^2{\pth{1-{2C_1\over M}}^{-p}\over (\Delta/2\sigma)^p}.
\end{align}

\section{Lower bound}
\begin{theorem}
	 For an absolute constant $C>0$ such that the following holds true. If the error distributions are chosen from $\calR_p(\sigma)$, then
	 $$\inf_{\hat z}\sup\EE_{z\in[k]^n}\qth{\ell(\hat z,z)}
	\geq {C\alpha\over k^2p }\cdot{1\over (\snr)^{p}(\log (\snr))^{1.5}}.$$
\end{theorem}
\begin{proof}
	We follow the proof technique of \cite[Theorem 3.3]{lu2016statistical}. For any $z\in [k]^n$, let us define $n_u(z)=\sum_{i=1}^n \indc{z_i=u}$. Let $z^*\in [k]^n$ satisfying $n_1(z^*)\leq n_2(z^*)\leq\dots\leq n_k(z^*)$, with $n_1(z^*)=n_2(z^*)=\floor{\alpha n}$. It is easy to check the existence of $z^*$. For each $u\in [k]$ we choose a subset of $\{i\in [n]: z^*(i)=u\}$ with cardinality $\ceil{n_u(z^*)-{\alpha n\over 4k}},$ denoted by $T_u$. Define $T=\cup_{u=1}^k T_u$ and
	$\calZ^* = \sth{z\in \calZ,z_i=z_i^* \text{ for all } i\in T}$. 
	A key observation is that for any $z\neq \tilde z\in\calZ^*$, we have $\frac 1n\sum_{i=1}^n\indc{z_i\neq \tilde z_i}\leq \frac kn\cdot \frac {\alpha n}{4k}=\frac \alpha 4$, and 
	$$
	\frac 1n\sum_{i=1}^n\indc{\pi(z_i)\neq \tilde z_i}\geq \frac 1n(\alpha n-{\alpha n\over 4k})\geq {\alpha\over 2}
	$$
	for all $\pi\in \calS_k$ which is not the identity permutation. Thus, $\ell(\tilde z,z)=\frac 1n\sum_{i=1}^n \indc{z_i\neq \tilde z_i}$ for all $z,\tilde z\in \calZ^*$. Then following the same arguments in the proof of \cite[Theorem 2]{gao2018community}, we can obtain
	\begin{align}\label{eq:gao2018}
	\inf_{\hat z}\sup_{z\in \calZ} \EE\qth{\ell(\hat z,z)}
	\geq {\alpha\over 6}
	\frac 1{T^c}\sum_{i\in T^c}\qth{\frac 1{2k^2}\inf_{\hat z_i}(\PP_1\qth{\hat z_i=2}+\PP_2\qth{\hat z_i=1})}.
	\end{align}
	Here $\PP_t,t\in \{1,2\}$ denote the probability distribution of our data given $z_i=t$. By Neyman-Pearson Lemma, the infimum of the right hand side of the last display is achieved by the likelihood ratio test 
	$$
	\hat z_i = \argmin_{g\in \{1,2\}}\|Y_i-\theta_g\|^2.
	$$
	Thus,
	$$
	\inf_{\hat z_i}\pth{\frac 12 \PP_1\qth{\qth{\hat z_i=2}+\frac 12\PP_2\qth{\hat z_i=1}}}
	=\PP\qth{\|\theta_1+w_i-\theta_2\|^2\leq \|w_i\|^2}
	=\PP\qth{\|\theta_1-\theta_2\|^2\leq 2\langle w_i,\theta_1-\theta_2\rangle}.
	$$
	 Note that as $|\langle w_i,\theta_1-\theta_2\rangle|\leq \|w_i\|\cdot\|\theta_1-\theta_2\|$, from the last display we get
	\begin{align}
		\label{eq:lb1}
	\inf_{\hat z_i}\pth{\frac 12 \PP_1\qth{\qth{\hat z_i=2}+\frac 12\PP_2\qth{\hat z_i=1}}}
	\geq \PP\qth{\|w_i\|\geq \frac 12\|\theta_1-\theta_2\|}
	\geq \PP\qth{\|w_i\|\geq \Delta/2}.
	\end{align}
	Next we choose all the errors to have the distribution
	\begin{align*}
	\begin{gathered}
		\{w_i\}_{i=1}^n\simiid R\cdot \Unif(\calS_{d-1}),\\ R = \sigma\pth{\xi\over pa\log a}^{\frac 1p}\tilde R,
	\ \PP\qth{\tilde R\geq r}=\frac {a(\log a)^{1+\xi}\indc{r\geq 0}}{(1+r^{p-1})(a+r)(\log(a+r))^{1+\xi}},\ a>1,\xi>0.
	\end{gathered}
	\end{align*}
	where $R$ is the radial distribution and $\Unif(\calS_{d-1})$ is the uniform distribution over the unit sphere, and they are independent.
	The $p$-th moment of $R$ is bounded from above by $\sigma^p$ follows from the fact that the $p$-th moment of $\tilde R$ is bounded from above as
	$$
	\EE\qth{\tilde R^{p}}
	=p\int_{0}^\infty  r^{p-1} \PP\qth{\tilde R > r} dr
	\leq \frac {pa\log a}\xi.
	$$
	This implies, with $a=2,\xi=\frac 12$, for an absolute constant $C>0$
	$$
	\PP\qth{\|w_i\|\geq \Delta/2}
	=\PP\qth{\tilde R\geq \frac{\Delta}{2\sigma}\pth{\xi\over pa\log a}^{-\frac 1p}}
	\geq C {1\over p(\Delta/2\sigma)^{p}(\log (\Delta/2\sigma))^{1.5}},
	$$
	where we used $\abs{\log\pth{\pth{\xi\over pa\log a}^{-1/p}}}\leq c$ for a small constant $c>0$. Thus using \eqref{eq:gao2018} and \eqref{eq:lb1} we conclude the result.
\end{proof}

\section{Minimax optimality with Sub-Gaussian mixtures}
In this section we prove that our algorithm achieves the optimal misclustering rate when the errors are generated from Sub-Gaussian mixture. In our model, the observed data $Y_1,\dots,Y_n\in \reals^d$ are distributed as
\begin{align}
	Y_i=\theta_{z_i}+w_i,\ i=1,\dots,n,
\end{align}
where $\sth{z_i}_{i=1}^n\in[k]^n$ denote the underlying unknown component labels of the points, and $w_i$-s denote the error variables. We assume that $w_i$-s are independent 0 mean Sub-Gaussian vectors with parameter $\sigma>0$, i.e.,
\begin{align}\label{eq:subg-defn}
	\EE\qth{e^{\langle a,w_i \rangle}}
	\leq e^{\sigma^2\|a\|^2\over 2}, \text{ for all $i\in \sth{1,\dots,n}$ and $a\in \reals^d$}.
\end{align}
We show the following.
Define the cluster-wise correct classification proportion at step $s$ as
\begin{align}
	H_s=\min_{g\in [k]}\sth{\min\sth{{n_{gg}^{(s)}\over n_g^*},{n_{gg}^{(s)}\over n_{g}^{(s)}}}}.
\end{align}
Our result is the following.
\begin{theorem}
	\label{thm:main-subg}
	There exists absolute constants $c_0,c_1,c_2,c_3,c_4>0$ such that the followings are satisfied.
	\begin{enumerate}[label=(\alph*)]
		\item \textbf{$\snr< c_0\sqrt {d/\alpha}$:} Assume $n\alpha^2\geq Ck\log n$ and ${\snr}\sqrt{\alpha\over 1+{dk\over n}}\geq C\sqrt k$ for a sufficiently large constant $C$. If the clustering initialization satisfies either one of the following conditions
		$${H_0}\geq 1-\frac 2{\sigma\sqrt d}\pth{\frac 12 - \frac {c_1/{\alpha}^{1/4}}{\pth{\snr}^{1/2}}}\quad  \text{ or } \quad \Lambda_0\leq \frac 12-{c_2/{\alpha}^{1/4}\over \pth{\snr}^{1/2}}.$$
		Then whenever $\snr\sqrt \alpha \geq M\geq c_3$,  we have $$\EE\qth{\ell(\hat z^{(s)},z)}\leq \exp\sth{-\frac 12\pth{1-{c_4\over \sqrt \snr}}(\snr)^2},
		\quad s\geq 3\log n.
		$$
		
		\item \textbf{$\snr\geq c_0\sqrt {d/\alpha}$:} Suppose the clustering initialization satisfies either one of the following conditions
		$${H_0}\geq \frac 12 +\gamma_0 \text{ with } \gamma_0>2.1\alpha \quad  \text{ or } \quad \Lambda_0\leq \frac 12-{c_2/{\alpha}^{1/4}\over \pth{\snr}^{1/2}}.$$
		Then whenever $\snr\sqrt \alpha \geq M\geq c_3$,  the $\cod$ algorithm with $\delta=\frac 12-{\gamma_0\over 4}$ achieves the misclustering rate
		$$
		\EE\qth{\ell(\hat z^{(s)},z)}\leq \exp\sth{-\frac 12\pth{1-{c_4\over \sqrt \snr}}{(\snr)^2}},
		\quad s\geq 1.
		$$
	\end{enumerate}
	
\end{theorem}
\begin{remark}
	The result \cite[Theorem 3.4]{lu2016statistical} shows that it is not possible to improve the misclustering error beyond the rate $e^{-\frac 12(1+o(1)){(\snr)^2}}$. This establishes the optimality of the coordinate-wise median based Lloyd algorithm.
\end{remark}

\begin{proof}[Proof of \prettyref{thm:main-subg}]
	The proof of part (a) is essentially the same as the proof of the similar result \cite[Theorem 3.2]{lu2016statistical} for usual $k$-means. This is because the part of the cluster, the mean of which we use to construct our centroid estimates, is of similar order as the full clusters themselves. As a result we can use the similar concentration bounds that were used to analyze the mean of the full sample in the classical $k$-means problems. We omit the proof here.
	
	To prove part (b), we use the following key lemma.
	\begin{lemma}
		\label{lmm:E-prob-subg}
		Fix $0<\tau,\epsilon_0<\frac 12$. There is a set $\calE_{\tau,\epsilon_0}$ with $\PP\qth{\calE_{\tau,\epsilon_0}}\geq 1-kn^{-c/2}-4e^{-0.3n}$ on which the following holds: 
		\begin{enumerate}[label=(\roman*)]
			\item For any $S\subseteq [n]$ with $|S|>\beta n$, the cardinality of the set 
			$$\sth{i\in S: \|{w_i}\|\leq \sigma \pth{\sqrt d + \sqrt{2\pth{\frac 1\tau\pth{1+\frac 1\beta}+\log(1/\tau)}}}}$$ 
			is at least $(1-\tau)|S|$.
			\item For any $\epsilon\in[\epsilon_0,1/2]$ and $g,h\in[k]$ we have
			$$\sum_{i:Y_i\in T_g^*}\indc{\epsilon^2\|\theta_g-\theta_h\|^2\leq \langle w_i,\theta_h-\theta_g\rangle}
			\leq \frac {5n_g^*}{4\epsilon_0^4(\Delta/\sigma)^2}$$
			\item For any symmetric matrix $A$, let $\lambda_{\max}(A)$ denote its maximum eigen value. Then 
			$$\lambda_{\max}\pth{\sum_{i:Y_i\in T_g^*} w_iw_i^{\sfT}}\leq 6\sigma^2(n_g^*+d) \text{ for all } g\in [k].$$
		\end{enumerate}
	\end{lemma} 
	To prove the above lemma, for each of the cases we separately construct sets of high probability on which the results hold. Then taking intersection we get the result. The analysis of (i) has been provided in \prettyref{lmm:norm-concentration-subg}, the statements (ii),(iii) are the exact results from \cite[Lemma 12, Lemma 13]{JKY2023}.
	
	Based on the above result we get the following results on step-wise clustering errors due to mislabelling.

\begin{lemma}\label{lmm:Gs-Ls-bound-subg}
	Fix $0<\epsilon_0\leq \frac 12,\frac 5{n\alpha} <\gamma_0 \leq \frac 12$. Let $r_k={\Delta\over\sigma}\sqrt{\alpha\over 1+{dk/n}}$. Then on the set $\calE_{\tau,\epsilon_0}$ with $\tau={\gamma_0\over 1+2\gamma_0}$ we have
	\begin{enumerate}[label=(\roman*)]
		\item If $\Lambda_s\leq \frac 12-\epsilon_0$ then $H_{s+1} \geq 1-{5\over \epsilon_0^4 r_k^2}
		-{48\Lambda_s^2\over \epsilon_0^4r_k^2}$,
		\item If $H_s\geq \frac 12+\gamma_0$ then $\Lambda_s\leq {8\sigma\over \Delta} \pth{\sqrt d + \sqrt{2\pth{{1+2\gamma_0\over \gamma_0}\pth{1+\frac 1\beta}+\log\pth{1+2\gamma_0\over \gamma_0}}}}$.
	\end{enumerate}
\end{lemma}

The proof of above result is straightforward. The proof of \prettyref{lmm:Gs-Ls-bound-subg}(i) is exactly the same as in \cite[Appendix C]{JKY2023}, so we skip it here. 
	We present below the proof of \prettyref{lmm:Gs-Ls-bound}(ii). We prove this using contradiction. For simplicity of notation we denote 
	$$D={\sigma} \pth{\sqrt d + \sqrt{2\pth{{1+2\gamma_0\over \gamma_0}\pth{1+\frac 1\beta}+\log\pth{1+2\gamma_0\over \gamma_0}}}}.$$ 
	Let us assume $\Lambda_{s} > {6D\over \Delta}$. This implies that there exists a cluster $h$ such that the centroid estimation error satisfies 
	$$\|\hat \theta_h^{(s+1)}-\theta_h\|> {6D}.$$ 
	

Next we use the above results to prove \prettyref{thm:main-subg}(ii). For $c_1$ to be chosen later, we define
$$\epsilon_0={c_1/\alpha^{1/4}\over \pth{\snr}^{1/2}}.$$
Let $G_s$ be the mislabeling proportion as defined before in \eqref{eq:mislabel}. Then from \prettyref{lmm:Gs-Ls-bound-subg} it follows that we can choose $c_0,c_1>0$ such that on the set $\calE_{{\gamma_0\over 1+2\gamma_0},\epsilon_0}$:
\begin{itemize}
	\item if $H_0\geq \frac 12+\gamma_0$ then $\Lambda_0\leq 0.3$,
	\item if $\Lambda_0\leq \frac 12-\epsilon_0$ then $H_1\geq 0.7$.
\end{itemize}
A second application of \prettyref{lmm:Gs-Ls-bound-subg} guarantees that we can choose $c_0$ large enough such that if  
$\snr\geq c_0\sqrt{d/\alpha}$
then on the set $\calE_{{5\over 26},0.2}$, with $\epsilon_1=\gamma_1=0.2$,
\begin{itemize}
	\item if $G_s\leq 0.3$ then
	\begin{align}
		\label{eq:Ls}
		\Lambda_s&\leq {12\sqrt 2/\alpha^{1/2}\over \sqrt{0.2}\snr} \leq 0.3,
	\end{align}
	\item if $\Lambda_s\leq 0.3$ then
	\begin{align}
		\label{eq:Gs}
		G_{s+1}&\leq {5/\alpha\over (0.2)^4(\snr)^2}+{48(0.3)^2/\alpha\over (0.2)^4(\snr)^2}\leq 0.3.
	\end{align}		
\end{itemize}
and whenever 
Combining the above displays we get that on the set
\begin{align}
	\label{eq:Prob-E}
	\calE&=\calE_{{\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{{5\over 26},0.2}
	\nonumber\\
	\PP\qth{\calE}
	&\geq 1-4kn^{-c/4}-4e^{-0.3n}
\end{align} 
we have
\begin{align}
	\label{eq:ht14}
	\Lambda_s\leq 0.3,G_{s+1}\leq 0.3 \text{ for all } s\ge 0.
\end{align}
The rest of the analysis is 
identical to that of the proof of \cite[Theorem 1]{JKY2023} where it is shown that once we achieve $\Lambda_s\leq 0.3$ for all $s\geq 3$, the mislabeling rate follows. We omit it here.
\end{proof}


\section{Clustering in presence of adversarial outliers \nb{TBD}}

\subsection{Error distributions with moment constraints}

\subsection{Sub-Gaussian error distributions}
Suppose that an adversary adds $n^{\out}$ many points to our existing data set. Then we have the following guarantees.
\begin{theorem}
	\label{thm:optim-outl}
	Suppose that $n\alpha\geq c\log n$ for some $c>0$. There exists absolute constants $c_1,c_2,c_3,c_4,c_5>0$ such that the followings are satisfied. For any $\eta\in(0,1]$, if the clustering initialization satisfies either one of the following conditions
	$${H_0}\geq \frac 12+\frac {c_1/\alpha}{\pth{\snr}^2}\quad  \text{ or } \quad \Lambda_0\leq \frac 12-{c_2/\alpha\over \pth{\snr}^{\frac 12(1-\eta)}},$$
	then whenever $$\snr\sqrt\alpha\geq M\geq c_3,$$ 
	for any $n^{\out}\leq n\alpha(1-c_4M^{-2\eta})$ our algorithm guarantees $$\EE\qth{\ell(\hat z^{(s)},z)}\leq \exp\sth{-\frac 12\pth{1-{c_5\over \sqrt M}}{(\snr)^2}},
	\quad s\geq 1.
	$$
\end{theorem}


\subsection{Step-wise clustering errors due to mislabelling (in presence of outliers)}
The proof of the above theorem hinges on the following lemma, similar to \prettyref{lmm:Gs-Ls-bound}.

\begin{lemma}\label{eq:HsLs-bound}
	Fix $\epsilon_0,\gamma_0\in (0,\frac 12]$ and suppose that an adversary added $n\beta$ many outliers with $\beta\leq\alpha(1-\delta)$ for some $\delta>0$. Let $r_k={\Delta\over\sigma}\sqrt{\alpha\over 1+{dk/n}}$. Then on the set $\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0} $ we have
	\begin{enumerate}[label=(\roman*)]
		\item If $\Lambda_s\leq \frac 12-\epsilon_0$ then $H_{s+1} \geq \frac 12 +\min\sth{{\delta-2\tau\over 2(2-\delta)},1-\tau}$ where $\tau={5\over 2\epsilon_0^4 r_k^2}
		+{24\Lambda_s^2\over \epsilon_0^4r_k^2}$,
		\item If $H_s\geq \frac 12+\gamma_0$ then $\Lambda_s\leq {3\sigma\over \Delta} \pth{\sqrt d + \sqrt{2\pth{{1+2\gamma_0\over \gamma_0}\pth{1+\frac 1\beta}+\log\pth{1+2\gamma_0\over \gamma_0}}}}$.
	\end{enumerate}
\end{lemma}

\begin{proof}
	
	The proof of part (i) borrows results from the proof of \prettyref{lmm:Gs-Ls-bound}(i). Notice that we can show for each $h\neq g$
	\begin{align}
		\label{eq:km22}
		n_{gh}^{(s+1)}
		&\leq 
		\frac{5n_g^*\sigma^2}{4\epsilon_0^4\Delta^2}
		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2}\pth{{n_g^*}+  d}.
	\end{align}
	Using the last display and noting that $k\leq \frac 1{\alpha}$ and $n_g^*\geq n\alpha$ we get
	\begin{align}\label{eq:km23}
		{\sum_{h\in[k]\atop h\neq g}n_{gh}^{(s+1)}\over n_g^*}
		\leq \tau,\quad \tau=
		\frac{5\sigma^2}{2\epsilon_0^4\Delta^2\alpha}
		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2\alpha}\pth{1+ {dk\over n}}.
	\end{align}
	Using $n_g^{*}=\sum_{h\in [k]}n_{gh}^{(s+1)}$ for all $s\geq 0$, we get 
	\begin{align}\label{eq:km24}
		{n_{gg}^{(s+1)}\over n_g^*}\geq 1-\tau.
	\end{align}	 
	Next we switch $g,h$ in \eqref{eq:km22} and sum over $h\in [k], h\neq g$. We get
	\begin{align}
		\sum_{h\in[k]\atop h\neq g}n_{hg}^{(s+1)}
		\leq \frac{5n\sigma^2}{2\epsilon_0^4\Delta^2}
		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2}\pth{n+ kd}
		\leq n\alpha\tau.
	\end{align}
	Using the above and noticing that in addition to the points in $\cup_{h\in[k]}\sth{T_{h}^*\cap T_g^{(s+1)}}$, $T_g^{(s+1)}$ can at most have $n\beta$ many extra points, accounting for the outliers, we get
	\begin{align}
		{n_{gg}^{(s+1)}\over n_g^{(s+1)}}\geq {n_{gg}^{(s+1)}\over n_{gg}^{(s+1)}+n\alpha\tau+n^{\out}}
		\geq \frac 1{1+{n_g^*(1-\delta+\tau)\over n_{gg}^{(s+1)}}}
		\geq \frac 1{1+{1-\delta+\tau\over 1-\tau}}
		=\frac 12 + {\delta-2\tau\over 2(2-\delta)}.
	\end{align}
	Combining the last display with \eqref{eq:km24} we get
	\begin{align*}
		H_{s+1}=\min_{g\in [k]}\sth{\min\sth{{n_{gg}^{(s)}\over n_g^*},{n_{gg}^{(s)}\over n_{g}^{(s)}}}}
		\geq \frac 12+\min\sth{{\delta-2\tau\over 2(2-\delta)},\frac 12-\tau},
	\end{align*}
	as required.
	
	The proof of (ii) follows a similar strategy as in the proof of \prettyref{lmm:Gs-Ls-bound}, part (ii). Define as before
\end{proof}
\subsection{Proof of \prettyref{thm:optim-outl}}
Let $\beta=\alpha(1-\delta)$.  For $c_1,c_2$ to be chosen later, we define
$$\gamma_0=\frac {c_1}{\pth{{\Delta\over \sigma}\sqrt{\alpha\over d}}^2},\quad \epsilon_0={c_2\over \pth{{\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}^{\frac 12(1-\eta)}}.$$
Then from \prettyref{lmm:Gs-Ls-bound} it follows that, we can choose $c_1,c_2,c_3,c_4>0$ such that whenever $M>c_3$ and $\delta\geq c_4M^{-2\eta}$, on the set $\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0}$:
\begin{itemize}
	\item if $\Lambda_0\leq \frac 12-\epsilon_0$ then $H_1\geq \frac 12 + {\delta\over 6}$.
	\item if $H_0\geq \frac 12+\gamma_0$ then $\Lambda_0\leq 0  .3$,
\end{itemize}
A second application of \prettyref{lmm:Gs-Ls-bound} guarantees that we can choose $c_3$ large enough such that if  
$$M=\min \sth{{\Delta\over \sigma}\sqrt{\alpha\over d},{\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}\geq c_3$$
then on the set $\calE_{{2\gamma_1\over 1+2\gamma_1},\epsilon_1}\cap \calE_{\frac 14,\epsilon_1}$, with $\epsilon_1=\gamma_1=0.2$, if $H_{s}\geq \frac 12 +\frac \delta6$ then $\Lambda_s\leq {12\sqrt 2\over \sqrt{0.2}M} \leq 0.3$ and if $\Lambda_s\leq 0.3$ then $H_{s+1}\geq \frac 12 +\frac \delta6$.
Combining the above displays we get that on the set
\begin{align}
	\label{eq:Prob-E2}
	\calE&=\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0} \cap \calE_{{2\gamma_1\over 1+2\gamma_1},\epsilon_1}\cap \calE_{\frac 14,\epsilon_1}
	\nonumber\\
	\PP\qth{\calE}
	&\geq 1-4(k^2+k)n^{-c/4}-16de^{-0.3n}
\end{align} 
we have
\begin{align}
	\label{eq:km27}
	\Lambda_s\leq 0.3,\quad H_{s+1}\geq \frac 12 +\frac \delta6 \text{ for all } s\ge 2.
\end{align}
We will show that $\PP\qth{\left.z_i\neq \hat z_i^{(s+1)}\right|\calE}$ is small for each $i\in [n]$. This will imply that on the set $\calE$, $A_{s+1}=\frac 1n\sum_{i=1}^n\indc{z_i\neq \hat z_i^{(s+1)}}$ is also small in probability. From this, using a Markov inequality we will conclude the result. The analysis is 
identical to that of the proof of \cite[Theorem 1]{JKY2023} where it is shown that once we achieve $\Lambda_s\leq 0.3$ for all $s\geq 3$, the mislabeling rate follows. We omit it here.


\section{Suboptimality of the Lloyd algorithm}

\begin{theorem}
Suppose that $d=1,k=2$ and the errors $\sth{w_i:i=1,\dots,n}$ are independently distributed according to the standard Cauchy distribution. Then there exists a constant $\gamma>0$ such that for any random initialization satisfying $H_0\in (\frac 12,\frac 12 + \gamma)$ the Lloyd algorithm produces suboptimal mislabeling. 
\end{theorem}

\begin{proof}
	Note that the model in this specific case is given by
	\begin{align}
		Y_i=\theta_{z_i}+w_i,\quad \sth{w_i}_{i=1}^n\simiid w\ \PP\qth{w>x} = \int_{x}^\infty \frac {dx}{\pi(1+x^2)},\ x\in (-\infty,\infty).
	\end{align}
	We assume that the clusters $T_1,T_2$ are of the same size $\frac n2$. Suppose that the centroids are $\theta_1,\theta_2$ with $\theta_2>\theta_1$ and let $T_j^{(0)}=\sth{i\in [n]:z_i=j}$ for $j\in\{1,2\}$. The we have $\Delta=\theta_2-\theta_1$ and $\alpha=\frac 12$.Fix $\tau\in(0,1)$ and define the two events
	\begin{align}
		\begin{gathered}
			A=\sth{\sum_{i\in T_1^{(0)}}w_i-\sum_{i\in T_2^{(0)}}w_i>2\gamma \Delta},\\
		B= \cap_{j\in\{1,2\}}\sth{|\sth{i\in T_j:|Y_i-\theta_j|<{\Delta\over 2}}|\geq (1-\tau)\frac n2}.
		\end{gathered}
	\end{align}
	We analyze the probabilities of the above events. To analyze the event $A$, as the errors are independent Cauchy random variables, note that ${\sum_{i\in T_1^{(0)}}w_i-\sum_{i\in T_2^{(0)}}w_i\over 2}$ is also distributed as a standard Cauchy random variable. This implies when $\gamma \Delta\geq 1$
	\begin{align}\label{eq:ht0}
		\PP\qth{A} = \int_{\gamma \Delta}^\infty \frac {dx}{\pi(1+x^2)}
		\geq \frac 1{2\pi\gamma\Delta}.
	\end{align}
	Next note that for a standard Cauchy random variable $Z$ we have
	$$\PP\qth{Z>x}\leq \frac 1\pi\cdot \frac 1x,\quad x>-\infty,$$
	and hence $Z\in \calR_1(\frac 1{\pi})$. In view of \prettyref{lmm:norm-concentration} with $\beta=\frac 12,\sigma=\frac 1{\pi}$, the last statement implies that
	$$\PP\qth{\abs{\sth{i\in T_j: \abs{w_i}\leq \frac {e^{\frac 1\tau (1+\frac 1\beta)}}{\pi\tau}}}\geq (1-\tau)\frac n2}\geq 1-e^{-0.3 n}.$$
	Then we get whenever $\frac \Delta2\geq \frac {e^{\frac 1\tau (1+\frac 1\beta)}}{\pi\tau}$, we have
	$$
		\PP\qth{|\sth{i\in T_j:|Y_i-\theta_j|<{\Delta\over 2}}|\geq (1-\tau)\frac n2}
		\geq 1-e^{-0.3n},
	$$
	and hence $\PP\qth{B}\geq 1-2e^{-0.3n}$. In view of \eqref{eq:ht0} the last display implies 
	\begin{align}\label{eq:ht1}
		\PP\qth{A\cap B} \geq \PP[A]-\PP[B^c]\geq \frac 1{8\pi\gamma\Delta}-2e^{-0.3n}.
	\end{align}
	For the rest of the analysis we condition on the event $A\cap B$. Note that upon initialization with proportion of correct labels $H_0$, after the first iteration, the new centroid estimates become
	\begin{align}
		\begin{gathered}
			\hat \theta_1^{(0)} = (\frac 12 + \gamma)\sth{\theta_1+\sum_{i\in T_1^{(0)}}w_i}+(\frac 12 - \gamma)\sth{\theta_2 + \sum_{i\in T_2^{(0)}}w_i},\\
		\hat \theta_2^{(0)} = (\frac 12 + \gamma)\sth{\theta_2+\sum_{i\in T_2^{(0)}}w_i}+(\frac 12 - \gamma)\sth{\theta_1 + \sum_{i\in T_1^{(0)}}w_i}
		\end{gathered}.
	\end{align}
	Simple algebraic manipulation implies that on the event $A$ we have $\hat \theta_1^{(0)}\geq \hat \theta_2^{(0)}$. This implies the order of the centroid estimates (according to the magnitude) switches from the true ones. Note that in all subsequent iterations this order of the estimates stay the same. This is because the in the subsequent estimates the data labels are estimated using the Voronoi regions, which is just a single division of the real line, and then the means are estimated using the data points on the two half lines. Hence, the least amount of mislabeling produced, when we condition on the event $B$ is $(1-\tau)\over 2$. Hence, in view of \eqref{eq:ht1}, the expected proportion of mislabeling produced by the $k$-means algorithm at any step $s\geq 1$, can be bounded from below as
	\begin{align}
		\EE\qth{\ell(\hat z^{(s)},z)}\geq \PP[A\cap B]\cdot \PP\qth{\ell(\hat z^{(s)},z)|A\cap B}
		\geq \frac {(1-\tau)}{16\pi\gamma\Delta}-(1-\tau)e^{-0.3n}.
	\end{align}
	On the other hand, note that \prettyref{thm:main} implies that, for any $\gamma\geq (\frac 1{n\alpha},\frac 12)$ and $k=2$, whenever $H_0\geq \frac 12+\gamma$, the mislabeling achieved by the \cod algorithm with $\delta=\frac 12-\frac \gamma4$ is at most $(1+o(1)){16/\pi\over \Delta}$, where the $o(1)$ term goes to zero as $\Delta$ becomes large. Hence choosing a small but constant value of $\gamma$ we can conclude that the mislabeling produced by $k$-means is suboptimal.
\end{proof}

%
%\section{Related estimation guarantees in absence of outliers}
%\label{sec:other-est-no-outliers}
%%We mention the centrality property here:
%%
%%\begin{enumerate}[label=(Q)]
%%	\item \label{eq:Q}(Quantile detection) Given a real random variable $W$ and $q\in(0,\frac 12]$, we say $x,y$ are sufficient to detect its $q,1-q$-th quantiles if
%%	\begin{align*}
%%		\PP\qth{W\geq x}\leq q,\quad \PP\qth{W\leq y}\leq 1-q.
%%	\end{align*}
%%\end{enumerate}
%
%\begin{theorem}
%	Let $F_{ij}$ denote the distribution of the $j$-th coordinate of the $i$-th data point $Y_i$. Suppose that $n\alpha\geq c\log n$ for some $c>0$ and the constraints in \prettyref{thm:main} on $G_s,\Lambda_s$ are satisfied. Then given any $\tau >0$, there exists absolute constants $C:=C(\tau)>0$ such that whenever $M=\min \sth{{\Delta\over \sigma}\sqrt{\alpha\over d}, {\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}\geq C$
%	with probability at least $1-\frac 1n-4(k^2+k)n^{-(c/2-2)}-16dn^4e^{-0.3n}- 2k^2\exp\sth{-{\Delta\over 8\sigma}}$ we have
%	$$
%	\|\hat \theta_g^{(s)}-\theta_g\|^2\leq {d}
%	\qth{\max_{i:Y_i\in T_g^*}\max_{j\in [d]} \max\sth{\abs{F_{ij}^{-1}\pth{\frac 12 +x_0}},\abs{F_{ij}^{-1}\pth{\frac 12 -x_0}}}}^2,\quad s\geq 2,
%	$$
%	where 
%	$x_0= \sqrt{3\log n\over n_g^*}+e^{-{\Delta^2\over (8+\tau)\sigma^2}}$.
%\end{theorem}
%
%\begin{remark} \nb{EDIT THIS FOR NEW NOTATIONS}
%	In particular, if the errors of the $g$-th cluster are distributed as the univariate Gaussian distribution with variance $\sigma^2$, then for any value of $n_g^*$ the conditions in the above theorems are satisfied with $$x_0=C\sigma\pth{{\sqrt{\log n\over {n_g^*}}+e^{-{\Delta^2\over 24\sigma^2}}}}$$ for some large constant $C>0$. This implies that when $\Delta\gtrsim \sigma\log n$ we achieve the optimal rate of estimating the centroids.
%\end{remark}
%\begin{proof}
%	The results in the last section implies that there is an absolute constant $C>0$ such that whenever 
%	$$
%	\min\sth{{\Delta\over \sigma}\sqrt{\alpha\over d},{\Delta\over \sigma}\sqrt{\alpha\over 1+{kd/n}}}\geq C
%	$$
%	we get for any $g\in [k]$
%	\begin{align}
%		\max\sth{\sum_{h\in[k]\atop h\ne g}n_{hg}^{(s)},\sum_{h\in[k]\atop h\ne g}n_{gh}^{(s)}}
%		\leq \sum_{i=1}^n\indc{\hat z_i^{(s)}\neq z_i}
%		=nA_s, \quad s\geq 3.
%	\end{align}
%	Using the above we get
%	\begin{align}
%		G_s=\max_{g\in [k]} \sth{\max\sth{{\sum_{h\in[k]\atop h\neq g} n_{gh}^{(s)}\over n_g^*},{\sum_{h\in[k]\atop h\neq g} n_{hg}^{(s)}\over n_g^{(s)}}}}
%		\leq nA_s\cdot \max_{g\in [k]}\sth{\max\sth{\frac 1{n_g^*},\frac 1{n_g^{(s)}}}}.
%	\end{align}
%	As $G_s\leq \frac 12$ for all $s\geq 3$, we get $n\alpha\leq n_g^*\leq 2n_{gg}^{(s)}\leq 2n_{g}^{(s)}$. Using this we have
%	\begin{align}\label{eq:km26}
%		n_{g}^*\geq n_{gg}^{(s)}\geq n_g^{(s)}-nA_s\geq n_g^{(s)}\pth{1-\frac 2\alpha A_s},
%		\quad n_{g}^{(s)}\geq n_{gg}^{(s)}\geq n_g^*-nA_s\geq n_g^*\pth{1-\frac 1\alpha A_s}.
%	\end{align}
%	Fix $g\in [k]$. Let $U_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^{(s)}$, $V_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^*\cap T_g^{(s)}$, and $W_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^*$. Then we get
%	\begin{align*}
%		U_j^{(\ceil{ {n_g^{(s)}/2}})}
%		&\stepa{\leq} V_j^{(\ceil{n_g^{(s)}/2}-n_g^{(s)}+n_{gg}^{(s)})}
%		\nonumber\\
%		&\stepb{\leq }
%		V_j^{(\floor{{n_g^{(s)}\over 2}-nA_s})}
%		\stepc{\leq} W_j^{(\floor{{n_g^{(s)}\over 2}-nA_s})}
%		\stepd{\leq} W_j^{(\floor{{n_g^{*}\over 2}-{3nA_s\over 2}})}
%		\stepe{\leq} W_j^{(\floor{{n_g^*}(\frac 12-\frac 1\alpha A_s)})},
%	\end{align*}
%	where
%	\begin{itemize}
%		\item (a) followed using \prettyref{lmm:ord-stat_after_addn} with
%		$
%		X=V_j,\ \tilde X=U_j,\ \ell=n_g^{(s)}-n_{gg}^{(s)},\ t=\ceil{n_g^{(s)}\over 2},
%		$
%		\item (b) followed using $n_g^{(s)}-n_{gg}^{(s)}\leq nA_s$ and $\ceil{x}-y\geq \floor{x-y}$ for $x,y\geq 0$
%		
%		\item (c) followed using \prettyref{lmm:ord-stat_after_addn} with 
%		$X=V_j,\ \tilde X=W_j,\ \ell=n_g^*-n_{gg}^{(s)},\ t=\floor{{n_g^{(s)}\over 2} -nA_s},$
%		
%		\item (d) followed using \eqref{eq:km26} and (e) followed using $n_g^*\geq n\alpha$.
%	\end{itemize}
%	Similarly we also have
%	\begin{align*}
%		U_j^{(\ceil{ {n_g^{(s)}/2}})}
%		&\stepa{\geq} V_j^{(\ceil{n_g^{(s)}/2})}
%		\nonumber\\
%		&\stepb{\geq} 
%		V_j^{(\ceil{{n_g^*\over 2}\cdot \frac 1{1-{2A_s/\alpha}}})}
%		\stepc{\geq} 
%		V_j^{(\ceil{{n_g^*}(\frac 12+\frac 2\alpha A_s)})}
%		\stepd{\geq} W_j^{(\ceil{{n_g^*}(\frac 12+\frac 2\alpha A_s)}+\sum_{h=[k]\atop h\neq k}n_{gh})}
%		\stepe{\geq} W_j^{(\ceil{{n_g^*}(\frac 12+\frac 3\alpha A_s)})}.
%	\end{align*}
%	\begin{itemize}
%		\item (a) followed using \prettyref{lmm:ord-stat_after_addn} with
%		$
%		X=V_j,\ \tilde X=U_j,\ \ell=n_g^{(s)}-n_{gg}^{(s)},\ t=\ceil{n_g^{(s)}\over 2},
%		$
%		
%		\item (b) followed using \eqref{eq:km26} and (c) followed using $(1-x)^{-1}\leq 1+2x$ for $x=\frac 2\alpha A_s\leq \frac 12$.
%		
%		\item (d) used \prettyref{lmm:ord-stat_after_addn} with 
%		$X=V_j,\ \tilde X=W_j,\ \ell=\sum_{h=[k]\atop h\neq k}n_{gh},\ t=\ceil{{n_g^*\over 2}(1+\frac 4\alpha A_s)}+\sum_{h=[k]\atop h\neq k}n_{gh},$
%		
%		
%		\item (e) used that for any $x>0$ and positive integer $y$, $\ceil{x}+y = \ceil{x+y}$, and $\sum_{h=[k]\atop h\neq k}n_{gh}\leq nA_s$.
%	\end{itemize}
%	Then \prettyref{thm:main} implies that given any $\tau>0$, there exists $C:=C(\tau)$ such that whenever $M\geq C(\tau)$, we have $\frac 6\alpha A_s\leq e^{-{\Delta^2\over (8+\tau)\sigma^2}}$. Using this we combine the last two displays to get
%	\begin{align}
%		W_j^{(\ceil{{n_g^*\pth{\frac 12+e^{-{\Delta^2\over (8+\tau)\sigma^2}}}}})}
%		\leq U_j^{(\floor{{n_g^{(s)}/2}})}\leq W_j^{(\floor{{n_g^*\pth{\frac 12-e^{-{\Delta^2\over (8+\tau)\sigma^2}}}}})}.
%	\end{align}
%	Then using the result \prettyref{lmm:order-concentration-smallx} on the concentration of the order statistics
%	we conclude our results.
%\end{proof}
%
%\nb{TBD: Add a remark about spectral initialization}
%
%\section{Optimality in the presence of outliers}
%
% Suppose that an adversary adds $n^{\out}$ many points to our existing data set. Our results for the adversarial addition regime is based on the cluster-wise correct classification proportion at step $s$, defined as
%\begin{align}
%	H_s=\min_{g\in [k]}\sth{\min\sth{{n_{gg}^{(s)}\over n_g^*},{n_{gg}^{(s)}\over n_{g}^{(s)}}}}.
%\end{align}
%\begin{theorem}
%	\label{thm:optim-outl}
%	 Suppose that $n\alpha\geq c\log n$ for some $c>0$. There exists absolute constants $c_1,c_2,c_3,c_4,c_5>0$ such that the followings are satisfied. For any $\eta\in(0,1]$, if the clustering initialization satisfies either one of the following conditions
%	$${H_0}\geq \frac 12+\frac {c_1}{\pth{{\Delta\over \sigma}\sqrt{\alpha\over d}}^2}\quad  \text{ or } \quad \Lambda_0\leq \frac 12-{c_2\over \pth{{\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}^{\frac 12(1-\eta)}},$$
%	then whenever $$M=\min \sth{{\Delta\over \sigma}\sqrt{\alpha\over d}, {\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}\geq c_3,$$ 
%	for any $n^{\out}\leq n\alpha(1-c_4M^{-2\eta})$ our algorithm guarantees $$A_s\leq \exp\sth{-\pth{1-{c_5\over \sqrt M}}{\Delta^2\over 8\sigma^2}+{\Delta\over \sigma}},
%	\quad s\geq 2
%	$$
%	with probability $1-4(k^2+k)n^{-(c/2-2)}-16dn^4e^{-0.3n}- 2k^2\exp\sth{-{\Delta\over 8\sigma}}.$
%\end{theorem}
%
%\begin{remark}
%    When we initialize with the constraint on $H_0$ we can allow $\eta=1$.\nb{Check proof}
%\end{remark}
%
%The proof of the above theorem hinges on the following lemma, similar to \prettyref{lmm:Gs-Ls-bound}.
%
%\begin{lemma}\label{eq:HsLs-bound}
%	Fix $\epsilon_0,\gamma_0\in (0,\frac 12]$ and suppose that an adversary added $n\beta$ many outliers with $\beta\leq\alpha(1-\delta)$ for some $\delta>0$. Let $r_k={\Delta\over\sigma}\sqrt{\alpha\over 1+{dk/n}}$. Then on the set $\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0} $ we have
%	\begin{enumerate}[label=(\roman*)]
%		\item If $\Lambda_s\leq \frac 12-\epsilon_0$ then $H_{s+1} \geq \frac 12 +\min\sth{{\delta-2\tau\over 2(2-\delta)},1-\tau}$ where $\tau={5\over 2\epsilon_0^4 r_k^2}
%		+{24\Lambda_s^2\over \epsilon_0^4r_k^2}$,
%		\item If $H_s\geq \frac 12+\gamma_0$ then $\Lambda_s\leq {12\sqrt 2\over \Delta/\sigma}\sqrt{d \over  {\gamma_0\alpha}}$.
%	\end{enumerate}
%\end{lemma}
%
%\begin{proof}
%	
%	The proof of part (i) borrows results from the proof of \prettyref{lmm:Gs-Ls-bound}(i). Notice that we can show for each $h\neq g$
%	\begin{align}
%		\label{eq:km22}
%		n_{gh}^{(s+1)}
%		&\leq 
%		\frac{5n_g^*\sigma^2}{4\epsilon_0^4\Delta^2}
%		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2}\pth{{n_g^*}+  d}.
%	\end{align}
%	Using the last display and noting that $k\leq \frac 1{\alpha}$ and $n_g^*\geq n\alpha$ we get
%	\begin{align}\label{eq:km23}
%		{\sum_{h\in[k]\atop h\neq g}n_{gh}^{(s+1)}\over n_g^*}
%		\leq \tau,\quad \tau=
%		\frac{5\sigma^2}{2\epsilon_0^4\Delta^2\alpha}
%		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2\alpha}\pth{1+ {dk\over n}}.
%	\end{align}
%	Using $n_g^{*}=\sum_{h\in [k]}n_{gh}^{(s+1)}$ for all $s\geq 0$, we get 
%	\begin{align}\label{eq:km24}
%		{n_{gg}^{(s+1)}\over n_g^*}\geq 1-\tau.
%	\end{align}	 
%	Next we switch $g,h$ in \eqref{eq:km22} and sum over $h\in [k], h\neq g$. We get
%	\begin{align}
%		\sum_{h\in[k]\atop h\neq g}n_{hg}^{(s+1)}
%		\leq \frac{5n\sigma^2}{2\epsilon_0^4\Delta^2}
%		+{24\Lambda_s^2\sigma^2\over \epsilon_0^4\Delta^2}\pth{n+ kd}
%		\leq n\alpha\tau.
%	\end{align}
%	Using the above and noticing that in addition to the points in $\cup_{h\in[k]}\sth{T_{h}^*\cap T_g^{(s+1)}}$, $T_g^{(s+1)}$ can at most have $n\beta$ many extra points, accounting for the outliers, we get
%	\begin{align}
%		{n_{gg}^{(s+1)}\over n_g^{(s+1)}}\geq {n_{gg}^{(s+1)}\over n_{gg}^{(s+1)}+n\alpha\tau+n^{\out}}
%		\geq \frac 1{1+{n_g^*(1-\delta+\tau)\over n_{gg}^{(s+1)}}}
%		\geq \frac 1{1+{1-\delta+\tau\over 1-\tau}}
%		=\frac 12 + {\delta-2\tau\over 2(2-\delta)}.
%	\end{align}
%	Combining the last display with \eqref{eq:km24} we get
%	\begin{align*}
%		H_{s+1}=\min_{g\in [k]}\sth{\min\sth{{n_{gg}^{(s)}\over n_g^*},{n_{gg}^{(s)}\over n_{g}^{(s)}}}}
%		\geq \frac 12+\min\sth{{\delta-2\tau\over 2(2-\delta)},\frac 12-\tau},
%	\end{align*}
%	as required.
%	
%	The proof of (ii) follows a similar strategy as in the proof of \prettyref{lmm:Gs-Ls-bound}, part (ii). Define as before
%	\begin{align}
%		\begin{gathered}
%			\hat \theta_g^{(s)}=\med(T_g^{(s)}),\quad \tilde \theta_g^{(s)}=\med(T_g^{(s)}\cap T_g^*)\\
%			U_j=\text{the set of $j^{\rm{th}}$ coordinates of $T_g^{(s)}$},\quad
%			V_j=\text{the set of $j^{\rm{th}}$ coordinates of $T_g^{(s)}\cap T_g^*$}.
%		\end{gathered}
%	\end{align} 
%%	Then as we have
%%	\begin{align}
%%			n_{gg}^{(s)}\geq (\frac 12+\gamma_0)n_g^{(s)}\geq {n_g^{(s)}\over 2}+5,\quad
%%			n_{g}^{(s)}-n_{gg}^{(s)}\leq (\frac 12-\gamma_0)n_g^{(s)}\leq {n_g^{(s)}\over 2}-5
%%	\end{align}
%%	we can use \prettyref{lmm:ord-stat_after_addn} with
%%	$X=V_j,\tilde X=U_j,m=n_{gg}^{(s)},\ell=n_{g}^{(s)}-n_{gg}^{(s)},
%%	t=\ceil{n_g^{(s)}\over 2}$
%%	to get
%%	\begin{align}
%%		V_j^{(\ceil{ {n_g^{(s)}/2}})}
%%		\leq \med(U_j)
%%		\leq V_j^{(\floor{\gamma_0 n_{g}^{(s)}})}.
%%	\end{align}
%%	Using the definition of order statistics we also have
%%	\begin{align}
%%	V_j^{(\ceil{ {n_g^{(s)}/2}})}
%%	\leq V_j^{(\ceil{n_{gg}^{(s)}/2})}=\med(V_j)
%%	\leq  V_j^{(\floor{\gamma_0 n_{g}^{(s)}})}.
%%	\end{align}
%%	Combining the last two displays we get
%	Then using essentially the same strategy we show
%	\begin{align}\label{eq:km32}
%	\|\hat \theta_g^{(s)}-\tilde\theta_g^{(s)}\|_2^2\leq \sum_{j=1}^d\abs{\med(U_j)-\med(V_j)}^2
%	&\leq \abs{V_j^{(\floor{\gamma_0 n_g^{(s)}})}-V_j^{(\ceil{ {n_g^{(s)}/2}})}}.
%	\end{align}
%	Then as $H_s\geq \frac 12+\gamma_0$ guarantees ${1\over 1+2\gamma_0}n_{gg}^{(s)} \geq {n_g^{(s)}\over 2}\leq \gamma_0 n_g^{(s)}\geq \gamma_0 n_{gg}^{(s)}$, we get that
%	\begin{align}
%		\|\hat \theta_g^{(s)}-\tilde\theta_g^{(s)}\|_2^2
%		\leq \sum_{j=1}^d\abs{V_j^{(\floor{\gamma_0 n_{gg}^{(s)}})}-V_j^{(\ceil{{1\over 1+2\gamma_0}n_{gg}^{(s)}})}}^2
%	\end{align}
%	The rest of the proof then follows using the concentration bound of order statistics for the sets $V_1,\dots,V_d$ As these sets do not involve any outliers, our usual concentration bound for $\subG(\sigma^2)$, provided in \prettyref{lmm:order-concentration}, applies.
%	
%\end{proof}
%
%\begin{proof}[Proof of \prettyref{thm:optim-outl}]
%	Let $\beta=\alpha(1-\delta)$.  For $c_1,c_2$ to be chosen later, we define
%	$$\gamma_0=\frac {c_1}{\pth{{\Delta\over \sigma}\sqrt{\alpha\over d}}^2},\quad \epsilon_0={c_2\over \pth{{\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}^{\frac 12(1-\eta)}}.$$
%	Then from \prettyref{lmm:Gs-Ls-bound} it follows that, we can choose $c_1,c_2,c_3,c_4>0$ such that whenever $M>c_3$ and $\delta\geq c_4M^{-2\eta}$, on the set $\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0}$:
%	\begin{itemize}
%		\item if $\Lambda_0\leq \frac 12-\epsilon_0$ then $H_1\geq \frac 12 + {\delta\over 6}$.
%		\item if $H_0\geq \frac 12+\gamma_0$ then $\Lambda_0\leq 0  .3$,
%	\end{itemize}
%	A second application of \prettyref{lmm:Gs-Ls-bound} guarantees that we can choose $c_3$ large enough such that if  
%	$$M=\min \sth{{\Delta\over \sigma}\sqrt{\alpha\over d},{\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}\geq c_3$$
%	then on the set $\calE_{{2\gamma_1\over 1+2\gamma_1},\epsilon_1}\cap \calE_{\frac 14,\epsilon_1}$, with $\epsilon_1=\gamma_1=0.2$, if $H_{s}\geq \frac 12 +\frac \delta6$ then $\Lambda_s\leq {12\sqrt 2\over \sqrt{0.2}M} \leq 0.3$ and if $\Lambda_s\leq 0.3$ then $H_{s+1}\geq \frac 12 +\frac \delta6$.
%	Combining the above displays we get that on the set
%	\begin{align}
%		\label{eq:Prob-E2}
%		\calE&=\calE_{{2\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{\frac 14,\epsilon_0} \cap \calE_{{2\gamma_1\over 1+2\gamma_1},\epsilon_1}\cap \calE_{\frac 14,\epsilon_1}
%		\nonumber\\
%		\PP\qth{\calE}
%		&\geq 1-4(k^2+k)n^{-c/4}-16de^{-0.3n}
%	\end{align} 
%	we have
%	\begin{align}
%		\label{eq:km27}
%		\Lambda_s\leq 0.3,\quad H_{s+1}\geq \frac 12 +\frac \delta6 \text{ for all } s\ge 2.
%	\end{align}
%	We will show that $\PP\qth{\left.z_i\neq \hat z_i^{(s+1)}\right|\calE}$ is small for each $i\in [n]$. This will imply that on the set $\calE$, $A_{s+1}=\frac 1n\sum_{i=1}^n\indc{z_i\neq \hat z_i^{(s+1)}}$ is also small in probability. From this, using a Markov inequality we will conclude the result. The analysis is 
%	identical to that of the proof of \prettyref{thm:main} after \eqref{eq:km14} which relies solely on the fact that $\Lambda_s\leq 0.3$ for all $s\geq 3$. We omit it here.
%\end{proof}
%
%
%
%\subsection*{Adversarial data corruption}
%	
%	\begin{remark}
%		Mention that it is equivalent to adversarial data addition but the result changes a bit
%	\end{remark}
%
%\section{Centroid estimation in presence of outliers}
%For this section, let us define the ratio of total outliers with respect to individual clusters as
%\begin{align}
%    \beta_g^\out = {n^{\out}\over n_g^*},\quad g=1,2,\dots,k.
%\end{align}
%Note that in order to identify all the clusters accurately we require $\max_g\beta_g^\out<1$; otherwise, given any algorithm, an adversary can always create a constellation involving only the outliers that will force the algorithm to detect it as an individual cluster.
%
%\begin{theorem} 
%	Suppose that $n\alpha\geq c\log n$ for some $c>0$ and the constraints in \prettyref{thm:optim-outl} on $H_s,\Lambda_s$ are satisfied. Then given any $\tau >0$, there exists absolute constants $C:=C(\tau)>0$ such that whenever $M=\min \sth{{\Delta\over \sigma}\sqrt{\alpha\over d}, {\Delta\over \sigma}\sqrt{\alpha\over 1+dk/n}}\geq C$, then
%	with probability at least $1-\frac 1n-4(k^2+k)n^{-(c/2-2)}-16dn^4e^{-0.3n}- 2k^2\exp\sth{-{\Delta\over 8\sigma}}$ we have
%	$$
%	\|\hat \theta_g^{(s)}-\theta_g\|^2\leq {d}
%	\qth{\max_{i:Y_i\in T_g^*}\max_{j\in [d]} \max\sth{\abs{F_{ij}^{-1}\pth{\frac 12 +x_0}},\abs{F_{ij}^{-1}\pth{\frac 12 -x_0}}}}^2,\quad s\geq 2,
%	$$
%	where 
%	$x_0= \sqrt{3\log n\over n_g^*}+e^{-{\Delta^2\over (8+\tau)\sigma^2}}+{\beta_g^\out\over 1+\beta_g^\out}$.
%\end{theorem}
%
%\begin{remark} \nb{EDIT THIS FOR NEW NOTATIONS}
%	In particular, if the errors of the $g$-th cluster are distributed as the multivariate Gaussian distribution with variance $\sigma^2$, then for any $\beta_g^{\out}\leq c \pth{\sqrt{3\log n\over n_g^*}+e^{-{\Delta^2\over (8+\tau)\sigma^2}}}$ the conditions in the above theorems are satisfied with $$x_0=C\sigma\pth{{\sqrt{\log n\over {n_g^*}}+e^{-{\Delta^2\over 24\sigma^2}}}}$$ for some large constant $C>0$. This implies that when $\Delta\gtrsim \sigma\log n$ we achieve the optimal rate of estimating the centroids.
%\end{remark}
%\begin{proof}
%	From the definition of $A_s$ we have
%	we get for any $g\in [k]$
%	\begin{align}\label{eq:29}
%		\max\sth{\sum_{h\in[k]\atop h\ne g}n_{hg}^{(s)},\sum_{h\in[k]\atop h\ne g}n_{gh}^{(s)}}
%		\leq \sum_{i=1}^n\indc{\hat z_i^{(s)}\neq z_i}
%		=nA_s, \quad s\geq 3.
%	\end{align}
%	Note that using $n\leq {n_g^*\over \alpha}$ and $n_{gg}^{(s)}\geq n_{g}^*-nA_s\geq n_g^*(1-A_s/\alpha)$, using the last display we can write
%	\begin{align*}
%		{n_{gg}^{(s)}\over n_g^{(s)}}\geq {n_{gg}^{(s)}\over n_{gg}^{(s)}+\sum_{h\in[k]\atop h\ne g}n_{hg}^{(s)}+n^{\out}}
%		\geq \frac 1{1+{n_g^*(\frac 1\alpha A_s+\beta_g^{\out})\over n_{gg}^{(s+1)}}}
%		\geq \frac 1{1+{\beta_g^{\out}+ A_s/\alpha\over 1-A_s/\alpha}}
%		=\frac 12 + {1-\beta_g^{\out}-\frac 2\alpha A_s\over 2(1+{\beta_g^{\out}})},
%	\end{align*}
%	which implies
%	\begin{align}\label{eq:km30}
%		\ceil{ {n_g^{(s)}/2}}-n_g^{(s)}+n_{gg}^{(s)}\geq n_{gg}^{(s)}-{n_g^{(s)}\over 2}
%		\geq \pth{1-\beta_g^{\out}-\frac 2\alpha A_s\over 1+\beta_g^{\out}}{n_g^{(s)}\over 2}
%		= \pth{\frac 12-{\beta_g^{\out}+A_s/\alpha \over 1+\beta_g^{\out}}}{n_g^{(s)}}
%	\end{align}
%	As $n_g^*\geq n\alpha$, the above implies for all $g\in [k]$
%	\begin{gather}
%			n_g^{(s)}\geq 	n_{gg}^{(s)}=n_g^*-\sum_{h\in[k]\atop h\ne g}n_{gh}^{(s)}
%			\geq n_g^*-nA_s \geq n_g^*\pth{1-\frac 1\alpha A_s}
%			\label{eq:km31}
%	\end{gather}
%	Fix $g\in [k]$. Let $U_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^{(s)}$, $V_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^*\cap T_g^{(s)}$, and $W_j$ denote the set of real numbers consisting of the $j^{\text{th}}$ coordinates of $T_g^*$.Then we get
%	\begin{align*}
%		U_j^{(\ceil{ {n_g^{(s)}/2}})}
%		&\stepa{\leq} V_j^{(\ceil{n_g^{(s)}/2}-n_g^{(s)}+n_{gg}^{(s)})}
%		\nonumber\\
%		&\stepb{\leq }
%		V_j^{(\floor{\pth{1-\beta_g^{\out}-\frac 2\alpha A_s\over 1+\beta_g^{\out}}{n_g^{(s)}\over 2}})}
%		\nonumber\\
%		&\stepc{\leq} W_j^{(\floor{\pth{1-\beta_g^{\out}-\frac 2\alpha A_s\over 1+\beta_g^{\out}}{n_g^{(s)}\over 2}})}
%		\stepd{\leq} W_j^{(\floor{{n_g^{*}}\pth{\frac 12-{\beta_g^{\out}+A_s/\alpha \over 1+\beta_g^{\out}}}\pth{1-\frac 1\alpha A_s}})}
%		\leq W_j^{(\floor{{n_g^{*}}\pth{\frac 12-{\beta_g^{\out}\over 1+\beta_g^{\out}}-\frac 5{2\alpha}A_s}})},
%	\end{align*}
%	where
%	\begin{itemize}
%		\item (a) followed using \prettyref{lmm:ord-stat_after_addn} with
%		$
%		X=V_j,\ \tilde X=U_j,\ \ell=n_g^{(s)}-n_{gg}^{(s)},\ t=\ceil{n_g^{(s)}\over 2},
%		$
%		\item (b) followed using \eqref{eq:km32} \eqref{eq:km30} and $\ceil{x}-y\geq \floor{x-y}$ for $x,y\geq 0$
%		
%		\item (c) followed using \prettyref{lmm:ord-stat_after_addn} with 
%		$X=V_j,\ \tilde X=W_j,\ \ell=n_g^*-n_{gg}^{(s)},\ t=\floor{\pth{\frac 12-{\beta_g^{\out}+ A_s/\alpha\over 1+\beta_g^{\out}}}{n_g^{(s)}}},$
%		
%		\item (d) followed using \eqref{eq:km31}.
%	\end{itemize}
%	Similarly, we also have
%	\begin{align*}
%		U_j^{(\ceil{ {n_g^{(s)}/2}})}
%		&\stepa{\geq} V_j^{(\ceil{n_g^{(s)}/2})}
%		\nonumber\\
%		&\stepb{\geq} 
%		V_j^{(\ceil{{n_g^*\over 2}\cdot \frac 1{1-{2A_s/\alpha}}})}
%		\stepc{\geq} 
%		V_j^{(\ceil{{n_g^*}(\frac 12+\frac 2\alpha A_s)})}
%		\stepd{\geq} W_j^{(\ceil{{n_g^*}(\frac 12+\frac 2\alpha A_s)}+\sum_{h=[k]\atop h\neq k}n_{gh})}
%		\stepe{\geq} W_j^{(\ceil{{n_g^*}(\frac 12+\frac 3\alpha A_s)})}.
%	\end{align*}
%	\begin{itemize}
%		\item (a) followed using \prettyref{lmm:ord-stat_after_addn} with
%		$
%		X=V_j,\ \tilde X=U_j,\ \ell=n_g^{(s)}-n_{gg}^{(s)},\ t=\ceil{n_g^{(s)}\over 2},
%		$
%		
%		\item (b) followed using \eqref{eq:km31} and (c) followed using $(1-x)^{-1}\leq 1+2x$ for $x=\frac 2\alpha A_s\leq \frac 12$.
%		
%		\item (d) used \prettyref{lmm:ord-stat_after_addn} with 
%		$X=V_j,\ \tilde X=W_j,\ \ell=\sum_{h=[k]\atop h\neq k}n_{gh},\ t=\ceil{{n_g^*\over 2}(1+\frac 4\alpha A_s)}+\sum_{h=[k]\atop h\neq k}n_{gh},$
%		
%		
%		\item (e) used that for any $x>0$ and positive integer $y$, $\ceil{x}+y = \ceil{x+y}$, and $\sum_{h=[k]\atop h\neq k}n_{gh}\leq nA_s$.
%	\end{itemize}
%	Then \prettyref{thm:main} implies that given any $\tau>0$, there exists $C:=C(\tau)$ such that whenever $M\geq C(\tau)$, we have $\frac 6\alpha A_s\leq e^{-{\Delta^2\over (8+\tau)\sigma^2}}$. Using this we combine the last two displays to get
%	\begin{align}
%		W_j^{(\ceil{{n_g^*\pth{\frac 12+e^{-{\Delta^2\over (8+\tau)\sigma^2}}}}})}
%		\leq U_j^{(\floor{{n_g^{(s)}/2}})}\leq W_j^{(\floor{{n_g^*\pth{\frac 12-{\beta_g^{\out}\over 1+\beta_g^{\out}}-e^{-{\Delta^2\over (8+\tau)\sigma^2}}}}})}.
%	\end{align}
%	Then using the result \prettyref{lmm:order-concentration-smallx} on the concentration of the order statistics
%	we conclude our results.
%\end{proof}

==> tex/outlier-genr.tex <==










==> tex/subG-app.tex <==

\section{Technical results for clustering with Sub-Gaussian errors}
\label{app:subg-technical}
\begin{lemma}\label{lmm:norm-concentration-subg}
	There is a set with probability at least $1-e^{-0.3n}$ on which the following happens. For any $\tau>0$ and any $S\subseteq [n]$ with $|S|\geq {n\beta}$, the cardinality of the set $$\sth{i\in S: \|{w_i}\|\leq \sigma \pth{\sqrt d + \sqrt{2\pth{\frac 1\tau\pth{1+\frac 1\beta}+\log(1/\tau)}}}}$$ 
	is at least $(1-\tau)|S|$.
\end{lemma}
\begin{proof}
	It suffices to show that for any set $S\subseteq [n]$
	$$
	\PP\qth{\sum_{i\in S}\indc{\norm{w_i} > \sigma \pth{\sqrt d + \sqrt{2\pth{\frac 1\tau\pth{1+\frac 1\beta}+\log(1/\tau)}}}}\geq \tau |S|}
	\leq e^{-n},
	$$
	and then use the union bound over different choices of $S$ to get the result. We define 
	$$
	F_i=\indc{\norm{w_i} > \sigma \pth{\sqrt d + \sqrt{2\pth{\frac 1\tau\pth{1+\frac 1\beta}+\log(1/\tau)}}}}.
	$$
	In view of the above definitions it is enough to show that
	\begin{align}
		\label{eq:ht8}
		\PP\qth{\sum_{i\in S} F_{i} \geq \tau |S|}\leq e^{-n} \text{ for all } S\subseteq [n].
	\end{align}
	Note that, by \cite[Theorem 2.1]{hsu2012tail}, we have
	$$
	\PP\qth{\|w_i\|\leq \sigma (\sqrt d+\sqrt{2t})}\leq e^{-t}, t\geq 0.
	$$
	This implies
	\begin{align}
		&\PP_{w_i\in \subG(\sigma^2)}\qth{\norm{w_i} > \sigma \pth{\sqrt d + \sqrt{2\pth{\frac 1\tau\pth{1+\frac 1\beta}+\log(1/\tau)}}}}
		\leq \tau e^{-\frac 1\tau\pth{1+\frac 1\beta}}
		.
	\end{align}
	This implies $\sum_{i\in S}F_i$ is stochastically larger than $\Binom(|S|,\tau e^{-\frac 1{\tau}(1+\frac 1\beta)})$. Using Chernoff's inequality \prettyref{lmm:chernoff}
	with $a=\tau e^{-\frac 1{\tau}(1+\frac 1\beta)}$, $m=|S|$. Using $x\log x\geq -0.5$ for $x\in (0,1)$ we get
	\begin{align}\label{eq:ht7}
		\PP\qth{\sum_{i\in S} F_{i} \geq \tau|S|}
		&\leq \exp\pth{-mh_{\tau}(a)}
		\nonumber\\
		&\leq \exp\pth{-m\pth{a\log{a\over \tau}+(1-a)\log{1-a\over 1-\tau}}}
		\nonumber\\
		&\leq  \exp\pth{-m\sth{a\log a+(1-a)\log(1-a)+{(1+ 1/\beta)}}}
		\leq e^{-n}.
	\end{align}
	Finally taking an union bound over all choices of $S$ we get the desired bound.
\end{proof}

==> tex/subG-ht.tex <==
\section{Mislabeling rates for the \codelta algorithm for sub-Gaussian mixtures}
In this section we prove mislabeling rate for our algorithm when the errors are generated from Sub-Gaussian mixture. In the sub-Gaussian model, the observed data $Y_1,\dots,Y_n\in \reals^d$ are distributed as
\begin{align}
	Y_i=\theta_{z_i}+w_i,\ i=1,\dots,n,
\end{align}
where $\sth{z_i}_{i=1}^n\in[k]^n$ denote the underlying unknown component labels of the points, and $w_i$-s denote the error variables. We assume that $w_i$-s are independent zero mean sub-Gaussian vectors with parameter $\sigma>0$, i.e.,
\begin{align}\label{eq:subg-defn}
	\EE\qth{e^{\langle a,w_i \rangle}}
	\leq e^{\sigma^2\|a\|^2\over 2}, \text{ for all $i\in \sth{1,\dots,n}$ and $a\in \reals^d$}.
\end{align}
For the results in this section we define the signal to noise ratio by $
\snr={\Delta\over 2\sigma}$. Notably, this definition differs from the usual definition in the moment constrained case as in the parameter $\sigma$ here is primarily used to characterize the variance of randomness in each individual coordinate and the bound on the norm of the random error should differ, on average, with dimension as well.
Our result is the following.
\begin{theorem}
	\label{thm:main-subg}
	There exists absolute constants $c_0,c_1,c_2,c_3,c_4>0$ such that the followings are satisfied.
	\begin{enumerate}[label=(\alph*)]
		\item \textbf{$\snr< c_0\sqrt {d/\alpha}$:} Assume $n\alpha^2\geq Ck\log n$ and ${\snr}\sqrt{\alpha\over 1+{dk\over n}}\geq C\sqrt k$ for a sufficiently large constant $C$. If the clustering initialization satisfies either one of the following conditions
		$${H_0}\geq 1-\frac 2{\sigma\sqrt d}\pth{\frac 12 - \frac {c_1/{\alpha}^{1/4}}{\pth{\snr}^{1/2}}}\quad  \text{ or } \quad \Lambda_0\leq \frac 12-{c_2/{\alpha}^{1/4}\over \pth{\snr}^{1/2}}.$$
		Then whenever $\snr\sqrt \alpha \geq M\geq c_3$,  we have $$\EE\qth{\ell(\hat z^{(s)},z)}\leq \exp\sth{-\frac 12\pth{1-{c_4\over \sqrt \snr}}(\snr)^2},
		\quad s\geq 3\log n.
		$$
		
		\item \textbf{$\snr\geq c_0\sqrt {d/\alpha}$:} Suppose the clustering initialization satisfies either one of the following conditions
		$${H_0}\geq \frac 12 +\gamma_0 \text{ with } \gamma_0>2.1\alpha \quad  \text{ or } \quad \Lambda_0\leq \frac 12-{c_2/{\alpha}^{1/4}\over \pth{\snr}^{1/2}}.$$
		Then whenever $\snr\sqrt \alpha \geq M\geq c_3$,  the \codelta algorithm with $\delta=\frac 12-{\gamma_0\over 4}$ achieves the misclustering rate
		$$
		\EE\qth{\ell(\hat z^{(s)},z)}\leq \exp\sth{-\frac 12\pth{1-{c_4\over \sqrt \snr}}{(\snr)^2}},
		\quad s\geq 1.
		$$
	\end{enumerate}
	
\end{theorem}
\begin{remark}
	The result \cite[Theorem 3.4]{lu2016statistical} shows that it is not possible to improve the misclustering error beyond the rate $e^{-\frac 12(1+o(1)){(\snr)^2}}$. This establishes the optimality of the coordinate-wise median based Lloyd algorithm.
\end{remark}

\begin{proof}[Proof of \prettyref{thm:main-subg}]
	The proof of part (a) is essentially the same as the proof of the similar result \cite[Theorem 3.2]{lu2016statistical} for usual $k$-means. This is because the part of the cluster, the mean of which we use to construct our centroid estimates, is of similar order as the full clusters themselves. As a result we can use the similar concentration bounds that were used to analyze the mean of the full sample in the classical $k$-means problems. We omit the proof here.
	
	To prove part (b), we use the following key lemma.
	\begin{lemma}
		\label{lmm:E-prob-subg}
		Fix $0<\tau,\epsilon_0<\frac 12$. There is a set $\calE_{\tau,\epsilon_0}$ with $\PP\qth{\calE_{\tau,\epsilon_0}}\geq 1-kn^{-c/2}-4e^{-0.3n}$ on which the following holds: 
		\begin{enumerate}[label=(\roman*)]
			\item For any $S\subseteq [n]$ with $|S|>\beta n$, the cardinality of the set 
			$$\sth{i\in S: \|{w_i}\|\leq \sigma \pth{\sqrt d + \sqrt{2\pth{\frac 1\tau\pth{1+\frac 1\beta}+\log(1/\tau)}}}}$$ 
			is at least $(1-\tau)|S|$.
			\item For any $\epsilon\in[\epsilon_0,1/2]$ and $g,h\in[k]$ we have
			$$\sum_{i:Y_i\in T_g^*}\indc{\epsilon^2\|\theta_g-\theta_h\|^2\leq \langle w_i,\theta_h-\theta_g\rangle}
			\leq \frac {5n_g^*}{4\epsilon_0^4(\Delta/\sigma)^2}$$
			\item For any symmetric matrix $A$, let $\lambda_{\max}(A)$ denote its maximum eigen value. Then 
			$$\lambda_{\max}\pth{\sum_{i:Y_i\in T_g^*} w_iw_i^{\sfT}}\leq 6\sigma^2(n_g^*+d) \text{ for all } g\in [k].$$
		\end{enumerate}
	\end{lemma} 
	To prove the above lemma, for each of the cases we separately construct sets of high probability on which the results hold. Then taking intersection we get the result. The analysis of (i) has been provided in \prettyref{lmm:E-norm}, the statements (ii),(iii) are the exact results from \cite[Lemma 12, Lemma 13]{JKY2023}.
	
	Based on the above result we get the following results on step-wise clustering errors due to mislabelling.
	
	\begin{lemma}\label{lmm:Gs-Ls-bound-subg}
		Fix $0<\epsilon_0\leq \frac 12,\frac 5{n\alpha} <\gamma_0 \leq \frac 12$. Let $r_k={\Delta\over\sigma}\sqrt{\alpha\over 1+{dk/n}}$. Then on the set $\calE_{\tau,\epsilon_0}$ with $\tau={\gamma_0\over 1+2\gamma_0}$ we have
		\begin{enumerate}[label=(\roman*)]
			\item If $\Lambda_s\leq \frac 12-\epsilon_0$ then $H_{s+1} \geq 1-{5\over \epsilon_0^4 r_k^2}
			-{48\Lambda_s^2\over \epsilon_0^4r_k^2}$,
			\item If $H_s\geq \frac 12+\gamma_0$ then $\Lambda_s\leq {8\sigma\over \Delta} \pth{\sqrt d + \sqrt{2\pth{{1+2\gamma_0\over \gamma_0}\pth{1+\frac 1\beta}+\log\pth{1+2\gamma_0\over \gamma_0}}}}$.
		\end{enumerate}
	\end{lemma}
	
	The proof of above result is straightforward. The proof of \prettyref{lmm:Gs-Ls-bound-subg}(i) is exactly the same as in \cite[Appendix C]{JKY2023}, so we skip it here. 
	We present below the proof of \prettyref{lmm:Gs-Ls-bound}(ii). We prove this using contradiction. For simplicity of notation we denote 
	$$D={\sigma} \pth{\sqrt d + \sqrt{2\pth{{1+2\gamma_0\over \gamma_0}\pth{1+\frac 1\beta}+\log\pth{1+2\gamma_0\over \gamma_0}}}}.$$ 
	Let us assume $\Lambda_{s} > {6D\over \Delta}$. This implies that there exists a cluster $h$ such that the centroid estimation error satisfies 
	$$\|\hat \theta_h^{(s+1)}-\theta_h\|> {6D}.$$ 
	
	
	Next we use the above results to prove \prettyref{thm:main-subg}(ii). For $c_1$ to be chosen later, we define
	$$\epsilon_0={c_1/\alpha^{1/4}\over \pth{\snr}^{1/2}}.$$
	Let $H_s$ be the correct-labeling proportion as defined before in \eqref{eq:mislabel}. Then from \prettyref{lmm:Hs-Ls-bound-subg} it follows that we can choose $c_0,c_1>0$ such that on the set $\calE_{{\gamma_0\over 1+2\gamma_0},\epsilon_0}$:
	\begin{itemize}
		\item if $H_0\geq \frac 12+\gamma_0$ then $\Lambda_0\leq 0.3$,
		\item if $\Lambda_0\leq \frac 12-\epsilon_0$ then $H_1\geq 0.7$.
	\end{itemize}
	A second application of \prettyref{lmm:Gs-Ls-bound-subg} guarantees that we can choose $c_0$ large enough such that if  
	$\snr\geq c_0\sqrt{d/\alpha}$
	then on the set $\calE_{{5\over 26},0.2}$, with $\epsilon_1=\gamma_1=0.2$,
	\begin{itemize}
		\item if $H_s\geq 0.7$ then
		\begin{align}
			\label{eq:Ls}
			\Lambda_s&\leq {12\sqrt 2/\alpha^{1/2}\over \sqrt{0.2}\snr} \leq 0.3,
		\end{align}
		\item if $\Lambda_s\leq 0.3$ then
		\begin{align}
			\label{eq:Gs}
			G_{s+1}&\leq {5/\alpha\over (0.2)^4(\snr)^2}+{48(0.3)^2/\alpha\over (0.2)^4(\snr)^2}\leq 0.3.
		\end{align}		
	\end{itemize}
	and whenever 
	Combining the above displays we get that on the set
	\begin{align}
		\label{eq:Prob-E}
		\calE&=\calE_{{\gamma_0\over 1+2\gamma_0},\epsilon_0}\cap \calE_{{5\over 26},0.2}
		\nonumber\\
		\PP\qth{\calE}
		&\geq 1-4kn^{-c/4}-4e^{-0.3n}
	\end{align} 
	we have
	\begin{align}
		\label{eq:ht14}
		\Lambda_s\leq 0.3,G_{s+1}\leq 0.3 \text{ for all } s\ge 0.
	\end{align}
	The rest of the analysis is 
	identical to that of the proof of \cite[Theorem 1]{JKY2023} where it is shown that once we achieve $\Lambda_s\leq 0.3$ for all $s\geq 3$, the mislabeling rate follows. We omit it here.
\end{proof}


